Information Design for Hybrid Work under Infectious Disease Transmission Risk

We study a planner's provision of information to manage workplace occupancy when strategic workers (agents) face risk of infectious disease transmission. The planner implements an information mechanism to signal information about the underlying risk of infection at the workplace. Agents update their belief over the risk parameter using this information and choose to work in-person or remotely. We address the design of the optimal signaling mechanism that best aligns the workplace occupancy with the planner's preference (i.e., maintaining safe capacity limits and operational efficiency at workplace). For various forms of planner preferences, we show numerical and analytical proof that interval-based information mechanisms are optimal. These mechanisms partition the continuous domain of the risk parameter into disjoint intervals and provision information based on interval-specific probability distributions over a finite set of signals. When the planner seeks to achieve an occupancy that lies in one of finitely many pre-specified ranges independent of the underlying risk, we provide an optimal mechanism that uses at most two intervals. On the other hand, when the preference on the occupancy is risk-dependent, we show that an approximately optimal interval-based mechanism can be computed efficiently. We bound the approximation loss for preferences that are expressed through a Lipschitz continuous function of both occupancy and risk parameter. We provide examples that demonstrate the improvement of proposed signaling mechanisms relative to the common benchmarks in information provision. Our findings suggest that information provision over the risk of disease transmission is an effective intervention for maintaining desirable occupancy levels at the workplace.

==> CDC_Submission/junk.tex <==

% \noindent We can accordingly use Definition $\ref{defn:pse}$ to determine the set of $(a,b) \in \mathbb{R}_+^2$ such that $x_{F,s} \in \mathcal{Y}$. Specifically, for any interval ${P_{i,\ubar{c},\bar{c}} = \{\sum_{j=0}^{j=i-1} \mathbf{e}_j + c\cdot \mathbf{e}_i | c \in [\ubar{c},\bar{c}]\}}$ on $\mathcal{Z}(x_I)$, note that the set ${\mathcal{A}_i  = \{(a,b)| r_i+(\ubar{c}+\sum_{j=1}^{i-1})x_j) a \leq b \leq r_i+(\bar{c}+\sum_{j=1}^{i-1})x_j) a\}}$ precisely defines the set of $(a,b)$ such that $x_F \in \mathcal{A}_i$. We define $\mathcal{A} = \cup_i \mathcal{A}_i$. This implies that for a public signalling equilibrium, we can simply re-express the objective as follows:

% \begin{figure}[h!]
%     \centering
%         \centering
%     \begin{tikzpicture}
% \draw[axis] (0,0) -- (8,0) node[right=2* \nudge cm] {\(x_1\)};
% \draw[axis] (0,0) -- (0,9) node[above=2*\nudge cm] {\(x_2\)};
% \node[black] at (1.2,6) {$\lonesimplex$};
% \node[fill,circle,red,minimum size=0.01cm] at (3.8,2.2) {};
% \begin{scope}
% \draw[line,line width=0.05cm] (8,0) -- (0,8) coordinate (ineq1);
% \node[fill,triangle,black,minimum size=0.01cm] at (3.1,2.2) {};
% \node[fill,square,black,minimum size=0.01cm] at (0,0.5) {};
% \node[teal] at (1.6,1.6) {$\mathcal{Y}$};
% \node[orange] at (-0.2,2.2) {$Q_1$};
% \node[black] at (0.3,0.5) {$\xh$};
% \node[black] at (3.15,1.95) {$\xl$};
% \node[black] at (3.8,1.95) {$\mathbf{x}_I$};
% \node[orange] at (3.3,2.4) {$Q_2$};
% \node[blue] at (2,2.4) {$P_2$};
% \node[blue] at (-0.2,1.4) {$P_1$};
% \node[purple] at (-0.2,0.25) {$Q_0$};
% \draw[line,thick,orange] (3.8,2.2) -- (3.1,2.2) coordinate (move1);
% \draw[line,thick,blue] (3.1,2.2) -- (0.8,2.2) coordinate (move2);
% \draw[line,thick,orange] (0.8,2.2) -- (0,2.2) coordinate (move3);
% \draw[line,thick,orange] (0.03,2.2) -- (0.03,2) coordinate (move4);
% \draw[line,thick,blue] (0.03,2) -- (0.03,0.5) coordinate (move5);
% \draw[line,thick,purple] (0.03,0.5) -- (0.03,0) coordinate (move6);
% \clip (0,1) -- (0,2) -- (2.6,2.8) -- (4,1) -- (2,0.5)  -| (0,1);
% \fill[teal,opacity=.5] (0,0) rectangle (8,8);
% \end{scope}
% \end{tikzpicture}
%     \caption{Example partition of $\mathcal{Z}(\mathbf{x}_I)$.}
% \label{fig:demonstration}
% \end{figure}

% \noindent As commonly used previous literature, we can define a mean-preserving contractions $\mathcal{Q}$ (reverse of mean-preserving spreads) of the distribution $\mathcal{P}$ and denote them accordingly as $\mathcal{Q} \prec \mathcal{P}$. From Stiglitz and Blackwell, it is commonly known that the set of all distributions and set of tuples is equivalent to the set of all mean-preserving contractions. 
% \subsubsection{Information Benchmarks}
% \noindent Notice that under no information, if $\bar{a} = \int a\cdot d\mathcal{P}(a,b)$ and $\bar{b} = \int a\cdot d\mathcal{P}(a,b)$ are such that $(\bar{a},\bar{b}) \in \mathcal{A}$ then $V^* = 1$. Else if $(\bar{a},\bar{b}) \notin \mathcal{A}$, then $V^* = 0$. 

% \noindent Under fully informative signalling, we correspondingly know that $V^* = \mathbb{P}[(a,b) \in \mathcal{A}]$. Notice if $\mathcal{Y}$ consists of a finite union of singletons (excluding corner points) and $\mathcal{P}$ is a continuously defined distribution then $V^* = 0$. 

% \subsubsection{Optimal Mechanism}
% \begin{lemma}
% The optimal mechanism $(\pi, \mathcal{S})$ can be determined by solving the following optimization problem:
% \begin{align*}
%     \max_{\mathcal{Q} \prec \mathcal{P}} \int_{\mathcal{A}} d\mathcal{Q}(a,b)
% \end{align*}
% \end{lemma}
% \begin{proof}
% Sketch - follows from definition.
% \end{proof}

% \begin{lemma}
% The optimal public signalling mechanism is equivalent to one with $|\mathcal{S}| \leq 2\mathcal{K}+1$. 
% \end{lemma}
% \begin{proof}
% Sketch - convexity of map from (a,b) to [0,1] in the objective is sufficient to show this property.
% \end{proof}

% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
% \begin{axis}[
%     axis lines = middle,
%     xlabel = {$a$},
%     ylabel = {$b$},
%     xmin=0, xmax=5.5,
%     ymin=0, ymax=7]
%  \filldraw [teal!20] (axis cs: 2, 4) circle [radius=3]; 
% % Plot 1
% \addplot [name path = A,
%     -latex,
%     domain = 0:4.5,
%     samples = 1000] {5+0.35*x} 
%     node [pos=0.6, above] {$b=(\bar{c}+\sum x_{i=1}^{k-1})a+r_k$};
 
% % Plot 2
% \addplot [name path = B,
%     -latex,
%     domain = 0:4.5] {5+0.25*x} 
%     node [pos=0.4, below] {$b=(\ubar{c}+\sum x_{i=1}^{k-1})a+r_k$};
 

% % Fill area between paths
% \addplot [blue!30] fill between [of = A and B, clip={domain=0:4}];
 
% \end{axis}
% % \end{tikzpicture}
% %     \caption{Ex: Distribution $\mathcal{P}$ shown in teal and $\mathcal{A}_k$ shown in between two lines. }
% %     \label{fig:my_label}
% % \end{figure}

% \subsection{IID Signalling}
% We will assume for now that all agents at all $\safe[k]$ for all $k$ are receiving signals drawn from the same distribution $\pi_{a,b}(s)$ and that each of these draws are independent irrespective of $k$. Via the law of large numbers, in IID signalling, this implies that for each $k$ and for a true parameter state of $(a,b)$, a mass of $x_k \pi_{a,b}(s)$ will observe signal $s$. These agents that observe $s$ maintain a posterior distribution $\mathcal{P}_s$ over $(a,b)$ and will commonly believe that the masses of agents receiving other signals is given by $\pi_{a,b}(s)$. Hence given $(a,b)$ the equilibrium mass should be fixed. \\
% Consequently, strategies now must be defined in terms of the signal received and the position of the agent. Hence $\sigma_i(x_i, s)$ can accordingly factor in the equilibrium definition as agents receiving $s$ have posterior $\mathcal{P}_s$. 

% \begin{defn}
% \label{defn:iidse}
% We define an IID signalling equilibrium in this setting to be the tuple $(\mathbf{\sigma}(p_s))_{s \in \mathcal{S}}$ inducing $(\mathbf{x}^*_{F,a,b})_{a,b \in \mathbb{R}^2}$ such that $(\mathbf{x}_{F,a,b})_i = \{\sum_{s \in \mathcal{S}} \sigma_i(s) \}$ where $y_{a,b}^* = 1-\sum_i \sigma_i(p_{a,b})$, such that for all $s$:\\
% $\sigma_i(x_i,s) \in (0,q_s x_{I,s})$ iff $r_k =\int b-a\cdot y^*_{a,b} d\mathcal{P}(a,b)$ \\
% $\sigma_i(x_i,s) = 0$ iff $r_k < \int b-a\cdot y^*_{a,b} d\mathcal{P}(a,b)$\\
% $\sigma_i(x_i,s)  = q_s x_{I,s}$ iff $r_k >\int b-a\cdot y^*_{a,b} d\mathcal{P}(a,b)$
% \end{defn}
% \noindent The first observation is that as before we can restrict the size of the signal alphabet. 
% \begin{lemma}
% The optimal  IID signalling mechanism is equivalent to one with $|\mathcal{S}| \leq 2M+1$. 
% \end{lemma}



% \begin{figure}
%     \centering
%     \includegraphics[width=80mm]{boxplot_x.png}
%     \caption{$\beta(y) = \theta y^2$; ratio between infectious risk ($\theta y^3$) and social surplus ($\sum_i v_i (x_i - y_i)$). There is no gains from signalling since any information revelation exacerbates the externality. Social surplus maximizing choice maximizes this difference.}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=80mm]{tradeoff_x.png}
%     \caption{$\beta(y) = \theta y^2$; trade-off between total infectious risk ($\theta y^3$) and social surplus ($\sum_i v_i (x_i - y_i)$). There is no gains from signalling since any information revelation exacerbates the externality. }
%     \label{fig:my_label}
% \end{figure}







% \begin{tikzpicture}
% \begin{axis}[no markers, domain=0:7, samples=100,
% axis lines*=left,  
% height=3cm, width=10cm,
% xticklabels={,,$\theta_1^1$,$\theta_1^2$, $\bar{\theta}$,,$\theta_2^1$,$\theta_2^2$}, ytick=\empty,
% enlargelimits=false, clip=false, axis on top]
% \addplot [fill=green!20, draw=none, domain=-3:3] {gauss(0,1)} \closedcycle;
% \end{axis}
% \draw[line,line width=1mm,blue] (1.42,0.01) -- (2.84,0.01);
% \draw[line,line width=1mm,blue] (5.62,0.02) -- (7.05,0.02);
% \node[fill,black,triangle] at (2.84,0.01);
% \node[fill,black,triangle] at (5.62,0.01);
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis}[no markers, domain=0:7, samples=100,
% axis lines*=left, 
% height=3cm, width=10cm,
% xticklabels={,,,, $\bar{\theta}$,$\theta_1^1$,$\theta_1^2$,}, ytick=\empty,
% enlargelimits=false, clip=false, axis on top]
% \addplot [fill=green!20, draw=none, domain=-3:3] {gauss(0,1)} \closedcycle;
% \addplot [fill=orange!20, draw=none, domain=-1.2:3] {gauss(0,1)} \closedcycle;
% \end{axis}
% \draw[line,line width=1mm,blue] (5.62,0.02) -- (7.05,0.02);
% \node[fill,black,triangle] at (5.62,0.01);
% \node[fill,black,triangle] at (1.9,0.01);
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis}[no markers, domain=0:7, samples=100,
% axis lines*=left, xlabel=$\Theta$,
% height=3cm, width=10cm,
% xticklabels={,,$\theta_1^1$,$\theta_1^2$, $\bar{\theta}$,,,}, ytick=\empty,
% enlargelimits=false, clip=false, axis on top]
% \addplot [fill=green!20, draw=none, domain=-3:3] {gauss(0,1)} \closedcycle;
% \addplot [fill=orange!20, draw=none, domain=1.25:3] {gauss(0,1)} \closedcycle;
% \end{axis}
% \draw[line,line width=1mm,blue] (1.42,0.01) -- (2.84,0.01);
% \node[fill,black,triangle] at (2.84,0.01);
% \node[fill,black,triangle] at (6.5,0.01);
% \end{tikzpicture}



% The set of all mechanisms is known to be compact; see \cite{candogan_persuasion_2019}. So notice that an optimal mechanism $\pi = \langle \{g_\theta\}_{\theta \in \Theta}, \I \rangle$ must exist. Suppose by contradiction that $|\I| > \KK+1$. Then, there must exist $i,j,l$ such that $\theta_i, \theta_j \in [\theta_l^1.\theta_l^2]$ or $\theta_i, \theta_j \notin [\theta_l^1.\theta_l^2]$ for all $l$. In the first scenario, consider the mechanism $\tilde{\pi} = \langle \{\tilde{g}_\theta\}_{\theta \in \Theta}, \I\cup{\tilde{i}}\setminus \{i,j\} \rangle$ where . It is easily verified that under the modified mechanism $\theta_{\tilde{i}} \in [\theta_i,\theta_j] \subset [\theta_l^1.\theta_l^2]$ and the remaining posterior means and associated probabilities are unchanged. By Equation \ref{eqn:red_1_form}, the objective $V(\tilde{\pi}) = V(\pi)$ which is a contradiction as $\tilde{\pi}$ uses a strictly smaller signalling set. 






%% INTRO

% It takes time for the organization to react due to the presence of asymptomatic
% individuals (e.g. in schools (Viner et al., 2020)), delayed display of symptoms and a variety
% of organizational frictions.1 Taking this reaction time as given we explore the best way to
% rotate groups in order to minimize the expected terminal infection We show XXX The key intuition XXX \\
% Lockdowns and confinement measures constitute effective non-pharmaceutical interventions for slowing the spread of an epidemic (Anderson et al. 2020, Fowler et al. 2020).
% These measures enable the deployment of more time-consuming medical responses and
% may even bring the spread of the virus to a halt (Ferguson et al. 2020, Ji et al. 2020).
% The efficacy of these restrictions, however, relies heavily on individual compliance (Wright
% et al. 2020), which political leaders and governmental agencies influence by disseminating information on the epidemic’s severity (Webster et al. 2020). However, several factors
% greatly complicate the proper choice of a communication strategy to influence the public
% compliance.
% First, implementing confinement measures requires making trade-offs between health
% benefits and the economic costs that social distancing brings about (Hargreaves Heap et al.
% 2020, IMF 2020). 
% These messages affect the population’s perception of the risk associated with social
% interactions. However, compliance with confinement measures also depends on the socioeconomic status of individuals (Atchison et al. 2020, Van Rooij et al. 2020). In deciding
% to remain isolated, individuals weigh the benefits to their health against the income they
% might forgo (Wright et al. 2020, Gitmez et al. 2020). Thus, part of the population might
% have preferences that do not fully align with the government’s priorities. The more heterogeneous a population is, the more individual preferences may differ (Bottan et al. 2020).
% Furthermore, the choice of an individual to remain isolated (or not) creates externalities
% for the rest of the population. The more individuals isolate themselves, the less exposed
% the population is, which decreases the expected health risk for everyone (Bethune and
% Korinek 2020). This, however, decreases the incentive to remain confined and thus gives
% rise to strategic interactions within the population.
% This paper explores how policymakers may efficiently inform the public about the severity of an epidemic to induce public compliance with their confinement measures. To address
% this question, we develop an information design framework, which accounts for the healtheconomy trade-off faced by both governments and individuals, the socioeconomic heterogeneity within the population and the externalities that social distancing brings about.
% Our analysis reveals that governments should always fully disclose their information
% about the epidemic when they weigh the economy and population health relatively equally.
% Consistent with the existing literature and several pieces of anecdotal evidence (e.g., Alizamir et al. 2020, Paz 2020), we also find that governments sometimes have a rationale to
% misrepresent information on the epidemic. If the government’s priorities are heavily biased
% toward the economy or the population’s health, they may indeed downplay or exaggerate the severity of the epidemic, respectively. These distortions occur when the public
% incentives are in fact overall aligned with the government’s priorities.
% More specifically, consider a government that is heavily biased toward protecting the
% population’s health over minimizing economic losses. When the symptoms of the disease
% are generally mild, individuals do not have strong incentives to isolate themselves, which
% does not fully align with the government’s objective. Nevertheless, we find in our setup that
% the government always fully discloses its information about the severity of the epidemic.
% In contrast, when symptoms are serious, individuals have a strong incentive to remain
% confined, which does align with the government’s priorities. However, we find that the
% government sometimes exaggerates the severity of the epidemic. In fact, when symptoms
% are extremely serious, the government does not disclose any information. We obtain similar
% results in the opposite direction when the government is heavily biased toward minimizing
% economic costs. In this case, the government may downplay the severity of the epidemic
% when the symptoms are mild, which, again, does not align with the government’s priorities.
% Further, we find that the level of economic inequality in the population has an effect on
% these misrepresentations. The more heterogeneous the disease’s economic impact is, the
% less the government exaggerates and the more it downplays the severity of the epidemic. In
% other words, the government of a population with significant levels of economic disparity
% has a greater tendency to downplay the severity of the epidemic than the government of a
% more economically equal society.
% The general information design framework we consider in this paper was introduced by
% Kamenica and Gentzkow (2011), with growing applications in operations research and management science (see Candogan 2020, and the references therein; see also online Appendix E
% for a literature review). In particular, this approach has been especially fruitful for studying
% broad public health questions such as ours (e.g., Shi 2013, Alizamir et al. 2020). Our findings also complement the rapidly growing literature on global health and disaster management that has emerged since the COVID-19 outbreak, which analyzes different approaches
% to limit the spread of the disease (e.g., Birge et al. 2020, Housni et al. 2020 and Ramdas
% et al. 2020). In contrast to this literature, our study explores the role of information and
% public behavior in containing the epidemic and is related to agency problems and strategic
% behaviors in healthcare systems (e.g., Adida et al. 2017, Zorc et al. 2017).

% Karin et al. (2020) propose rotation of the economic activities as a safe path to reopening
% the economy.5 We share with Karin et al. (2020) the motivation of understanding rotation
% mechanisms in the diffusion of disease, and our work is complementary to theirs. Their
% focus and recommendation over the rotation’s frequency differ from those in our paper.
% They exploit particular biological facts about the length of the covid-19 incubation and
% infectiousness periods to design a cycle in which each person is active about one third of
% the times so that she is likely to be isolated during her possible infectious period. We,
% instead, focus on uncertainty over the exposure period and show that the frequency of
% rotation has large effects even if the timing of infectiousness is not carefully exploited. This
% is an adequate approach when there are organizational frictions and, therefore, organizations
% cannot be trusted to react immediately to the first displays of symptoms. Vice versa, there
% is no uncertainty over the length of the diffusion of the disease in Karin et al. (2020).
% Additionally, we require that half of the individuals are active at any time, and thus the
% policy experiment evaluated by Karin et al. (2020) is infeasible in our model. Finally, we
% explain the role of aggregate uncertainty over infections when we study the effect of mixing
% members of the rotating groups; aggregate uncertainty is absent in Karin et al. (2020).
% Relatedly, Akbarpour et al. (2020) show, in a SIR-based network model calibrated to two
% US agglomerations, that rotation of workforce has strong contagion-mitigation effect with
% small disruption costs.
% Recent contributions in epidemiology, computer science and economics investigate targeted lock-downs and other social-distancing measures typically within variants of the SIR
% diffusion model, see, e.g., Acemoglu et al. (2020), Eichenbaum et al. (2020) and Brother hood et al. (2020). We take a complementary micro-level approach and our analysis uncover
% some mechanisms that could allow decision-makers to re-design the workplace to increase
% organizational resilience to new Covid-19 outbreaks. We do not attempt to model the whole
% economy, and instead take the infection rate outside of the studied organization as given.Some of the greatest economic crises that societies have faced involve some form of contagion. Notable examples include financial contagion, where investors acquire toxic assets that decrease the
% total value of their portfolios—e.g., the global financial crisis of 2008 (GFC); epidemiological contagion, where an infectious disease is spread in a population, impacting its productivity, growth,
% and employment—e.g., the Covid-19 pandemic; and monetary contagion, where the debasement
% of commodity money and the counterfeiting of fiat money reduce the frequency with which goods
% and services are exchanged—e.g., the debasement crisis of medieval France and England and the
% current wave of counterfeiting boosted by the digital era.1
% While contagion problems can be devastating per se, the propagation of their deleterious effects
% is facilitated by the weak response of economic systems, which is typically hampered by externalities and coordination failure. The reason for this is that individuals fail to internalize the whole
% effect their efforts have on curbing contagion and are unable to coordinate their responses to increase the effectiveness of their actions. The thesis of this paper is that governments or regulators
% can alleviate these frictions by managing the disclosure of information they possess in a way that
% aligns individuals’ behavior to what would be the optimal behavior from society’s perspective.2
% We analyze the role of information design to shape individuals’ incentives in a decentralized
% environment susceptible to contagion. In our setup, infected and susceptible individuals match
% randomly and pairwise. The infection rate of the population is initially unknown, as well as
% the infectious status of each individual. The government (the sender in our setting) has a test
% available that can reveal the infectious status of any tested individual. There is a continuum of
% individuals; thus, the government learns the infection rate by testing a positive fraction of the
% population. Critically, the government may strategically reveal the infection rate to the public or
% opt to (partially) conceal such information.
% 1According to Quercioli and Smith (2015), about one in 10,000 U.S. dollar notes is counterfeit, with the
% domestic public losing 80 million in 2011, more than doubling since 2003. Meanwhile, Rolnick et al. (1996)
% observe that between 1285 and 1490, France had 123 debasements of silver coins, 112 of more than 5 percent,
% with the highest being 50 percent.
% 2
% Information management can be a powerful but fuzzy policy instrument. As a testament of the former, the
% final report of the Commission that studied the GFC concluded that the “liberal” policies undertaken by credit
% rating agencies were instrumental in the downfall of financial markets (cf. Financial-Crisis-Inquiry-Commission,
% 2011). In turn, as an illustration of the latter, it is noteworthy that the WHO advices full transparency regarding
% the transmission of sanitary information for containing epidemics, but it is silent about the communication
% policies that governments should follow with respect to their assessment of how widespread contagion is (cf.
% World-Health-Organization, 2018).
% 2
% Electronic copy available at: https://ssrn.com/abstract=3988157�
% Testing partitions the population in two types: non-tested and tested-negative. Testedpositive individuals are isolated by the government—in line with the policies that have been used
% to manage contagion in different historical contexts—and play no role in our model. Non-isolated
% individuals interact in a decentralized environment and make strategic choices of vigilance efforts.
% In a matching, a passage function maps individuals’ vigilance efforts to a probability of contagion, whenever one of the individuals is infected and the other is not. Vigilance reduces the probability of contagion, and, hence, the passage function is decreasing in the effort of both matched
% individuals. As a consequence, the effort of non-tested individuals—who are uncertain about their
% infectious status—generates a positive externality that benefits both other non-tested individuals
% who may not be infected with positive probability and tested-negative individuals who are certainly not infected. Moreover, we distinguish two cases with respect to the interaction of efforts:
% (i) when the marginal benefit of an individual’s effort is decreasing in the effort of the other individual, i.e, when efforts are strategic substitutes; and (ii) when the marginal benefit of an individual’s
% effort is increasing in the effort of the other individual, i.e., when efforts are strategic complements.
% Finally, the government is benevolent and aims to minimize society’s expected welfare losses,
% which include both the cost of vigilance and losses associated to contagion. The only available
% instrument is the choice of an information disclosure policy that is used to manage individuals’
% vigilance efforts.
% A key departure of our analysis from standard applications of information design is our focus
% on how the government attempts to correct inefficiencies caused by externalities and coordination failure. Additionally, in our model, testing generates individuals’ types—i.e., non-tested
% and tested-negative—which, in turn, influence individuals’ behavior. Finally, individuals can take
% continuous vigilance efforts based on their testing status, instead of the usual binary-action framework used in models of persuasion. This feature allows us to provide a comprehensive account of
% the role of strategic complementarity and substitutability in the design of the optimal policy.
% Overview of the results Our results reveal that the optimal information disclosure policy can
% be passive, i.e., fully revealing, or involve obfuscation, driven by three qualitatively different impacts on individuals’ vigilance that the government may be aiming for: (i) smoothing the variation
% of vigilance across different infection rate realizations; (ii) enlarging the set of events for which individuals exert vigilance; and (iii) enlarging the set of events for which individuals’ effort is maximal.
% Methodologically, we adapt techniques developed in Dworczak and Martini (2019) and Dworczak and Kolotilin (2019), writing the expected payoffs of individuals and the government as
% functions of the conditional first and second moments of the infection rate. This approach reveals
% 3
% Electronic copy available at: https://ssrn.com/abstract=3988157
% that, if the government’s payoff function is convex, then full disclosure is optimal (Lemma 2). Intuitively, convexity implies that, on average, variation in interim beliefs of individuals—and their
% corresponding efforts—reduce the ex-ante expected loss associated to contagion and vigilance
% costs.
% For strategic substitutes, we provide simple sufficient conditions for convexity of the government’s payoff function—and hence, for the optimality of full revelation. As exposure risk
% increases, when the infection rate gets closer to one half of the population (where the largest
% exposure risk is attained), the incentives to exert vigilance effort increase, buffering contagion.
% This results in convexity of the government payoff function, provided that the buffering effects
% are not dominated by decreasing returns of effort externalities. Proposition 1 provides the precise
% condition on the magnitude of these effects for convexity to hold.
% When convexity is violated, involving convex combinations of beliefs in the support of the
% distribution of posteriors that arises under full revelation, the optimal information disclosure
% involves obfuscation (Lemma 3). In particular, Proposition 2 provides an optimal information
% policy that applies when the government’s payoff function is concave over some regions. Here, the
% government uses obfuscation to smooth non-tested individuals’ vigilance effort across different
% realizations of the infection rate. By concavity, reducing the variation of individuals efforts across
% different states of the world ex-ante increases the expected payoff of the government.
% For strategic complements, the game played by non-isolated individuals is supermodular and
% exhibits multiple equilibria. Our analysis focuses on the largest equilibria, which involve the highest vigilance effort that can be sustained in equilibrium.3 When the complementarity of effort is
% strong, the equilibria that arise are bang-bang, jumping from inaction (no effort) to frenzy (full
% effort), as exposure risk increases. The optimal policy in this scenario requires to pool intermediate infection rates—which is associated to high exposure risk because there are large fractions
% of both infected and non-infected individuals (Proposition 3).4 Here, obfuscation allows the government to stretch the set of infection rates within which effort is exerted. This is attained by
% pooling intermediate infection rates—for which effort has a high private marginal benefit—with
% more extreme infection rates—for which effort has a low private marginal benefit (not enough to
% make effort worthy under full disclosure).
% 3The other natural alternative would be considering the smallest equlibria; i.e., those involving the smallest
% effort. Typically, as in our leading example, those equilibira involve no effort at all. In that scenario, contagion
% management is better addressed through policies that force behavior, such as lock-downs and curfews (cf. Alvarez
% et al., 2021).
% 4The government may fully disclose extreme infection rates, either low or high, or can pool such states. Either
% way individuals will exert no effort.
% 4
% Electronic copy available at: https://ssrn.com/abstract=3988157
% Finally, when the degree of complementarity is low, the largest equilibrium is not bang-bang,
% and the analysis is qualitatively similar to the case of strategic substitutes. In Proposition 4,
% we provide an optimal information disclosure that arises in the presence of kinks in the payoff
% function of the government. In this case, obfuscation decreases the government expected losses
% by stretching the set of realizations of infection rates for which effort is maximal.

==> Journal_Version/2b_Notation_Table.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex

\section{Notation Table}\label{sec:numberical}
\begin{table}[h]
\caption{Notation}
\begin{tabularx}{\textwidth}{@{}XX@{}}
\toprule
  $\wrr$ & Remote work\\
  $\ws$ & Shared workspace\\
  $\benefit$ & Private benefit from in-person work\\
  $\maximal$ & Maximal value of infectious risk \\
  $\paramspace$ & Domain of the infectious risk, i.e., $[0,\maximal]$ \\
  $\param$ & Parameter to describe risk \\
  $\trueparam$ & Random variable describing the true realized risk \\
  $\dist$ & Distribution from which the true risk parameter is drawn ($\trueparam \sim \dist$; this is common knowledge) \\
  $\priormean$ & Prior mean belief over risk parameter ($\E_{\trueparam\sim\dist}[\trueparam]$)\\
  $\fin$ & remote mass\\
  $z_\theta(i)$\\
  $\I$\\
  $\pi$\\
  $\signal$ & Random variable describing realized signal from chosen mechanism $\pi$\\
  $\popdist$ & Distribtion v \\
  $\popdist^{-1}$ & $\sup\{t: \popdist(t) \leq u\}$ \\
  $\costfxn{\fin}{\param}$ &  \\
  $\costperparam$ & Coefficient on \\
  $\constantcost$ & $\sup\{t: \popdist(t) \leq u\}$ \\
  $\maxcost$ & $\costperparam(0) = \maxcost$ \\
  $H$ & parameter used for mean-preserving contractions $H \preccurlyeq F$\\
  $\final$ & Equilibrium in-person mass\\
  $\posterior{\signal}$ & posterior mean belief upon receiving signal $s$\\
  $\obj$ & Objective function to evaluate outcome given \\
  $\goal$ & Set of desirable outcomes (or correspondence in abuse of notation) for indicator-based objectives\\
  $\mfxn$ & Function from posterior mean belief to remote mass\\
%   Utility function for $v$\\
%   Strategies \\
%   Strategy space \\
%   Critical type \\
%   $\epsilon$ & error bounds\\
%   Lipschitz constants\\
%   Discretized distributions \\
%   Adherence model \\ 
%   Platform utility \\
%   Platform goal itnervals \\
%   Direct mechanism terminology\\
%   R2a tools\\
%   Theorem 5.1 terms\\
\bottomrule
\end{tabularx}
\end{table}

==> Journal_Version/4_-_old_Approximation.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex
\section{State-dependent Preferences}
\label{sec:stateful}

In this section, we consider state-dependent preferences for the planner. We assume that the planner's preference can be modelled with a utility function~$\obj(\fin;\trueparam)$ that expresses the planner's utility when the equilibrium outcome is $\fin$ and the state is $\trueparam$. 

To introduce state-dependence into the set-based model (ref. Sec.~\ref{sec:static_id}), we can consider that preferred range of agent distributions across in-person and remote work varies with the state, as captured by the utility function~$\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{y \in \goal(\trueparam)\}$. In general, this is a correspondence from the state-space~$\paramspace$ to the set of mass distributions preferred by the planner. Here, we consider a \emph{state-dependent set-based preference} modelled as: $\goal(\trueparam) = [a(\trueparam),b(\trueparam)] \subseteq [0,1]$. The choice of $a(\trueparam),b(\trueparam)$ for each value~$\trueparam$ is driven by practical considerations such as how the preferred set of agent occupancies at the workplace vary as a function of the true transmissivity and severity of the disease. For example, the planner may allow a wider range of remote mass under smaller values of state (e.g., more flexibility with regards to in-person mass), but seek to enforce a narrower range with larger values for remote mass when the disease state increases (e.g., remote work necessary for most agents).  

The planner's expected objective $V_{F,\obj}(\pi)$ for a signaling mechanism $\pi = \langle \I, \{z_\param\}_{\param \in \paramspace} \rangle $ then becomes $V_{F,\obj}(\pi) = \mathbb{P}\{\final(i) \in \goal(\trueparam)\}=\mathbb{P}\{\final({\signal}) \in [a(\trueparam),b(\trueparam)]\}$, where $\final({\signal})$ is the agents' equilibrium response to~$\pi$. Following Prop.~\ref{prop:eqbm_formula_prop_1}, the problem of maximizing planner's objective~\eqref{eqn:gen_objective_stateful} is: 
\begin{align}
        V_{F,h}^* &= \max_{\pi: \langle \I,  \{z_\param\}_{\param \in \paramspace}\rangle} \mathbb{P}\{a(\trueparam) \leq m(\posterior{\signal}) \leq b(\trueparam)\}. \label{eq:statedependentsetobj}
\end{align}

The design problem is more challenging in comparison to Sec. \ref{sec:static_id} due to the fact that the set of preferred equilibrium outcomes depends on the true state; hence it is no longer sufficient to identify preferred posterior means $\posterior{\signal}$. Instead, we must identify both preferred posterior means and states $(\param,\posterior{\signal})$. Consequently, modifying the probability of generating signal $\signal$ when the state is $\param$ (i.e. $z_{\param}(\signal)$) is not straightforward -- any modification in the mechanism to change $\posterior{\signal}$ so that $m( \posterior{\signal})$ moves into $\goal(\param)$ could cause $m( \posterior{\signal})$ to move out of $\goal(\param')$ for some other state $\param'$. Thus, the planner may elect to generate signals in a way that forgoes any utility in a particular realization of the state $\trueparam$ to generate posterior means that are preferred in other realizations of the state $\trueparam$. As a result, the structure of the optimal signalling mechanisms can be more amorphous and are not guaranteed to maintain monotone partitional structure. 

The following example demonstrates that optimal solution to~\eqref{eq:statedependentsetobj} may require pooling of states from disconnected regions of the state-space, even under a simple set-based, state-dependent preference. 
%Thus, optimal mechanism in this setting does not admit a MPS.  
\begin{example}\label{ex:statefulpool}
Let $\dist$ be uniform over $[0,1]$ ($\priormean = 0.5$). Let $\goal(\trueparam)=[m(\frac{1}{3}\trueparam-\epsilon),m(\frac{1}{3}\trueparam+\epsilon)]$ (i.e. $a(\trueparam) = m( \frac{1}{3}\trueparam-\epsilon)$ and $b(\trueparam) = m( \frac{1}{3}\trueparam+\epsilon)$) for some arbitrary small $\epsilon>0$. \\
Then any signaling mechanism with MPS has an objective value no larger than $6\epsilon$. To see this, observe that without loss of generality, any mechanism satisfying MPS generates a signal $s$ over some interval $[t_{j-1}, t_{j}]$ where $t_j > 0$. This mechanism induces a posterior mean~$\posterior{s}=\frac{t_{j-1}+t_{j}}{2}$ for signal~$s$. For any $t_j > 6\epsilon$ and for all $\trueparam \in [t_{j-1}, t_{j}]$ observe that $\frac{t_{j-1}+t_{j}}{2} \geq \frac{t_{j}}{2} > \frac{t_{j}}{3}+\epsilon \geq \frac{\trueparam}{3}+\epsilon$, which implies that $m(\posterior{s}) > b(\trueparam)$. Thus, all such signals do not contribute to planner's objective. This holds for all values of $\trueparam>6 \epsilon$; hence the planner's objective under MPS-based signaling is less than $\P[\trueparam \leq 6 \epsilon] = 6\epsilon$.  

Now consider the mechanism: $\pi^\mathrm{pool} = \langle \I, \{z_\param\}_{\param\in\paramspace}\rangle$ where $\I = \{\mathbf{1},\mathbf{2},\mathbf{3}\}$ and $z_{\theta}(s)$ is as follows:
\begin{align*}
z_\theta(\cdot) = \begin{cases}
& \mathbf{1} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_1\coloneqq[0,0.12]\cup[0.52,0.56]\\
& \mathbf{2} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_2\coloneqq[0.12,0.30]\cup[0.80,0.82]\\
& \mathbf{3} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_3\coloneqq[0,1]\setminus\{\mathcal{S}_1\cup\mathcal{S}_2\}
\end{cases}
\end{align*}
The resulting posterior means are $\posterior{\mathbf{1}} = 0.18, \posterior{\mathbf{2}} = 0.27$ and $\posterior{\mathbf{3}} \approx 0.65$. Hence, for $\trueparam \in [0.54-3\epsilon,0.54+3\epsilon] \subset \mathcal{S}_1$ and $\trueparam \in [0.81-3\epsilon,0.81+3\epsilon] \subset \mathcal{S}_2$, $\pi^\mathrm{pool}$ generates posterior beliefs that induce equilibrium outcomes in $\goal(\trueparam)$. Thus $\pi^\mathrm{pool}$ achieves an objective value of $12\epsilon$, exceeding the performance of any MPS-based mechanism. 
%; therefore, no signalling mechanism with MPS can be optimal for this setting.
\hfill{\vartriangleleft}
\end{example}

The previous example demonstrates that an MPS-based signalling mechanism may not necessarily be optimal with state-dependent preference. Due to the added technical challenge and suboptimality of MPS-based signalling schemes even under this simple state-dependent preference, we now motivate a search for approximately optimal designs. In particular, we develop a computational approach that provides an approximate solution with interval-based signalling structure for two state-dependent preference models: (i) a Lipschitz continuous preference model where the
planner’s utility is jointly Lipschitz in both the remote mass and the true state and (ii) a scaled-capacity preference model where the planner seeks outcomes that
satisfy capacity limits which become progressively restrictive in the state. Our solution approach entails discretizing the continuous distribution $\dist$ (see Sec.~\ref{subsec:discretization_lp}) in order to limit the number of states $\param$ for which we need to consider preferences $\obj(\cdot;\param)$. This reduces the scope of the problem, thereby allowing us to find optimal solutions under this discretization. Particularly, we show that a linear programming algorithm admits an optimal solution for this discretized problem's model of uncertainty. We subsequently use this algorithm in Sec.~\ref{subsec:scaled_capacity} and Sec.~\ref{subsec:lipschitz_continuous} to provide provably approximately optimal solutions for both models of preference (Prop.~\ref{thm:scaled_capacity} and Thm.~\ref{thm:stateful}). Finally, in Sec.~\ref{subsec:numerical}, we numerically assess the quality of the approximate solution against known benchmarks and assess the suboptimality of the approximation as we scale the granularity of the discretization.

\subsection{Discretization Scheme and Linear Programming Formulation}
\label{subsec:discretization_lp}
\begin{figure}[h!]
\centering
% [Distribution of $\dist$ over $\trueparam$]
{\begin{tikzpicture}
    \draw[->] (0,0) -- (\rb+0.5,0);
    \draw[->] (0,0) -- (0,\rb);
    \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$M$};
    \draw[] (0,0) -- (0,-0.25) node[below] {$0$};
    \draw[] (\rb-0.5,\rb-2) node[below] {$F$};
    
    \draw[blue, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{sin(deg(\x))+\x});
    
\end{tikzpicture}}
% [Distribution of discretized distribution $\dist_\delta$]
{\begin{tikzpicture}
    \draw[->] (0,0) -- (\rb+0.5,0);
    \draw[->] (0,0) -- (0,\rb);
    \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$\nu_N$};
    \draw[] (1.8,-0.14) -- (1.8,-0.14) node[below] {$\cdots$};
    \draw[] (0,0) -- (0,-0.15) node[below] {$\nu_1$};
    \draw[] (0.4,0) -- (0.4,-0.15) node[below] {$\nu_2$};
    \draw[] (\rb-0.5,\rb-2) node[below] {$F_\delta$};
    
    \foreach \x in {0,1,...,9} 
    \draw[blue, -, domain=0.4*\x:0.4*\x+0.4, smooth, samples=100, variable=\y] plot ({\y},{sin(deg(0.4*(\x+1)))+0.4*(\x+1)});
\end{tikzpicture}}
\caption{Distribution over $\trueparam$ (left) and discretized distribution $\dist_\delta$ (right).}
\label{fig:discretization_fig}
\end{figure}
Now, we provide a discretization scheme that modifies the distribution $\dist$ over the continuous space $\paramspace$ into a discrete distribution $\dist_\delta$. It turns out that when an optimal design is achieved for this particular distribution, we can argue that a signalling mechanism for the continuous distribution $\dist$ can be mapped from the discrete solution without much loss of planner objective value. In particular, we take a uniform partition of $\paramspace$ with $N \coloneqq M\delta$ intervals $[\frac{j-1}{\delta},\frac{j}{\delta})$ each of length $\frac{1}{\delta}$. Moreover, we assign all the probability mass in the interval to the minimum of that interval $\nu_j \coloneqq \frac{j-1}{\delta}$ (see Fig. \ref{fig:discretization_fig}), and we denote the collection of $\nu_j$ by $\discpspace \coloneqq \{\nu_1, ...,\nu_N\}$.

\begin{definition}
\label{defn:discretized_dist}
The \textit{$\delta$-discretization} $\dist_\delta$ of any continuous distribution $\dist$ is a discrete probability distribution over $\discpspace$ such that $\hat{\theta} \sim \dist_\delta$ has $\mathbb{P}[\hat{\theta} = \nu_j] \coloneqq p_{j} = \dist(\frac{j}{\delta})-F(\frac{j-1}{\delta})$.
\end{definition}

Observe that $\dist_\delta$ does not necessarily have the same mean as $\dist$ since the probability mass of each interval is shifted towards the minimum of the interval. In fact, $\mathbb{E}_{\trueparam \sim \dist}[\trueparam] \geq \mathbb{E}_{\nu \sim \dist_\delta}[\nu]$. 

When the state is distributed according to a discrete distribution, we can computationally derive the optimal design for objectives $\obj$ that have regularity in their dependence over $\fin$. Particularly, this regularity can be achieved by requiring that $\obj$ is locally constant in $\fin$ which subsequently enables the optimal design to require only finitely many signals (i.e. $|\I|<\infty$). The following lemma establishes that if $\obj(\fin;\nu)$ is piecewise constant in $\fin$ then an optimal design can be achieved using linear programming.

\begin{lemma}
\label{lemma:lp_discrete}
Let $\trueparam\sim H$ with $H$ supported over the finite set $\{\nu_1,..,\nu_N\}$ (denote: $p_j \coloneqq \P[\trueparam = \nu_j]=H(\nu_j)-H(\nu_{j-1})$). Suppose that we are given constants $K \in \mathbb{N}$, $\mathbf{y} \in \R^{K+1}$ and $\mathbf{c}\in\R^{N\times K}$ with $y_0 \coloneqq 0  < y_1 < .. < y_{K-1} < y_{K}\coloneqq 1$ such that for all $\nu_j \in\discpspace$ and $\fin \in [y_{k-1},y_k]$, $\obj(\fin;\nu_j) = c_{jk}$.
Then, an optimal design $\pi_{H,\obj}^\ast = \langle \I, \{z_{\param}\}_{\param \in \discpspace} \rangle$ can be constructed from optimal solution $\{z_{ji}^\ast\}$ of the following linear program \textbf{LP($H,\mathbf{y}, \mathbf{c}$)}  by choosing $\I = [K]$ and $z_{\nu_j}(\signal) = 0$ if $p_j = 0$ and $z_{\nu_j}(\signal) = \frac{z_{ji}^\ast}{p_j}$ otherwise for all $\signal \in \I$ and $j \in [N]$.\\
\begin{tagblock}[tagname={\textbf{LP}},content={\label{My first LP Block}}]
    \begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle&\sum_{j=1}^N \sum_{i=1}^{K} c_{ji} z_{ji} &\\
\text{subject to}& \displaystyle&\sum_{i=1}^{N+1}  z_{ji} = p_j,  &j=1 ,\dots, N\\
   &\displaystyle &z_{ji} \geq 0,\hspace{0.5cm} &j=1 ,\dots, N,\quad i=1 ,\dots, K \\
    &\displaystyle m^{-1}(y_{i-1})&\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, &i=1 ,\dots, K \\
    &\displaystyle&\sum_{j=1}^N \nu_j z_{ji} \leq m^{-1}(y_i)\sum_{j=1}^N z_{ji}, &i=1 ,\dots, K
\end{array}
\end{equation*}
\end{tagblock}
\end{lemma}
\begin{proof}

\noindent For the discrete distribution, the optimization (see \eqref{eqn:gen_objective_stateful}) can be reformulated as: 
\begin{align*}
V_{H,\obj}^\ast &= \max_{\langle \{z_\param\}_{\param \in \{\nu_j\}_{j=1}^{N}},\I\rangle} \mathbb{E}[h(m(\posterior{i}),\trueparam)]\\
&= \max_{\langle \{z_\param\}_{\param \in \{\nu_j\}_{j=1}^{N}},\I\rangle} \sum_{j=1}^N \sum_{s\in|\I|} \mathbb{P}\{\signal=s,\trueparam=\nu_j\}\obj(m(\posterior{s}),\nu_j)\\
&= \max_{\langle \{z_\param\}_{\param \in \{\nu_j\}_{j=1}^{N}},\I\rangle} \sum_{j=1}^N \sum_{s\in|\I|} p_j z_{\nu_j}(s)\obj(m(\posterior{s}),\nu_j)
\end{align*}
Analogous to Lemma~\ref{lemma:num_signals_bdd}, the objective value remains unchanged when any two signals $s_1,s_2$ with $\posterior{s_1}, \posterior{s_2} \in [m^{-1}(y_{k-1}),m^{-1}(y_k))$ for any $k \in [K]$ are consolidated to a signal $s$ ($\posterior{s_1} \leq \posterior{s} \leq \posterior{s_2}$). Therefore, we define $\I = [K]$ with $m^{-1}(y_{\signal-1})\leq\posterior{\signal}<m^{-1}(y_\signal)$ for all $\signal \in \I$.
Choosing the parameterization $z_{ji} = p_j z_{\nu_j}(i)$, we can rewrite the above optimization problem as:
\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle&\sum_{j=1}^N \sum_{i=1}^{K} c_{ji} z_{ji} &\\
\text{subject to}& \displaystyle&\sum_{i=1}^{K}  z_{ji} = p_j,  &j=1 ,\dots, N\\
   &\displaystyle &z_{ji} \geq 0,\hspace{0.5cm} &j=1 ,\dots, N,\quad i=1 ,\dots, K \\
    &\displaystyle m^{-1}(y_{i-1})& \leq  \posterior{i} = \frac{\sum_{j=1}^N \nu_j z_{ji}}{\sum_{j=1}^N z_{ji}} \leq m^{-1}(y_i), &i=1 ,\dots, K
\end{array}
\end{equation*}
Expanding the last inequalities we arrive at \textbf{LP($H,\mathbf{y}, \mathbf{c}$)} with optimal solution $\pi_{H,\obj}^\ast$.\qed
\end{proof}

We note that the linear program \textbf{LP}($\dist_\delta,\mathbf{y}, \mathbf{c}$) has $NK$ variables $z_{ij}$. Appealing to the results presented by \cite{vaidya_speeding-up_1989}, the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Thus, \textbf{LP}($\dist_\delta,\mathbf{y}, \mathbf{c}$) has time complexity $O(N^{2.5}K^{2.5})$, i.e. polynomial in the number of partitions to describe the piecewise function ($K$) and the size of the support for the discretized distribution $H$ ($N$).

\subsection{$\epsilon$-optimal Design}
\label{subsec:epsilon_optimal_design}
To generalize the optimal solution obtained from Lemma 4 for the discrete distribution $\dist_\delta$ to the original continuous distributions $\dist$, we seek an \textit{$\epsilon$-optimal} signalling mechanisms $\hat{\pi}$ that satisfies the following definition.

\begin{definition}
\label{defn:eps_approx}
A mechanism $\hat{\pi}$ is $\epsilon$-optimal for a problem instance \eqref{eqn:gen_objective_stateful} defined by distribution $\dist$ over $\paramspace$ and utility function $\obj$ (under $V_{\dist,\obj}$) if $|V_{\dist,\obj}(\hat{\pi}) - V_{\dist,\obj}(\pi^\ast)| \leq \epsilon$.
\end{definition}

Thus, the $\epsilon$-optimal signalling mechanism $\hat{\pi}$ must be \textit{close} to $\pi^\ast$ when evaluated according to the planner's objective 
\textit{in expectation} with the true prior distribution $\dist$. However, the tuples $\pi^\ast$ and $\hat{\pi}$ themselves need not be ``close" and cannot be compared in a straightforward manner. 
% In fact, since the agents' strategic decisions are conditionally independent of the mechanism $\pi$ given the generated posterior mean by Prop.~\ref{prop:eqbm_formula_prop_1}, for state-independent objectives we were able to compare two distinct mechanisms $\pi_1, \pi_2$ by the induced distributions of posterior means $\dist \preccurlyeq H_1, H_2$ alone. However, with state-dependent preferences, $V_{\dist,\obj}^\ast$ crucially depends on the product distribution that the signalling mechanism specifies over $(\trueparam, \posterior{\signal})$. This is clear, since even if the marginals of this product distribution on $\posterior{\signal}$ (i.e. $H_1$ and $H_2$) were identically distributed, the objectives will differ due to the added dependence on $\trueparam$. 

To construct $\hat{\pi}$, our general procedure is to first solve for the optimal solution $\pi_{\dist_\delta,\obj}^\ast = \langle \{z^\delta_{\nu}\}_{\nu \in \discpspace}, \I_\delta \rangle$ under the discrete distribution of state $\dist_\delta$ (Lemma~\ref{lemma:lp_discrete}). We then construct $\hat{\pi}_{\dist_\delta,h} = \langle \{\hat{z}_\param\}_{\param \in \paramspace}, \I_\delta \rangle$ such that for all $j \in [N], \param \in [\nu_{j-1},\nu_j), \signal \in \I_\delta$,  $\hat{z}_\param(\signal) = z^\delta_{\nu_j}(\signal)$. That is, the distribution used to generate signals when in state $\nu_j$
suggested by the discretized optimal solution is applied to the entire 
corresponding interval of states in the continuous adaptation of the mechanism we propose. To bound the quality of $\hat{\pi}_{\dist_\delta,h}$, we consider the unknown true optimal signalling mechanism $\pi_{\dist,\obj}^\ast = \langle \I, \{z^\ast_{\param}\}_{\param \in \paramspace} \rangle$ and another signalling mechanism $\pi_{\dist,h}' = \langle \I, \{z'_\param\}_{\param \in \discpspace \subseteq \paramspace} \rangle$ for the discretized distribution $\dist_\delta$. The mechanism $\pi_{\dist,h}'$ is obtained by modifying the  design by averaging the distributions used to generate signals over the intervals
 where for all $j \in [N], \signal \in \I$:
\begin{align}
\label{eqn:z'}
z'_{\nu_j}(\signal) = \frac{\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} z^\ast_\param(\signal) dF(\param)}{p_j}
\end{align}

\noindent To summarize, the four signalling mechanisms are: 
\begin{itemize}
\item Optimal solution to original design: $\pi_{\dist,\obj}^\ast = \langle \I, \{z^\ast_{\param}\}_{\param \in \paramspace} \rangle$
\item Averaging $\pi_{\dist,\obj}^\ast$ for discretized distribution $\dist_\delta$ (constructed from $\pi_{\dist,\obj}^\ast$): $\pi_{\dist,h}' = \langle \I , \{z'_{\param}\}_{\param \in \paramspace^\delta}\rangle$
\item Optimal solution in Lemma~\ref{lemma:lp_discrete}: $\pi_{\dist_\delta,\obj}^\ast = \langle \I_\delta , \{z^\delta_{\param}\}_{\param \in \discpspace} \rangle$
\item Proposed $\epsilon$-optimal solution (constructed from $\pi_{\dist_\delta,\obj}^\ast$): $\hat{\pi}_{\dist_\delta,\obj} = \langle \I_\delta , \{\hat{z}_\param\}_{\param \in \paramspace} \rangle$
\end{itemize}

To show $\epsilon$-optimality of $\hat{\pi}_{\dist_\delta,\obj}$, it suffices to show that $V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj}) \leq \epsilon$. 
Note that:
\begin{align}
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj})
    &=
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj}) \nonumber \\ 
    &=
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}') + V_{\dist_\delta,\obj}(\pi_{\dist,h}')-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj}) \nonumber \\ 
    &\leq
    \underbrace{V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}')}_{\textbf{(i)}} + \underbrace{V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj})}_{\textbf{(ii)}} \label{eq:i_ii}
\end{align}
The terms in expression (i) and (ii) can be treated separately. The first term is the loss due to averaging the true optimum's signal generation distribution across each discretized interval, and the second term represents the loss incurred by applying the discrete optimum's signal generation distribution across intervals. Following Definition \ref{defn:eps_approx}, bounding both of these terms by $\frac{\epsilon}{2}$ is sufficient to ensure the $\epsilon$-optimality of $\hat{\pi}_{\dist_\delta,h}$.

Observe that in (i), both $\pi_{\dist,\obj}^\ast$ and $\pi_{\dist,h}'$ use an identical set of signals $\I$; in term (ii), both $\pi^\ast_{\dist_\delta,\obj}$ and $\hat{\pi}_{\dist_\delta,\obj}$ use $\I_\delta$. One can conclude by the construction that for each signal $\signal \in \I$ (resp. $\signal\in\I_\delta$) the corresponding signal incidence probabilities $q_{\signal}^\ast$ and $q_{\signal}'$ (resp. $\hat{q}_{\signal}$ and $q_{\signal}^\delta$) are equal across $\pi_{\dist,h}^\ast$ and $\pi_{\dist,h}'$ (resp. $\pi_{\dist_\delta,h}^\ast$ and $\hat{\pi}_{\dist_\delta,h}$). Moreover, in both Lemmas \ref{lemma:posteriors_close_I} and \ref{lemma:posteriors_close_I_delta} (see appendix), we show that the impact of our chosen discretization scheme on the posterior means induced by $\pi_{\dist,\obj}^\ast$ and $\pi_{\dist,h}'$ (i.e., $\posterior{\signal}^\ast$ and $\posterior{\signal}'$ for $\signal \in \I$) can be controlled; similarly for the posterior means induced by $\pi^\ast_{\dist_\delta,\obj}$ and $\hat{\pi}_{\dist_\delta,\obj}$  (i.e., $\posterior{\signal}^\delta$ and $\hat{\posterior{\signal}}$ for $\signal \in \I_\delta$).

Using these results, our strategy will be to bound the two terms in \eqref{eq:i_ii} (or corresponding terms suitably adapted to problem instance). 


\subsection{Lipschitz-Continuous Preferences}
\label{subsec:lipschitz_continuous}
We consider a planner with preferences modelled by a real-valued function $\obj(\fin;\trueparam)$ such that $\obj:[0,1]\times\paramspace\rightarrow\R$. We assume that the function is doubly-Lipschitz across both the remote mass and the true state.\footnote{Recall, a real function $f:\Omega \rightarrow \R $ is $\eta$-Lipschitz continuous if for all $\omega_1, \omega_2 \in \Omega$, $|f(\omega_1)-f(\omega_2)| \leq \eta |\omega_1-\omega_2|$.}
This allows us to model the preferences of planners who face trade-offs between controlling disease transmissivity and allowing social activity. The authors in~\cite{de_vericourt_informing_2021} provide one such example, but our model of doubly-Lipschitz continuous $\obj$ allows for much richer preferences. 

Recall that Lemma \ref{lemma:lp_discrete} requires a piecewise constant objective function $\obj$ (i.e., not Lipschitz continuous). Still, we can use that result to develop an $\epsilon$-optimal solution for the discretized problem. To achieve this, we approximate our  Lipschitz objective $\obj(\cdot, \param)$ for each value of $\param \in \paramspace$ by a piecewise constant function $\obj_\tau$, where $\tau$ is another discretization parameter. Precisely, for a fixed $\tau$, we create uniform intervals of length $\frac{1}{\tau}$ over $[0,1]$ with the discretized function taking a constant value over each interval equal to the average of the minimum and maximum over this interval. 
\begin{definition}
The \textit{$\tau$-discretization} $\obj_\tau$ of any continuous function $\obj:[0,1]\times\param\rightarrow \R$ is a piecewise constant function such that for all $k \in [\tau], \param\in\paramspace,x \in[\frac{k-1}{\tau},\frac{k}{\tau})$:
\begin{align*}
    h_\tau(x,\param) = \frac{\min_{x\in[\frac{k-1}{\tau},\frac{k}{\tau}]}h(x,\param)+\max_{x\in[\frac{k-1}{\tau},\frac{k}{\tau}]}h(x,\param)}{2} 
\end{align*}
\end{definition}

Consequently, we can solve for $\pi_{\dist_\delta,\obj_\tau}^\ast$ using the linear program in Lemma \ref{lemma:lp_discrete} and adapt that solution to a continuous signalling mechanism $\hat{\pi}_{\dist_\delta,\obj_\tau}$ as described above (ref. Sec. \ref{subsec:epsilon_optimal_design}). We argue that, subject to regularity on the distribution of agents' value of in-person work and the Lipschitz continuity, this solution $\hat{\pi}_{\dist_\delta,\obj_\tau}$ is $\epsilon$-optimal (ref. Definition \ref{defn:eps_approx}) and hence achieves an objective $\epsilon$-close to that of $\pi_{\dist,\obj}^\ast$. 

\begin{theorem}\label{thm:stateful}
Let $\obj(\fin; \trueparam)$ be uniformly $\eta_{1}$-Lipschitz for all $\trueparam \in \paramspace$ and uniformly $\eta_{2}$-Lipschitz for all $\fin \in [0,1]$. Then, if $\popdist$ is continuously differentiable with $0 < \frac{d\popdist}{dv} \leq \kappa$\footnote{This condition is justified by the fact that highly concentrated distribution $G$ can lead to a high sensitivity of equilibrium mass of remote agents to the induced posterior means, thus making approximation difficult.}, the signalling mechanism $\hat{\pi}_{\dist_\delta,\obj_\tau}$ constructed from $\pi_{\dist_\delta,\obj_\tau}^\ast$ (Lemma \ref{lemma:lp_discrete} and Sec. \ref{subsec:epsilon_optimal_design}) is $\epsilon$-optimal for $\delta > \frac{4\eta_{2} +4\eta_{1} \kappa}{\epsilon}$, $\tau > \frac{2\eta_{1}}{\epsilon}$. 
\end{theorem}
\begin{proof}
Observe that we aim to bound $V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau})$. Following \eqref{eq:i_ii}, observe that:
\begin{align}
V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau})
    % &=
    % V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau}) \nonumber \\ 
    % &=
    % V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}') + V_{\dist_\delta,\obj}(\pi_{\dist,h}')-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau}) \nonumber \\ 
    &\leq
    \underbrace{V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}')}_{\textbf{(i)}} + \underbrace{V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau})}_{\textbf{(ii)}} \label{eq:i_ii_iii}
    \end{align}
The proof proceeds in two parts - bounding terms \textbf{(i)} and \textbf{(ii)} from \eqref{eq:i_ii_iii}. To do this, we refer to Lemma \ref{lemma:m_lipschitz} (see appendix) which establishes the $C\kappa$-Lipschitz continuity of the remote-mass function $m(\cdot)$.

Next, we recall from Prop. \ref{prop:eqbm_formula_prop_1} that the equilibrium remote mass induced by any signaling mechanism is a function of the induced posterior mean. Hence, from 
Lemma \ref{lemma:m_lipschitz} and the conditions of the theorem, we can conclude that planner's objective function $\obj(m(\posterior{\signal}), \trueparam)$ is uniformly Lipschitz continuous in the induced posterior mean.  
\begin{lemma}
\label{lemma:h_lipschitz_posterior}
$\obj(m(\posterior{\signal}),\trueparam)$ is uniformly $C\kappa\eta_{1}$-Lipschitz in $\posterior{\signal}$.
\end{lemma}
\begin{subproof}
This is immediate by the conservation of Lipschitz continuity under composition.
\end{subproof}

We can now analyze (i):
\begin{align*}
       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}') &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z^\ast_{\param}}[\obj(m(\posterior{\signal}); \param^\ast)] - \mathbb{E}_{\param' \sim \dist_\delta, \signal \sim 
       \hat{z}_{\param'}}[\obj(m(\posterior{\signal}'); \param')] \\
       &= \sum_{i \in \I}\int_{\param \in \paramspace}\obj(m(\posterior{\signal}); \param) z_{\param}(i) dF(\param) - \sum_{i \in \I}\sum_{\nu \in \paramspace^\delta}\obj(m(\posterior{\signal}'); \nu) p_\nu z_{\nu}(i)  \\
       % &= \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}); \param) z_{\param}(i) d\dist(\param) - \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}'); \nu) z_{\nu_k}(i)d\dist(\param)  \\
       &= \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}); \param) z_{\param}(i) d\dist(\param) - \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}'); \nu_k) z_{\nu_k}(i) d\dist(\param) \Big) \\
        &\stackrel{\eqref{eqn:z'}}{=} \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big(\obj(m(\posterior{\signal}); \param) -\obj(m(\posterior{\signal}'); \nu_k)\big)z_{\param}(i) d\dist(\param) \Big) \\
        \intertext{By Lemma \ref{lemma:posteriors_close_I} and Lemma \ref{lemma:h_lipschitz_posterior} and since $|\nu_k-\param| < \frac{1}{\delta}$ for all $\param \in [\frac{k-1}{\delta},\frac{k}{\delta}]$:}
        &\leq \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big(\obj(m(\posterior{\signal}); \nu_k) -\obj(m(\posterior{\signal}'); \nu_k)+\frac{\eta_{2}}{\delta}\big)z_{\param}(i) d\dist(\param) \Big) \\
         &\leq \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\big(\frac{C\kappa\eta_{1}}{\delta}+\frac{\eta_{2}}{\delta}\big)z_{\param}(i) d\dist(\param) \Big)  \\
         &= \frac{C\kappa\eta_{1}}{\delta}+\frac{\eta_{2}}{\delta} \\
         &< \frac{\epsilon}{2}
\end{align*}
We can analogously simplify expression (ii) using the same decomposition. 
\begin{align*}
       V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z^\ast_{\param}}[\obj(m(\posterior{\signal}); \param^\ast)] - \mathbb{E}_{\param' \sim \dist_\delta, \signal \sim 
       \hat{z}_{\param'}}[\obj(m(\posterior{\signal}'); \param')] \\
       &= \sum_{i \in \I}\int_{\param \in \paramspace}\obj(m(\posterior{\signal}); \param) z_{\param}(i) dF(\param) - \sum_{i \in \I}\sum_{\nu \in \paramspace^\delta}\obj(m(\posterior{\signal}'); \nu) p_\nu z_{\nu}(i)  \\
       % &= \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}); \param) z_{\param}(i) d\dist(\param) - \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}'); \nu) z_{\nu_k}(i)d\dist(\param)  \\
       &= \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}); \param) z_{\param}(i) d\dist(\param) - \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\obj(m(\posterior{\signal}'); \nu_k) z_{\nu_k}(i) d\dist(\param) \Big) \\
        &= \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big(\obj(m(\posterior{\signal}); \param) -\obj(m(\posterior{\signal}'); \nu_k)\big)z_{\param}(i) d\dist(\param) \Big) \\
        \intertext{By Lemma \ref{lemma:posteriors_close_I} and Lemma \ref{lemma:h_lipschitz_posterior} and since $|\nu_k-\param| < \frac{1}{\delta}$ for all $\param \in [\frac{k-1}{\delta},\frac{k}{\delta}]$:}
        &\leq \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big(\obj(m(\posterior{\signal}); \nu_k) -\obj(m(\posterior{\signal}'); \nu_k)+\frac{\eta_{2}}{\delta}\big)z_{\param}(i) d\dist(\param) \Big) \\
         &\leq \sum_{i \in \I}\sum_{k=1}^{N}  \Big(\big(\frac{C\kappa\eta_{1}}{\delta}+\frac{\eta_{2}}{\delta}\big)z_{\param}(i) d\dist(\param) \Big)  \\
         &= \frac{C\kappa\eta_{1}}{\delta}+\frac{\eta_{2}}{\delta} \\
         &< \frac{\epsilon}{2}
\end{align*}
Hence, $V_{\dist,\obj}(\pi^\ast_{\dist,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau}) \leq \epsilon$ and thus $\hat{\pi}_{\dist_\delta,\obj_\tau}$ is $\epsilon$-optimal. \qedsymbol
\end{proof}

As mentioned before, the computation of $\hat{\pi}_{\dist_\delta,\obj_\tau}$ requires the solution of \textbf{LP} with $O(\delta \tau)$ variables since there are $\tau$ components to the piecewise-constant objective and the distribution's support is of size $\delta$. We can conclude the time complexity of \textbf{LP} is $O(M^{2.5}\frac{\eta_{1}^5\eta_{2}^{2.5} \kappa^{2.5}}{\epsilon^5})$.
% which can be upper bounded by $O(\frac{(\kappa \eta_{1}^2+\eta_{2}\eta_{1})^{2.5}}{\epsilon^5})$.



\subsection{Scaled-Capacity Preferences}
\label{subsec:scaled_capacity}
Consider a planner with preferences modelled by $\obj(\fin;\trueparam)$ and a correspondence of sets $\goal(\trueparam) = [a(\trueparam),1]$ for a weakly increasing function $a: \paramspace \rightarrow [0,1] $ such that $\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{y \in \goal(\trueparam)\} = \mathbb{I}\{y \geq a(\trueparam)\}$. Hence, under these preferences, the planner is willing to accept size distributions where the remote mass exceeds (in-person mass falls below) some threshold that gets larger (smaller) as $\trueparam$ increases. We refer to this setting as \emph{scaled capacity preferences}. This family of preferences is driven by the practical considerations of agent occupancies at the workplace that get more restrictive as the true disease severity and risk of community disease spread from the disease increases. Observe that this is an example of state-dependent set-based preference as described in Eq.~\eqref{eq:statedependentsetobj} where $b(\param) = 1$ for all $\theta$.

Reformulating~\eqref{eqn:gen_objective_stateful} with Prop.~\ref{prop:eqbm_formula_prop_1}, we can express the objective of the planner as follows: 
\begin{align}
    V_{\dist,\obj}^\ast &= \max_{\langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \mathbb{P}\{\final(i) \in \goal(\trueparam)\} \label{eqn:scaled_capacity_1}\\
    &= \max_{\langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \mathbb{P}\{m(\posterior{i}) \geq a(\trueparam)\} \label{eqn:scaled_capacity_2}
\end{align}

To reflect the progressive strictness of the capacity restriction, we assume that $a$ is a weakly increasing function. For technical convenience, we also assume that this is a step-function so that the capacity limit $a(\param)$ at state $\param$ can only take finitely many values. 

We can likewise achieve an approximation guarantee on the quality of the estimated solution $\hat{\pi}_{\dist_\delta,h}$. Observe that $\obj(\fin, \trueparam) = \mathbb{I}\{\fin \geq a(\trueparam)\}$ is already a piecewise-constant function as necessitated by Lemma \ref{lemma:lp_discrete}. 

\begin{theorem}\label{thm:scaled_capacity}
Suppose there exists $K < \infty, 0 \coloneqq y_0 < y_1 < .. < y_K \coloneqq 1, 0 \leq  a_1 < a_2 < .. < a_K \leq 1, $ such that $a(x) = a_{i}$ is constant for all $x \in [y_{i-1},y_i]$ for each $i \in [K]$. Then, if both $\dist$ and $\popdist$ are continuously differentiable with $0 < \frac{d\dist}{d\param}, \frac{d\popdist}{dv} \leq \kappa$, the solution $\hat{\pi}_{\dist_\delta,\obj}$ constructed from $\pi_{\dist_\delta,\obj}^\ast$ (ref. Lemma \ref{lemma:lp_discrete} and Sec. \ref{subsec:epsilon_optimal_design}) is $\epsilon$-optimal for $\delta > \frac{4K\kappa C'}{\epsilon}$ where $C' = \max\{C,1\}$. 
\end{theorem}
\begin{proof}
Observe that we aim to bound $V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj})$. Modifying Equation \eqref{eq:i_ii}, observe that if we let $g(\fin;\param) = \mathbb{I}\{\fin \geq a(\param)+\frac{C'\kappa}{\delta}\}$ and modify $\pi_{\dist,h}'$ off $\pi_{\dist,\obj}^\ast$:
\begin{align}
V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj}) \leq
\underbrace{V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,g}(\pi_{\dist,g}^\ast)}_{(i)}+\underbrace{V_{\dist,g}(\pi_{\dist,g}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}')}_{(ii)} + \underbrace{V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj})}_{(iii)} \label{eq:i_ii_iii_iv}
    \end{align}
The proof proceeds in three parts - bounding terms \textbf{(i)}, \textbf{(ii)} and \textbf{(iii)} from \eqref{eq:i_ii_iii_iv}. 
Simplifying expression (i):
\begin{align*}
       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,g}(\pi_{\dist,g}^\ast) &\leq V_{\dist_\delta+\frac{1}{\delta},\obj}(\pi_{\dist,\obj}')-V_{\dist_\delta,g}(\pi_{\dist,g}')
\end{align*}
This is equivalent to modifying constants $\nu_j, p_j, m^{-1}(y_i)$ terms in the linear program by $O(\frac{1}{\delta})$. However, there are $O(K\delta)$ variables and terms so this adds constant error. 
\todo[inline]{Previous proof strategy is incorrect for (i). For the uniform distribution $F$ we can upper bound the difference in (i) by the difference between applying $\pi_{F,h}^\ast$ on the distribution supported $[]$.}
Simplifying expression (ii):
\begin{align*}
       V_{\dist,\obj}(\pi_{\dist,g}^\ast)-V_{\dist_\delta,\obj}(\pi_{\dist,h}') &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z^\ast_{\param}}[g(m(\posterior{\signal}^\ast); \param^\ast)] - \mathbb{E}_{\param' \sim \dist_\delta, \signal \sim 
       \hat{z}_{\param'}}[\obj(m(\posterior{\signal}'); \param')] \\
       &= \sum_{i \in \I}\int_{\param \in \paramspace}g(m(\posterior{\signal}^\ast); \param) z^\ast_{\param}(i) dF(\param) 
       - 
       \sum_{i \in \I}\sum_{\nu \in \discpspace}\obj(m(\posterior{\signal}'); \nu) p_\nu z_{\nu}'(i) \\
       &\stackrel{\eqref{eqn:z'}}{=} \sum_{i \in \I}\int_{\param \in \paramspace}g(m(\posterior{\signal}^\ast); \param) z^\ast_{\param}(i) dF(\param) 
       - 
       \sum_{i \in \I}\sum_{j=1}^N \obj(m(\posterior{\signal}'); \nu_j)(\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} dF(\param)) \frac{\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} z^\ast_\param(\signal) dF(\param)}{\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} dF(\param)} \\ 
&\stackrel{\ref{eqn:scaled_capacity_2}}{=} \sum_{i \in \I}\sum_{j=1}^N \int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} \mathbb{I}\{m(\posterior{\signal}^\ast) \geq a(\param)+\frac{C'\kappa}{\delta}\} z^\ast_{\param}(i) dF(\param) 
       - 
       \sum_{i \in \I}\sum_{j=1}^N \mathbb{I}\{m(\posterior{\signal}') \geq a(\nu_j)\}\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} z^\ast_\param(\signal) dF(\param) \\     
&\leq \sum_{i \in \I}\sum_{j=1}^N \int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} \mathbb{I}\{m(\posterior{\signal}^\ast) \geq a(\param)+\frac{C'\kappa}{\delta}, m(\posterior{\signal}') < a(\nu_j)\} z^\ast_{\param}(i) dF(\param)         
        \intertext{By Lemma \ref{lemma:posteriors_close_I} and Lemma \ref{lemma:m_smooth}, it is known that $m(\posterior{i}') + \frac{C'\kappa}{\delta} \geq m(\posterior{i}^\ast)$ for all $i \in \I$:}
        &= \sum_{i \in \I}\sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\param)\} z_{\nu_{j-1}}^\delta(i)  d\dist(\param) + \sum_{i \in \I}\int_{\paramspace} \mathbb{I}\{m(\posterior{\signal}^\ast) - \frac{C'\kappa}{\delta} \geq a(\param) > m(\posterior{\signal}')\} z^\ast_{\param}(i) dF(\param)\\
        &= \sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\param)\} d\dist(\param) \\
        &\leq \sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\nu_j)\} d\dist(\param)  \\ 
        &\leq \sum_{j=1}^{N}\mathbb{I}\{a(\nu_{j-1})\neq a(\nu_j)\} \kappa \frac{1}{\delta} \\ 
         &= \frac{2K \kappa}{\delta}\\
         &\leq \frac{\epsilon}{2}
\end{align*}
We can also simplify expression (iii) using the same decomposition. 
\begin{align*}
V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj}) &= \mathbb{E}_{\param' \sim \dist_\delta, \signal \sim 
       z_{\param}^\delta}[\obj(m(\posterior{\signal}'); \param')] - \mathbb{E}_{\param^\ast \sim \dist, i \sim \hat{z}_{\param}}[\obj(m(\posterior{\signal}); \param^\ast)] \\
       &= \sum_{i \in \I}\sum_{\nu \in \paramspace^\delta}\obj(m(\posterior{\signal}^\delta); \nu) p_\nu z_{\nu}^\delta(i) - \sum_{i \in \I}\int_{\param \in \paramspace}\obj(m(\hat{\posterior{\signal}}); \param) \hat{z}_{\param}(i) dF(\param) \\
       &=\sum_{i \in \I}\sum_{j=1}^{N}\mathbb{I}\{m(\posterior{i}^\delta)\geq a(\nu_{j-1})\} (\int_{\nu_{j-1}}^{\nu_j} d\dist(\param)) z_{\nu_{j-1}}^\delta(i) - \sum_{i \in \I}\int_{\param \in \paramspace} \mathbb{I}\{m(\hat{\posterior{i}})\geq a(\param)\}\hat{z}_{\param}(i) dF(\param) \\
       &=\sum_{i \in \I}\sum_{j=1}^{N}(\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{m(\posterior{i}^\delta)\geq a(\nu_{j-1})\}z_{\nu_{j-1}}^\delta(i)  d\dist(\param))  - \sum_{i \in \I} \sum_{j=1}^{N} \int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{m(\hat{\posterior{i}})\geq a(\param)\}\hat{z}_{\param}(i) dF(\param) \\       
       &=\sum_{i \in \I}\sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{m(\posterior{i}^\delta)\geq a(\nu_{j-1})\} z_{\nu_{j-1}}^\delta(i) 
 d\dist(\param)  - \sum_{i \in \I} \sum_{j=1}^{N} \int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{m(\hat{\posterior{i}})\geq a(\param)\}z_{\nu_{j-1}}^\delta(i)  dF(\param) \\  
&\leq \sum_{i \in \I}\sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{m(\posterior{i}^\delta)\geq a(\nu_{j-1}), m(\hat{\posterior{i}})< a(\param)\} z_{\nu_{j-1}}^\delta(i)  d\dist(\param)\\   
&\leq \sum_{i \in \I}\sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\param)\} z_{\nu_{j-1}}^\delta(i)  d\dist(\param) + \sum_{i \in \I}\sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{m(\posterior{i}^\delta)\geq a(\nu_{j-1})> m(\hat{\posterior{i}})\} z_{\nu_{j-1}}^\delta(i)  d\dist(\param)\\  
        \intertext{By Lemma \ref{lemma:posteriors_close_I} and Lemma \ref{lemma:m_smooth}, it is known that $m(\hat{\posterior{i}}) \geq m(\posterior{i}^\delta)$ for all $i \in \I$:}
        &= \sum_{i \in \I}\sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\param)\} z_{\nu_{j-1}}^\delta(i)  d\dist(\param) \\
        &= \sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\param)\} d\dist(\param) \\
        &\leq \sum_{j=1}^{N}\int_{\nu_{j-1}}^{\nu_j} \mathbb{I}\{a(\nu_{j-1})\neq a(\nu_j)\} d\dist(\param) \\ 
        &\leq \sum_{j=1}^{N}\mathbb{I}\{a(\nu_{j-1})\neq a(\nu_j)\} \kappa \frac{1}{\delta}\\ 
         &= \frac{2K \kappa}{\delta} \\
         &\leq \frac{\epsilon}{2}
\end{align*}
Hence, $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}_{\dist_\delta,\obj_\tau}) \leq \frac{\epsilon}{2}$. Combining both parts we achieve the statement of the theorem. \qedsymbol
\end{proof}

\input{Journal Version/case_study.tex}

==> Journal_Version/TO_DO_check.tex <==
SA_Approximation

%!TEX root = Opt_Info_Provision_Hybrid.tex
\newpage
\section{State-dependent Preferences}
%!TEX root = Opt_Info_Provision_Hybrid.tex
\label{sec:stateful}

In this section, we consider a class of state-dependent preferences for the planner. Here the planner's preferred range of agent distributions across in-person and remote work may vary with the state, as captured by the utility function~$\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{y \in \goal(\trueparam)\}$. In general, this is a correspondence from the state-space~$\paramspace$ to the set of mass distributions preferred by the planner. In contrast to Sec.~\ref{sec:static_id} where the planner's preference was captured by a union of state-independent closed intervals, we model a \emph{state-dependent set-based preference} as: $\goal(\trueparam) = [a(\trueparam),b(\trueparam)] \subseteq [0,1]$. Here, the choice of $a(\trueparam),b(\trueparam)$ for each value~$\trueparam$ is driven by practical considerations such as how the preferred set of agent occupancies at workplace vary as a function of the true transmissivity and severity of the disease. For example, the planner may allow a wider range of remote mass under smaller values of state (e.g., more flexibility with regards to in-person mass), but likely enforce a narrower range with larger values for remote mass when the disease state increases (e.g., remote work necessary for most agents).  

The planner's expected objective $V_{F,\obj}(\pi)$ for a signaling mechanism $\pi = \langle \I, \{z_\param\}_{\param \in \paramspace} \rangle $ then becomes $V_{F,\obj}(\pi) = \mathbb{P}\{\final(i) \in \goal(\trueparam)\}=\mathbb{P}\{\final({\signal}) \in [a(\trueparam),b(\trueparam)]\}$, where $\final({\signal})$ is the agents' equilibrium response to~$\pi$. Following Prop.~\ref{prop:eqbm_formula_prop_1}, the problem of maximizing planner's objective~\eqref{eqn:gen_objective_stateful} is: 
\begin{align}
        V_{F,h}^* &= \max_{\pi: \langle \I,  \{z_\param\}_{\param \in \paramspace}\rangle} \mathbb{P}\{a(\trueparam) \leq m(\posterior{\signal}) \leq b(\trueparam)\}. \label{eq:statedependentsetobj}
\end{align}

The design problem posed in Equation~\eqref{eq:statedependentsetobj} is categorically more complex than those posed in Section \ref{sec:static_id}. Intuitively this is clear because now that the set of preferred equilibrium outcomes also depends on the true state, one cannot alone identify preferred posterior means $\posterior{\signal}$, but we must identify preferred tuples of posterior means and state $(\param,\posterior{\signal})$. Consequently, modifying the probability of generating $\signal$ when the state is $\param$ (i.e. $z_{\param}(\signal)$) is not straightforward since any such modification to change $\posterior{\signal}$ so that $m( \posterior{\signal})$ moves into $\goal(\param)$ could cause $m( \posterior{\signal})$ to move out of $\goal(\param')$ for some other state $\param'$. 

The following example demonstrates that optimal solution to~\eqref{eq:statedependentsetobj} may require pooling of states from disconnected regions of the state-space, even under a simple set-based preference. 
%Thus, optimal mechanism in this setting does not admit a MPS.  
\begin{example}\label{ex:statefulpool}
Let $\dist$ be uniform over $[0,1]$ ($\priormean = 0.5$). Let $\goal(\trueparam)=[m(\frac{1}{3}\trueparam-\epsilon),m(\frac{1}{3}\trueparam+\epsilon)]$ (i.e. $a(\trueparam) = m( \frac{1}{3}\trueparam-\epsilon)$ and $b(\trueparam) = m( \frac{1}{3}\trueparam+\epsilon)$) for some arbitrary small $\epsilon>0$. \\
Then any signaling mechanism with MPS has an objective no larger than $6\epsilon$. To see this, observe that without loss of generality, any mechanism satisfying MPS generates a signal $s$ over some interval $[t_{j-1}, t_{j}]$ where $t_j > 0$. This mechanism subsequently induces a posterior mean~$\posterior{s}=\frac{t_{j-1}+t_{j}}{2}$ for signal~$s$. For any $t_j > 6\epsilon$ and for all $\trueparam \in [t_{j-1}, t_{j}]$ observe that $\frac{t_{j-1}+t_{j}}{2} \geq \frac{t_{j}}{2} > \frac{t_{j}}{3}+\epsilon \geq \frac{\trueparam}{3}+\epsilon$, which implies that $m(\posterior{s}) > b(\trueparam)$. Thus, all such signals~$s$ do not contribute to planner's objective. This holds for all values of $\trueparam>6 \epsilon$; hence the planner's objective under MPS-based signaling is less than $\P[\trueparam \leq 6 \epsilon] = 6\epsilon$.  

Now consider the mechanism: $\pi^\mathrm{pool} = \langle \I, \{z_\param\}_{\param\in\paramspace}\rangle$ where $\I = \{\mathbf{1},\mathbf{2},\mathbf{3}\}$ and $z_{\theta}(s)$ is as follows:
\begin{align*}
z_\theta(\cdot) = \begin{cases}
& \mathbf{1} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_1\coloneqq[0,0.12]\cup[0.52,0.56]\\
& \mathbf{2} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_2\coloneqq[0.12,0.30]\cup[0.80,0.82]\\
& \mathbf{3} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_3\coloneqq[0,1]\setminus\{\mathcal{S}_1\cup\mathcal{S}_2\}
\end{cases}
\end{align*}
The resulting posterior means are $\posterior{\mathbf{1}} = 0.18, \posterior{\mathbf{2}} = 0.27$ and $\posterior{\mathbf{3}} \approx 0.65$. Hence, for $\trueparam \in [0.54-3\epsilon,0.54+3\epsilon] \subset \mathcal{S}_1$ and $\trueparam \in [0.81-3\epsilon,0.81+3\epsilon] \subset \mathcal{S}_2$, $\pi^\mathrm{pool}$ generates posterior beliefs that induce equilibrium outcomes in $\goal(\trueparam)$. Thus $\pi^\mathrm{pool}$ achieves an objective value of $12\epsilon$, exceeding the performance of any MPS-based mechanism. 
%; therefore, no signalling mechanism with MPS can be optimal for this setting.
\end{example}

This example shows that pooling the states non-sequentially may be required at optimality. This also verifies that it is not necessary that a mechanism with MPS will be optimal under this model of planner preferences. 

Consequently, due to the described added complexity and suboptimality of signalling schemes with MPS, we instead search for approximately optimal designs. 

We define a discretization of the continuous
distribution over state and identify solutions for the discretized distribution. We then introduce two
models of preference: (i) a scaled-capacity preference model where the planner seeks outcomes that
satisfy state-dependent capacity limits and (ii) a Lipschitz continuous preference model when the
planner’s utility is jointly Lipschitz in both the remote mass and the true state. We provide algorithms
that admit approximately optimal solutions for both models of preference in Propositions 4 and 5
respectively. We finally analytically and numerically assess the quality of the approximate solution our
algorithm produces.
%so optimal design is too technically challenging to tackle directly
%The example demonstrates that pooling the states non-sequentially may be required so optimal design is too technically challenging to tackle directly. 

In the following subsections, we will seek \textit{approximations} to the optimal design that can be efficiently derived computationally.

Motivated by practical considerations, we consider a \textit{scaled-capacity preference} model, in which the capacity limits at workplace facilities are state-dependent; in particular, they get progressively tighter as transmissivity and severity of the disease increases. In Prop.~\ref{prop:stateful} we provide a computational approach that guarantees an approximately optimal signaling mechanism for the scaled capacity preference model. This approach is generalizable to settings in which the planner's utility cannot be captured by a set-based preference, but rather expressed as a function of the agents’ size distribution and the state. 

% In this section, we consider a setting under which the planner maintains a model of preferences over the
% size distribution of agents across in-person and remote work that also \textit{may vary} as a function of the state. We first demonstrate through an example that optimal design with MPS is no longer guaranteed under this setting as pooling states from disconnected regions of the state space is necessary to produce optimal solutions for certain objectives. We then introduce a \textit{scaled-capacity} preference model where the planner seeks outcomes that satisfy state-dependent capacity limits. We provide an approximately optimal solution in Proposition \ref{prop:stateful}. We then leverage the insights of this computational approach to address the general setting when the planner’s utility is jointly Lipschitz in both the remote mass and the true state. We finally analytically and numerically assess the quality of the approximate solution our algorithm produces. 
\subsection{Discretization Procedure and Linear Programming Formulation}


\subsection{Scaled-Capacity Objectives}
\label{sec:scaled_capaci}
% \begin{figure}[h]
% \centering     %%% not \center
% \subfigure[Goal sets for stateful objective when $\K = N = 2$ ($\nu_1 < \nu_2$).]{\label{fig:a}\includegraphics[width=40mm]{img/stateful}}
% \subfigure[A more general nested structure of goal sets. ]{\label{fig:b}\includegraphics[width=40mm]{img/nested}}
% \end{figure}
% \noindent In this section, we consider a stateful scaled capacity objective $\{\goal(\param)\}_{\param \in \paramspace}$ that is defined by a collection of sets $\goal(\param) = \{\fin: \|\fin\| \geq b(\param)\}$ for some increasing function $b(\cdot)$ in the domain $\paramspace$. Such sets are practically relevant because they model a capacity limit on in-person work that gets more stringent as the infectious risk increases.

% \noindent To proceed with analyzing the stateful case, for some $N > 0$ we restrict $\paramspace \coloneqq \{\nu_1, \nu_2, .., \nu_N\}$ with $0 < \nu_1 < .. < \nu_N$. We denote $\mathbb{P}[\param = \nu_i] = p_i$ for all $i \in [N]$. To simplify notation, we also denote $b(\nu_i) = b_i$ for all $i \in [N]$ where $b_i$ is strictly increasing in $i$; see Fig. \ref{fig:a}. 

% \noindent Using \eqref{eqn:objective_stateful}, we can express the objective of the planner by: 
% \begin{align}
%     V^* &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \mathbb{P}\{\final(i) \in \goal(\nu)\} \\
%      &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_\nu(i) \mathbb{I}\{\final(i) \in \goal(\nu_j)\}  \label{eqn:stateful_a}
% \end{align}
% As with the stateless design, $\final(i)$ only depends on the induced posterior mean $\param_i$ and $\final(i) \in \goal(\nu_j)$ if and only $\final(i) \in \goal(\nu_j) \cap \curve$. The latter follows if and only if $b_j \leq \|\final(i)\| \leq 1$ or $0 \leq m(\param_i) \leq 1-b_j$. Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, observe that this corresponds to $\param_i \in [\gamma_j,\infty)$ for some constants $\gamma_j$ that are strictly increasing in $j$. For completeness, we denote $\gamma_0 = 0$ and $\gamma_{N+1} = \infty$.
% We can then reformulate \eqref{eqn:stateful_a} as follows:
% \begin{align}
%     V^* &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{\gamma_j \leq \param_i < \infty\} \label{eqn:stateful_b}
% \end{align}
% We highlight that despite these simplifications, our analysis is extensible to other practically relevant objectives aside from the scaled capacity objective. Suppose that the desirable sets satisfy Assumption A1 and are also (i) nested with $\goal(\nu_{i+1})\subset \goal(\nu_{i})$ for all $i \in [N-1]$, and (ii) half-bounded with $\init \in \goal(\nu_i)$ for all initial mass vectors $\init$ and all $i \in [N]$; see Fig. \ref{fig:b}. Then we arrive at an identical formulation to \eqref{eqn:stateful_b} since the minimal posterior mean beliefs for the agent outcomes to enter each $\goal(\nu_j)$ is an increasing sequence $\gamma_j$.

% \noindent Using a similar reduction as in stateless design, we can restrict our mechanism to induce a single posterior mean $\param_i$ to lie in each interval $[\gamma_{i-1},\gamma_{i})$ for $i \in [N+1]$. These $\param_i$ consequently induce equilibrium outcomes that lie in $\goal(\nu_j)$ if and only if $\param_i \geq \gamma_j$ or equivalently $i \geq j+1$. This implies that an optimal mechanism can be described by at most $N+1$ signals. In the proposition below, we provide a linear program (LP) to compute an optimal signalling mechanism for the stateful scaled capacity objective. We first introduce the LP:
% \begin{align*}
%     V^* &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% \begin{prop}
% \label{prop:stateful}
% The optimal value $V^*$ to the above LP is equal to $\max_{\pi: \langle \{z_\param\}_{\param \in \paramspace},\I\rangle} V(\pi)$ in \eqref{eqn:objective_stateful} under the stateful scaling capacity objective. For an optimal solution $\{z_{ji}^*\}_{j \in [N], i\in[N+1]}$ of the LP, the optimal signalling mechanism is given by $\pi^* = \langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle$ where $\I \coloneqq [N+1]$ and $z_{\nu_j}(i) = \frac{z_{ji}^*}{p_j}$ for all $i \in \I,j \in [N]$. 
% \end{prop}
% Using this result, we can efficiently compute the optimal objective $V^*$ and an optimal signalling mechanism $\pi^*$ in polynomial time. 

% \noindent If the $b_j$ and hence $\goal(\nu_j)$ were all identical, our setting becomes the stateless setting solved by Theorem $\ref{thm:stateless}$. In this special case, all $\nu_j$ correspond to a single $\gamma=\gamma_j$ and only two posterior means $\param_1 < \gamma \leq \param_2$ are required. If $\mu = \sum_{j \in [N]} p_j \nu_j \geq \gamma$ then this corresponds to regime R1 and non-informative mechanism is optimal. If $\mu < \gamma$ this corresponds to regime R4 and likewise we recover a discretized interval-based signalling mechanism over $\I = \{1,2\}$ by solving the LP and we can check that there exists a $\hat{j} \in [N]$ such that for all $j < \hat{j}$, $z_{\nu_j}(1) = 1$ and for all $j > \hat{j}$, $z_{\nu_j}(2) = 1$.  

\noindent Finally, for any mechanism $\pi$, the probability of complying with the capacity limit conditioned on $\param = \nu_j$ can be represented by $V_j(\pi) \coloneqq  \mathbb{P}\{\final(i) \in \goal(\param)|\param=\nu_j\}$. Observe that $V(\pi) = p_j V_j(\pi)$ is a weighted average of the compliance for each possible realization of $\param$. However, practically planners may face significantly more adverse risks of being overcapacitated as the infectiousness increases, and weight compliance heterogeneously across realizations of $\param$. For this slightly more general objective, an optimal signalling mechanism for a different weighted sum $\sum_{j=1}^{N} \alpha_j V_j(\pi)$ for $\alpha_j \geq 0$ can likewise be solved using the linear program above by replacing the objective with $\max_{\{ z_{ji}\}} \sum_{i=j+1}^{N+1} \frac{\alpha_j}{p_j}z_{ji}$.

The previous section demonstrates that generally one cannot expect to find MPS solutions under our model for general objectives, but we consider our second class of objectives which are state-dependent. Namely, we consider a scaling capacity objective where $\goal(\param) = \{y: y \geq b(\param)\}$ for some non-increasing function $b$. 
In this section, we consider stateful goal sets where generally the set of outcomes that the principal seeks to guide equilibrium for the true parameter $\param$ is $\goal(\param)$. In this stateful setting, we cannot reduce the search over $\pi$ by searching over the corresponding direct mechanisms $\mathcal{T}_\pi$. This is because a posterior mean $\param_i$ will induce a specific equilibrium outcome $\final(i)$ but we cannot evaluate whether $\final(i) \in \goal(\param)$ if we only know $\param_i$ and not the true $\param$.

\noindent Observe that each design problem is tailored to an initial population allocation across the groups $\init$. For this particular $\init$, achievable equilibria lie on a one-dimensional manifold as shown in Lemma \ref{lemma:intervals}, so we can decompose the intersection of $\curve$ and each of our goal sets $\goal(\param)$ as the objects of interest. Namely we will impose the following assumptions to be as general as possible: \\
\noindent \textbf{(A2)} $\goal(\param)$ is closed for all $\param$. \\
\noindent \textbf{(A3)} $\goal(\param) \cap \curve = \cup_{i=1}^{P} [a_{i}(\param), b_{i}(\param)]$ for finite $P$, $0 \leq a_i(\param), b_i(\param) \leq 1$ for all $\param$.\\
\noindent \textbf{(A4)} For all $i \in [P]$, $a_i(\cdot),b_i(\cdot)$ are $\eta_1$-Lipschitz. 

\noindent Observe that \textbf{(A3)} can be satisfied if $\goal(\param)$ is convex for all $\param$, but the assumption allows for a more general description. Assumption \textbf{(A4)} while seemingly restrictive merely requires that the goal sets are smooth in $\param$ and that there are no sudden discontinuities. Observe that some of the $P$ intervals where we only assume $P$ is finite can be empty so the shape of the intersection can change significantly as $\param$ increases.

\noindent The following proposition establishes a linear program that is capable of approximating the optimal solution to the information design problem posed in Equation \eqref{eqn:objective_stateful}. We first introduce the following LP:
\begin{align*}
    V^* &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
    &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
    &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
    &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
    &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
\end{align*}

\subsection{Stateful Scaled Capacity Model}
\label{sec:stateful}
\begin{figure}[h]
\centering     %%% not \center
\subfigure[Goal sets for stateful objective when $\K = N = 2$ ($\nu_1 < \nu_2$).]{\label{fig:a}\includegraphics[width=40mm]{img/stateful}}
\subfigure[A more general nested structure of goal sets. ]{\label{fig:b}\includegraphics[width=40mm]{img/nested}}
\end{figure}
\noindent In this section, we consider a stateful scaled capacity objective $\{\goal(\param)\}_{\param \in \paramspace}$ that is defined by a collection of sets $\goal(\param) = \{\fin: \|\fin\| \geq b(\param)\}$ for some increasing function $b(\cdot)$ in the domain $\paramspace$. Such sets are practically relevant because they model a capacity limit on in-person work that gets more stringent as the infectious risk increases.

\noindent To proceed with analyzing the stateful case, for some $N > 0$ we restrict $\paramspace \coloneqq \{\nu_1, \nu_2, .., \nu_N\}$ with $0 < \nu_1 < .. < \nu_N$. We denote $\mathbb{P}[\param = \nu_i] = p_i$ for all $i \in [N]$. To simplify notation, we also denote $b(\nu_i) = b_i$ for all $i \in [N]$ where $b_i$ is strictly increasing in $i$; see Fig. \ref{fig:a}. 

\noindent Using \eqref{eqn:objective_stateful}, we can express the objective of the planner by: 
\begin{align}
    V^* &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \mathbb{P}\{\final(i) \in \goal(\nu)\} \\
     &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_\nu(i) \mathbb{I}\{\final(i) \in \goal(\nu_j)\}  \label{eqn:stateful_a}
\end{align}
As with the stateless design, $\final(i)$ only depends on the induced posterior mean $\param_i$ and $\final(i) \in \goal(\nu_j)$ if and only $\final(i) \in \goal(\nu_j) \cap \curve$. The latter follows if and only if $b_j \leq \|\final(i)\| \leq 1$ or $0 \leq m(\param_i) \leq 1-b_j$. Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, observe that this corresponds to $\param_i \in [\gamma_j,\infty)$ for some constants $\gamma_j$ that are strictly increasing in $j$. For completeness, we denote $\gamma_0 = 0$ and $\gamma_{N+1} = \infty$.
We can then reformulate \eqref{eqn:stateful_a} as follows:
\begin{align}
    V^* &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{\gamma_j \leq \param_i < \infty\} \label{eqn:stateful_b}
\end{align}
We highlight that despite these simplifications, our analysis is extensible to other practically relevant objectives aside from the scaled capacity objective. Suppose that the desirable sets satisfy Assumption A1 and are also (i) nested with $\goal(\nu_{i+1})\subset \goal(\nu_{i})$ for all $i \in [N-1]$, and (ii) half-bounded with $\init \in \goal(\nu_i)$ for all initial mass vectors $\init$ and all $i \in [N]$; see Fig. \ref{fig:b}. Then we arrive at an identical formulation to \eqref{eqn:stateful_b} since the minimal posterior mean beliefs for the agent outcomes to enter each $\goal(\nu_j)$ is an increasing sequence $\gamma_j$.

\noindent Using a similar reduction as in stateless design, we can restrict our mechanism to induce a single posterior mean $\param_i$ to lie in each interval $[\gamma_{i-1},\gamma_{i})$ for $i \in [N+1]$. These $\param_i$ consequently induce equilibrium outcomes that lie in $\goal(\nu_j)$ if and only if $\param_i \geq \gamma_j$ or equivalently $i \geq j+1$. This implies that an optimal mechanism can be described by at most $N+1$ signals. In the proposition below, we provide a linear program (LP) to compute an optimal signalling mechanism for the stateful scaled capacity objective. We first introduce the LP:
\begin{align*}
    V^* &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
    &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
    &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
    &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
    &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
\end{align*}

\begin{prop}
\label{prop:stateful}
The optimal value $V^*$ to the above LP is equal to $\max_{\pi: \langle \{z_\param\}_{\param \in \paramspace},\I\rangle} V(\pi)$ in \eqref{eqn:objective_stateful} under the stateful scaling capacity objective. For an optimal solution $\{z_{ji}^*\}_{j \in [N], i\in[N+1]}$ of the LP, the optimal signalling mechanism is given by $\pi^* = \langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle$ where $\I \coloneqq [N+1]$ and $z_{\nu_j}(i) = \frac{z_{ji}^*}{p_j}$ for all $i \in \I,j \in [N]$. 
\end{prop}
\begin{proof}
\noindent Observe that we can expand the optimization in \eqref{eqn:stateful_b} to include the constraints as follows:
\begin{align*}
    V^* &= \max_{\langle \{z_\nu\}_{\nu \in \Theta},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{c_j \leq \theta_i \leq \infty\} \\
    &\text{s.t. }\sum_{i=1}^{|\I|} z_{\nu_j}(i) = 1, \forall j\in[N] \\
    &\hspace{1cm} 0 \leq z_{\nu_j}(i) \leq 1, \forall i\in |\I|,j\in[N] \\
    &\hspace{1cm}\theta_i = \frac{\sum_{j=1}^N \nu_j p_j z_{\nu_j}(i)}{\sum_{j=1}^N p_j z_{\nu_j}(i)}, \hspace{0.5cm} \forall i \in |\I|
    % &\hspace{1cm}G \succcurlyeq F
\end{align*}
As mentioned, analogous to Lemma \ref{lemma:num_signals_bdd}, if two signals $i_1, i_2$ are such that there exists $\gamma_{j} \leq \theta_{i_1}, \theta_{i_2} < \gamma_{j+1}$, we can merge the signals without loss. Therefore, for each interval $[\gamma_{i-1},\gamma_{i})$ with $i\in [N+1]$, at most one posterior mean need be present so $\I = [N+1]$ with $\theta_i \in [\gamma_{i-1},\gamma_{i})$ for all $i$. 
Reducing by observing that $\theta_i \geq \gamma_j$ for all $i \geq j+1$:
\begin{align}
    V^* &= \max_{\{ z_{\nu_j}(i)\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} p_j z_{\nu_j}(i) \\
    &\text{s.t. }\sum_{i=1}^{N+1}  z_{\nu_j}(i) = 1, \hspace{0.5cm}\forall j\\
    &\hspace{1cm} 0 \leq z_{\nu_j}(i) \leq 1,\hspace{0.5cm} \forall i,j \\
    &\hspace{1cm} \gamma_{i-1} \leq  \frac{\sum_{j=1}^N \nu_j p_j z_{\nu_j}(i)}{\sum_{j=1}^N p_j z_{\nu_j}(i)} \leq \gamma_{i}, \hspace{0.5cm} \forall i\in[N+1]
    % &\sum_{j=1}^N p_j z_{\nu_j}(i) (\theta_i - \nu_j)= 0,\hspace{0.4cm} \forall i \in [N+1]
    % &\sum_{i=1}^{m} (\sum_{j=1}^N p_j z_{\nu_j}(N+1-i))\theta_{N+1-i} \geq \int_0^{\sum_{i=1}^{m} q_{N+1-i}} \dist^{-1}(t)dt\hspace{0.25cm} \forall m \in [N+1]
\end{align}
By renaming $z_{ji} = p_j z_{\nu_j}(i)$ and expanding the final constraint, we arrive at the linear program.\qed
\end{proof}
Using this result, we can efficiently compute the optimal objective $V^*$ and an optimal signalling mechanism $\pi^*$ in polynomial time. 

\noindent If the $b_j$ and hence $\goal(\nu_j)$ were all identical, our setting becomes the stateless setting solved by Theorem $\ref{thm:stateless}$. In this special case, all $\nu_j$ correspond to a single $\gamma=\gamma_j$ and only two posterior means $\param_1 < \gamma \leq \param_2$ are required. If $\mu = \sum_{j \in [N]} p_j \nu_j \geq \gamma$ then this corresponds to regime R1 and non-informative mechanism is optimal. If $\mu < \gamma$ this corresponds to regime R4 and likewise we recover a discretized interval-based signalling mechanism over $\I = \{1,2\}$ by solving the LP and we can check that there exists a $\hat{j} \in [N]$ such that for all $j < \hat{j}$, $z_{\nu_j}(1) = 1$ and for all $j > \hat{j}$, $z_{\nu_j}(2) = 1$.  

\noindent Finally, for any mechanism $\pi$, the probability of complying with the capacity limit conditioned on $\param = \nu_j$ can be represented by $V_j(\pi) \coloneqq  \mathbb{P}\{\final(i) \in \goal(\param)|\param=\nu_j\}$. Observe that $V(\pi) = p_j V_j(\pi)$ is a weighted average of the compliance for each possible realization of $\param$. However, practically planners may face significantly more adverse risks of being overcapacitated as the infectiousness increases, and weight compliance heterogeneously across realizations of $\param$. For this slightly more general objective, an optimal signalling mechanism for a different weighted sum $\sum_{j=1}^{N} \alpha_j V_j(\pi)$ for $\alpha_j \geq 0$ can likewise be solved using the linear program above by replacing the objective with $\max_{\{ z_{ji}\}} \sum_{i=j+1}^{N+1} \frac{\alpha_j}{p_j}z_{ji}$.




\subsection{Numerical Experiments}
% \textcolor{blue}{Outline: create analogous curve for the stateful setting for a discrete distribution - show the improved comparative benefit from stateful signalling in this regime relative to even the stateless setting. Here, we again have a stateful capacity based objective (simple LP solves this).}
\noindent For the stateful capacity case, we highlight a specific instance where we scale-down the in-person capacity limit as the infectious risk increases. Consequently, the minimal posterior mean to induce outcomes in $\goal(\nu_j)$ are represented by $\gamma_j$ that are increasing in $j$. To gain intuition, we choose the specific set of tuples for $N=3$ where $\{p_i\}_{i \in \{1,2,3\}} = (0.3,0.3,0.4), \{\nu_i\}_{i \in \{1,2,3\}} = (0.4,0.6,1.0), \{\gamma_i\}_{i \in \{1,2,3\}} = (0.5, 0.9, 1.2)$ and compare the performance of the optimal mechanism against the same two benchmarks as in the stateless case.
In Fig. \ref{table:stateful_vary_capacity}, we tabulate each information mechanism's performance. Observe that under no information, agents mean belief over $\theta = \mu = \sum_{j=1}^N p_j \nu_j = 0.7$. Since agents receive no signal, the equilibrium outcome is independent of $\theta$ and agents only comply if $\gamma_j < \mu$ which happens with probability $p_1 = 0.3$. Under full information, agents perfectly observe $\theta$, so the outcome is compliant with the limit if and only if $\theta_j \geq \gamma_j$. This occurs with probability $0$ in our example. Thus, the stateful design significantly improves the probability of compliance relative to both benchmarks. We also observe that the stateful design does no worse in this setting than either benchmark in any of the conditional compliance measures $V_j(\pi)$.
\begin{figure}
    \centering
    \begin{tabular}{ |c|c|c|c|c| } 
    \hline
    Information Scheme & $V(\pi)$ & $V_1(\pi)$ & $V_2(\pi)$ & $V_3(\pi)$ \\     
    \hline
    No Information & 0.300 &1& 0& 0 \\ 
    Full Information  & 0.000 & 0& 0 &0 \\ 
    Stateful Design & 0.425 & 1& 0.417 &0 \\ 
 \hline
\end{tabular}
    
    \caption{Comparison of non-informative, fully informative and optimal stateful signalling in terms of the overall probability of compliance and conditional probabilities of compliance. }
    \label{table:stateful_vary_capacity}
\end{figure}
\label{sec:approximation}
In the previous section, we demonstrated that MPS mechanisms can achieve optimal design for particular state-independent objective  functions. However, we also provided state-dependent counterexamples where no MPS mechanism is able to achieve or closely approximate optimal design. 
In this section, we seek a methodology to provide \textit{approximate} optimal design for a general form of state-dependent objective functions. Because we seek a method that will generalize to a general form of objective functions $\obj$, observe that a closed-form description of the optimal signalling mechanism will be difficult to obtain under arbitrary objectives.
% \srs{sentence seems unnecessary - The approach we  produces a signalling mechanism that will \textit{$\epsilon$-approximate} the optimal solution to \eqref{eqn:gen_objective_stateful} by using $O(\frac{1}{\epsilon})$ discrete signals and $O(\frac{1}{\epsilon^2})$ computational complexity.}

% \begin{figure}
%     \centering
%     \input{presentations/stateful_c.tex}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
\noindent Formally, we characterize an $\epsilon$-approximation of the optimal signalling mechanism using the following definition.

The previous example demonstrates that generally one cannot expect to find MPS solutions under our model for general objectives, but we consider our second class of objectives which are state-dependent. Namely, we consider a scaling capacity objective where $\goal(\param) = \{y: y \geq b(\param)\}$ for some non-increasing function $b$. In this section, we consider stateful goal sets where generally the set of outcomes that the principal seeks to guide equilibrium for the true parameter $\param$ is $\goal(\param)$. In this stateful setting, we cannot reduce the search over $\pi$ by searching over the corresponding direct mechanisms $\mathcal{T}_\pi$. This is because a posterior mean $\param_i$ will induce a specific equilibrium outcome $\final(i)$ but we cannot evaluate whether $\final(i) \in \goal(\param)$ if we only know $\param_i$ and not the true $\param$.

\noindent Observe that each design problem is tailored to an initial population allocation across the groups $\init$. For this particular $\init$, achievable equilibria lie on a one-dimensional manifold as shown in Lemma \ref{lemma:intervals}, so we can decompose the intersection of $\curve$ and each of our goal sets $\goal(\param)$ as the objects of interest. Namely we will impose the following assumptions to be as general as possible: \\
\noindent \textbf{(A2)} $\goal(\param)$ is closed for all $\param$. \\
\noindent \textbf{(A3)} $\goal(\param) \cap \curve = \cup_{i=1}^{P} [a_{i}(\param), b_{i}(\param)]$ for finite $P$, $0 \leq a_i(\param), b_i(\param) \leq 1$ for all $\param$.\\
\noindent \textbf{(A4)} For all $i \in [P]$, $a_i(\cdot),b_i(\cdot)$ are $\eta_1$-Lipschitz. 

\noindent Observe that \textbf{(A3)} can be satisfied if $\goal(\param)$ is convex for all $\param$, but the assumption allows for a more general description. Assumption \textbf{(A4)} while seemingly restrictive merely requires that the goal sets are smooth in $\param$ and that there are no sudden discontinuities. Observe that some of the $P$ intervals where we only assume $P$ is finite can be empty so the shape of the intersection can change significantly as $\param$ increases.

\noindent The following proposition establishes a linear program that is capable of approximating the optimal solution to the information design problem posed in Equation \eqref{eqn:objective_stateful}. We first introduce the following LP:
\begin{align*}
    V^* &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
    &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
    &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
    &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
    &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
\end{align*}
\begin{defn}
\label{defn:eps_approx}
A mechanism $\hat{\pi}$ is $\epsilon$-optimal for a problem instance defined by distribution $\dist$ over $\Theta$ and utility function $\obj$ if $|V_{\dist,\obj}(\hat{\pi}) - V_{\dist,\obj}(\pi^*)| \leq \epsilon$.
\end{defn}

Note that on expectation when evaluated by the planner's objective, both an optimal signalling mechanism $\pi^*$ and an \textit{approximately} optimal mechanism $\hat{\pi}$ are necessarily close, but the tuples $\pi^*$ and $\hat{\pi}$ themselves may not behave similarly. Furthermore, since the agents' strategic decisions are conditionally independent on the mechanism given the generated posterior mean, two mechanisms $\pi_1, \pi_2$ can generally be compared by the induced distributions of posterior means $H_1, H_2 \preccurlyeq \dist$. However, recall from \eqref{eqn:gen_objective_stateful} that $V_{\dist,\obj}(\pi_j) = \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[\obj(\final(i), \param)] = \mathbb{E}_{\param \sim \dist, \theta_i \sim H_j}[\obj(m(\param_i), \param)]$ and consequently the objective critically depends on the product distribution that the signalling mechanism specifies over $(\theta, \theta_i)$. However, clearly even if $H_1$ and $H_2$ were identically distributed, the corresponding product distributions may not be. 

The approach we demonstrate to find an approximately optimal solution will be to adapt the present general setting to the linear programming methodology used in Section \ref{sec:stateful} without loss. In order to do this, the distribution over the parameter $\param$ must be discretized to a discrete distribution and the objective must be analogously adapted to be piecewise-constant. The following definition describes a systematic discretization of a general distribution $\dist$ so that the discretization uniformly partitions $\paramspace$ into intervals of length $\frac{1}{\delta}$ and places all the probability on the midpoint of that interval. 
\begin{defn}
The \textit{$\delta$-discretization} $F_\delta$ of any continuous distribution $F$ is a discrete probability distribution over $\{\frac{(2k-1)}{2\delta}\}_{k=1}^{M\delta}$ such that $\hat{\theta} \sim F_\delta$ has $\mathbb{P}[\hat{\theta} = \frac{(2k-1)}{2\delta}] = F(\frac{k}{\delta})-F(\frac{k-1}{\delta})$.
\end{defn}
\begin{figure}
    \centering
    \begin{tikzpicture}
    \draw[->] (0,0) -- (\rb+0.5,0);
    \draw[->] (0,0) -- (0,\rb);
    % \draw[dashed] (\ra,0) -- (\ra,1) node[above] {$a$};
    \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$1$};
    \draw[] (\rb+0.5,-0.25) node[below] {$y$};
    \draw[] (\rb-0.5,\rb-1) node[below] {$\obj(y;\cdot)$};
    
    \draw[red, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{2*sin(deg(\x))+2});
    \draw[red!90,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.9*sin(deg(\x))+1.9});
    \draw[red!80blue!40,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.6*sin(deg(\x))+1.5});
    \draw[red!70blue!30,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.4*sin(deg(\x))+1.2});
    \draw[red!60!blue!40-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.2*sin(deg(\x))+0.9});
    \draw[red!50!blue!50,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{sin(deg(\x))+0.8});
\end{tikzpicture}
    
    \begin{tikzpicture}
    \draw[->] (0,0) -- (\rb+0.5,0);
    \draw[->] (0,0) -- (0,\rb+0.5);
    % \draw[dashed] (\ra,0) -- (\ra,1) node[above] {$a$};
\draw[] (\rb,0) -- (\rb,-0.25) node[below] {$1$};
    \draw[] (\rb+0.5,-0.25) node[below] {$y$};
    \draw[] (\rb-0.5,\rb) node[below] {$\obj(y;\nu)$};
    \draw[dotted,thick,red] (1.6,0) -- (1.3,-0.3) node[below] {$\theta_{s'}$};
    \draw[dotted,thick,red] (1.8,0) -- (2.1,-0.3) node[below] {$\theta_{s''}$};
    % \draw[dashed] (1.0,0) -- (1.0,-1.5) node[below] {$m(\gamma_{i+1})$};
    
    %Right-Hand
    \foreach \x in {1,...,\rb} % <--- my issues
    \draw[thick, fill=red!25] (\x-.5,0) -- (\x-.5,{2*sin(deg(\x-0.25))+2.05}) -- (\x,{2*sin(deg(\x-0.25))+2.05}) -- (\x,0) -- cycle;
    \foreach \x in {1,...,\rb} % <--- my issues
    \draw[thick, fill=green!25] (\x-1,0) -- (\x-1,{2*sin(deg(\x-0.5-0.25))+2.05}) -- (\x-0.5,{2*sin(deg(\x-0.5-0.25))+2.05}) -- (\x-0.5,0) -- cycle;
    
    % %Left-Hand
    % \foreach \x in {\ra,-0.5,...,\rbtwo} % <--- my issues
    % \draw[thick, fill=blue!25] (\x,0) -- (\x,{sin(deg(\x))}) -- (\x+.5,{sin(deg(\x))}) -- (\x+.5,0) -- cycle;
    
    \draw[ultra thick, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{2*sin(deg(\x))+2});
    
\end{tikzpicture}\caption{$\delta$-discretization of $F$ and $\omega$-discretization of $\obj$.}
    \label{fig:discretization}
\end{figure}
Analogously, to adapt a continuous objective function $h(\cdot, \param)$ to a piecewise constant, we can parameterize the discretization by $\omega$ and choose to uniformly create intervals of length $\frac{1}{\omega}$ over $[0,1]$ with the discretized function taking a constant value over each interval equal to the average of the minimum and maximum on this interval. 
\begin{defn}
The \textit{$\omega$-discretization} $h_\omega$ of any continuous function $h:[0,1]\rightarrow \R$ is a piecewise constant function such that for all $k \in [\omega], x \in[\frac{k-1}{\omega},\frac{k}{\omega}]$:
\begin{align*}
    h_\omega(x) = \frac{\min_{x\in[\frac{k-1}{\omega},\frac{k}{\omega}]}h(x)+\max_{x\in[\frac{k-1}{\omega},\frac{k}{\omega}]}h(x)}{2} 
\end{align*}
\end{defn}

Consider the following linear program parameterized by a sequence of parameters $\langle P, Q, \{\alpha_{ji}\}_{i \in [P], j\in[Q]},\{\gamma_{i}\}_{i \in [P]},\{\nu_{j}\}_{j\in[Q]}\rangle$:
\begin{align*}
    V^* &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} \alpha_{ji}z_{ji} \\
    &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
    &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
    &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
    &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
\end{align*}

\noindent To eliminate instances of our problem when the objective is erratically constructed, we impose the following assumptions on the problem setting.

\textbf{Assumptions}
\\
\noindent \textbf{A3} $\popdist$ is continuously differentiable with $0 < \frac{d\popdist}{dv} \leq \eta_\beta$. 

\noindent \textbf{A4} $h(x; \cdot)$ is uniformly $\eta_{h,1}$-Lipschitz

\noindent \textbf{A5} $h(\cdot; \theta)$ is uniformly $\eta_{h,2}$-Lipschitz

\noindent \textbf{A6} $h(x; \theta)$ is jointly differentiably continuous

\begin{theorem}\label{thm:stateful}
Under assumptions A3-A5, the solution $\pi^*(F_\delta,h_\omega)$ for $\delta > \frac{2\eta_{2,h} +2\eta_{1,h} \eta_{\beta}}{\epsilon}$, $\omega > \frac{2\eta_{1,h}}{\epsilon}$ is $\epsilon$-optimal and $\pi^*(F_\delta,z_\omega)$ can be computed using \textbf{LP} with parameters:. 
\end{theorem}
\begin{proof}
The proof proceeds in four major steps: (i) we first establish that the assumptions guarantee that the objective function as a function of the parameter and posterior mean belief is Lipschitz continuous, (ii) we next establish we can discretize the distribution over the risk parameter $\dist$ without loss, (iii) we then argue that we can replace a general objective function $\obj$ with a piecewise constant function without loss, (iv) we finally argue that the optimal solution using a discretized distribution $\dist$ and a piecewise constant $\obj$ can be solved using \textbf{LP}.
First, we argue that there is Lipschitz continuity in the map $m$ from the posterior mean belief to the remote mass. By conservation of Lipschitz continuity under composition, this suggests that the planner's objective as a function of $\param$ and $\param_i$ is Lipschitz-continuous.
\begin{subproof}
\begin{lemma}
\label{lemma:m_lipschitz}
$m(t)$ is $C \eta_\beta$-Lipschitz.
\end{lemma}
\begin{subproof}
Recall that $m(t) \coloneqq \inf\{u \geq 0: G^{-1}(u) \geq c_1(u)t+c_2(u)\}$ and, by Assumption \textbf{A3}, $G$ is continuously differentiable and monotone so $G^{-1}$ is continuous. Since $c_1, c_2$ are also continuous:
\begin{align*}
    m(t) &= \begin{cases}
    u & G^{-1}(u) = c_1(u)t + c_2(u), 0 < u < 1 \\
    0 & G^{-1}(0) \geq c_1(0)t + c_2(0) \\
    1 & G^{-1}(1) \leq c_1(1)t + c_2(1)\\
    \end{cases}
\end{align*}
Suppose by contradiction the claim is false, then there exists $0\leq t_1 < t_2 \leq M$ with $z_2 \coloneqq m(t_2)$, $z_1 \coloneqq m(t_1)$ such that $z_2 - z_1 > C \eta_\beta (t_2-t_1)$. Since $z_1 > z_2$:
\begin{align*}
    \popdist^{-1}(z_1) &\geq c_1(z_1)t_1+c_2(z_1)\\
    \popdist^{-1}(z_2) &\leq c_1(z_2)t_2+c_2(z_2)
\end{align*}
Therefore:
\begin{align*}
    z_1 &\geq \popdist(c_1(z_1)t_1+c_2(z_1))\\
    z_2 &\leq \popdist(c_1(z_2)t_2+c_2(z_2))
\end{align*}
Observe that:
\begin{align*}
    \popdist(c_1(z_2)t_2+c_2(z_2)) - \popdist(c_1(z_1)t_1+c_2(z_1)) &\geq z_2 - z_1\\
    &> C \eta_\beta (t_2-t_1)
    % \frac{G^{-1}(m(t_1))-c_2(m(t_1))}{c_1(m(t_1))} - \frac{G^{-1}(m(t_2))-c_2(m(t_2))}{c_1(m(t_2))} = t_2 - t_1 \\
    % \frac{c_1(m(t_2))G^{-1}(m(t_1))-c_1(m(t_2))c_2(m(t_1))-c_1(m(t_1))G^{-1}(m(t_2))+c_1(m(t_1))c_2(m(t_2))}{c_1(m(t_1))c_1(m(t_2))} = t_2 - t_1     \\
    % \frac{c_1(z_2)G^{-1}(z_1)-c_1(z_2)c_2(z_1)-c_1(z_1)G^{-1}(z_2)+c_1(z_1)c_2(z_2)}{c_1(z_1)c_1(z_2)} = t_2 - t_1    
\end{align*}
However:
\begin{align*}
    \popdist(c_1(z_2)t_2+c_2(z_2)) - \popdist(c_1(z_1)t_1+c_2(z_1)) &\leq \eta_\beta(c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1)) \\
    &\leq \eta_\beta(c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_2))\\
    &\leq \eta_\beta(c_1(z_2)t_2-c_1(z_1)t_1) \\
    &\leq \eta_\beta(c_1(z_2)t_2-c_1(z_2)t_1) \\
    &\leq C \eta_\beta(t_2-t_1)
    % \popdist(c_1(z_2)t_2+c_2(z_2))-\popdist(c_1(z_1)t_1+c_2(z_1)) > \eta_\beta (t_2-t_1)\\
    % t_2 - t_1 \leq t_2 - t_1) \\
    %   c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1) > t_2-t_1\\
    % c_1(z_2)t_2-c_1(z_1)t_1+c_2(z_2)-c_2(z_1) > t_2-t_1\\
    % c_1(z_2)t_2-c_1(z_1)t_1 > t_2-t_1\\
    % c_1(z_2)(t_2-t_1) > t_2-t_1\\ 
\end{align*}
This is a contradiction, hence $m$ must be $C \eta_\beta$-Lipschitz. 
\end{subproof}
\end{subproof}
\begin{subproof}
\begin{lemma}
\label{lemma:h_comp_lipschitz}
$\tilde{h}(\param_i; \param) = h(m(\param_i);\param)$ is $C \eta_{h,1}\eta_\beta$-Lipschitz in $\theta_i$ for all $\param \in \paramspace$.
\end{lemma}
\begin{subproof}
This follows directly from Lemma \ref{lemma:m_lipschitz} since the Lipschitz continuity is preserved under composition with constant as product. 
\end{subproof}
\end{subproof}
Next, we establish a procedure that produces a solution $\pi'$ using $\dist_\delta$ that performs well compared to the optimal $\pi^*_{\dist,\obj}$. For readability, let $V(\cdot) \coloneqq V_{\dist,\obj}(\cdot), V_\delta(\cdot) \coloneqq V_{\dist_\delta,\obj}(\cdot), \pi^* \coloneqq \pi^*_{\dist,\obj} = \langle \{z_\param\}_{\param \in \paramspace}, \I\rangle, \pi_\delta \coloneqq \pi^*_{\dist_\delta,\obj}= \langle \{s_\param\}_{\param \in \{\frac{2k-1}{2\delta}\}_{k=1}^\delta \subseteq \paramspace}, \I_\delta \rangle$. Specifically, our approach, for sufficiently large $\delta$, will solve for optimality using the $\delta$-discretization of $\dist$, $\dist_\delta$, to produce $\pi_\delta$. We then modify the mechanism to $\pi' = \langle \{s'_\param \}_{\param \in \paramspace},\I_\delta \rangle$ which uses the same set of signals as $\pi_\delta$ but is expanded to the full domain of the distribution $\dist$ by having for all $k \in [M\delta], \theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]$, $s_\theta'(\cdot) = s_{\frac{2k-1}{2\delta}}(\cdot)$. The following lemma establishes that using $\pi'$ is close to $\pi^*$ in the planner's true objective under the true distribution $\dist$.
\begin{subproof}
\begin{lemma}
For $\delta > \frac{\eta_{2,h}+ C\eta_{1,h} \eta_{\beta}}{\epsilon}$, $|V(\pi')-V(\pi^*)| \leq \epsilon$.
\end{lemma}
\begin{subproof}
By definition, $V(\pi') \leq V(\pi^*)$ so it suffices to show that $V(\pi^*)-V(\pi') \leq \epsilon$. 
Observe that if we define $\hat{\pi} = \langle \{\hat{g}_\param\}_{\param \in \{\frac{2k-1}{2\delta}\}_{k=1}^{M\delta} \subseteq \paramspace}, \I \rangle$ where for all $k \in [M\delta], i \in \I, \hat{g}_{\frac{2k-1}{2\delta}}(i) = \frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}$:
\begin{align*}
    V(\pi^*)-V(\pi') &\leq
    V(\pi^*)-V_\delta(\pi') + V_\delta(\pi') -V(\pi') \\
    &=
    V(\pi^*)-V_\delta(\pi_\delta) + V_\delta(\pi_\delta) -V(\pi') \\
    &=
    V(\pi^*)-V_\delta(\hat{\pi}) + V_\delta(\hat{\pi})-V_\delta(\pi_\delta) + V_\delta(\pi_\delta) -V(\pi')\\
    &\leq
    \underbrace{V(\pi^*)-V_\delta(\hat{\pi})}_{\textbf{(i)}} + \underbrace{V_\delta(\pi_\delta) -V(\pi')}_{\textbf{(ii)}}
\end{align*}
The terms in expression (i) and (ii) can be simplified independently. Observe that in term (i), both $\pi^*$ and $\hat{\pi}$ use the same set of signals $\I$; in term (ii), both $\pi_{\delta}$ and $\pi'$ use the same set of signals $\I_\delta$. \\
For (i), we can consider the corresponding direct mechanisms $T_{\pi^*} = \{(q_i^*, \param_i^*)\}_{i \in \I}$ for $\pi^*$ in combination with distribution $\dist$ and $T_{\hat{\pi}} = \{(\hat{q}_i,\hat{\param}_i)\}_{i \in \I}$ for $\hat{\pi}$ in combination with distribution $\dist_\delta$. Observe that by construction:
\begin{align*}
    \hat{q}_i &= \sum_{k=1}^{M\delta} \mathbb{P}_{\dist_\delta}\big[\theta =\frac{2k-1}{2\delta}]\\ 
    &= \sum_{k=1}^{M\delta} \mathbb{P}_{\dist}\big[\theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]\big] \hat{g}_{\frac{2k-1}{2\delta}}(i)\\
    &=\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)\frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}\\
    &=\sum_{k=1}^{M\delta}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)\\    
    &= q_i^*
\end{align*}
Furthermore, for all $i \in \I$, we can bound the difference between $\param_i^*$ and $\hat{\param}_i$:
\begin{align*}
|\hat{\param}_i-\param_i^*| &= \Big|\frac{\int_{0}^{M} \param \hat{g}_{\param}(i) d\dist_\delta(\param) }{\int_{0}^{M} \hat{g}_{\param}(i) d\dist_\delta(\param) }-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{\int_{0}^{M} z_{\param}(i) d\dist(\param) }\Big|\\
&= \Big|\frac{\int_{0}^{M} \param \hat{g}_{\param}(i) d\dist_\delta(\param) }{q_i^*}-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{q_i^*}\Big|\\
&= \frac{1}{q_i^*}\Big|\int_{0}^{M} \param \hat{g}_{\param}(i) d\dist_\delta(\param) -\int_{0}^{M} \param z_{\param}(i) d\dist(\param)\Big|\\
&= \frac{1}{q_i^*}\Big|\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\frac{2k-1}{2\delta})\hat{g}_{\frac{2k-1}{2\delta}}(i)d\dist(\param) -\sum_{k=1}^{M\delta}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \param z_\param(i) dF(\param)\Big|\\
&= \frac{1}{q_i^*}\Big|\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\frac{2k-1}{2\delta}-\param)z_{\theta}(i)d\dist(\param)\Big|\\
&\leq \frac{1}{q_i^*}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big|\frac{2k-1}{2\delta}-\param\big|z_{\theta}(i)d\dist(\param)\\
&\leq \frac{1}{q_i^*}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\frac{1}{2\delta}z_{\theta}(i)d\dist(\param) \\
&\leq \frac{1}{2\delta}
\end{align*}
Therefore, simplifying expression (i):
\begin{align*}
       V(\pi^*)-V_\delta(\hat{\pi}) &= \mathbb{E}_{\param^* \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^*); \param^*)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
       \hat{g}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
       &= \mathbb{E}_{i}[\mathbb{E}_{\param^* }[\obj(m(\theta_i^*); \param^*)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
\end{align*}\end{subproof}
By Fubini's theorem:
\begin{align*}
V(\pi^*)-V_\delta(\hat{\pi}) &= \mathbb{E}_{\param^* \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^*); \param^*)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
       \hat{g}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
       &=  \sum_{i \in \I}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^*_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \frac{2k-1}{2\delta})) z_{\param}(i) dF(\param)\\
       &=  \sum_{i \in \I}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^*_i; \param)) -\obj(m(\hat{\param}_i; \frac{2k-1}{2\delta}))  \Big) z_{\param}(i)dF(\param)\\
       &=  \sum_{i \in \I}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
      \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\obj(m(\param^*_i; \param)) -\obj(m(\param^*_i; \frac{2k-1}{2\delta}))  \Big) z_{\param}(i)dF(\param)\\      
       &=  \sum_{i \in \I}\sum_{k=1}^{M\delta} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
      \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
  &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
  &\leq  \frac{\epsilon}{2}
\end{align*}
We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi_\delta} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi_\delta$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_\delta(\pi_\delta) -V(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V(\pi')-V(\pi^*)| \leq \epsilon. \blacksquare$
\end{subproof}
The final step of the proof is to show that by approximating our general objective function $\obj$ by its $\omega-$discretization that we also achieve arbitrarily small loss. For readability, let $V(\cdot) \coloneqq V_{\dist_\delta,\obj}(\cdot), V_\omega(\cdot) \coloneqq V_{\dist_\delta,\obj_\omega}(\cdot), \pi^* \coloneqq \pi^*_{\dist_\delta,\obj} = \langle \{z_\param\}_{\param \in \paramspace}, \I\rangle, \pi_\omega \coloneqq \pi^*_{\dist_\delta,\obj_\omega}= \langle \{s_\param\}_{\param \in \{\frac{2k-1}{2\delta}\}_{k=1}^\delta \subseteq \paramspace}, \I_\delta \rangle$. 
\begin{lemma}
For $\omega > \frac{\eta_{\obj,1}}{\epsilon}$, $|V_{F,\obj}(\pi^*_{F_\delta,\obj_\omega})-V_{F,\obj}(\pi^*_{F_\delta,\obj})| \leq \epsilon$ 
\end{lemma}
\begin{subproof}

Observe that:
\begin{align*}
    V_{\delta}(\pi)-V(\pi_\delta) &\leq
    V_{\dist_{\delta},\obj}(\pi^*_{\dist,h})-V_{\dist,\obj}(\pi'_{F,h}) \\
    &= \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i), \param)] - \mathbb{E}_{\param \sim \dist_\delta, i \sim z_{\param}}[\obj(m(\theta_i), \param)] \\
   &= \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\obj(m(\theta_i+\sigma_1), \param+\sigma_2)-\obj(m(\theta_i), \param)]] \\
   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} +  \obj(m(\theta_i+\sigma_1), \param)-\obj(m(\theta_i), \param)]] \\
   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} + \sigma_1 \eta_{1,h}\eta_{\beta}+ \obj(m(\theta_i), \param)-\obj(m(\theta_i), \param)]] \\
   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} + \sigma_1 \eta_{1,h}\eta_{\beta}]]
    \\
   &\leq \frac{\eta_{2,h} +  \eta_{1,h}\eta_{\beta}}{\delta} \\
   &\leq  \epsilon
\end{align*}
\end{subproof}
\begin{lemma}
The result of \textbf{LP} is equivalent to $\pi^*(F_\delta,z_\omega)$.
\end{lemma}
\end{proof}

The complexity of the above LP is consequently polynomial in $M,\eta_{1,g}, \eta_{2,g}, \eta_{\beta}$ and $\frac{1}{\epsilon^2}$. Observe that appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Consequently, we can bound the overall complexity in the following corollary:
\begin{corollary}
Under assumptions $A3-A5$, the linear program provided above has polynomial time complexity with $O(\frac{\eta_{1,\obj}^5\eta_{2,\obj}^{2.5} \eta_{\beta}^{1.5}}{\epsilon^5})$ runtime produces $\hat{\pi}$ such that $\big|V(\pi^*)-V(\hat{\pi})\big| \leq \epsilon$.
\end{corollary}
\begin{proof}
The linear program \textbf{LP} has $O(\delta \omega)$ variables $z_{ij}$. 
\end{proof}
\subsection{Numerical Experiments}
In this subsection, we provide the results an reproduce the plot that exists in \cite{de_vericourt_informinz_2021} showing the improved gain and matching the mechanisms to the solutions they produce. Some additional pruning is necessary to compare apples to apples computationally. In this subsection, we provide the results for a more general setting than the DeVericourt analysis. We can consider another epidemiologically motivated setting with non-uniform cost distribution and non-concave objectives if sufficiently motivated and show our results.
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{img/DV.png}
    \caption{Error of $\hat{V}$ against discretization of $\obj$}
    \label{fig:results}
\end{figure}


% Observe that by construction:
% \begin{align*}
%     \hat{q}_i &= \sum_{k=1}^{N} \mathbb{P}_{\dist_\delta}\big[\theta =\nu_k]\hat{z}_{\nu_k}(i)\\ 
%     &= \sum_{k=1}^{N} \mathbb{P}_{\dist}\big[\theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]\big] \hat{z}_{\nu_k}(i)\\
%     &=\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)\frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}\\
%     &=\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)\\    
%     &= q_i^\ast
% \end{align*}
% Furthermore, for all $i \in \I$, we can bound the difference between $\param_i^\ast$ and $\hat{\param}_i$:
% \begin{align*}
% |\hat{\param}_i-\param_i^\ast| &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{\int_{0}^{M} \hat{z}_{\param}(i) d\dist_\delta(\param) }-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{\int_{0}^{M} z_{\param}(i) d\dist(\param) }\Big|\\
% &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{q_i^\ast}-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{q_i^\ast}\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) -\int_{0}^{M} \param z_{\param}(i) d\dist(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k)\hat{z}_{\nu_k}(i)d\dist(\param) -\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \param z_\param(i) dF(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k-\param)z_{\theta}(i)d\dist(\param)\Big|\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big|\nu_k-\param\big|z_{\theta}(i)d\dist(\param)\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\frac{1}{2\delta}z_{\theta}(i)d\dist(\param) \\
% &\leq \frac{1}{2\delta}
% \end{align*}
% Therefore, simplifying expression (i):
% \begin{align*}
%     V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{P}\{m(\posterior{i}) \geq b(\trueparam)\}
% \end{align*}

% Therefore, simplifying expression (i):
% \begin{align*}
%       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
% \end{align*}
% By Fubini's theorem:
% \begin{align*}
% V_{\dist,\obj}(\pi_{\dist,\obj})-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\kappa}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\kappa}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
%   &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
%   &\leq  \frac{\epsilon}{2}
% \end{align*}
% We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi_{\dist,\obj})| \leq \epsilon. \blacksquare$
% \end{proof}
% \begin{align*}
%       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
% \end{align*}
% By Fubini's theorem:
% \begin{align*}
% V_{\dist,\obj}(\pi_{\dist,\obj})-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\kappa}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\kappa}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
%   &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
%   &\leq  \frac{\epsilon}{2}
% \end{align*}
% We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi_{\dist,\obj})| \leq \epsilon. \blacksquare$
% \end{proof}

% The complexity of the above LP is consequently polynomial in $M,\eta_{1,g}, \eta_{2,g}, \eta_{\beta}$ and $\frac{1}{\epsilon^2}$. Observe that appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Consequently, we can bound the overall complexity in the following corollary:
% \begin{corollary}
% The algorithm described in the proof of Theorem~\ref{thm:stateful} has time complexity equal to the time complexity of \textbf{LP}. The time complexity of \textbf{LP} is $O(\frac{\eta_{1,\obj}^5\eta_{2,\obj}^{2.5} \eta_{\beta}^{1.5}}{\epsilon^3})$.
% \end{corollary}
% \begin{proof}
% The linear program \textbf{LP} has $O(\delta \omega)$ variables $z_{ij}$. Appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables.
% \end{proof}
% As with the stateless design, $\final(i)$ only depends on the induced posterior mean $\param_i$ and $\final(i) \in \goal(\nu_j)$ if and only $\final(i) \in \goal(\nu_j) \cap \curve$. The latter follows if and only if $b_j \leq \|\final(i)\| \leq 1$ or $0 \leq m(\param_i) \leq 1-b_j$. Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, observe that this corresponds to $\param_i \in [\gamma_j,\infty)$ for some constants $\gamma_j$ that are strictly increasing in $j$. For completeness, we denote $\gamma_0 = 0$ and $\gamma_{N+1} = \infty$.
% We can then reformulate \eqref{eqn:stateful_a} as follows:
% \begin{align}
%     V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{\gamma_j \leq \param_i < \infty\} \label{eqn:stateful_b}
% \end{align}
% We highlight that despite these simplifications, our analysis is extensible to other practically relevant objectives aside from the scaled capacity objective. Suppose that the desirable sets satisfy Assumption A1 and are also (i) nested with $\goal(\nu_{i+1})\subset \goal(\nu_{i})$ for all $i \in [N-1]$, and (ii) half-bounded with $\init \in \goal(\nu_i)$ for all initial mass vectors $\init$ and all $i \in [N]$; see Fig. \ref{fig:b}. Then we arrive at an identical formulation to \eqref{eqn:stateful_b} since the minimal posterior mean beliefs for the agent outcomes to enter each $\goal(\nu_j)$ is an increasing sequence $\gamma_j$.

% \noindent Using a similar reduction as in stateless design, we can restrict our mechanism to induce a single posterior mean $\param_i$ to lie in each interval $[\gamma_{i-1},\gamma_{i})$ for $i \in [N+1]$. These $\param_i$ consequently induce equilibrium outcomes that lie in $\goal(\nu_j)$ if and only if $\param_i \geq \gamma_j$ or equivalently $i \geq j+1$. This implies that an optimal mechanism can be described by at most $N+1$ signals. In the proposition below, we provide a linear program (LP) to compute an optimal signalling mechanism for the stateful scaled capacity objective.












% Using this result, we can efficiently compute the optimal objective $V^\ast$ and an optimal signalling mechanism $\pi^\ast$ in polynomial time. 

% \noindent If the $b_j$ and hence $\goal(\nu_j)$ were all identical, our setting becomes the stateless setting solved by Theorem $\ref{thm:stateless}$. In this special case, all $\nu_j$ correspond to a single $\gamma=\gamma_j$ and only two posterior means $\param_1 < \gamma \leq \param_2$ are required. If $\mu = \sum_{j \in [N]} p_j \nu_j \geq \gamma$ then this corresponds to regime R1 and non-informative mechanism is optimal. If $\mu < \gamma$ this corresponds to regime R4 and likewise we recover a discretized interval-based signalling mechanism over $\I = \{1,2\}$ by solving the LP and we can check that there exists a $\hat{j} \in [N]$ such that for all $j < \hat{j}$, $z_{\nu_j}(1) = 1$ and for all $j > \hat{j}$, $z_{\nu_j}(2) = 1$.  

% \noindent Finally, for any mechanism $\pi$, the probability of complying with the capacity limit conditioned on $\param = \nu_j$ can be represented by $V_j(\pi) \coloneqq  \mathbb{P}\{\final(i) \in \goal(\param)|\param=\nu_j\}$. Observe that $V_{\dist,\obj}(\pi) = p_j V_j(\pi)$ is a weighted average of the compliance for each possible realization of $\param$. However, practically planners may face significantly more adverse risks of being overcapacitated as the infectiousness increases, and weight compliance heterogeneously across realizations of $\param$. For this slightly more general objective, an optimal signalling mechanism for a different weighted sum $\sum_{j=1}^{N} \alpha_j V_j(\pi)$ for $\alpha_j \geq 0$ can likewise be solved using the linear program above by replacing the objective with $\max_{\{ z_{ji}\}} \sum_{i=j+1}^{N+1} \frac{\alpha_j}{p_j}z_{ji}$.

% The previous section demonstrates that generally one cannot expect to find MPS solutions under our model for general objectives, but we consider our second class of objectives which are state-dependent. Namely, we consider a scaling capacity objective where $\goal(\param) = \{y: y \geq b(\param)\}$ for some non-increasing function $b$. 
% In this section, we consider stateful goal sets where generally the set of outcomes that the principal seeks to guide equilibrium for the true parameter $\param$ is $\goal(\param)$. In this stateful setting, we cannot reduce the search over $\pi$ by searching over the corresponding direct mechanisms $\mathcal{T}_\pi$. This is because a posterior mean $\param_i$ will induce a specific equilibrium outcome $\final(i)$ but we cannot evaluate whether $\final(i) \in \goal(\param)$ if we only know $\param_i$ and not the true $\param$.

% \noindent Observe that each design problem is tailored to an initial population allocation across the groups $\init$. For this particular $\init$, achievable equilibria lie on a one-dimensional manifold as shown in Lemma \ref{lemma:intervals}, so we can decompose the intersection of $\curve$ and each of our goal sets $\goal(\param)$ as the objects of interest. Namely we will impose the following assumptions to be as general as possible: \\
% \noindent \textbf{(A2)} $\goal(\param)$ is closed for all $\param$. \\
% \noindent \textbf{(A3)} $\goal(\param) \cap \curve = \cup_{i=1}^{P} [a_{i}(\param), b_{i}(\param)]$ for finite $P$, $0 \leq a_i(\param), b_i(\param) \leq 1$ for all $\param$.\\
% \noindent \textbf{(A4)} For all $i \in [P]$, $a_i(\cdot),b_i(\cdot)$ are $\eta_1$-Lipschitz. 

% \noindent Observe that \textbf{(A3)} can be satisfied if $\goal(\param)$ is convex for all $\param$, but the assumption allows for a more general description. Assumption \textbf{(A4)} while seemingly restrictive merely requires that the goal sets are smooth in $\param$ and that there are no sudden discontinuities. Observe that some of the $P$ intervals where we only assume $P$ is finite can be empty so the shape of the intersection can change significantly as $\param$ increases.

% \noindent The following proposition establishes a linear program that is capable of approximating the optimal solution to the information design problem posed in Equation \eqref{eqn:objective_stateful}. We first introduce the following LP:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% \subsection{Stateful Scaled Capacity Model}
% \label{sec:stateful}
% \begin{figure}[h]
% \centering     %%% not \center
% \subfigure[Goal sets for stateful objective when $\K = N = 2$ ($\nu_1 < \nu_2$).]{\label{fig:a}\includegraphics[width=40mm]{img/stateful}}
% \subfigure[A more general nested structure of goal sets. ]{\label{fig:b}\includegraphics[width=40mm]{img/nested}}
% \end{figure}

% \noindent Using \eqref{eqn:objective_stateful}, we can express the objective of the planner by: 
% \begin{align}
%     V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \mathbb{P}\{\final(i) \in \goal(\nu)\} \\
%      &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_\nu(i) \mathbb{I}\{\final(i) \in \goal(\nu_j)\}  \label{eqn:stateful_a}
% \end{align}
% As with the stateless design, $\final(i)$ only depends on the induced posterior mean $\param_i$ and $\final(i) \in \goal(\nu_j)$ if and only $\final(i) \in \goal(\nu_j) \cap \curve$. The latter follows if and only if $b_j \leq \|\final(i)\| \leq 1$ or $0 \leq m(\param_i) \leq 1-b_j$. Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, observe that this corresponds to $\param_i \in [\gamma_j,\infty)$ for some constants $\gamma_j$ that are strictly increasing in $j$. For completeness, we denote $\gamma_0 = 0$ and $\gamma_{N+1} = \infty$.
% We can then reformulate \eqref{eqn:stateful_a} as follows:
% \begin{align}
%     V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{\gamma_j \leq \param_i < \infty\} \label{eqn:stateful_b}
% \end{align}
% We highlight that despite these simplifications, our analysis is extensible to other practically relevant objectives aside from the scaled capacity objective. Suppose that the desirable sets satisfy Assumption A1 and are also (i) nested with $\goal(\nu_{i+1})\subset \goal(\nu_{i})$ for all $i \in [N-1]$, and (ii) half-bounded with $\init \in \goal(\nu_i)$ for all initial mass vectors $\init$ and all $i \in [N]$; see Fig. \ref{fig:b}. Then we arrive at an identical formulation to \eqref{eqn:stateful_b} since the minimal posterior mean beliefs for the agent outcomes to enter each $\goal(\nu_j)$ is an increasing sequence $\gamma_j$.

% \noindent Using a similar reduction as in stateless design, we can restrict our mechanism to induce a single posterior mean $\param_i$ to lie in each interval $[\gamma_{i-1},\gamma_{i})$ for $i \in [N+1]$. These $\param_i$ consequently induce equilibrium outcomes that lie in $\goal(\nu_j)$ if and only if $\param_i \geq \gamma_j$ or equivalently $i \geq j+1$. This implies that an optimal mechanism can be described by at most $N+1$ signals. In the proposition below, we provide a linear program (LP) to compute an optimal signalling mechanism for the stateful scaled capacity objective. We first introduce the LP:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% Using this result, we can efficiently compute the optimal objective $V^\ast$ and an optimal signalling mechanism $\pi^\ast$ in polynomial time. 

% \noindent If the $b_j$ and hence $\goal(\nu_j)$ were all identical, our setting becomes the stateless setting solved by Theorem $\ref{thm:stateless}$. In this special case, all $\nu_j$ correspond to a single $\gamma=\gamma_j$ and only two posterior means $\param_1 < \gamma \leq \param_2$ are required. If $\mu = \sum_{j \in [N]} p_j \nu_j \geq \gamma$ then this corresponds to regime R1 and non-informative mechanism is optimal. If $\mu < \gamma$ this corresponds to regime R4 and likewise we recover a discretized interval-based signalling mechanism over $\I = \{1,2\}$ by solving the LP and we can check that there exists a $\hat{j} \in [N]$ such that for all $j < \hat{j}$, $z_{\nu_j}(1) = 1$ and for all $j > \hat{j}$, $z_{\nu_j}(2) = 1$.  

% \noindent Finally, for any mechanism $\pi$, the probability of complying with the capacity limit conditioned on $\param = \nu_j$ can be represented by $V_j(\pi) \coloneqq  \mathbb{P}\{\final(i) \in \goal(\param)|\param=\nu_j\}$. Observe that $V_{\dist,\obj}(\pi) = p_j V_j(\pi)$ is a weighted average of the compliance for each possible realization of $\param$. However, practically planners may face significantly more adverse risks of being overcapacitated as the infectiousness increases, and weight compliance heterogeneously across realizations of $\param$. For this slightly more general objective, an optimal signalling mechanism for a different weighted sum $\sum_{j=1}^{N} \alpha_j V_j(\pi)$ for $\alpha_j \geq 0$ can likewise be solved using the linear program above by replacing the objective with $\max_{\{ z_{ji}\}} \sum_{i=j+1}^{N+1} \frac{\alpha_j}{p_j}z_{ji}$.

% \subsection{Numerical Experiments}
% % \textcolor{blue}{Outline: create analogous curve for the stateful setting for a discrete distribution - show the improved comparative benefit from stateful signalling in this regime relative to even the stateless setting. Here, we again have a stateful capacity based objective (simple LP solves this).}
% \noindent For the stateful capacity case, we highlight a specific instance where we scale-down the in-person capacity limit as the infectious risk increases. Consequently, the minimal posterior mean to induce outcomes in $\goal(\nu_j)$ are represented by $\gamma_j$ that are increasing in $j$. To gain intuition, we choose the specific set of tuples for $N=3$ where $\{p_i\}_{i \in \{1,2,3\}} = (0.3,0.3,0.4), \{\nu_i\}_{i \in \{1,2,3\}} = (0.4,0.6,1.0), \{\gamma_i\}_{i \in \{1,2,3\}} = (0.5, 0.9, 1.2)$ and compare the performance of the optimal mechanism against the same two benchmarks as in the stateless case.
% In Fig. \ref{table:stateful_vary_capacity}, we tabulate each information mechanism's performance. Observe that under no information, agents mean belief over $\theta = \mu = \sum_{j=1}^N p_j \nu_j = 0.7$. Since agents receive no signal, the equilibrium outcome is independent of $\theta$ and agents only comply if $\gamma_j < \mu$ which happens with probability $p_1 = 0.3$. Under full information, agents perfectly observe $\theta$, so the outcome is compliant with the limit if and only if $\theta_j \geq \gamma_j$. This occurs with probability $0$ in our example. Thus, the stateful design significantly improves the probability of compliance relative to both benchmarks. We also observe that the stateful design does no worse in this setting than either benchmark in any of the conditional compliance measures $V_j(\pi)$.
% \begin{figure}
%     \centering
%     \begin{tabular}{ |c|c|c|c|c| } 
%     \hline
%     Information Scheme & $V_{\dist,\obj}(\pi)$ & $V_1(\pi)$ & $V_2(\pi)$ & $V_3(\pi)$ \\     
%     \hline
%     No Information & 0.300 &1& 0& 0 \\ 
%     Full Information  & 0.000 & 0& 0 &0 \\ 
%     Stateful Design & 0.425 & 1& 0.417 &0 \\ 
%  \hline
% \end{tabular}
    
%     \caption{Comparison of non-informative, fully informative and optimal stateful signalling in terms of the overall probability of compliance and conditional probabilities of compliance. }
%     \label{table:stateful_vary_capacity}
% \end{figure}
% \label{sec:approximation}
% In the previous section, we demonstrated that MPS mechanisms can achieve optimal design for particular state-independent objective  functions. However, we also provided state-dependent counterexamples where no MPS mechanism is able to achieve or closely approximate optimal design. 
% In this section, we seek a methodology to provide \textit{approximate} optimal design for a general form of state-dependent objective functions. Because we seek a method that will generalize to a general form of objective functions $\obj$, observe that a closed-form description of the optimal signalling mechanism will be difficult to obtain under arbitrary objectives.
% % \srs{sentence seems unnecessary - The approach we  produces a signalling mechanism that will \textit{$\epsilon$-approximate} the optimal solution to \eqref{eqn:gen_objective_stateful} by using $O(\frac{1}{\epsilon})$ discrete signals and $O(\frac{1}{\epsilon^2})$ computational complexity.}

% % \begin{figure}
% %     \centering
% %     \input{presentations/stateful_c.tex}
% %     \caption{Caption}
% %     \label{fig:my_label}
% % \end{figure}
% \noindent Formally, we characterize an $\epsilon$-approximation of the optimal signalling mechanism using the following definition.

% The previous example demonstrates that generally one cannot expect to find MPS solutions under our model for general objectives, but we consider our second class of objectives which are state-dependent. Namely, we consider a scaling capacity objective where $\goal(\param) = \{y: y \geq b(\param)\}$ for some non-increasing function $b$. In this section, we consider stateful goal sets where generally the set of outcomes that the principal seeks to guide equilibrium for the true parameter $\param$ is $\goal(\param)$. In this stateful setting, we cannot reduce the search over $\pi$ by searching over the corresponding direct mechanisms $\mathcal{T}_\pi$. This is because a posterior mean $\param_i$ will induce a specific equilibrium outcome $\final(i)$ but we cannot evaluate whether $\final(i) \in \goal(\param)$ if we only know $\param_i$ and not the true $\param$.

% \noindent Observe that each design problem is tailored to an initial population allocation across the groups $\init$. For this particular $\init$, achievable equilibria lie on a one-dimensional manifold as shown in Lemma \ref{lemma:intervals}, so we can decompose the intersection of $\curve$ and each of our goal sets $\goal(\param)$ as the objects of interest. Namely we will impose the following assumptions to be as general as possible: \\
% \noindent \textbf{(A2)} $\goal(\param)$ is closed for all $\param$. \\
% \noindent \textbf{(A3)} $\goal(\param) \cap \curve = \cup_{i=1}^{P} [a_{i}(\param), b_{i}(\param)]$ for finite $P$, $0 \leq a_i(\param), b_i(\param) \leq 1$ for all $\param$.\\
% \noindent \textbf{(A4)} For all $i \in [P]$, $a_i(\cdot),b_i(\cdot)$ are $\eta_1$-Lipschitz. 

% \noindent Observe that \textbf{(A3)} can be satisfied if $\goal(\param)$ is convex for all $\param$, but the assumption allows for a more general description. Assumption \textbf{(A4)} while seemingly restrictive merely requires that the goal sets are smooth in $\param$ and that there are no sudden discontinuities. Observe that some of the $P$ intervals where we only assume $P$ is finite can be empty so the shape of the intersection can change significantly as $\param$ increases.

% \noindent The following proposition establishes a linear program that is capable of approximating the optimal solution to the information design problem posed in Equation \eqref{eqn:objective_stateful}. We first introduce the following LP:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}
% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%     \draw[->] (0,0) -- (\rb+0.5,0);
%     \draw[->] (0,0) -- (0,\rb);
%     % \draw[dashed] (\ra,0) -- (\ra,1) node[above] {$a$};
%     \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$1$};
%     \draw[] (\rb+0.5,-0.25) node[below] {$y$};
%     \draw[] (\rb-0.5,\rb-1) node[below] {$\obj(y;\cdot)$};
    
%     \draw[red, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{2*sin(deg(\x))+2});
%     \draw[red!90,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.9*sin(deg(\x))+1.9});
%     \draw[red!80blue!40,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.6*sin(deg(\x))+1.5});
%     \draw[red!70blue!30,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.4*sin(deg(\x))+1.2});
%     \draw[red!60!blue!40-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.2*sin(deg(\x))+0.9});
%     \draw[red!50!blue!50,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{sin(deg(\x))+0.8});
% \end{tikzpicture}
    
%     \begin{tikzpicture}
%     \draw[->] (0,0) -- (\rb+0.5,0);
%     \draw[->] (0,0) -- (0,\rb+0.5);
%     % \draw[dashed] (\ra,0) -- (\ra,1) node[above] {$a$};
% \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$1$};
%     \draw[] (\rb+0.5,-0.25) node[below] {$y$};
%     \draw[] (\rb-0.5,\rb) node[below] {$\obj(y;\nu)$};
%     \draw[dotted,thick,red] (1.6,0) -- (1.3,-0.3) node[below] {$\theta_{s'}$};
%     \draw[dotted,thick,red] (1.8,0) -- (2.1,-0.3) node[below] {$\theta_{s''}$};
%     % \draw[dashed] (1.0,0) -- (1.0,-1.5) node[below] {$m(\gamma_{i+1})$};
    
%     %Right-Hand
%     \foreach \x in {1,...,\rb} % <--- my issues
%     \draw[thick, fill=red!25] (\x-.5,0) -- (\x-.5,{2*sin(deg(\x-0.25))+2.05}) -- (\x,{2*sin(deg(\x-0.25))+2.05}) -- (\x,0) -- cycle;
%     \foreach \x in {1,...,\rb} % <--- my issues
%     \draw[thick, fill=green!25] (\x-1,0) -- (\x-1,{2*sin(deg(\x-0.5-0.25))+2.05}) -- (\x-0.5,{2*sin(deg(\x-0.5-0.25))+2.05}) -- (\x-0.5,0) -- cycle;
    
%     % %Left-Hand
%     % \foreach \x in {\ra,-0.5,...,\rbtwo} % <--- my issues
%     % \draw[thick, fill=blue!25] (\x,0) -- (\x,{sin(deg(\x))}) -- (\x+.5,{sin(deg(\x))}) -- (\x+.5,0) -- cycle;
    
%     \draw[ultra thick, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{2*sin(deg(\x))+2});
    
% \end{tikzpicture}\caption{$\delta$-discretization of $F$ and $\omega$-discretization of $\obj$.}
%     \label{fig:discretization}
% \end{figure}
% Analogously, to adapt a continuous objective function $h(\cdot, \param)$ to a piecewise constant, we can parameterize the discretization by $\omega$ and choose to uniformly create intervals of length $\frac{1}{\omega}$ over $[0,1]$ with the discretized function taking a constant value over each interval equal to the average of the minimum and maximum on this interval. 
% \begin{defn}
% The \textit{$\omega$-discretization} $h_\omega$ of any continuous function $h:[0,1]\rightarrow \R$ is a piecewise constant function such that for all $k \in [\omega], x \in[\frac{k-1}{\omega},\frac{k}{\omega}]$:
% \begin{align*}
%     h_\omega(x) = \frac{\min_{x\in[\frac{k-1}{\omega},\frac{k}{\omega}]}h(x)+\max_{x\in[\frac{k-1}{\omega},\frac{k}{\omega}]}h(x)}{2} 
% \end{align*}
% \end{defn}

% Consider the following linear program parameterized by a sequence of parameters $\langle P, Q, \{\alpha_{ji}\}_{i \in [P], j\in[Q]},\{\gamma_{i}\}_{i \in [P]},\{\nu_{j}\}_{j\in[Q]}\rangle$:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} \alpha_{ji}z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% \noindent To eliminate instances of our problem when the objective is erratically constructed, we impose the following assumptions on the problem setting.

% \textbf{Assumptions}
% \\
% \noindent \textbf{A3} $\popdist$ is continuously differentiable with $0 < \frac{d\popdist}{dv} \leq \kappa$. 

% \noindent \textbf{A4} $h(x; \cdot)$ is uniformly $\eta_{h,1}$-Lipschitz

% \noindent \textbf{A5} $h(\cdot; \theta)$ is uniformly $\eta_{h,2}$-Lipschitz

% \noindent \textbf{A6} $h(x; \theta)$ is jointly differentiably continuous

% \begin{theorem}\label{thm:stateful}
% Under assumptions A3-A5, the solution $\pi^\ast(F_\delta,h_\omega)$ for $\delta > \frac{2\eta_{2,h} +2\eta_{1,h} \eta_{\beta}}{\epsilon}$, $\omega > \frac{2\eta_{1,h}}{\epsilon}$ is $\epsilon$-optimal and $\pi^\ast(F_\delta,z_\omega)$ can be computed using \textbf{LP} with parameters:. 
% \end{theorem}
% \begin{proof}
% The proof proceeds in four major steps: (i) we first establish that the assumptions guarantee that the objective function as a function of the parameter and posterior mean belief is Lipschitz continuous, (ii) we next establish we can discretize the distribution over the risk parameter $\dist$ without loss, (iii) we then argue that we can replace a general objective function $\obj$ with a piecewise constant function without loss, (iv) we finally argue that the optimal solution using a discretized distribution $\dist$ and a piecewise constant $\obj$ can be solved using \textbf{LP}.
% First, we argue that there is Lipschitz continuity in the map $m$ from the posterior mean belief to the remote mass. By conservation of Lipschitz continuity under composition, this suggests that the planner's objective as a function of $\param$ and $\param_i$ is Lipschitz-continuous.
% \begin{subproof}
% \begin{lemma}
% \label{lemma:m_lipschitz}
% $m(t)$ is $C \kappa$-Lipschitz.
% \end{lemma}
% \begin{subproof}
% Recall that $m(t) \coloneqq \inf\{u \geq 0: G^{-1}(u) \geq c_1(u)t+c_2(u)\}$ and, by Assumption \textbf{A3}, $G$ is continuously differentiable and monotone so $G^{-1}$ is continuous. Since $c_1, c_2$ are also continuous:
% \begin{align*}
%     m(t) &= \begin{cases}
%     u & G^{-1}(u) = c_1(u)t + c_2(u), 0 < u < 1 \\
%     0 & G^{-1}(0) \geq c_1(0)t + c_2(0) \\
%     1 & G^{-1}(1) \leq c_1(1)t + c_2(1)\\
%     \end{cases}
% \end{align*}
% Suppose by contradiction the claim is false, then there exists $0\leq t_1 < t_2 \leq M$ with $z_2 \coloneqq m(t_2)$, $z_1 \coloneqq m(t_1)$ such that $z_2 - z_1 > C \kappa (t_2-t_1)$. Since $z_1 > z_2$:
% \begin{align*}
%     \popdist^{-1}(z_1) &\geq c_1(z_1)t_1+c_2(z_1)\\
%     \popdist^{-1}(z_2) &\leq c_1(z_2)t_2+c_2(z_2)
% \end{align*}
% Therefore:
% \begin{align*}
%     z_1 &\geq \popdist(c_1(z_1)t_1+c_2(z_1))\\
%     z_2 &\leq \popdist(c_1(z_2)t_2+c_2(z_2))
% \end{align*}
% Observe that:
% \begin{align*}
%     \popdist(c_1(z_2)t_2+c_2(z_2)) - \popdist(c_1(z_1)t_1+c_2(z_1)) &\geq z_2 - z_1\\
%     &> C \kappa (t_2-t_1)
%     % \frac{G^{-1}(m(t_1))-c_2(m(t_1))}{c_1(m(t_1))} - \frac{G^{-1}(m(t_2))-c_2(m(t_2))}{c_1(m(t_2))} = t_2 - t_1 \\
%     % \frac{c_1(m(t_2))G^{-1}(m(t_1))-c_1(m(t_2))c_2(m(t_1))-c_1(m(t_1))G^{-1}(m(t_2))+c_1(m(t_1))c_2(m(t_2))}{c_1(m(t_1))c_1(m(t_2))} = t_2 - t_1     \\
%     % \frac{c_1(z_2)G^{-1}(z_1)-c_1(z_2)c_2(z_1)-c_1(z_1)G^{-1}(z_2)+c_1(z_1)c_2(z_2)}{c_1(z_1)c_1(z_2)} = t_2 - t_1    
% \end{align*}
% However:
% \begin{align*}
%     \popdist(c_1(z_2)t_2+c_2(z_2)) - \popdist(c_1(z_1)t_1+c_2(z_1)) &\leq \kappa(c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1)) \\
%     &\leq \kappa(c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_2))\\
%     &\leq \kappa(c_1(z_2)t_2-c_1(z_1)t_1) \\
%     &\leq \kappa(c_1(z_2)t_2-c_1(z_2)t_1) \\
%     &\leq C \kappa(t_2-t_1)
%     % \popdist(c_1(z_2)t_2+c_2(z_2))-\popdist(c_1(z_1)t_1+c_2(z_1)) > \kappa (t_2-t_1)\\
%     % t_2 - t_1 \leq t_2 - t_1) \\
%     %   c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1) > t_2-t_1\\
%     % c_1(z_2)t_2-c_1(z_1)t_1+c_2(z_2)-c_2(z_1) > t_2-t_1\\
%     % c_1(z_2)t_2-c_1(z_1)t_1 > t_2-t_1\\
%     % c_1(z_2)(t_2-t_1) > t_2-t_1\\ 
% \end{align*}
% This is a contradiction, hence $m$ must be $C \kappa$-Lipschitz. 
% \end{subproof}
% \end{subproof}
% \begin{subproof}
% \begin{lemma}
% \label{lemma:h_comp_lipschitz}
% $\tilde{h}(\param_i; \param) = h(m(\param_i);\param)$ is $C \eta_{h,1}\kappa$-Lipschitz in $\theta_i$ for all $\param \in \paramspace$.
% \end{lemma}
% \begin{subproof}
% This follows directly from Lemma \ref{lemma:m_lipschitz} since the Lipschitz continuity is preserved under composition with constant as product. 
% \end{subproof}
% \end{subproof}
% Next, we establish a procedure that produces a solution $\pi'$ using $\dist_\delta$ that performs well compared to the optimal $\pi^\ast_{\dist,\obj}$. For readability, let $V_{\dist,\obj}(\cdot) \coloneqq V_{\dist,\obj}(\cdot), V_{\dist_\delta,\obj}(\cdot) \coloneqq V_{\dist_\delta,\obj}(\cdot), \pi^\ast \coloneqq \pi^\ast_{\dist,\obj} = \langle \{z_\param\}_{\param \in \paramspace}, \I\rangle, \pi^\ast_{\dist_\delta,\obj} \coloneqq \pi^\ast_{\dist_\delta,\obj}= \langle \{s_\param\}_{\param \in \{\nu_k\}_{k=1}^\delta \subseteq \paramspace}, \I_\delta \rangle$. Specifically, our approach, for sufficiently large $\delta$, will solve for optimality using the $\delta$-discretization of $\dist$, $\dist_\delta$, to produce $\pi^\ast_{\dist_\delta,\obj}$. We then modify the mechanism to $\pi' = \langle \{s'_\param \}_{\param \in \paramspace},\I_\delta \rangle$ which uses the same set of signals as $\pi^\ast_{\dist_\delta,\obj}$ but is expanded to the full domain of the distribution $\dist$ by having for all $k \in [N], \theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]$, $s_\theta'(\cdot) = s_{\nu_k}(\cdot)$. The following lemma establishes that using $\pi'$ is close to $\pi^\ast$ in the planner's true objective under the true distribution $\dist$.
% \begin{subproof}
% \begin{lemma}
% For $\delta > \frac{\eta_{2,h}+ C\eta_{1,h} \eta_{\beta}}{\epsilon}$, $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi^\ast)| \leq \epsilon$.
% \end{lemma}
% \begin{subproof}
% By definition, $V_{\dist,\obj}(\pi') \leq V_{\dist,\obj}(\pi^\ast)$ so it suffices to show that $V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\pi') \leq \epsilon$. 
% Observe that if we define $\hat{\pi} = \langle \{\hat{z}_\param\}_{\param \in \{\nu_k\}_{k=1}^{N} \subseteq \paramspace}, \I \rangle$ where for all $k \in [N], i \in \I, \hat{z}_{\nu_k}(i) = \frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}$:
% \begin{align*}
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\pi') &\leq
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\pi') + V_{\dist_\delta,\obj}(\pi') -V_{\dist,\obj}(\pi') \\
%     &=
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \\
%     &=
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) + V_{\dist_\delta,\obj}(\hat{\pi})-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi')\\
%     &\leq
%     \underbrace{V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi})}_{\textbf{(i)}} + \underbrace{V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi')}_{\textbf{(ii)}}
% \end{align*}
% The terms in expression (i) and (ii) can be simplified independently. Observe that in term (i), both $\pi^\ast$ and $\hat{\pi}$ use the same set of signals $\I$; in term (ii), both $\pi_{\delta}$ and $\pi'$ use the same set of signals $\I_\delta$. \\
% For (i), we can consider the corresponding direct mechanisms $T_{\pi^\ast} = \{(q_i^\ast, \param_i^\ast)\}_{i \in \I}$ for $\pi^\ast$ in combination with distribution $\dist$ and $T_{\hat{\pi}} = \{(\hat{q}_i,\hat{\param}_i)\}_{i \in \I}$ for $\hat{\pi}$ in combination with distribution $\dist_\delta$. Observe that by construction:
% \begin{align*}
%     \hat{q}_i &= \sum_{k=1}^{N} \mathbb{P}_{\dist_\delta}\big[\theta =\nu_k]\\ 
%     &= \sum_{k=1}^{N} \mathbb{P}_{\dist}\big[\theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]\big] \hat{z}_{\nu_k}(i)\\
%     &=\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)\frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}\\
%     &=\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)\\    
%     &= q_i^\ast
% \end{align*}
% Furthermore, for all $i \in \I$, we can bound the difference between $\param_i^\ast$ and $\hat{\param}_i$:
% \begin{align*}
% |\hat{\param}_i-\param_i^\ast| &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{\int_{0}^{M} \hat{z}_{\param}(i) d\dist_\delta(\param) }-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{\int_{0}^{M} z_{\param}(i) d\dist(\param) }\Big|\\
% &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{q_i^\ast}-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{q_i^\ast}\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) -\int_{0}^{M} \param z_{\param}(i) d\dist(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k)\hat{z}_{\nu_k}(i)d\dist(\param) -\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \param z_\param(i) dF(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k-\param)z_{\theta}(i)d\dist(\param)\Big|\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big|\nu_k-\param\big|z_{\theta}(i)d\dist(\param)\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\frac{1}{2\delta}z_{\theta}(i)d\dist(\param) \\
% &\leq \frac{1}{2\delta}
% \end{align*}
% Therefore, simplifying expression (i):
% \begin{align*}
%       V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
% \end{align*}\end{subproof}
% By Fubini's theorem:
% \begin{align*}
% V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\kappa}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\kappa}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
%   &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
%   &\leq  \frac{\epsilon}{2}
% \end{align*}
% We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi^\ast)| \leq \epsilon. \blacksquare$
% \end{subproof}
% The final step of the proof is to show that by approximating our general objective function $\obj$ by its $\omega-$discretization that we also achieve arbitrarily small loss. For readability, let $V_{\dist,\obj}(\cdot) \coloneqq V_{\dist_\delta,\obj}(\cdot), V_\omega(\cdot) \coloneqq V_{\dist_\delta,\obj_\omega}(\cdot), \pi^\ast \coloneqq \pi^\ast_{\dist_\delta,\obj} = \langle \{z_\param\}_{\param \in \paramspace}, \I\rangle, \pi_\omega \coloneqq \pi^\ast_{\dist_\delta,\obj_\omega}= \langle \{s_\param\}_{\param \in \{\nu_k\}_{k=1}^\delta \subseteq \paramspace}, \I_\delta \rangle$. 
% \begin{lemma}
% For $\omega > \frac{\eta_{\obj,1}}{\epsilon}$, $|V_{F,\obj}(\pi^\ast_{F_\delta,\obj_\omega})-V_{F,\obj}(\pi^\ast_{F_\delta,\obj})| \leq \epsilon$ 
% \end{lemma}
% \begin{subproof}

% Observe that:
% \begin{align*}
%     V_{\delta}(\pi)-V_{\dist,\obj}(\pi^\ast_{\dist_\delta,\obj}) &\leq
%     V_{\dist_{\delta},\obj}(\pi^\ast_{\dist,h})-V_{\dist,\obj}(\pi'_{F,h}) \\
%     &= \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i), \param)] - \mathbb{E}_{\param \sim \dist_\delta, i \sim z_{\param}}[\obj(m(\theta_i), \param)] \\
%   &= \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\obj(m(\theta_i+\sigma_1), \param+\sigma_2)-\obj(m(\theta_i), \param)]] \\
%   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} +  \obj(m(\theta_i+\sigma_1), \param)-\obj(m(\theta_i), \param)]] \\
%   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} + \sigma_1 \eta_{1,h}\eta_{\beta}+ \obj(m(\theta_i), \param)-\obj(m(\theta_i), \param)]] \\
%   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} + \sigma_1 \eta_{1,h}\eta_{\beta}]]
%     \\
%   &\leq \frac{\eta_{2,h} +  \eta_{1,h}\eta_{\beta}}{\delta} \\
%   &\leq  \epsilon
% \end{align*}
% \end{subproof}
% \begin{lemma}
% The result of \textbf{LP} is equivalent to $\pi^\ast(F_\delta,z_\omega)$.
% \end{lemma}
% \end{proof}

% The complexity of the above LP is consequently polynomial in $M,\eta_{1,g}, \eta_{2,g}, \eta_{\beta}$ and $\frac{1}{\epsilon^2}$. Observe that appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Consequently, we can bound the overall complexity in the following corollary:
% \begin{corollary}
% Under assumptions $A3-A5$, the linear program provided above has polynomial time complexity with $O(\frac{\eta_{1,\obj}^5\eta_{2,\obj}^{2.5} \eta_{\beta}^{1.5}}{\epsilon^5})$ runtime produces $\hat{\pi}$ such that $\big|V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\hat{\pi})\big| \leq \epsilon$.
% \end{corollary}
% \begin{proof}
% The linear program \textbf{LP} has $O(\delta \omega)$ variables $z_{ij}$. 
% \end{proof}
% \subsection{Numerical Experiments}
% In this subsection, we provide the results an reproduce the plot that exists in \cite{de_vericourt_informinz_2021} showing the improved gain and matching the mechanisms to the solutions they produce. Some additional pruning is necessary to compare apples to apples computationally. In this subsection, we provide the results for a more general setting than the DeVericourt analysis. We can consider another epidemiologically motivated setting with non-uniform cost distribution and non-concave objectives if sufficiently motivated and show our results.
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{img/DV.png}
%     \caption{Error of $\hat{V}$ against discretization of $\obj$}
%     \label{fig:results}
% \end{figure}






% 
\newpage
\subsection{Scaled Capacity}
\begin{prop}
\label{prop:scaled_capacity} The corresponding solution  of \textbf{LP} for the scaled capacity model with $\gamma_i = m^{-1}(b(\nu_i))$ will produce $\hat{\pi}$ that is $\epsilon$-optimal.
\end{prop}

\begin{itemize}
\item \textbf{LP} has $O(N^2) = O(M^2 \delta^2)$ variables and $O(N^2) = O(M^2 \delta^2)$ constraints
\end{itemize}


Moreover, given an optimal solution to \textbf{LP} $\{z_{ji}^\ast\}$, define the following signalling mechanism.  The following theorem shows that $\pi'$ is $\epsilon$-optimal under $V_{\dist,\obj}$ for sufficiently large $\delta$.
\begin{prop}\label{prop:lipschitz}
Suppose that $\popdist$ is continuously differentiable with $0 < \frac{d\popdist}{dv} \leq \kappa$ and $b(\cdot)$ is continuously differentiable with $0 < \frac{db}{dt} \leq \eta_b$, then for $\delta > \frac{2\eta_{2,h} +2\eta_{1,h} \eta_{\beta}}{\epsilon}$, $\pi'$ is $\epsilon$-optimal under $V_{\dist,\obj}$.
\end{prop}
\begin{proof}
The proof proceeds in three major steps: (i) we first establish that the assumptions guarantee that $m(\cdot)$ is Lipschitz continuous, (ii) we solve for  $V_{\dist_\delta,\obj}^\ast$ and $\pi_{\dist_\delta,\obj}^\ast$ using a linear program, (ii) we next establish that $V_{\dist,\obj}(\pi')$ is close to $V_{\dist_\delta,\obj}(\pi_{\dist_\delta,\obj}^\ast)$ and then that $V_{\dist_\delta,\obj}(\pi_{\dist_\delta,\obj}^\ast)$ is close to $V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)$.\\
First, we argue that there is Lipschitz continuity in the map $m$ from the posterior mean belief to the remote mass. 
\begin{subproof}
\end{subproof}
Finally, we establish $\pi'$ is $\epsilon$-optimal for \textcolor{blue}{$\delta > \frac{\eta_{2,h}+ C\eta_{1,h} \eta_{\beta}}{\epsilon}$}. The discrete solution (we know this precisely from Lemma~\ref{lemma:lp_discrete}).
\end{proof}

Therefore, simplifying expression (i):
\begin{align*}
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{P}\{m(\posterior{i}) \geq b(\trueparam)\}
\end{align*}

==> Journal_Version/case_study.tex <==
\section{Computational Study}
\label{subsec:numerical}

In this section, we apply our approach to compute optimal signalling mechanism for a class of operationally relevant planner preferences, and demonstrate that we asymptotically recover the optimal planner utility. We also compare with the the model studied in~\cite{de_vericourt_informing_2021}, which corresponds to the distribution of agent's value of in-person work $\popdist \sim Unif[0,6]$. However, in contrast to binary-valued state in their work, we consider continuous valued state $\trueparam\sim Unif[0,10]$. 

In this subsection, we present a numerical analysis demonstrating the generality of our result to apply to various planner preferences that have not been considered in the literature. 

\noindent Consider the preference model presented in~\cite{de_vericourt_informing_2021} by accordingly choosing $\popdist \sim Unif[0,6]$ and $\dist\sim Unif[0,10]$\footnote{In terms of the notation presented in ~\cite{de_vericourt_informing_2021}, we choose $\lambda = \frac{1}{2},\kappa = 1, \theta = 3, \sigma = \sqrt{3}, p_\ell = \frac{1}{2}, \omega_\ell = 0, \omega_h = 10$.}:
\begin{align*}
\obj_{\text{ref}(\lambda)}(\fin;\trueparam) = \lambda \mathbb{E}_{v \sim G}[v\mathbb{I}\{v\geq G^{-1}(\fin)\}]- (1-\lambda) \trueparam (1-\fin)^2
\end{align*}

The preference model equally weighs the \textit{total} disutility all agents cumulatively expect to incur from the disease spread ($\trueparam (1-\fin)^2$) and the gains it expects to receive from the in-person workers (i.e., those that receive benefits larger than $G^{-1}(\fin)$, $\mathbb{E}_{v \sim G}[v\mathbb{I}\{v\geq G^{-1}(\fin)\}]$). Although this preference description is a reasonable model and the results in ~\cite{de_vericourt_informing_2021} provide a closed form representation of the optimal signalling mechanism, a planner in practice may seek to regularize the results of such an optimization and maintain in-person masses that do not involve fully remote or fully in-person work. Intuitively, the workplace facilities may only be viable if a moderate in-person mass is present irrespective of state. The planner can achieve this by augmenting their objective with an additive concave term taking maximal values in the center of $\fin\in[0,1]$ such as $\fin(1-\fin)$. Choosing this as an example we consider the modified objective function (by choosing $\lambda = \frac{1}{2}$):
\begin{align*}
\obj_\rho(\fin;\trueparam) = \frac{1}{2}\big((1-\rho)(5(1-\fin^2) -  \trueparam (1-\fin)^2)\big)  + \rho \fin(1-\fin)
\end{align*}

We provide a characterization of the error obtained by our $\epsilon$-optimal solution $\hat{\pi}_{\dist_\delta,,\obj_\tau}$ as we vary the discretization. In contrast to ~\cite{de_vericourt_informing_2021}, we consider the distribution to be $\dist \sim Unif[0,10]$ where now $\dist$ is continuously valued. Observe that our new model satisfies all the assumptions of Theorem \ref{thm:stateful} and consequently with sufficient discretization (i.e., $\delta, \tau$ large enough) we can acheieve $\epsilon$-optimal solutions using \textbf{LP}.

\begin{align*}
\obj_{\text{ref}(\lambda)}(\fin;\trueparam) = 5\lambda(1-\fin^2) - (1-\lambda) \trueparam (1-\fin)^2 
\end{align*}

We plot the error of our solutions against the true optimum\footnote{The true optimum is unknown in this setting so rely on the correctness of Theorem \ref{thm:stateful} and approximate the solution when $\tau=10^5$ is sufficiently close to the true optimum.} in Fig. ~\ref{fig:continuous_error} as we increase $\delta=\tau$for various degrees of regularization $\rho$. \footnote{For brevity, we only consider one such weighting $\lambda$, but our analysis is general to the chosen weighting.} As demonstrated, the error of the computational solution provided by our linear program rapidly reduces to the limits of numerical precision quickly and faster than the rate of $\frac{1}{\epsilon^5}$ described in our result. This suggests that in practice, the convergence to the true optimum in terms of the discretization in $\tau$ is faster than the rate we provide. Because the structure of the true optimal solution can numerically be verified to being close to interval-based (see \ref{subsec:theta_y_plots}), the fast convergence can coincide with linear programming's ease of traversing extreme points since interval-based schemes correspond to the extreme points of the polytope containing all signalling mechanisms.

\noindent The added regularization term rewards remote masses that are more moderate. While the optimal mechanism has characteristics of full information disclosure and no information disclosure (see \ref{fig:y_theta_plot}) which does not qualitatively differ from the closed form result in ~\cite{de_vericourt_informing_2021}, observe the distribution we consider takes on a more general form of uncertainty and the added regularization term has a more complex dependence on the posterior mean directly. This added complexity makes much of the analysis in ~\cite{de_vericourt_informing_2021} seeking to identify the concave envelope of the posterior mean analytically intractable. Still, while the results of ~\cite{de_vericourt_informing_2021} do not directly apply, our solution still provides approximate solutions of high quality. Moreover, our linear programming technique that produces the $\epsilon$-optimal signalling mechanism is able to achieve more precise approximations at the expense of more time complexity with the error scaling to zero with sufficient discretization.

\begin{figure}[h!]
\label{fig:continuous_error}
\centering
\begin{tikzpicture}
\begin{axis}[
% scaled y ticks=-12:0,
% ytick scale label code/.code={},
symbolic x coords={1,3,10,32,100,316},
xticklabels={$10^{0}$,$10^{0.5}$,$10^{1}$,$10^{1.5}$,$10^{2}$,$10^{2.5}$},
xtick=data,
height=9cm,
width=15cm,
grid=major,
xlabel={$(\tau,\delta)$},
ylabel={$\log(V_{F,h_{\lambda,\rho)}}^\ast - V_{\bar{F},h_{\lambda,\rho)}}(\hat{\pi}_{\bar{F},h_{\tau}}))$},
legend style={
cells={anchor=east},
legend pos=south east,
}
]
\addplot[-,dashed,gray] coordinates {
(1,-1.39188)  (3,-1.79188)  (10,-2.19188)  (32,-2.59188)  (100,-2.99188)  (316,-3.39188)};
\addplot[red,mark=*] coordinates {
(1,-1.39188)  
(3,-2.88172)  
(10,-4.02515)  
(32,-6.75781)  
(100,-7.92214)
(316,-16.27845)
};
\addplot[green,mark=*] coordinates {
(1,-2.20855)  
(3,-3.59715)  
(10,-4.55526)  
(32,-7.02078)  
(100,-9.84782)
(316,-11.79503) 
};
\addplot[blue,mark=*] coordinates {
(1,-9.50138)  
(3,-9.50127)  
(10,-4.84466)  
(32,-7.11988)  
(100,-11.38512) 
(316,-12.96203)
};

\legend{Thm. \ref{thm:stateful},$\rho = 0.0$,$\rho = 0.5$,$\rho = 1.0$}
\end{axis}
\end{tikzpicture}

\caption{Error of computed $\epsilon$-optimal solution $\hat{\pi}_{F_\delta,h_{\tau}}$ as discretization ($\delta,\tau$; assume equal) increases and the regularizations $\rho$ are varied. $\lambda = 0.5$.}
\end{figure}



==> Journal_Version/old/3_-_State_Independent.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex
\newpage
\section{State-Independent, Set-Based Preferences}
\label{sec:static_id}

In this section, we consider the setting in which the planner maintains a set-based preference over the size distribution of agents across in-person and remote work, identical for all values of the state. This preference is represented by the union of finitely many ($\numintervals$) closed intervals: $\goal =\cup_{k=1}^{\numintervals} \Omega_k\subseteq [0,1]$ where $\Omega_k \coloneqq [\wll{k}, \wlh{k}]$. Without loss of generality, we can assume that these intervals are disjoint and increasing, that is $0\leq \wlh{k} < \wll{k+1} \leq 1$ for all $k$. We refer to this setting as \emph{state-independent set-based preference}. 

The choice of $\Omega_k$ is driven by practical considerations such as feasible set of agent occupancies at the workplace, as driven by the number of workplace  facilities, their sizes, and minimum/maximum number of occupants and public health guidelines at each facility. As an example, $\numintervals=1$ and $\goal = [\wll{1}, \wlh{1}]$ would mean that the planner with two workplace facilities prefers the in-person mass of agents to be in the interval $[0, \wll{1})$ or $(\wlh{1}, 1]$; this corresponds to a occupancy limit below $\wll{1}$ in the first facility, and a minimum (resp. maximum) limit $(\wlh{1}-\wll{1})$ (resp. ($1-\wll{1})$) in the second facility (which is to be used when the first facility's occupancy limit is reached). 

The planner's utility for state-independent set-based preferences can be defined as $\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{y \in \goal\}$. Her expected objective $V_{F,\obj}(\pi)$ for a signaling mechanism $\pi = \langle \I, \{z_\param\}_{\param \in \paramspace} \rangle $ then becomes~$V_{F,\obj}(\pi) = \mathbb{P}\{\final(i) \in \goal\}=\mathbb{P}\{\final({\signal}) \in \cup_{k=1}^{\numintervals} \Omega_k\}$, where $\final({\signal})$ is the agent's equilibrium remote mass in response to signal $i\in\I$ that is realized with probability $z_\trueparam(i)$. Following Prop.~\ref{prop:eqbm_formula_prop_1}, we can  write the problem of maximizing planner's objective~\eqref{eqn:gen_objective_stateful} as follows: 
\begin{align}
        V_{F,h}^* = \max_{\pi: \langle \I,  \{z_\param\}_{\param \in \paramspace}\rangle} \sum_{k=1}^{\numintervals} \mathbb{P}\{\wll{k} \leq m(\posterior{\signal}) \leq \wll{k}\}, \label{eqn:value_c_i}
\end{align}
where $\posterior{\signal}$ is the posterior mean belief induced by the signal $i$. For any $k=1,\ldots,\numintervals$, Lemma~\ref{lemma:m_smooth} implies that the preimage of $m(\cdot)$ over $\Omega_k=[\wll{k}, \wlh{k}]$ is a closed interval $[\lol{k}, \hil{k}]\eqqcolon \bar{\Theta}_k\subseteq \paramspace$. Hence, the occurrence of event $\{m(\posterior{\signal})\in \Omega_k\}$ is equivalent to that of the event $\{\posterior{\signal} \in \bar{\Theta}_k\}$. Furthermore, the monotonicity of $m(\cdot)$ implies that $\lol{k}$ and $\hil{k}$ are increasing in $k$. By exploiting this structure, the problem~\eqref{eqn:value_c_i} can be re-written as optimization over direct mechanisms of the form $\mathcal{T}_{\pi} = \{(q_\signal, \posterior{\signal})\}_{\signal \in \I}$:  
\begin{align}
        V_{F,h}^* &= \max_{\mathcal{T}_\pi: \{(q_i, \posterior{i})\}_{i \in \I}} \sum_{i \in \I} \sum_{k=1}^{K} q_i \mathbb{I}\{\lol{k} \leq \posterior{i} \leq \hil{k}\},         
        \label{eqn:red_1_form}
\end{align}
where $q_i$ and $\posterior{i}$ are the signal probability and posterior mean belief corresponding to signal~$i$ realized by mechanism $\pi$ (refer to~\eqref{eqn:q_i} and \eqref{eqn:theta_i}). 

Now consider the no informative mechanism $\pi_{\mathrm{NI}}$ which can be constructed by choosing $\I$ as a singleton set (say $\{s\}$) and $z_\param=1$ for all $\param \in \paramspace$. The corresponding direct mechanism is $\mathcal{T}_\mathrm{NI}=\{(1, \priormean)\}$, where $\priormean$ is the mean for prior distribution $\dist$ over the true state~$\trueparam$. From~\eqref{eqn:red_1_form}, we note that the no informative mechanism achieves maximum planner utility of $1$ if and only if there exists an interval  $k=[\numintervals]$ for which the prior mean belief $\priormean\in\bar{\Theta}_k$. On the other hand, if $\priormean\notin\bar{\Theta}_k$ for all $k=[\numintervals]$, then the planner achieves a utility of $0$ under $\pi_{\mathrm{NI}}$.  

Consequently, to solve~\eqref{eqn:red_1_form}, it is useful to distinguish the following qualitative different cases (\emph{regimes}) based on the position of $\priormean$ relative to the intervals $\{[\lol{k},\hil{k}]\}_{k \in [K]}$. These regimes can be defined in terms of $\cup_{k=1}^K \bar{\Theta}_k$ as follows: 
\begin{itemize}
    \item[] $(\mathrm{R1})$: $\priormean \in \cup_{k=1}^K \bar{\Theta}_k$. The prior mean $\priormean$ lies in one of the intervals $\bar{\Theta}_k$ (and as noted above $\pi_{\mathrm{NI}}$ is optimal in this regime).     
    \item[]  $(\mathrm{R2})$: $\priormean > \sup \cup_{k=1}^K\bar{\Theta}_k$. Equivalently, $\hil{\numintervals}<\priormean\leq \maximal$, where $\maximal$ is the maximum value of the state.  
    \item[]  $(\mathrm{R3})$: $\priormean < \inf \cup_{k=1}^K\bar{\Theta}_k$. Equivalently, $0\leq\priormean < \lol{1}$.
    \item[] $(\mathrm{R4})$: $\priormean \notin \cup_{k=1}^K \bar{\Theta}_k\; \wedge \; \inf \cup_{k=1}^K\bar{\Theta}_k < \priormean < \sup \cup_{k=1}^K\bar{\Theta}_k $. That is, $\priormean$ does not lie in any interval but lies in the gap between two contiguous intervals ($\exists k\in[\numintervals]$ such that $\priormean\in( \hil{k}, \lol{k+1})$). 
\end{itemize}

Furthermore, in any regime, any direct mechanism~$\mathcal{T}_\pi$ that solves~\eqref{eqn:red_1_form} is not unique in general. This follows from the fact that any signal $i\in\I$ with signal probability~$q_i$ and posterior mean~$\posterior{i}$ can be forked into two signals $i_i$, $i_2$ uniformly at random to induce symmetric posterior means~$\posterior{i_1}=\posterior{i_2}=\posterior{i}$ with probability~$\sfrac{q_i}{2}$ each, and hence such a construction achieves the same planner objective. However, the following lemma shows that the search for an optimal mechanism can be limited to the class of direct mechanisms that use a set of signals~$\I$ of size at most $|\I|=\numintervals+1$. 
\begin{lemma}
\label{lemma:num_signals_bdd}
There exists a direct mechanism~$\mathcal{T}_{\pi}^\ast=\{(q_\signal, \posterior{\signal})\}_{\signal \in [\numintervals+1]}$ that achieves optimal planner objective in~\eqref{eqn:red_1_form} and satisfies following constraints:
\[\posterior{i} \in \bar{\Theta}_i,\quad i=1,\dots,\numintervals, \quad \text{and} \quad \posterior{K+1} \notin \cup_{k=1}^K \bar{\Theta}_k.\]
\end{lemma}
That is, to solve for an optimal mechanism, we need at most one signal for each of the $\numintervals$ intervals  (i.e., $\bar{\Theta}_i,\; i=1,\dots,\numintervals$) to induce posterior mean in the desirable set, and one additional signal that induces posterior mean that does not lie in any of these sets. We henceforth use this insight to search over mechanisms that can be represented by the set of tuples~$\{(q_\signal, \posterior{\signal})\}_{\signal \in [\numintervals+1]}$, and define the (cumulative) distribution of posterior means for such a set of tuples as $H(t) = \sum_{k=1}^{K+1} q_k \mathbb{I}\{\posterior{k} \leq t\}$.

We say that posterior mean distribution $H$ corresponding to~$\mathcal T_\pi=\{(q_\signal, \posterior{\signal})\}_{\signal \in [\numintervals+1]}$ is a \emph{mean-preserving contraction} if and only if for any $y\in \paramspace$, $\int_0^y H(t)dt \leq \int_0^y F(t)dt$, with equality for $y=\maximal$. If $H$ is a mean-preserving contraction of $\dist$ we write $H \succcurlyeq \dist$ (i.e., $H$ majorizes $\dist$). \textcolor{blue}{This relationship can be expressed as following equivalent constraints: 
\begin{align}
   \int_0^y (1-H(t)) dt \geq \int_0^y (1-F(t)) dt,  \forall y\in \paramspace \quad \Leftrightarrow \quad \int_0^x H^{-1}(s) ds \geq \int_0^x F^{-1}(s) ds, \forall x\in [0,1]\label{eq:MPC_constraint1}
\end{align}
with equality at $y=\maximal$ (resp. $x=1$).}

Following the seminal result from~\cite{gentzkow_rothschild-stiglitz_2016,blackwell_theory_1954}, we know that set of tuples~$\{(q_\signal, \posterior{\signal})\}_{\signal \in [\numintervals+1]}$ is implementable via a signaling mechanism~$\pi$ \emph{if and only if} the corresponding posterior mean distribution~$H\succcurlyeq \dist$, i.e., $H$ is a mean-preserving contraction of the prior distribution~$\dist$. Intuitively, implementability requires that the mechanism shifts the probability mass from the tails of the prior distribution~$\dist$ ``inward'' in a manner that preserves the mean of the distribution (both $\dist$ and posterior distribution~$H$ have equal means).  

\textcolor{blue}{We note that $f(x)=\int_0^x F^{-1}(s) ds$ is convex in $x$ with $f(0)=0$. Furthermore, by definition of $H$, $\int_0^u H^{-1}(s) ds$ is a piecewise linear function in $u$ with breakpoints in the set~$\{\sum_{j}^m q_j: m\in[\numintervals+1]\}$.} Hence, we obtain that to ensure $H\succcurlyeq \dist$, it suffices to enforce the constraint~\eqref{eq:MPC_constraint1} at these breakpoints. The following lemma captures this observation:
\begin{lemma}
For the posterior distribution of means defined as $H(t)=\sum_{k=1}^{K+1} q_k \mathbb{I}\{\posterior{k} \leq t\}$ for all $t\in\paramspace$, enforcing that $H\succcurlyeq \dist$ is equivalent to the following constraints:
\begin{subequations}\label{eq:MPCall}
\begin{align}
    &\sum_{j=1}^{m} q_j\posterior{j} \geq \int_0^{\sum_{j=1}^{m} q_j} \dist^{-1}(s)ds,\quad \forall m \in [\numintervals] \label{eqn:MPC}\\
 &\sum_{j=1}^{\numintervals+1} q_j \posterior{j} = \priormean. \label{eqn:mean_mean}
\end{align}
\end{subequations}
\end{lemma}

Finally, we highlight a class of signaling mechanisms that plays an important role in our subsequent results. We say that a signaling mechanism~$\pi$ has a \emph{Monotone Partitional Structure} (MPS) if there exists a finite partition of the state-space~$\paramspace$, defined as $\mathcal{P} \coloneqq \{\paramspace_j\}_{j=1}^m = \{[t_{j-1},t_j]\}_{j=1}^m$  for some $m$ with $0=t_0<t_1<\dots<t_{m-1}<t_m = \maximal$, such that $\I=[m]$ and for any $\param\in\paramspace$, $z_\param(j) = \mathbb{I}\{\param \in [t_{j-1}, t_j]\}$. The corresponding direct counterpart can be written as the set of tuples~$\{(q_j, \posterior{j})\}_{j \in [m]}$, where following~\eqref{eqn:q_i} and \eqref{eqn:theta_i}, $q_j = \dist(t_j) - \dist(t_{j-1})$ and $\posterior{j} = \sfrac{\int_{t_{j-1}}^{t_j} \param d\dist(\param)}{q_j}$. 

We are now in the position to characterize the optimal signaling mechanism for the regimes $\mathrm{R1}-\mathrm{R3}$ (we already know that $\pi_{\mathrm{NI}}$ is optimal in regime~$\mathrm{R1}$). The following proposition shows that the optimal signaling mechanism in these three regimes has a monotone partitional structure. (This property does not necessarily hold for regime $\mathrm{R4}$, as discussed subsequently.) Before proceeding we define the increasing function for any $\param\in\paramspace$:
\begin{align}
    \bar f(\param) \coloneqq \sup\left\{x:\int_0^x F^{-1}(s)ds \leq x \param\right\},\label{eq:barffn}
\end{align}
and note that for any~$\param\in\paramspace$ the constraint $\param x\geq f(x)$ is satisfied if and only if $0\leq x\leq \bar f(\param)$. 

\begin{prop}
The optimal value of planner's objective~$V_{F,h}^\ast$ and the corresponding signaling mechanism~$\pi_{F,\obj}^\ast$ for the regimes~$\mathrm{R1}-\mathrm{R3}$ are as follows:
\begin{itemize}
    \item[] $(\mathrm{R1})$: $V_{F,h}^\ast=1$ and $\pi_{F,\obj}^\ast=\langle \{1\}, \{z_\param\}_{\param \in \paramspace}\rangle$ with $z_\param(1) = 1$ for all $\param\in\paramspace$. 
    \item[]  $(\mathrm{R2})$: $V_{F,\obj}^\ast = q_1^\ast$ where  $ q_1^\ast\coloneqq \min\left\{\bar f(\hil{\numintervals}),\frac{M-\priormean}{M-\hil{\numintervals}}\right\}$ and $\pi_{F,\obj}^\ast = \langle \{z_\param\}_{\param \in \paramspace}, \{1,2\}\rangle$ with $z_\param(1) = 1$ for $\param \leq F^{-1}(q_1^\ast)$ and $z_\param(2) = 1$ for $\param > F^{-1}(q_1^\ast)$.
  
    \item[] $(\mathrm{R3})$: $V_{F,\obj}^\ast = 1-q_2^\ast$ where $q_2^\ast \coloneqq \inf\left\{q \geq \frac{\lol{1}-\priormean}{\lol{1}}:q \leq \bar f(\lol{1}-\frac{\lol{1}-\priormean}{q})\right \}$ and $\pi_{F,\obj}^* = \langle \{z_\param\}_{\param \in \paramspace}, \{1,2\}\rangle$ with $z_\param(1) = 1$ for $\param > F^{-1}(q_2^\ast)$ and $z_\param(2) = 1$ for $\param \leq F^{-1}(q_2^\ast)$. 
\end{itemize}
Thus, $\pi_{F,\obj}^\ast$ has a monotone partitional structure in regimes~$\mathrm{R1}-\mathrm{R3}$: $t_0 = 0$ and $t_1 = M$ for $(\mathrm{R1})$; $t_0 = 0$, $t_1 = F^{-1}(q_1^*)$ and $t_2 = M$ for $(\mathrm{R2})$; and $t_0 = 0$, $t_1 = F^{-1}(q_2^*)$ and $t_2 = M$ for $(\mathrm{R3})$.  
\label{prop:r123}
\end{prop}

\begin{proof}
In $\mathrm{R1}$, we know that $\pi_{F,\obj}^\ast=\pi_{\mathrm{NI}}$, and hence $\mathcal T_{NI}=\{(1, \priormean)\}$. From~\eqref{eqn:red_1_form}, we obtain~$V_{F,h}^\ast=1$ (the maximum value of planner's objective function).

In general, appealing to lemma~\ref{lemma:num_signals_bdd}, we can simplify the objective function in~\eqref{eqn:red_1_form} as follows:
\begin{align*}
    \sum_{i =1}^{\numintervals+1} \sum_{k=1}^{\numintervals} q_i \mathbb{I}\{\lol{k} \leq \posterior{i} \leq \hil{k}\}=\sum_{i=1}^\numintervals q_i = \left(1-q_{\numintervals+1}\right). 
\end{align*}
Hence, the problem of optimal signaling mechanism design can be expressed as follows:
\begin{align*}
    &\min_{\mathcal{T}_\pi: \{(q_i, \posterior{i})\}_{i \in [\numintervals+1]}}  q_{\numintervals+1}\\
    \text{s.t.} & \quad H\succcurlyeq \dist, \\ 
    & \quad   \posterior{i} \in \bar{\Theta}_i,\quad i\in[\numintervals],  
\end{align*}
where the second constraint ensures that posterior distribution $H$ is a mean-preserving contraction of prior distribution~$\dist$. Using~lemma~\eqref{eq:MPCall}, the definitions of sets~$\bar{\Theta}_i$, and the fact that all signal probabilities must sum to~$1$, we can re-write the above problem:  
\begin{subequations}\label{eq:equivalentopt}
\begin{align}
 &\min q_{\numintervals+1} \label{eq:qkplus1}\\ 
    \text{s.t.}   &\sum_{i \in [\numintervals+1]} q_i=1 \label{eq:probsum}\\ 
    & \lol{i}\leq \posterior{i} \leq \hil{i}, \quad \forall i\in[\numintervals] \label{eq:posteriorbounds}\\
    & \eqref{eqn:MPC}, \eqref{eqn:mean_mean} \nonumber. 
\end{align}
\end{subequations}
We now proceed to solve for the optimal signaling mechanism for~$\mathrm{R2}$; the proof for~$\mathrm{R3}$ is analogous. \textcolor{blue}{For simplicity and without loss of generality, we assume $\maximal=1$ since any optimal solution is invariant to linear scaling.}

\underline{Claim 1.} $\posterior{\numintervals+1} \geq \priormean$ and $q_{\numintervals+1} > 0$, hence $q_{\numintervals+1}^\ast > 0$. 

Under~$\mathrm{R2}$, we know that $\hil{\numintervals}<\priormean$. From constraint $\posterior{\numintervals}\leq\hil{\numintervals}$, we obtain $\posterior{\numintervals}\leq \hil{\numintervals}<\priormean$. \\
Suppose that $\posterior{\numintervals+1}<\priormean$. Then by~\eqref{eqn:mean_mean} and by condition of $\mathrm{R2}$, we obtain $\priormean=\sum_{i=1}^{\numintervals+1} q_i \posterior{i}< \sum_{i=1}^{\numintervals+1} q_i \priormean = \priormean$. However, this is a contradiction. Hence, we conclude that  $\mu_{\numintervals+1}\geq\priormean$.\\
Next, suppose that $q_{\numintervals+1}=0$. Then, $\priormean=\sum_{i=1}^\numintervals q_i \posterior{i}\leq \sum_{i=1}^\numintervals q_i \hil{i} \leq \hil{\numintervals} \sum_{i=1}^\numintervals q_i = \hil{\numintervals}$. However, this is a contradiction since under~$\mathrm{R2}$, $\hil{\numintervals}<\priormean$. Hence, we conclude that  $q_{\numintervals+1}>0$ (and hence $q_{\numintervals+1}^\ast > 0$).

\underline{Claim 2.} $q_j^* = 0$ for all $j < \numintervals$.\\ 
Suppose for the sake of contradiction that $q_j^\ast > 0$ for some $j < \numintervals$, and let the corresponding distribution of posterior means by denoted~$H^\ast$. Now consider the new distribution of signal probabilities obtained by decreasing $q_j^\ast$ by $\tfrac{(\posterior{\numintervals+1}^\ast-\posterior{\numintervals}^\ast)}{(\posterior{\numintervals+1}^\ast-\posterior{j}^\ast)}\epsilon$, increasing $q_{\numintervals}^*$ by $\epsilon$, decreasing $q_{\numintervals+1}^*$ by $\tfrac{(\posterior{\numintervals}^\ast-\posterior{j}^\ast)}{(\posterior{\numintervals+1}^\ast-\posterior{j}^\ast)}\epsilon$, for a small $\epsilon>0$. Then, the value of objective~\eqref{eq:qkplus1} strictly increases and constraints~\eqref{eq:probsum} and~\eqref{eq:posteriorbounds} are still satisfied. Furthermore, this is a convex stochastic modification of the original mechanism; hence the modified set of tuples generates a distribution of posterior means such that~$H'\succcurlyeq H^\ast$ (refer to~Theorem 3.A.7. of \cite{shaked_univariate_2007}). By transitivity, we obtain that $H'\succcurlyeq \dist$, which implies that constraints~\eqref{eqn:MPC}, \eqref{eqn:mean_mean} for ensuring mean-preserving contraction also hold. This establishes the contradiction. Hence, $q_j^* = 0$ for all $j < \numintervals$.  

Following these results, we can simply rename $q_{\numintervals}$ to $q_1$ and $q_{\numintervals+1}$ to $q_2$ (and similarly for $\posterior_\numintervals$ and $\posterior_{\numintervals+1}$), and simplify~\eqref{eq:equivalentopt} as follows: 
\begin{subequations}\label{eq:simpleopt}
\begin{align}
   & \max_{q_1,q_2,\posterior{1},\posterior{2}} q_1 \\
  \text{s.t.}\quad & q_1+q_2=1 \\
   & \lol{\numintervals} \leq  \posterior{1} \leq \hil{\numintervals} \\
   & \priormean \leq \posterior{2} \leq \maximal \\
   & q_1\posterior{1} \geq \int_0^{q_1} \dist^{-1}(s)ds \label{eqn:convv_new}\\ 
   & q_1 \posterior{1} + q_2 \posterior{2} = \priormean. 
\end{align}
\end{subequations}
Suppose that~$q_1^\ast,q_2^\ast,\posterior{1}^\ast,\posterior{2}^\ast$ is an optimal solution of ~\eqref{eq:simpleopt} with~$\posterior{1}^* < \hil{\numintervals}$. Then we can find another optimal solution by choosing same signal probabilities~$q_1'=q_1^\ast$, $q_2'=q_2^\ast$, but the posterior means as $\posterior{1}'=\hil{\numintervals}$ and $\posterior{2}'=\priormean+\tfrac{(\posterior-\hil{\numintervals})(\posterior{2}^\ast-\priormean)}{(\priormean-\posterior{1}^\ast)}$ (this follows by noting that all the constraints in~\eqref{eq:simpleopt} are satisfied). Hence, we can restrict~$\posterior{1}=\hil{\numintervals}$ in the optimal design. Following~\eqref{eq:barffn}, we can rewrite~\eqref{eqn:convv_new} as $0\leq q_1 \leq \bar f(\hil{\numintervals})$ and substitute $q_2$ with $1-q_1$ to obtain:
\begin{subequations}\label{eq:finalopt}
\begin{align}
    &\max_{q_1,\posterior{2}} q_1 \\
    \text{ s.t.   } &q_1 \hil{\numintervals} + (1-q_1) \posterior{2} = \priormean \label{eq:finalopt1}\\
    & 0 \leq q_1 \leq h(\hil{\numintervals}) \label{eq:finalopt2}\\
    % & \int_{0}^{q_1} \dist^{-1}(t) dt \leq q_1 \hil{\numintervals}\\
  & \priormean \leq \posterior{2} \leq M \label{eq:finalopt3}
\end{align}
\end{subequations}

From~\eqref{eq:finalopt1} we obtain  $q_1=\frac{\posterior{2}-\priormean}{\posterior{2}-\hil{\numintervals}}$ and using $\hil{\numintervals}\leq \priormean \leq \posterior{2} \leq M$ (Claim 1 and~\eqref{eq:finalopt3}), we know that $q_1\leq \frac{\maximal-\priormean}{\maximal-\hil{\numintervals}}$. Combining with~\eqref{eq:finalopt2}, the optimal value of~\eqref{eq:finalopt} is $q_1^\ast=\min\{\bar f(\hil{\numintervals}),\frac{M-\priormean}{M-\hil{\numintervals}}\}$. Finally, $\posterior{2}^\ast=\frac{\priormean-q_1^\ast \hil{\numintervals}}{1-q_1^\ast}$, $\posterior{1}^\ast=\hil{\numintervals}$, and $q_2^\ast=1-q_1^\ast$, specifies the optimal direct mechanism~$\mathcal T^\ast=$  




\vspace{2cm}
 

\end{proof}














\newpage
\st{\noindent In this section, we consider planners with state-independent, set-based preferences $\obj(\fin; \trueparam) = \mathbb{I}\{\fin\in\goal\}$ for some set of desirable masses $\goal$ that is specified for the planner. In Sec. \ref{subsec:max_static}, we show that when $\dist$ and $\goal$ obey certain regularity conditions, the optimal signalling mechanism has MPS. We then provide some numerical results to validate the improvement of this optimal mechanism against classical information benchmarks in Sec. \ref{subsec:numerical_state_indpt}. }
% Finally, in Sec. \ref{subsec:counterexample_mps} we demonstrate with an example that as preferences become state-dependent, monotone partitional signalling is not sufficient to achieve optimal design. 

\subsection{Optimal Information Design for State-Independent Objectives}
\label{subsec:max_static}
\noindent 
\st{We consider preferences of the form $\obj(\fin; \trueparam) = \mathbb{I}\{\fin\in\goal\}$ and solve for the optimal design formulated in \eqref{eqn:opt_v}. Observe that for preferences of this form, the planner is equivalently maximizing the probability the remote mass lies in $\goal$ irrespective of $\trueparam$. We make the following assumption that $\goal$ is well-behaved by which it can be expressed as a finite collection of closed intervals $\Omega_i=[\wll{i}, \wlh{i}]$. Practically, the choice of $\Omega_i$ could be driven by a combination of feasible capacities for possible workplace venues and capacity limits adhering to public safety guideliens. These intervals could also be motivated by a more general continuous form of preferences $\obj$ where certain remote masses achieve sufficiently high planner utility (i.e. $\{y: \E_{\trueparam\sim\dist}[\obj(\fin;\trueparam) ]\geq \mathcal{C}\}$ for some given utility baseline $\mathcal{C}$).}


\begin{ass*}[\textbf{A1}]
\st{$\goal = \cup_{k=1}^{\numintervals}\Omega_k\coloneqq\cup_{k=1}^{\numintervals} [\wll{k}, \wlh{k}]$ can be expressed as the union of finitely many closed intervals ($\numintervals < \infty$) where $0 \leq \wll{k} \leq \wlh{k} \leq 1$ for all $k$. Without loss of generality, these intervals are increasing and disjoint (i.e. $\wlh{k} < \wll{k+1}$ for all $k$).}
\end{ass*}


\st{\noindent We can now reformulate \eqref{eqn:opt_v} to simply depend on whether the remote masses lie in one of the disjoint intervals $\Omega_i$:}
\begin{align}
    V_{F,h}^* &= \max_{\pi: \langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \mathbb{P}\{\final({\signal}) \in \goal\} \nonumber\\
         &= \max_{\pi: \langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \mathbb{P}\{\final({\signal}) \in \cup_{k=1}^{\numintervals} \Omega_k\} \nonumber\\
         &= \max_{\pi: \langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \sum_{k=1}^{\numintervals} \mathbb{P}\{\wll{k} \leq m(\posterior{\signal}) \leq \wll{k}\} 
 %        \label{eqn:value_c_i}
\end{align}

\st{Using Lemma $\ref{lemma:m_smooth}$, observe that the preimage of $m(\cdot)$ over the closed interval $[\wll{k},\wlh{k}]$ is another closed interval $[\lol{k}, \hil{k}]$ where $m(\posterior{\signal}) \in \Omega_k$ if and only if $\posterior{\signal} \in \bar{\Theta}_k \coloneqq [\lol{k}, \hil{k}]$. Observe by the monotonocity of $m$, $\lol{k}$ and $\hil{k}$ are increasing in $k$. 
Exploiting this fact and by searching over all mechanism $\pi$'s corresponding direct mechanisms $\mathcal{T}_\pi$ as computed in \eqref{eqn:q_i} and \eqref{eqn:theta_i}, we can reformulate the planner's problem as:}
\begin{align}
        V_{F,h}^* &= \max_{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in \I}} \sum_{s \in \I} \sum_{k=1}^{K} q_s \mathbb{I}\{\lol{k} \leq \posterior{s} \leq \hil{k}\}           
  %      \label{eqn:red_1_form}
\end{align}

\st{\noindent We make some immediate observations about this formulation for the optimal design. Consider a non-informative mechanism $\pi_{NI}$ which can be constructed by selecting $\I =\{s\}$ to be a singleton which yields a direct mechanism $\mathcal{T}_{NI} = \{(1,\priormean)\}$. If the prior mean belief $\E_{\param \sim \dist}[\param] \coloneqq \priormean \in [\lol{k},\hil{k}]$ for some $k$, the planner achieves the maximum possible objective of $1$ by choosing $\pi_{NI}$. However, if $\priormean \notin [\lol{k},\hil{k}]$ for all $k$, then choosing $\pi_{NI}$ achieves an objective of 0. }

\st{\noindent Consequently, in order to solve for the optimal mechanism, it is useful to distinguish possible distributions $\dist$ based on the position of its corresponding prior mean $\priormean$ relative to the intervals $\{[\lol{k},\hil{k}]\}_{k \in [K]}$. In order to characterize these regimes, consider the following increasing functions $\ubar{s}(t) = \E[\param|\param \leq t]$ and $\bar{s}(t) = \E[\param|\param \geq t]$ which are computable from $\dist$. 
% Then, we can define $\delta(\alpha,\lambda, t) \coloneqq \frac{ \ubar{s}(t) \lambda F(t) +  \bar{s}(t) \alpha (1-F(t))}{\lambda F(t) +  \alpha (1-F(t))}$ to represent the posterior mean belief when receiving a signal that is generated with probability $\lambda$ for $\param \leq t$ and with probability $\alpha$ for $\param > t$. 
We breakout the following subcases on the prior distribution $\dist$ relative to $\cup_{k=1}^K \bar{\Theta}_k$:}
(let $p(t,\theta) = \frac{(1-F(t))(\bar{s}(t)-\theta)}{F(t)(\theta-\ubar{s}(t))}$)
\begin{align*}
&\text{(R1): } \priormean \in \cup_{k=1}^K \bar{\Theta}_k \\
&\text{(R2): } \priormean > \sup \cup_{k=1}^K\bar{\Theta}_k \\
&\text{(R3): } \priormean < \inf \cup_{k=1}^K\bar{\Theta}_k \\
&\text{(R4): } \priormean \notin \cup_{k=1}^K \bar{\Theta}_k, \inf \cup_{k=1}^K\bar{\Theta}_k < \priormean < \sup \cup_{k=1}^K\bar{\Theta}_k \\
&\hspace{5mm}\text{(R4a): } \exists \theta', \theta'' \in \cup_{k=1}^K \bar{\Theta}_k, \delta \in [0,1], t \in \paramspace \\
&\quad \quad \quad \quad \text{ s.t. } 0 \leq \delta p(t,\theta') \leq 1 \\ &\quad \quad \quad \quad \text{ s.t. } \delta p(t,\theta')+(1-\delta) p(t,\theta'') = 1
\end{align*}

\st{\noindent The above subcases are illustrated in Fig. \ref{fig:result}. (R1) captures the aforementioned case where the prior distribution's mean $\priormean$ already lies in an interval $\bar{\Omega}_k$ and the planner can consequently maximize its objective with the non-informative mechanism. Both (R2) and (R3) capture distributions where $\priormean$ lies outside the convex hull of the intervals. (R4) considers when $\priormean$ does not lie in any interval, but lies in the gap between two intervals.} 

Intuitively, in this case the planner seeks to spread mean beliefs outwards from the prior mean. However, this information design may not be feasible for distributions $\dist$ that induce beliefs that are tightly concentrated in this gap. Under this setting, either $\bar{s}(t)$ is close to $\priormean$ and $F(t)$ close to 0 or $\ubar{s}(t)$ is close to $\priormean$ and $F(t)$ close to 1 for most values of $t$. Consequently, we focus on a more likely case -- subcase (R4a) -- where the conditions are met when $\dist$ has sufficient probability mass outside the gap between two intervals surrounding $\priormean$.

\st{\noindent Before solving for an optimal mechanism in each regime, note that any direct mechanism $\mathcal{T}_\pi$ that is a solution to \eqref{eqn:red_1_form} is not unique in general. This is immediate as any signal $i \in \I$ can be forked into two signals $i_1, i_2$ uniformly at random and induce symmetric posterior means $\posterior{i} = \posterior{i_1} = \posterior{i_2}$ with probability $\frac{q_i}{2}$ each and hence achieve the same planner objective. To eliminate such multiplicity, we provide the following lemma: it shows that we need not consider mechanisms that use a set of signals $\I$ of size $|\I| > K +1$ since we require at most one signal to correspond to a posterior mean in each of the $K$ intervals and one extra signal whose posterior mean lies outside these sets. }
\begin{lemma}
%\label{lemma:num_signals_bdd}
\st{There exists an optimal mechanism $\pi_{F,\obj}^* = \langle \{z^*_\param\}_{\param \in \paramspace}, [K+1] \rangle$ where $V(\pi_{F,\obj}^*) = V_{F,\obj}^*$ such that for each $s \in [K]$, $\posterior{s} \in \bar{\Theta}_s$ and $\posterior{K+1} \notin \cup_{k=1}^K \bar{\Theta}_k$.}
\end{lemma}
\st{This insight consequently reduces the search problem (\eqref{eqn:red_1_form}) over all possible mechanisms $\pi$ to those that use at most $K+1$ signals. We equivalently search over all $\mathcal{T}_\pi$ with at most $K+1$ tuples with $\posterior{s}$ obeying the constraints determined by Lemma} \ref{lemma:num_signals_bdd}.\st{ In order to ensure we only search over the sets of $K+1$ tuples $\{(q_s,\posterior{s})\}_{s \in [K+1]}$ that correspond to $\mathcal{T}_\pi$ that are equivalent to a signalling mechanism $\pi$, define the posterior mean distribution $H$ specified by any set of tuples to have cumulative distribution $H(t) = \sum_{s=1}^{K+1} q_s \mathbb{I}\{\posterior{s} \leq t\}$.} 

\st{It is known that the posterior mean distribution $H$ corresponding to $\mathcal{T}_\pi = \{(q_s,\posterior{s})\}_{s \in [K+1]}$ must be a \textit{mean-preserving contraction} of $\dist$ if and only if the tuple $\mathcal{T}_\pi$ is implementable through a signalling mechanism $\pi$ \cite{gentzkow_rothschild-stiglitz_2016,blackwell_theory_1954}. Formally, $\dist \preccurlyeq H$ is a mean-preserving contraction if and only if $\forall c \in \paramspace$, $\int_{0}^{c} H(t)dt \leq \int_{0}^{c} \dist(t)dt$. Intuitively, the distribution of the posterior means must shift mass towards the mean from the tails of the distribution $\dist$. }

\st{\noindent We exploit the above reduction to solve for the optimal mechanism in $\eqref{eqn:red_1_form}$. The following theorem characterizes the optimal planner objective and optimal mechanism across R1, R2, and R3 (we discuss the optimal direct signalling mechanism for R2 in the proof of the theorem). We show that the optimal signalling mechanisms provided all have MPS.}

\begin{theorem}
\label{thm:stateless}
% $\min\{c(\hil{N}),\frac{\priormean}{\hil{N}}\}$
\st{Define the increasing function $h(\param) \coloneqq \sup\{s:\int_0^s F^{-1}(t)dt \leq s \param\}$. The optimal objective $V^*$ and a corresponding optimal mechanism can be computed as follows for each subcase:\\
(R1): 
$V_{F,\obj}^* = 1$ and $\pi_{F,\obj}^* = \langle \{z_\param\}_{\param \in \paramspace}, \{1\}\rangle$ with $z_\param(1) = 1$ for all $\theta$. This is a monotone partitional mechanism with $t_0 = 0$ and $t_1 = M$.  \\
(R2):
$V_{F,\obj}^* = q_1^* \coloneqq \min\{h(\hil{N}),\frac{M-\priormean}{M-\hil{N}}\}$ and $\pi_{F,\obj}^* = \langle \{z_\param\}_{\param \in \paramspace}, \{1,2\}\rangle$ with $z_\param(1) = 1$ for $\param \leq F^{-1}(q_1^*)$ and $z_\param(2) = 1$ for $\param > F^{-1}(q_1^*)$. This is a monotone partitional mechanism with $t_0 = 0$, $t_1 = F^{-1}(q_1^*)$ and $t_2 = M$. \\
(R3):
$V_{F,\obj}^* = 1-q_2^*$ where $q_2^* \coloneqq \inf\{q \geq \frac{\lol{1}-\priormean}{\lol{1}}:q \leq h(\lol{1}-\frac{\lol{1}-\priormean}{q}) \}$ and $\pi_{F,\obj}^* = \langle \{z_\param\}_{\param \in \paramspace}, \{1,2\}\rangle$ with $z_\param(2) = 1$ for $\param \leq F^{-1}(q_2^*)$ and $z_\param(1) = 1$ for $\param > F^{-1}(q_2^*)$. This is a monotone partitional mechanism with $t_0 = 0$, $t_1 = F^{-1}(q_2^*)$ and $t_2 = M$.}
\end{theorem}
\begin{proof}
 
\st{(R1) The proof for R1 follows from construction as $\pi_{F,\obj}^*$ induces $\mathcal{T}_{\pi_{F,\obj}^*} = \{(1,\priormean)\}$ and from Equation $\eqref{eqn:red_1_form}$ this implies that $V_{F,\obj}^* = 1$ which is maximal.} \\

(R2 \& R3) \\
\noindent The proofs for R2 and R3 are symmetric (can modify all objects in $\Theta$ by going from $\theta$ to $M-\theta$ and the proof is analogous) so we only prove R2. Moreover, without loss of generality, assume $M=1$ as an optimal signalling mechanism is invariant to linear scaling. Appealing to Lemma \ref{lemma:num_signals_bdd} and using the equivalence of mean-preserving contractions, observe:
\begin{align}
V_{F,h}^* &= \max_{\substack{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in [\numintervals+1]} \\ H \succcurlyeq \dist \\\posterior{s} \in \bar{\Theta}_s \forall s\in[\numintervals]} } \sum_{s =1}^{\numintervals+1} \sum_{k=1}^{\numintervals} q_s \mathbb{I}\{\posterior{s} \in \bar{\Theta}_k\} \nonumber\\
&= \max_{\substack{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in [\numintervals+1]} \\ H \succcurlyeq \dist \\\posterior{s} \in \bar{\Theta}_s \forall s\in[\numintervals]} } \sum_{s=1}^{\numintervals}q_s \nonumber\\
&= \max_{\substack{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in [\numintervals+1]} \\ H \succcurlyeq \dist \\\posterior{s} \in \bar{\Theta}_s \forall s\in[\numintervals]} } 1-q_{\numintervals+1} \nonumber\\
&= \min_{\substack{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in [\numintervals+1]} \\ H \succcurlyeq \dist \\\posterior{s} \in \bar{\Theta}_s \forall s\in[\numintervals]} } q_{\numintervals+1} \label{eqn:MPC_1}
\end{align}

\st{Observe that $H \succcurlyeq \dist$ if and only if $\int_{0}^{c} (1-H(t))dt \geq \int_{0}^{c} (1-\dist(t))dt$ for all $c \in [0,1]$ with equality at $c=1$. Taking the standard inverse in the quantile space, this is equivalent to $\int_{0}^{c} H^{-1}(t)dt \geq \int_{0}^{c} F^{-1}(t)dt$ for all $c \in [0,1]$ with equality at $c=1$. We will refer to each of these constraints as the \textit{MPC constraints}. Observe that $\int_0^c \dist^{-1}(t)dt$ is convex in $s$ and that $\int_0^c G^{-1}(t)dt$ is piecewise-linear in $c$ with breakpoints at $x \in \mathcal{S}\coloneqq \{\sum_{j=1}^m q_j: m \in [\numintervals+1]\}$. Consequently, enforcing all the MPC constraints is equivalent to only enforcing the MPC constraints for values of $c \in \mathcal{S}$ since the remaining constraints are implications of these constraints. Fully describing the optimization problem posed in \eqref{eqn:MPC_1}:}
 \begin{align}
 &\min q_{\numintervals+1}    \nonumber      \\
 \text{s.t. }&\sum_{s=1}^{\numintervals+1} q_s = 1 \nonumber\\
 & \lol{s} \leq \posterior{s} \leq \hil{s} \hspace{1cm} \forall s \in [\numintervals] \nonumber\\
%  & \priormean \leq \posterior{\numintervals+1} \leq 1\\
 & \sum_{j=1}^{m} q_j\posterior{j} \geq \int_0^{\sum_{j=1}^{m} q_j} \dist^{-1}(t)dt\hspace{0.25cm} \forall m \in [\numintervals] %\label{eqn:MPC}
 \\
 &\sum_{s=1}^{\numintervals+1} q_s \posterior{s} = \priormean 
 %\label{eqn:mean_mean}
\end{align}


{Under (R3), observe that for any feasible solution $\posterior{\numintervals+1} > \priormean$ and $q_{\numintervals+1} > 0$ since $\priormean > \sup \cup_{k=1}^{\numintervals} \bar{\Theta}_k$ and \eqref{eqn:mean_mean} would otherwise produce infeasibility. Consequently, $q_{\numintervals+1}^* > 0$. Suppose by contradiction that $q_j^* > 0$ for some $j < \numintervals$ and let the distribution of posterior means be designated by $H^*$. Consider decreasing $q_j^*$ by $(\frac{\theta^*_{\numintervals+1}-\theta^*_{\numintervals}}{\theta^*_{\numintervals+1}-\theta^*_{j}})\epsilon$, increasing $q_{\numintervals}^*$ by $\epsilon$, decreasing $q_{\numintervals+1}^*$ by $(\frac{\theta^*_{\numintervals}-\theta^*_{j}}{\theta^*_{\numintervals+1}-\theta^*_{j}})\epsilon$. Then, observe that the objective is strictly improved and all the non-MPC constraints are still obeyed by design. Moreover, applying Theorem 3.A.7. of \cite{shaked_univariate_2007}, this is a convex stochastic modification and hence the modified tuples generate a distribution of posterior means $H' \succcurlyeq H^*$ so by transitivity $H' \succcurlyeq \dist$ so it will trivially satisfy the MPC constraints in Equation \eqref{eqn:MPC}. This is a contradiction so $q_j^* = 0$ for all $j < \numintervals$.} \\

Renaming $q_{\numintervals}$ to $q_1$ and $q_{\numintervals+1}$ to $q_2$, we can reduce the optimization to:
 \begin{align}
 &\max q_1             \\
 \text{s.t. }& q_1 \posterior{1} + q_2 \posterior{2} = \priormean \\
 & q_1 + q_2 = 1 \\
 & q_1\posterior{1} \geq \int_0^{q_1} \dist^{-1}(t)dt \label{eqn:convv} \\
  & \lol{\numintervals} \leq  \posterior{1} \leq \hil{\numintervals} \\
 & \priormean \leq \posterior{2} \leq 1
\end{align}
 Suppose we find a solution $q_1^*, q_2^*, \posterior{1}^*, \posterior{2}^*$ where $\posterior{1}^* < \hil{\numintervals}$. Observe that we can find another solution with the same objective by choosing $q_1' = q_1^*, q_2' = q_2^*$, $\posterior{1}^{'} = \hil{\numintervals}$ and $\posterior{2}^{'} = \priormean+\frac{(\priormean-\hil{\numintervals})(\posterior{2}^* - \priormean)}{(\priormean-\posterior{1}^*)}$. Observe that this solution obeys all the previous constraints. Consequently, we can restrict $\posterior{1} = \hil{\numintervals}$ without loss.\\
Observing that $f(x) = \int_0^{x} \dist^{-1}(t)dt$ is convex with $f(0) = 0$ implies that $\theta x \geq f(x)$ for all $x \in [0,h(\theta)]$. Replacing $\posterior{\numintervals}$ with $\hil{\numintervals}$, $q_2$ with $1-q_1$ and then the constraint in \eqref{eqn:convv} with $0 \leq q_1 \leq h(\hil{\numintervals})$ results in the following optimization:
\begin{align*}
    &\max_{q_1,\posterior{2}} q_1 \\
    \text{ s.t.   } &q_1 \hil{\numintervals} + (1-q_1) \posterior{2} = \priormean\\
    & 0 \leq q_1 \leq h(\hil{\numintervals})\\
    % & \int_{0}^{q_1} \dist^{-1}(t) dt \leq q_1 \hil{\numintervals}\\
  & \priormean \leq \posterior{2} \leq M
\end{align*}
We then eliminate $\posterior{2}$ by using the first constraint as $\posterior{2} = \frac{\priormean-q_1 \hil{\numintervals}}{1-q_1}$. Since $\priormean \geq \hil{\numintervals}$, $\priormean \leq \posterior{2} \leq M$ simplifies to $q_1 \leq \frac{M-\priormean}{M-\hil{\numintervals}}$ and we admit the solution that $q_1^* = \min\{h(\hil{\numintervals}),\frac{M-\priormean}{M-\hil{\numintervals}}\}$.

\noindent Finally, given the objective value $V_{F,\obj}^*$ and the direct mechanism $\mathcal{T}^* = \{(q_1^*, \posterior{1}^*),(q_2^*, \posterior{2}^*)\}$, we solve the corresponding problem of finding a mechanism $\pi_{F,\obj}^* = \langle \{z_\theta\}_{\theta \in \Theta},\I \rangle$ that achieves in $V_{F,\obj}^*$ and implements $\mathcal{T}^*$. To solve this, we appeal to the results in Remark 1 and Proposition 1 in \cite{gentzkow_rothschild-stiglitz_2016} as well as Theorem 3.A.4 in \cite{shaked_univariate_2007}. Consider the discrete distribution $H$ that places probability $q_1^*$ on $\hil{\numintervals}$ and $1-q_1^*$ on $\posterior{2}^*$. Then, the corresponding function $g(x) = \int_{0}^x H(t) dt$ defined by:
\begin{align}
    g(x) &= \begin{cases} 0 & x \leq \hil{\numintervals} \\ q_1^* (x-\hil{\numintervals}) & \hil{\numintervals} < x \leq \posterior{2}^* \\ q_1^*(\posterior{2}^*-\hil{\numintervals})+(x-\posterior{2}^*) & x > \posterior{2}^* \end{cases}
\end{align}
It is known that $g$ is convex and that, for $f(x) = \int_{0}^x F(t) dt$, $g(x) \leq f(x)$ for all $x \in [0,1]$. Observe that $g'(0) = f'(0)$ and $g'(1) = f'(1)$. From \cite{shaked_univariate_2007} and \cite{ivanov_optimal_2021}, it is known that if there exists $s \in [\hil{\numintervals},\posterior{2}^*]$ such that $f(s) = g(s)$, then $g$ is tangent to $f$ at $s$ and therefore is tangent on each linear segment of $g$. It is then a result that the mechanism can then be implemented using a monotone partitional signalling mechanism with $t_0 = 0, t_1 = s, t_2 = 1$ with $s = F^{-1}(q_1^*)$. This is consistent since the probability signal $1$ is generated is represented by $q_1^*$ and $\mathbb{P}[\theta \in [0,s]] = F(s) = F(F^{-1}(q_1^*)) = q_1^*$.

\noindent To show this holds in this setting, suppose by contradiction that for all $s \in [\hil{\numintervals},\posterior{2}^*]$, $f(s) > g(s)$. Then since $f-g$ is convex over $[\hil{\numintervals},\posterior{2}^*]$, let $\inf_{t \in [\hil{\numintervals},\posterior{2}^*]} f(t)-g(t) = \epsilon > 0$ with some minimizer $t^* \in [\hil{\numintervals},\posterior{2}^*]$ such that $f(t^*)-g(t^*) = \epsilon$. Moreover, let $\tilde{\posterior{2}^*}$ solve $(q_1^*+\epsilon)(x-\hil{\numintervals}) = q_1^*(\posterior{2}^*-\hil{\numintervals})+(x-\posterior{2}^*)$. Then consider the function $\tilde{g}$ as follows:
\begin{align*}
    \tilde{g}(x) &= \begin{cases} 0 & x \leq \hil{\numintervals} \\ (q_1^*+\epsilon) (x-\hil{\numintervals}) & \hil{\numintervals} < x \leq \tilde{\posterior{2}^*} \\ (q_1^*+\epsilon)(\tilde{\posterior{2}^*}-\hil{\numintervals})+(x-\tilde{\posterior{2}^*}) & x > \tilde{\posterior{2}^*} \end{cases}
\end{align*}
Observe that $\tilde{g}$ is still convex and that $g\leq\tilde{g}\leq f$, so by \cite{gentzkow_rothschild-stiglitz_2016} the distribution over posterior means with $q_1^*+\epsilon$ on $\hil{\numintervals}$ and $1-q_1^*-\epsilon$ on $\tilde{\posterior{2}^*}$ is implementable through a signalling mechanism. However, this violates the optimality of $q_1^*$ and is a contradiction. Hence, there must exist an  $s \in [\hil{\numintervals},\posterior{2}^*]$ such that $f(s) = g(s)$.
\qed
\end{proof}



 Notice that in subcase (R1), an optimal mechanism is trivially monotone partitional with a single signal; in Figure \ref{fig:result}, the entire probability mass over $\paramspace$ maps to a single signal. In (R2) and (R3) an optimal mechanism is also monotone partitional with two signals, where a threshold is specified by the theorem and the $\paramspace$ is partitioned into a ``low" and ``high" interval, where each interval corresponds to a signal. Under these three subcases, an optimal signalling mechanism is produced by Theorem \ref{thm:stateless} that necessarily has MPS.
 
 The remaining subcase (R4) will not necessarily allow for an optimal mechanism that obeys MPS structure as evidenced by the following example. 
 \begin{example}
 Let $\dist$ be uniform on $[0,1]$ ($\priormean = 0.5$). Assume $K=2$ and for some small $\epsilon$,  $\bar{\Omega}_1 = [0.4-\epsilon,0.4+\epsilon]$ and $\bar{\Omega}_2 = [0.6-\epsilon,0.6+\epsilon]$. Observe that no signalling mechanism with MPS can achieve an objective of $1$. To see this, consider a mechanism with MPS with $t_1 \in (0,1]$. If $t_1 = 1$ this mechanism is equivalent to a non-informative mechanism and because $\priormean \notin \bar{\Omega}_1\cup\bar{\Omega}_2$ the objective by \eqref{eqn:red_1_form} would be 0. If $t_1 < 0.8-2\epsilon$, then $\posterior{1} < 0.4 -\epsilon$ so $\posterior{1} \notin \bar{\Omega}_1\cup\bar{\Omega}_2$. Hence, the objective is less than $1-F(t_1) < 1$. If $0.8-2\epsilon \leq t < 1$, then $\posterior{k} \notin \bar{\Omega}_1\cup\bar{\Omega}_2$ for all $k > 1$, so the objective is $F(t_1) < 1$. Hence, in all cases of $t_1$, the objective is strictly worse than $1$. However observe that by choosing $\I = \{1,2\}$ with $z_{\param}(1) = 0.7$ for all $\param \leq 0.5$ and $z_{\param}(1) = 0.3$ for all $\param \geq 0.5$, the posterior means are $\posterior{1} = 0.4$ and $\posterior{2} = 0.6$.  Hence, the planner earns a utility of 1. Therefore, no signalling mechanism with MPS can be optimal.
 \end{example}  
 The previous example illustrates that under the subcase (R4) it is generally not possible to guarantee an optimal mechanism has MPS. However, in the example, observe that an optimal mechanism was produced that still partitions the interval into two components and uses a fixed distribution $z_{\param}(\cdot)$ in each interval. The following proposition formalizes this intuition by specifying that under subcase (R4a) we can constructively provide the best mechanism for most $\dist$ by partitioning $\paramspace$ into two intervals and using an interval-specific signalling distribution. 
 
\begin{prop}
\label{prop:stateless_r4a}
Under subcase (R4a), for some $\theta', \theta'', t, \delta$, letting $\lambda = \delta p(t,\theta')$, the optimal objective $V_{F,\obj}^* = 1$ and $\pi_{F,\obj}^* = \langle \{z_\param\}_{\param \in \paramspace}, \{1,2\}\rangle$ with $z_\param(1) = \lambda \mathbb{I}\{\param \in [0, t]\}+\delta \mathbb{I}\{\param \in (t, M]\}$ and $g_\param(1) = (1-\lambda) \mathbb{I}\{\param \in [0, t]\}+(1-\delta) \mathbb{I}\{\param \in (t, M]\}$.
\end{prop}
\begin{proof}
The proof follows from construction as $\pi_{F,\obj}^*$ induces $\mathcal{T}_{\pi_{F,\obj}^*} = \{(\lambda F(t) +  \delta(1-F(t)),\theta'),((1-\lambda) F(t) +  (1-\delta) (1-F(t)), \theta'')\}$ and from Equation $\eqref{eqn:red_1_form}$ this implies that $V_{F,\obj}^* = 1$ which is maximal. \qed
\end{proof}
In (R4a), we create two signals and identify a threshold $t$ where we split $\paramspace$ into two intervals at that threshold. In each interval, we then reveal the first signal with probability $\delta$ if $\param \leq t$ and with probability $\lambda$ if $\param > t$. Otherwise, we reveal the second signal. Consequently, the signals are generated according to an interval-specific distribution over just two signals. 

The general case of (R4) can be solved, however we cannot obtain closed form results generally and will simply show that the optimal objective and a \textit{direct} optimal signalling mechanism can be found using a convex program. Mapping the direct signalling mechanism map to an implementable mechanism is not trivial more generally under this setting.

\begin{prop}
The optimal objective $V^*$ and an optimal \textit{direct} signalling mechanism $\mathcal{T}_{\pi^*}$ can be solved generally by taking the minimal solution of $\numintervals$ convex programs.
\end{prop}
\begin{proof}
From the proof of Theorem \ref{thm:stateless}, observe that we can reduce the statement of the design problem as follows:
\begin{align*}
V_{F,h}^* &=  \min_{\substack{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in [\numintervals+1]} \\ H \succcurlyeq \dist \\\posterior{s} \in \bar{\Theta}_s \forall s\in[\numintervals]} } q_{\numintervals+1}
\end{align*}

It is known that $\posterior{k}$ is increasing for all $k \in [\numintervals]$, however it is not known where the $\mu_{\numintervals+1}$ is ordered within the set $\{\posterior{k}\}_{k \in [\numintervals]}$. 

Consequently, to solve this problem we take the union over the $\numintervals+1$ partitions by iterating over all $\numintervals+1$ possible placements of $\posterior{\numintervals+1}$ relative to $\{\posterior{i}\}_{i\in[\numintervals]}$, with $\mu_{j-1} < \mu_{\numintervals+1} \leq \mu_j$ corresponding to $OPT(j)$ as follows:
\begin{align*}
V_{F,h}^j &=  \min_{\substack{\mathcal{T}_\pi: \{(q_s, \posterior{s})\}_{s \in [\numintervals+1]} \\ H \succcurlyeq \dist \\\posterior{s} \in \bar{\Theta}_s \forall s\in[\numintervals], \mu_{j-1} < \mu_{\numintervals+1} \leq \mu_j}} q_{\numintervals+1}
\end{align*}
Moreover, 
\begin{align*}
V_{F,h}^* &=  \min_{j \in [\numintervals+1]} V_{F,h}^j
\end{align*}
To solve for $V_{\dist,\obj}^j$, we can appeal to the same techniques in Theorem \ref{thm:stateless}. Namely, $H \succcurlyeq \dist$ if and only if $\int_{0}^{c} H^{-1}(t)dt \geq \int_{0}^{c} F^{-1}(t)dt$ for all $c \in [0,1]$ with equality at $c=1$. Moreover, by the convexity of $\int_0^c \dist^{-1}(t)dt$ is convex in $s$, these mean-preserving contstraints can be enforced only at $x \in \mathcal{S}\coloneqq \{\sum_{j=1}^m q_j: m \in [\numintervals+1]\}$ without loss.
\begin{align}
 V_{\dist,\obj}^j =&\min q_{\numintervals+1}    \nonumber      \\
 \text{s.t. }&\sum_{s=1}^{\numintervals+1} q_s = 1 \nonumber\\
 & \lol{s} \leq \posterior{s} \leq \hil{s} \hspace{1cm} \forall s \in [\numintervals] \nonumber\\
%  & \priormean \leq \posterior{\numintervals+1} \leq 1\\
 & \sum_{j=1}^{m} q_j\posterior{j} \geq \int_0^{\sum_{j=1}^{m} q_j} \dist^{-1}(t)dt\hspace{0.25cm} \forall m \in [\numintervals]\\
 &\sum_{s=1}^{\numintervals+1} q_s \posterior{s} = \priormean
\end{align}
To solve each of these subproblems, we can introduce variables $z_j \coloneqq q_j\posterior{j}$ as in \cite{candogan_optimal_2021} to convexify the form and make this into a convex optimization problem.
\begin{align}
 V_{\dist,\obj}^j =&\min q_{\numintervals+1}    \nonumber      \\
 \text{s.t. }&\sum_{s=1}^{\numintervals+1} q_s = 1 \nonumber\\
 & \lol{s} \leq \posterior{s} \leq \hil{s} \hspace{1cm} \forall s \in [\numintervals] \nonumber\\
%  & \priormean \leq \posterior{\numintervals+1} \leq 1\\
 & \sum_{j=1}^{m} z_j \geq \int_0^{\sum_{j=1}^{m} q_j} \dist^{-1}(t)dt\hspace{0.25cm} \forall m \in [\numintervals] \nonumber\\
 &\sum_{j=1}^{\numintervals+1} z_j = \priormean \nonumber
\end{align}
\end{proof}

\begin{figure}[h]
    \centering
\includegraphics[width=180mm]{img/theorem_1.png}
    \caption{The pdf for $\trueparam$ and the intervals $[\lol{k},\hil{k}]$ (blue) with the solution for the three cases from Theorem $\ref{thm:stateless}$ marked by the induced posterior means $\posterior{1}, \posterior{2}$ (star). The posteriors are induced by mapping the probability mass to signals as marked (green, violet, yellow).}
    \label{fig:result}
    \vspace{-0.6cm}
\end{figure}

\begin{figure}[h]
    \centering
\includegraphics[width=90mm]{img/Prop_2.png}
    \vspace{-0.6cm}
    \caption{The pdf for $\trueparam$ and the intervals $[\lol{k},\hil{k}]$ (blue) with the solution for the three cases from Proposition $\ref{prop:stateless_r4a}$ marked by the induced posterior means $\posterior{1}, \posterior{2}$ (star). The posteriors are induced by mapping the probability mass to signals as marked (green, blue).}
    \label{fig:result_2}
\end{figure}
\subsection{Numerical Experiments - State-independent}
\label{subsec:numerical_state_indpt}
\noindent We now present numerical experiments to illustrate the benefit of our optimally designed signalling mechanisms relative to no information and full information benchmarks. We consider a stateless case where the in-person safe capacity the planner seeks to implement does not depend on $\theta$. We vary the capacity limit to demonstrate how the relative improvement with regard to each benchmark changes. 

\noindent We implement an experiment where $\goal = \{\fin : \norm{\fin} \geq b\}$ and we vary the constants $b$ between 0 and 1 in increments of $\frac{1}{20}$. The number of groups is fixed at $\K = 10$ and for each $b$ we run $10,000$ simulations by drawing $ \mathbf{x} \sim Unif(L_1), v_i \sim Unif[0,10], \theta \sim Unif[5,20]$ ($\priormean = \frac{25}{2}$). We evaluate the optimal mechanism given by Theorem \ref{thm:stateless} against two benchmarks. The first benchmark is the non-informative mechanism where agents receive no added information and consequently have a posterior mean belief of $\priormean$ over $\Theta$. The second benchmark is the fully-informative mechanism, where the true value of $\theta$ is directly revealed so agents maintain posterior mean beliefs $\theta'$ where $\theta'$ is sampled from $Unif[5,20]$. 
The resulting objective that measures the probability of compliance is averaged across simulations for each $b$ and plotted in Figure \ref{fig:stateless_carying_capacity}. 
\begin{figure}
    \centering
    \includegraphics[width=55mm]{img/download.png}
    \caption{Capacity compliance across non-informative, fully-informative and optimal signalling.}
    \label{fig:stateless_carying_capacity}
\end{figure}
We indeed obtain that the optimal signalling mechanism strictly improves relative to both benchmarks. The improvement reduces as $b \nearrow 1$ as the intersection between the outcomes achievable in equilibrium and the outcomes the planner deems acceptable reduces to the empty set. Naturally, the mechanism's ability to influence agents to a set of outcomes decreases as the set of outcomes becomes smaller. Likewise, as $b \searrow 0$, the set of acceptable outcomes grows to encompass all outcomes. Hence, the mechanism approaches full compliance, but so do the benchmark mechanisms. Consequently, the relative value of our optimally-designed signalling mechanism decreases as the set of outcomes the planner is willing to accept grows. 

% \subsection{State-dependent, set-based preferences}
% \label{subsec:counterexample_mps}

\newpage

==> Journal_Version/old/4_-_Approximation.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex
\newpage
\section{State-dependent Preferences}
%!TEX root = Opt_Info_Provision_Hybrid.tex
\label{sec:stateful}
In this section, we consider a setting under which the planner maintains a model of preferences over the
size distribution of agents across in-person and remote work that also \textit{may vary} as a function of the state. We demonstrate through an example that optimal design with MPS is no longer guaranteed under this setting as pooling states from disconnected regions of the state space is necessary to produce optimal solutions for certain objectives. 

\noindent Consequently, due to the added complexity and infeasibility of interval-based signalling schemes at optimality, we search for approximately optimal designs. We define a discretization of the continuous distribution over state and identify solutions for the discretized distribution. We then introduce two models of preference: (i) a \textit{scaled-capacity} preference model where the planner seeks outcomes that satisfy state-dependent capacity limits and (ii) a Lipschitz continuous preference model when the planner’s utility is jointly Lipschitz in both the remote mass and the true state. We provide 
algorithms that admit approximately optimal solutions for both models of preference in Propositions \ref{prop:scaled_capacity} and \ref{prop:lipschitz} respectively. We finally analytically and numerically assess the quality of the approximate solution our algorithm produces. 

\subsection{State-Dependent Preference Problem Formulation and MPS}
Consider a planner with preferences modelled by $\obj(\fin;\trueparam)$ where now this function $\obj$ is free to vary as a function of $\fin$ and $\trueparam$.

Observe first, that since the design problem's objective both depends on $\fin$ (i.e. $m(\posterior{\signal})$) and $\trueparam$, two signalling mechanisms $\pi_1,\pi_2$ with an equivalent direct mechanism $\mathcal{T}_\pi$ do not necessarily produce an identical objective if the product distribution over $(\posterior{\signal},\trueparam)$ is distinct. Without this simplification, we cannot conduct our search over signalling mechanisms thru the mean-preserving contractions of the prior distribution $\dist$. 

An additional technical concern of deriving the optimal design, exact forms of optimal design for an arbitrary $\obj$ will not necessarily have MPS. As a motivating example, we build off the structure of the preferences modelled in Sec.~\ref{sec:stateful} where we were able to analytically derive optimal design and show it had MPS. Particularly, we consider preferences $\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{y \in \goal(\trueparam)\}$ where the preference is represented by a correspondence from the possible values of the state $\trueparam$ to sets of mass distributions acceptable to the planner which we will assume are closed intervals: $\goal(\trueparam) = [a(\trueparam),b(\trueparam)] \subseteq [0,1]$. We refer to this setting as \emph{state-dependent set-based preference}. 

The choice of $a(\trueparam),b(\trueparam)$ for each value of the state $\trueparam$ is driven by practical considerations such as feasible set of agent occupancies at the workplace as a function of the true severity of the disease. As an example, as $\trueparam$ increases, it is feasible that a planner would seek a larger equilibrium remote mass and consequently seek to induce higher beliefs on expectation (i.e. $a, b$ increasing). 

The planner's expected objective $V_{F,\obj}(\pi)$ for a signaling mechanism $\pi = \langle \I, \{z_\param\}_{\param \in \paramspace} \rangle $ then becomes~$V_{F,\obj}(\pi) = \mathbb{P}\{\final(i) \in \goal(\trueparam)\}=\mathbb{P}\{\final({\signal}) \in [a(\trueparam),b(\trueparam)]\}$, where $\final({\signal})$ is the agent's equilibrium remote mass in response to signal $i\in\I$ that is realized with probability $z_\trueparam(i)$. Following Prop.~\ref{prop:eqbm_formula_prop_1}, we can  write the problem of maximizing planner's objective~\eqref{eqn:gen_objective_stateful} as follows: 
\begin{align}
        V_{F,h}^\ast &= \max_{\pi: \langle \I,  \{z_\param\}_{\param \in \paramspace}\rangle} \mathbb{P}\{a(\trueparam) \leq m(\posterior{\signal}) \leq b(\trueparam)\} \label{eq:statedependentsetobj}
\end{align}
Even for this subclass of state-dependent preferences that is only specified by sets $\goal(\trueparam)$, we show in the following example that the optimal signalling mechanism will not necessarily have MPS:
\begin{ex}
Let $\dist$ be uniform on $[0,1]$ ($\priormean = 0.5$). Abstracting away equilibrium behavior, let $\Omega(\trueparam)$ be the preimage under $m(\cdot)$ of the set $\goal(\trueparam)$. Formally, let $\Omega(\trueparam) = [\frac{1}{3}\trueparam-\epsilon,\frac{1}{3}\trueparam+\epsilon]$ (i.e. $a(\trueparam) = m( \frac{1}{3}\trueparam-\epsilon)$ and $b(\trueparam) = m( \frac{1}{3}\trueparam+\epsilon)$) for some arbitrary small $\epsilon$. Observe that any signalling mechanism with MPS will achieve an objective less than $6\epsilon$.

To see this, consider any mechanism with MPS and any interval $[t_{j-1}, t_{j}]$ with $t_j > 0$ without loss of generality. Observe that the posterior mean $\posterior{j}$ on seeing signal $j$ is $\frac{t_{j-1}+t_{j}}{2}$. However, for any $t_j > 6\epsilon$, for all $\trueparam \in [t_{j-1}, t_{j}]$ observe that $\frac{t_{j-1}+t_{j}}{2} \geq \frac{t_{j}}{2} > \frac{t_{j}}{3}+\epsilon \geq \frac{\trueparam}{3}+\epsilon$. So $m(\posterior{j}) > b(\trueparam)$ and by~\eqref{eq:statedependentsetobj} these signals $j$ contribute 0 to the objective. Hence, no true state $\trueparam > 6 \epsilon$ can be in an interval that contributes positively to the objective and hence at best the planner can achieve an objective of $6\epsilon$. 

Consider the following mechanism: $\pi = \langle \I, \{z_\param\}_{\param\in\paramspace}\rangle$ where $\I = \{\mathbf{1},\mathbf{2},\mathbf{3}\}$ and $z_{\theta}(s)$ is as follows:
\begin{align*}
z_\theta(\cdot) = \begin{cases}
& \mathbf{1} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_1\coloneqq[0,0.12]\cup[0.52,0.56]\\
& \mathbf{2} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_2\coloneqq[0.12,0.30]\cup[0.80,0.82]\\
& \mathbf{3} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_3\coloneqq[0,1]\setminus\{\mathcal{S}_1\cup\mathcal{S}_2\}
\end{cases}
\end{align*}
Observe that $\posterior{\mathbf{1}} = 0.18, \posterior{\mathbf{2}} = 0.27$ and $\posterior{\mathbf{3}} \approx 0.65$. Hence, if $\trueparam \in [0.54-3\epsilon,0.54+3\epsilon] \subset \mathcal{S}_1$ or if $\trueparam \in [0.81-3\epsilon,0.81+3\epsilon] \subset \mathcal{S}_2$, the signal generates posterior beliefs that correspond to equilibria that lie in $\goal(\trueparam)$. This feasible mechanism achieves an objective of $12\epsilon$ which strictly outperforms $6\epsilon$; therefore, no signalling mechanism with MPS can be optimal for this setting.
\end{ex}

The above example demonstrates that MPS schemes are not sufficient to achieve optimality generally when the intervals become state-dependent. Intuitively, a signal $s$ will alert the agents that $\trueparam$ lies in some set ($\I_s \coloneqq \{\param: z_{\param}(s) > 0\}$), but generates a unique posterior mean $\posterior{s}$ and consequently a unique equilibrium outcome $m(\posterior{s})$. Hence, the optimal design must take care in the selection of the set of states $\I_s$ as it both affects $\posterior{s}$ which will consequently affect $\final(s)$ in the evaluation of $\obj$ but also the $\trueparam$ for the states corresponding to this equilibrium. In this example, this corresponds to carefully setting $\I_s$ so that the posterior mean $\posterior{s}$ is contained in preimage of $m(\cdot)$ over $\goal(\trueparam)$ for a large mass of $\trueparam \in \I_s$. The example demonstrates that pooling the states non-sequentially may be required so optimal design is too technically challenging to tackle directly. In the following subsections, we will seek \textit{approximate designs} that are interval-based in nature and can be efficiently computed.

% \subsection{General state-independent $\obj$ \srs{Comment out if not progressing more}}
% \label{subsec:gen_state_independent}
% Consider a general state-independent objective $\obj(y)$. The formulation we will typically consider will require $\obj$ to be concave. Then observe that the objective can be written as a function over posterior means $\tilde{h}(\theta_i) = h(m(\theta_i))$.
% It is known from \cite{gentzkow_rothschild-stiglitz_2016} that any signalling must induce a distribution over posterior means $S$ such that for all $x\in[0.M]$ $\ell(x) \coloneqq \int_{t = 0}^x F(t) dt \geq \int_{t = 0}^x S(t) dt $ with equality at $x=1$. An MPS scheme is optimal if a piecewise-linear, convex function $k(x) \leq \ell(x)$ for all $x\in[0,M]$ exists such that:
% \begin{align*}
%     &\max \sum_{i \in \I} p_i(\tilde{h}(x_i))\\
%     &\text{s.t. }\int_{t=0}^x F(t) dt \geq \sum_{i\in\I} s_i(x-x_i)^+, \forall x\in[0,M]\\
%     &\int_{t=0}^1 F(t) dt \geq \sum_{i\in\I} s_i(1-x_i)^+, \forall x\in[0,M]
% \end{align*}
% \begin{obs}
% \label{obs:to_prove}
% Suppose $F$ is a binary distribution and $\tilde{h}$ is concave over intervals $\cup_{i=1}^{T}[a_i,b_i]$ and convex over $[0,M]\setminus\cup_{i=1}^{T}[a_i,b_i]$. Then at most $T$ signals are used in the optimal mechanism. \srs{Provide example using DeVericourt model to show $\tilde{h}$ is in $\mathcal{C}^2$ and can be decomposed this way naturally.}
% \end{obs}
\subsection{Discretization Procedure and Linear Programming Formulation}
\begin{figure}[h!]
\begin{subfigure}[width=0.3\textwidth]{
\include{presentations/pres_fig/stateful_0.tex}}
\end{subfigure}
\begin{subfigure}{
\include{presentations/pres_fig/stateful_1.tex}}
\end{subfigure}
\end{figure}
% \include{presentations/pres_fig/stateful_0.tex}
The approach we describe in this section to generate an approximately optimal solution will be to discretize the distribution $\dist$ over the continuous space $\paramspace$ into a discrete distribution. The discretization we describe is such that when an optimal design is achieved for this discretized distribution, we can argue that a signalling mechanism for the continuous distribution $\dist$ can be mapped from the discrete solution without much planner objective loss. The following definition describes a systematic definition of a discretizated  distribution $\dist_\delta$ of $\dist$. In particular, we take a uniform partition of $\paramspace$ with $N \coloneqq M\delta$ intervals $[\frac{j-1}{\delta},\frac{j}{\delta}]$ each of length $\frac{1}{\delta}$. Moreover, we assign all the probability mass in the interval to the minimum of that interval $\nu_j \coloneqq \frac{j-1}{\delta}$. We denote the collection of $\nu_j$ by $\discpspace \coloneqq \{\nu_1, ...,\nu_N\}$.

\begin{defn}
The \textit{$\delta$-discretization} $\dist_\delta$ of any continuous distribution $\dist$ is a discrete probability distribution over $\discpspace$ such that $\hat{\theta} \sim \dist_\delta$ has $\mathbb{P}[\hat{\theta} = \nu_j] \coloneqq p_{j} = \dist(\frac{j}{\delta})-F(\frac{j-1}{\delta})$.
\end{defn}
Observe that this modified distribution $\dist_\delta$ will not necessarily have the same mean as $\dist$ since we only shift probability mass of $\dist$ towards the minimum within each of these intervals. Hence, in fact: $\mathbb{E}_{\trueparam \sim \dist}[\trueparam] \geq \mathbb{E}_{\nu \sim \dist_\delta}[\nu]$. 

By considering discrete prior distributions over the state, the planner's design problem is suitable to be solved using linear programming provided that the planner's objective $\obj$ has regularity in its dependence over $\fin$ that enables the design problem to have linear constraints and a linear objective. This regularity will be achieved by requiring that the number of signals needed at optimality is finite and that the locally constant. Hence, the following lemma establishes that if $\obj(\fin;\nu)$ is piecewise constant in $\fin$ then an optimal design can be achieved using linear programming. 

\begin{lemma}
\label{lemma:lp_discrete}
Suppose that $\trueparam\sim \dist_\delta$ ($p_j \coloneqq \P[\trueparam = \nu_j]$) and $\obj(\fin;\trueparam)$ is piecewise constant in $\fin$ such that there exists $y_0 \coloneqq 0  < y_1 < .. < y_K < y_{K+1}\coloneqq 1$ where for all $\nu_j \in\Theta^\delta$, $\obj(\fin;\nu_j) = c_{jk}$ is constant across $\fin \in [y_{k-1},y_k]$. Then given the optimal solution of the following linear program \textbf{LP} $\{z_{ji}^\ast\}$, 
 we can construct the optimal design $\pi_{\dist_\delta,\obj}^\ast = \langle \I, \{z_{\param}\}_{\param \in \Theta^\delta} \rangle$ with $\I = [K]$ and $z_{\nu_j}(\signal) = \frac{z_{ji}^\ast}{p_j}$ for all $\signal \in \I$ and $j \in [N]$.

\begin{align*}
    &\max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=1}^{K} c_{ji} z_{ji} \\
    &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
    &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[K],j\in[N] \\
    &\hspace{1cm} m^{-1}(y_{i-1})\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[K] \\
    &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq m^{-1}(y_i)\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[K]
\end{align*}
\end{lemma}
\begin{proof}

\noindent Observe that we can expand the optimization in \eqref{eqn:scaled_capacity_2} for $\dist_\delta$ to include the constraints as follows: 
\begin{align*}
V^\ast &= \max_{\langle \{z_\param\}_{\param \in \{\nu_j\}_{j=1}^{N}},\I\rangle} \mathbb{E}[h(m(\posterior{i}),\trueparam)]\\
&= \max_{\langle \{z_\param\}_{\param \in \{\nu_j\}_{j=1}^{N}},\I\rangle} \sum_{j=1}^N \sum_{s\in|\I|} \mathbb{P}\{\signal=s,\trueparam=\nu_j\}\obj(m(\posterior{s}),\nu_j)\\
&= \max_{\langle \{z_\param\}_{\param \in \{\nu_j\}_{j=1}^{N}},\I\rangle} \sum_{j=1}^N \sum_{s\in|\I|} p_j z_{\nu_j}(s)\obj(m(\posterior{s}),\nu_j)
\end{align*}
Next, observe that analogous to Lemma~\ref{lemma:num_signals_bdd}, the objective is constant if any two signals $s_1,s_2$ with $\posterior{s_1}, \posterior{s_2} \in [m^{-1}(y_{k-1}),m^{-1}(y_k))$ for any $k \in [K]$ are consolidated to a signal $s$ ($\posterior{s_1} \leq \posterior{s} \leq \posterior{s_2}$). Therefore, we can restrict the optimization further to $\I = [K]$ with $m^{-1}(y_{\signal-1})\leq\posterior{\signal}<m^{-1}(y_\signal)$ for all $\signal \in \I$.
Reparameterizing the optimization so that $z_{ji} = p_j z_{\nu_j}(i)$, we get:
\begin{align*}
    V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \Theta},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{N+1} c_{ji}z_{ji} \\
    &\text{s.t. }\sum_{i=1}^{N+1} z_{ji} = p_j, \forall j\in[N] \\
    &\hspace{1cm} z_{ji}\geq 0, \forall i\in [N+1],j\in[N] \\
    &\hspace{1cm} m^{-1}(y_{\signal-1})\leq\posterior{\signal} = \frac{\sum_{j=1}^N \nu_j z_{ji}}{\sum_{j=1}^N z_{ji}}\leq m^{-1}(y_{\signal}), \hspace{0.5cm} \forall i \in |\I|
    % &\hspace{1cm}G \succcurlyeq F
\end{align*} 
Expanding the last inequalities we arrive at \textbf{LP($\mathbf{c},\mathbf{p},\mathbf{y}$)}. Hence the optimal solution from \textbf{LP} will return $\pi_{\dist_\delta,\obj}^\ast$.\qed
\end{proof}

The following corollary establishes that the time complexity of the algorithm \textbf{LP} specified in Lemma~\ref{lemma:lp_discrete} is polynomial in the number of partitions to describe the piecewise function.
\begin{corollary}
\label{cor:lp_discrete_complexity}
The algorithm presented using \textbf{LP} to compute $\pi_{\dist_\delta,\obj}^\ast$ has time complexity $O(N^{2.5}K^{2.5})$.
\end{corollary}
\begin{proof}
The linear program \textbf{LP} has $O(NK)$ variables $z_{ij}$. Appealing to the results presented by \cite{vaidya_speeding-up_1989}, the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. \qed
\end{proof}
This corollary will be useful as we consider the two state-dependent classes of planner preferences.
 

\subsection{$\epsilon$-optimal Design}
\label{subsec:setup_epsilon_optimal_design}
As discussed in the previous subsection, we will seek \textit{$\epsilon$-optimal} signalling mechanisms $\hat{\pi}$ as described in the following definition.

\begin{defn}
\label{defn:eps_approx}
A mechanism $\hat{\pi}$ is $\epsilon$-optimal for a problem instance defined by distribution $\dist$ over $\paramspace$ and utility function $\obj$ (under $V_{\dist,\obj}$) if $|V_{\dist,\obj}(\hat{\pi}) - V_{\dist,\obj}(\pi^\ast)| \leq \epsilon$.
\end{defn}

Observe that the definition states that $\epsilon$-optimal signalling mechanism $\hat{\pi}$ is close on expectation to $\pi^\ast$ when evaluated according to the planner's objective with the prior distribution $\dist$. However, notice that the tuples $\pi^\ast$ and $\hat{\pi}$ themselves may not be close and are difficult objects to compare. In fact, since the agents' strategic decisions are conditionally independent of the mechanism $\pi$ given the generated posterior mean by Prop.~\ref{prop:eqbm_formula_prop_1}, in Sec.~\ref{sec:static_id} we were able to compare two distinct mechanisms $\pi_1, \pi_2$ by the induced distributions of posterior means $\dist \preccurlyeq H_1, H_2$ alone. However, observe that in~\eqref{eqn:scaled_capacity_1} that $V_{\dist,\obj}^\ast$ critically depends on the product distribution that the signalling mechanism specifies over $(\trueparam, \posterior{\signal})$. Hence, even if the if the marginals of this product distribution on $\posterior{\signal}$ (i.e. $H_1$ and $H_2$) were identically distributed, the corresponding product distributions may not be and hence the objectives will differ. 

To formulate $\hat{\pi}$, our general procedure will be to first solve for the optimal solution $\pi_{\dist_\delta,\obj}^\ast = \langle \{z^\delta_{\param}\}_{\param \in \discpspace}, \I_\delta \rangle$ under the discrete distribution of state $\dist_\delta$. We will then construct $\hat{\pi} = \langle \{\hat{z}_\param\}_{\param \in \paramspace}, \I_\delta \rangle$ such that for all $j \in [N], \param \in [\nu_{j-1},\nu_j), \signal \in \I_\delta$,  $\hat{z}_\param(\signal) = z^\delta_{\nu_j}(\signal)$. Intuitively, the distribution used to generate signals when in state $\nu_j$
suggested by the discretized optimal solution will be applied to the entire interval of states in the continuous adaptation of the mechanism we propose. 
\begin{itemize}
\item \underline{Optimal Solution to Original Design} $\pi_{\dist,\obj}^\ast = \langle \{z^\ast_{\param}\}_{\param \in \paramspace}, \I \rangle$
\item \underline{Application of $\pi_{\dist,\obj}^\ast$ to discrete distribution} $\pi' = \langle \{z'_{\param}\}_{\param \in \paramspace^\delta}, \I \rangle$
\item \underline{Proposed $\epsilon$-optimal Solution} $\hat{\pi} = \langle \{\hat{z}_\param\}_{\param \in \paramspace}, \I_\delta \rangle$
\item \underline{Optimal solution to discrete design}  $\pi_{\dist_\delta,\obj}^\ast = \langle \{z^\delta_{\param}\}_{\param \in \discpspace}, \I_\delta \rangle$
\end{itemize}
To bound the quality of this estimate, notationally allow the true optimal design $\pi_{\dist,\obj}^\ast = \langle \{z^\ast_{\param}\}_{\param \in \paramspace}, \I \rangle$. We consider another signalling mechanism for the discretized distribution $\dist_\delta$ that is obtained by modifying the true optimal design by averaging the distributions used to generate signals over the intervals
$\pi' = \langle \{z'_\param\}_{\param \in \Theta^\delta \subseteq \paramspace}, \I \rangle$ where for all $j \in [N], \signal \in \I, z'_{\nu_j}(\signal) = \frac{\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} z^\ast_\param(\signal) dF(\param)}{\int_{\frac{j-1}{\delta}}^{\frac{j}{\delta}} dF(\param)}$.

To show $\epsilon$-optimality of $\hat{\pi}$, it suffices to show that $V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi}) \leq \epsilon$. 
Observe:
\begin{align*}
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist,\obj}(\hat{\pi})
    &=
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi}) \\
    &=
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi') + V_{\dist_\delta,\obj}(\pi')-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi})\\
    &\leq
    \underbrace{V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\pi')}_{\textbf{(i)}} + \underbrace{V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\hat{\pi})}_{\textbf{(ii)}}
\end{align*}
The terms in expression (i) and (ii) can be simplified independently and represent the loss incurred by applying the discrete optimum's signal generation distribution across intervals or averaging the true optimum's signal generation distribution across an interval. In fact, observe that in term (i), both $\pi_{\dist,\obj}^\ast$ and $\hat{\pi}$ use the same set of signals $\I$; in term (ii), both $\pi^\ast_{\dist_\delta,\obj}$ and $\pi'$ use the same set of signals $\I_\delta$. Consequently, bounding both of these terms by $\frac{\epsilon}{2}$ is sufficient to ensure the $\epsilon$-optimality of the proposed solution $\hat{\pi}$.

\subsection{Scaled-Capacity Preferences}
\label{subsec:scaled_capacity}
% \begin{figure}[h]
% \centering     %%% not \center
% \subfigure[Goal sets for stateful objective when $\K = N = 2$ ($\nu_1 < \nu_2$).]{\label{fig:a}\includegraphics[width=40mm]{img/stateful}}
% \subfigure[A more general nested structure of goal sets. ]{\label{fig:b}\includegraphics[width=40mm]{img/nested}}
% \end{figure}

Consider a planner with preferences modelled by $\obj(\fin;\trueparam)$ and a correspondence of sets $\goal(\trueparam) = [b(\trueparam),1]$ for a weakly increasing function $b: \paramspace \rightarrow [0,1] $ such that $\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{y \in \goal(\trueparam)\} = \mathbb{I}\{y \geq b(\trueparam)\}$. Hence, under these preferences, the planner is willing to accept size distributions where the remote mass exceeds (in-person mass falls below) some threshold that gets larger (smaller) as $\trueparam$ increases. We refer to this setting as \emph{scaled capacity preferences}. This family of preferences is driven by the practical considerations of agent occupancies at the workplace that get more restrictive as the true disease severity and risk of community disease spread from the disease increases. 

Assume that $b$ is an weakly increasing step function with increments over $\nu_j$. Namely, we assume the following.
\begin{ass}$b(x)$ is constant for all $x \in [\frac{j-1}{\delta},\frac{j}{\delta}]$ for each $j \in [N]$.\end{ass}

Reformulating~\eqref{eqn:gen_objective_stateful} with Prop.~\ref{prop:eqbm_formula_prop_1}, we can express the objective of the planner as follows: 
\begin{align}
    V_{\dist,\obj}^\ast &= \max_{\langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \mathbb{P}\{\final(i) \in \goal(\trueparam)\} \label{eqn:scaled_capacity_1}\\
    &= \max_{\langle \{z_\param\}_{\param \in \paramspace},\I\rangle} \mathbb{P}\{m(\posterior{i}) \geq b(\trueparam)\} \label{eqn:scaled_capacity_2}
\end{align} 

To accomplish the linear programming component of solving the optimal signalling mechanism for the discretized $\dist_\delta$, consider the following \textbf{LP} where $\gamma_i = m^{-1}(b(\nu_i))$.  
% We will be able to lower bound objective using $\gamma_i$ and upper bound objective by using $\nu_{j}$'s set at maximum of intervals and using $\gamma_{i+1}$.

\begin{prop}
\label{prop:scaled_capacity} The application of \textbf{LP} for the scaled capacity model with $\gamma_i = m^{-1}(b(\nu_i))$ will produce $\hat{\pi}$ that is $\epsilon$-optimal.
\end{prop}

Observe that \textbf{LP} has $O(N^2) = O(M^2 \delta^2)$ variables and $O(N^2) = O(M^2 \delta^2)$ constraints. 


Moreover, given an optimal solution to \textbf{LP} $\{z_{ji}^\ast\}$, define the following signalling mechanism.  The following theorem shows that $\pi'$ is $\epsilon$-optimal under $V_{\dist,\obj}$ for sufficiently large $\delta$.
\begin{prop}\label{prop:lipschitz}
Suppose that $\popdist$ is continuously differentiable with $0 < \frac{d\popdist}{dv} \leq \eta_\beta$ and $b(\cdot)$ is continuously differentiable with $0 < \frac{db}{dt} \leq \eta_b$, then for $\delta > \frac{2\eta_{2,h} +2\eta_{1,h} \eta_{\beta}}{\epsilon}$, $\pi'$ is $\epsilon$-optimal under $V_{\dist,\obj}$.
\end{prop}
\begin{proof}
The proof proceeds in three major steps: (i) we first establish that the assumptions guarantee that $m(\cdot)$ is Lipschitz continuous, (ii) we solve for  $V_{\dist_\delta,\obj}^\ast$ and $\pi_{\dist_\delta,\obj}^\ast$ using a linear program, (ii) we next establish that $V_{\dist,\obj}(\pi')$ is close to $V_{\dist_\delta,\obj}(\pi_{\dist_\delta,\obj}^\ast)$ and then that $V_{\dist_\delta,\obj}(\pi_{\dist_\delta,\obj}^\ast)$ is close to $V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)$.\\
First, we argue that there is Lipschitz continuity in the map $m$ from the posterior mean belief to the remote mass. 
\begin{subproof}
\begin{lemma}
\label{lemma:m_lipschitz}
$m(\mu)$ is $C \eta_\beta$-Lipschitz.
\end{lemma}
\begin{subproof}
Recall that $m(\mu) \coloneqq \inf\{u \geq 0: G^{-1}(u) \geq c_1(u)\mu+c_2(u)\}$ and, by assumption, $G$ is continuously differentiable and monotone so $G^{-1}$ is continuous. Since $c_1, c_2$ are also continuous:
\begin{align*}
    m(\mu) &= \begin{cases}
    u & G^{-1}(u) = c_1(u)\mu + c_2(u), 0 < u < 1 \\
    0 & G^{-1}(0) \geq c_1(0)\mu + c_2(0) \\
    1 & G^{-1}(1) \leq c_1(1)\mu + c_2(1)\\
    \end{cases}
\end{align*}
Suppose by contradiction the claim is false, then there exists $0\leq \mu_1 < \mu_2 \leq M$ with $z_2 \coloneqq m(\mu_2)$, $z_1 \coloneqq m(\mu_1)$ such that $z_2 - z_1 > C \eta_\beta (\mu_2-\mu_1)$. Since $z_1 > z_2$:
\begin{align*}
    \popdist^{-1}(z_1) &\geq c_1(z_1)\mu_1+c_2(z_1)\\
    \popdist^{-1}(z_2) &\leq c_1(z_2)\mu_2+c_2(z_2)
\end{align*}
Therefore:
\begin{align*}
    z_1 &\geq \popdist(c_1(z_1)\mu_1+c_2(z_1))\\
    z_2 &\leq \popdist(c_1(z_2)\mu_2+c_2(z_2))
\end{align*}
Observe that:
\begin{align*}
    \popdist(c_1(z_2)\mu_2+c_2(z_2)) - \popdist(c_1(z_1)\mu_1+c_2(z_1)) &\geq z_2 - z_1\\
    &> C \eta_\beta (\mu_2-\mu_1)
    % \frac{G^{-1}(m(t_1))-c_2(m(t_1))}{c_1(m(t_1))} - \frac{G^{-1}(m(t_2))-c_2(m(t_2))}{c_1(m(t_2))} = t_2 - t_1 \\
    % \frac{c_1(m(t_2))G^{-1}(m(t_1))-c_1(m(t_2))c_2(m(t_1))-c_1(m(t_1))G^{-1}(m(t_2))+c_1(m(t_1))c_2(m(t_2))}{c_1(m(t_1))c_1(m(t_2))} = t_2 - t_1     \\
    % \frac{c_1(z_2)G^{-1}(z_1)-c_1(z_2)c_2(z_1)-c_1(z_1)G^{-1}(z_2)+c_1(z_1)c_2(z_2)}{c_1(z_1)c_1(z_2)} = t_2 - t_1    
\end{align*}
However:
\begin{align*}
    \popdist(c_1(z_2)\mu_2+c_2(z_2)) - \popdist(c_1(z_1)\mu_1+c_2(z_1)) &\leq \eta_\beta(c_1(z_2)\mu_2+c_2(z_2)-c_1(z_1)\mu_1-c_2(z_1)) \\
    &\leq \eta_\beta(c_1(z_2)\mu_2+c_2(z_2)-c_1(z_1)\mu_1-c_2(z_2))\\
    &\leq \eta_\beta(c_1(z_2)\mu_2-c_1(z_1)\mu_1) \\
    &\leq \eta_\beta(c_1(z_2)\mu_2-c_1(z_2)\mu_1) \\
    &\leq C \eta_\beta(\mu_2-\mu_1)
    % \popdist(c_1(z_2)t_2+c_2(z_2))-\popdist(c_1(z_1)t_1+c_2(z_1)) > \eta_\beta (t_2-t_1)\\
    % t_2 - t_1 \leq t_2 - t_1) \\
    %   c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1) > t_2-t_1\\
    % c_1(z_2)t_2-c_1(z_1)t_1+c_2(z_2)-c_2(z_1) > t_2-t_1\\
    % c_1(z_2)t_2-c_1(z_1)t_1 > t_2-t_1\\
    % c_1(z_2)(t_2-t_1) > t_2-t_1\\ 
\end{align*}
This is a contradiction, hence $m$ must be $C \eta_\beta$-Lipschitz. 
\end{subproof}
\end{subproof}
Finally, we establish $\pi'$ is $\epsilon$-optimal for \textcolor{blue}{$\delta > \frac{\eta_{2,h}+ C\eta_{1,h} \eta_{\beta}}{\epsilon}$}. The discrete solution (we know this precisely from Lemma~\ref{lemma:lp_discrete}).


For (i), we can consider the corresponding direct mechanisms $T_{\pi_{\dist,\obj}} = \{(q_i^\ast, \param_i^\ast)\}_{i \in \I}$ for $\pi_{\dist,\obj}^\ast$ in combination with distribution $\dist$ and $T_{\hat{\pi}} = \{(\hat{q}_i,\hat{\param}_i)\}_{i \in \I}$ for $\hat{\pi}$ in combination with distribution $\dist_\delta$. Observe that by construction:
\begin{align*}
    \hat{q}_i &= \sum_{k=1}^{N} \mathbb{P}_{\dist_\delta}\big[\theta =\nu_k]\hat{z}_{\nu_k}(i)\\ 
    &= \sum_{k=1}^{N} \mathbb{P}_{\dist}\big[\theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]\big] \hat{z}_{\nu_k}(i)\\
    &=\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)\frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}\\
    &=\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)\\    
    &= q_i^\ast
\end{align*}
\end{proof}



\subsection{Lipschitz-Continuous Preferences}
\label{subsec:lipschitz_continuous}
Furthermore, for all $i \in \I$, we can bound the difference between $\param_i^\ast$ and $\hat{\param}_i$:
\begin{align*}
|\hat{\param}_i-\param_i^\ast| &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{\int_{0}^{M} \hat{z}_{\param}(i) d\dist_\delta(\param) }-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{\int_{0}^{M} z_{\param}(i) d\dist(\param) }\Big|\\
&= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{q_i^\ast}-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{q_i^\ast}\Big|\\
&= \frac{1}{q_i^\ast}\Big|\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) -\int_{0}^{M} \param z_{\param}(i) d\dist(\param)\Big|\\
&= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k)\hat{z}_{\nu_k}(i)d\dist(\param) -\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \param z_\param(i) dF(\param)\Big|\\
&= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k-\param)z_{\theta}(i)d\dist(\param)\Big|\\
&\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big|\nu_k-\param\big|z_{\theta}(i)d\dist(\param)\\
&\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\frac{1}{2\delta}z_{\theta}(i)d\dist(\param) \\
&\leq \frac{1}{2\delta}
\end{align*}
Therefore, simplifying expression (i):
\begin{align*}
    V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{P}\{m(\posterior{i}) \geq b(\trueparam)\}
\end{align*}

Therefore, simplifying expression (i):
\begin{align*}
       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
\end{align*}
By Fubini's theorem:
\begin{align*}
V_{\dist,\obj}(\pi_{\dist,\obj})-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
      \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
      \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
  &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
  &\leq  \frac{\epsilon}{2}
\end{align*}
We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi_{\dist,\obj})| \leq \epsilon. \blacksquare$
\subsection{Time Complexity and Numerical Comparison}
The complexity of the above LP is consequently polynomial in $M,\eta_{1}, \eta_{2}, \eta_{3}$ and $\frac{1}{\epsilon^2}$. Observe that appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Consequently, we can bound the overall complexity in the following corollary:
\begin{corollary}
\label{cor:stateful}
The algorithms described in Prop.~\ref{prop:scaled_capacity} and Prop.~\ref{prop:lipschitz} has time complexity equal to the time complexity of \textbf{LP}. The time complexity of \textbf{LP} is $O(\frac{\eta_{1}^5\eta_{2}^{2.5} \eta_{3}^{1.5}}{\epsilon^3})$.
\end{corollary}
\begin{proof}
The linear program \textbf{LP} has $O(\delta \omega)$ variables $z_{ij}$. Appealing to the results presented by \cite{vaidya_speeding-up_1989}, the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables.
\end{proof}
\begin{figure}[h!]
\centering
\includegraphics[width=3in]{img/DV.png}
\caption{Numerical results indicating the error from the true optimal design $\pi^\ast$ and the produced algorithmic solution $\hat{\pi}$.}
\end{figure}
Analogous to the results presented in ~\cite{de_vericourt_informing_2021}, we will consider the family of preferences indicated by the function $\obj(\fin;\trueparam) = \lambda \trueparam \fin + (1-\lambda) \fin$. As an example, we choose $\lambda = 0.5$ and plot the error of our approximately optimal solution against the optimal solution provably shown to be optimal in ~\cite{de_vericourt_informing_2021}. Note that the distribution presented in ~\cite{de_vericourt_informing_2021} is a binary distribution, and our model is general to this distinction. In their results, $G$ is assumed to be uniform over $[0,1]$. We correspondingly adapt our solution by modifying the equation in Equation~\eqref{eqn:red_1_form} appropriately. The modified solution is shown to be full information revelation in ~\cite{de_vericourt_informing_2021}. As a result $\pi^\ast = <\I, g_\theta>$ where $\I = \Theta$ and $g_\theta(\theta) = 1$.
% Observe that by construction:
% \begin{align*}
%     \hat{q}_i &= \sum_{k=1}^{N} \mathbb{P}_{\dist_\delta}\big[\theta =\nu_k]\hat{z}_{\nu_k}(i)\\ 
%     &= \sum_{k=1}^{N} \mathbb{P}_{\dist}\big[\theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]\big] \hat{z}_{\nu_k}(i)\\
%     &=\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)\frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}\\
%     &=\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)\\    
%     &= q_i^\ast
% \end{align*}
% Furthermore, for all $i \in \I$, we can bound the difference between $\param_i^\ast$ and $\hat{\param}_i$:
% \begin{align*}
% |\hat{\param}_i-\param_i^\ast| &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{\int_{0}^{M} \hat{z}_{\param}(i) d\dist_\delta(\param) }-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{\int_{0}^{M} z_{\param}(i) d\dist(\param) }\Big|\\
% &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{q_i^\ast}-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{q_i^\ast}\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) -\int_{0}^{M} \param z_{\param}(i) d\dist(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k)\hat{z}_{\nu_k}(i)d\dist(\param) -\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \param z_\param(i) dF(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k-\param)z_{\theta}(i)d\dist(\param)\Big|\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big|\nu_k-\param\big|z_{\theta}(i)d\dist(\param)\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\frac{1}{2\delta}z_{\theta}(i)d\dist(\param) \\
% &\leq \frac{1}{2\delta}
% \end{align*}
% Therefore, simplifying expression (i):
% \begin{align*}
%     V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{P}\{m(\posterior{i}) \geq b(\trueparam)\}
% \end{align*}

% Therefore, simplifying expression (i):
% \begin{align*}
%       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
% \end{align*}
% By Fubini's theorem:
% \begin{align*}
% V_{\dist,\obj}(\pi_{\dist,\obj})-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
%   &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
%   &\leq  \frac{\epsilon}{2}
% \end{align*}
% We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi_{\dist,\obj})| \leq \epsilon. \blacksquare$
% \end{proof}
% \begin{align*}
%       V_{\dist,\obj}(\pi_{\dist,\obj}^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
% \end{align*}
% By Fubini's theorem:
% \begin{align*}
% V_{\dist,\obj}(\pi_{\dist,\obj})-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
%   &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
%   &\leq  \frac{\epsilon}{2}
% \end{align*}
% We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi_{\dist,\obj})| \leq \epsilon. \blacksquare$
% \end{proof}

% The complexity of the above LP is consequently polynomial in $M,\eta_{1,g}, \eta_{2,g}, \eta_{\beta}$ and $\frac{1}{\epsilon^2}$. Observe that appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Consequently, we can bound the overall complexity in the following corollary:
% \begin{corollary}
% The algorithm described in the proof of Theorem~\ref{thm:stateful} has time complexity equal to the time complexity of \textbf{LP}. The time complexity of \textbf{LP} is $O(\frac{\eta_{1,\obj}^5\eta_{2,\obj}^{2.5} \eta_{\beta}^{1.5}}{\epsilon^3})$.
% \end{corollary}
% \begin{proof}
% The linear program \textbf{LP} has $O(\delta \omega)$ variables $z_{ij}$. Appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables.
% \end{proof}
% As with the stateless design, $\final(i)$ only depends on the induced posterior mean $\param_i$ and $\final(i) \in \goal(\nu_j)$ if and only $\final(i) \in \goal(\nu_j) \cap \curve$. The latter follows if and only if $b_j \leq \|\final(i)\| \leq 1$ or $0 \leq m(\param_i) \leq 1-b_j$. Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, observe that this corresponds to $\param_i \in [\gamma_j,\infty)$ for some constants $\gamma_j$ that are strictly increasing in $j$. For completeness, we denote $\gamma_0 = 0$ and $\gamma_{N+1} = \infty$.
% We can then reformulate \eqref{eqn:stateful_a} as follows:
% \begin{align}
%     V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{\gamma_j \leq \param_i < \infty\} \label{eqn:stateful_b}
% \end{align}
% We highlight that despite these simplifications, our analysis is extensible to other practically relevant objectives aside from the scaled capacity objective. Suppose that the desirable sets satisfy Assumption A1 and are also (i) nested with $\goal(\nu_{i+1})\subset \goal(\nu_{i})$ for all $i \in [N-1]$, and (ii) half-bounded with $\init \in \goal(\nu_i)$ for all initial mass vectors $\init$ and all $i \in [N]$; see Fig. \ref{fig:b}. Then we arrive at an identical formulation to \eqref{eqn:stateful_b} since the minimal posterior mean beliefs for the agent outcomes to enter each $\goal(\nu_j)$ is an increasing sequence $\gamma_j$.

% \noindent Using a similar reduction as in stateless design, we can restrict our mechanism to induce a single posterior mean $\param_i$ to lie in each interval $[\gamma_{i-1},\gamma_{i})$ for $i \in [N+1]$. These $\param_i$ consequently induce equilibrium outcomes that lie in $\goal(\nu_j)$ if and only if $\param_i \geq \gamma_j$ or equivalently $i \geq j+1$. This implies that an optimal mechanism can be described by at most $N+1$ signals. In the proposition below, we provide a linear program (LP) to compute an optimal signalling mechanism for the stateful scaled capacity objective.












% Using this result, we can efficiently compute the optimal objective $V^\ast$ and an optimal signalling mechanism $\pi^\ast$ in polynomial time. 

% \noindent If the $b_j$ and hence $\goal(\nu_j)$ were all identical, our setting becomes the stateless setting solved by Theorem $\ref{thm:stateless}$. In this special case, all $\nu_j$ correspond to a single $\gamma=\gamma_j$ and only two posterior means $\param_1 < \gamma \leq \param_2$ are required. If $\mu = \sum_{j \in [N]} p_j \nu_j \geq \gamma$ then this corresponds to regime R1 and non-informative mechanism is optimal. If $\mu < \gamma$ this corresponds to regime R4 and likewise we recover a discretized interval-based signalling mechanism over $\I = \{1,2\}$ by solving the LP and we can check that there exists a $\hat{j} \in [N]$ such that for all $j < \hat{j}$, $z_{\nu_j}(1) = 1$ and for all $j > \hat{j}$, $z_{\nu_j}(2) = 1$.  

% \noindent Finally, for any mechanism $\pi$, the probability of complying with the capacity limit conditioned on $\param = \nu_j$ can be represented by $V_j(\pi) \coloneqq  \mathbb{P}\{\final(i) \in \goal(\param)|\param=\nu_j\}$. Observe that $V_{\dist,\obj}(\pi) = p_j V_j(\pi)$ is a weighted average of the compliance for each possible realization of $\param$. However, practically planners may face significantly more adverse risks of being overcapacitated as the infectiousness increases, and weight compliance heterogeneously across realizations of $\param$. For this slightly more general objective, an optimal signalling mechanism for a different weighted sum $\sum_{j=1}^{N} \alpha_j V_j(\pi)$ for $\alpha_j \geq 0$ can likewise be solved using the linear program above by replacing the objective with $\max_{\{ z_{ji}\}} \sum_{i=j+1}^{N+1} \frac{\alpha_j}{p_j}z_{ji}$.

% The previous section demonstrates that generally one cannot expect to find MPS solutions under our model for general objectives, but we consider our second class of objectives which are state-dependent. Namely, we consider a scaling capacity objective where $\goal(\param) = \{y: y \geq b(\param)\}$ for some non-increasing function $b$. 
% In this section, we consider stateful goal sets where generally the set of outcomes that the principal seeks to guide equilibrium for the true parameter $\param$ is $\goal(\param)$. In this stateful setting, we cannot reduce the search over $\pi$ by searching over the corresponding direct mechanisms $\mathcal{T}_\pi$. This is because a posterior mean $\param_i$ will induce a specific equilibrium outcome $\final(i)$ but we cannot evaluate whether $\final(i) \in \goal(\param)$ if we only know $\param_i$ and not the true $\param$.

% \noindent Observe that each design problem is tailored to an initial population allocation across the groups $\init$. For this particular $\init$, achievable equilibria lie on a one-dimensional manifold as shown in Lemma \ref{lemma:intervals}, so we can decompose the intersection of $\curve$ and each of our goal sets $\goal(\param)$ as the objects of interest. Namely we will impose the following assumptions to be as general as possible: \\
% \noindent \textbf{(A2)} $\goal(\param)$ is closed for all $\param$. \\
% \noindent \textbf{(A3)} $\goal(\param) \cap \curve = \cup_{i=1}^{P} [a_{i}(\param), b_{i}(\param)]$ for finite $P$, $0 \leq a_i(\param), b_i(\param) \leq 1$ for all $\param$.\\
% \noindent \textbf{(A4)} For all $i \in [P]$, $a_i(\cdot),b_i(\cdot)$ are $\eta_1$-Lipschitz. 

% \noindent Observe that \textbf{(A3)} can be satisfied if $\goal(\param)$ is convex for all $\param$, but the assumption allows for a more general description. Assumption \textbf{(A4)} while seemingly restrictive merely requires that the goal sets are smooth in $\param$ and that there are no sudden discontinuities. Observe that some of the $P$ intervals where we only assume $P$ is finite can be empty so the shape of the intersection can change significantly as $\param$ increases.

% \noindent The following proposition establishes a linear program that is capable of approximating the optimal solution to the information design problem posed in Equation \eqref{eqn:objective_stateful}. We first introduce the following LP:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% \subsection{Stateful Scaled Capacity Model}
% \label{sec:stateful}
% \begin{figure}[h]
% \centering     %%% not \center
% \subfigure[Goal sets for stateful objective when $\K = N = 2$ ($\nu_1 < \nu_2$).]{\label{fig:a}\includegraphics[width=40mm]{img/stateful}}
% \subfigure[A more general nested structure of goal sets. ]{\label{fig:b}\includegraphics[width=40mm]{img/nested}}
% \end{figure}

% \noindent Using \eqref{eqn:objective_stateful}, we can express the objective of the planner by: 
% \begin{align}
%     V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \mathbb{P}\{\final(i) \in \goal(\nu)\} \\
%      &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_\nu(i) \mathbb{I}\{\final(i) \in \goal(\nu_j)\}  \label{eqn:stateful_a}
% \end{align}
% As with the stateless design, $\final(i)$ only depends on the induced posterior mean $\param_i$ and $\final(i) \in \goal(\nu_j)$ if and only $\final(i) \in \goal(\nu_j) \cap \curve$. The latter follows if and only if $b_j \leq \|\final(i)\| \leq 1$ or $0 \leq m(\param_i) \leq 1-b_j$. Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, observe that this corresponds to $\param_i \in [\gamma_j,\infty)$ for some constants $\gamma_j$ that are strictly increasing in $j$. For completeness, we denote $\gamma_0 = 0$ and $\gamma_{N+1} = \infty$.
% We can then reformulate \eqref{eqn:stateful_a} as follows:
% \begin{align}
%     V^\ast &= \max_{\langle \{z_\nu\}_{\nu \in \paramspace},\I\rangle} \sum_{j=1}^N \sum_{i=1}^{|\I|} p_j z_{\nu_j}(i) \mathbb{I}\{\gamma_j \leq \param_i < \infty\} \label{eqn:stateful_b}
% \end{align}
% We highlight that despite these simplifications, our analysis is extensible to other practically relevant objectives aside from the scaled capacity objective. Suppose that the desirable sets satisfy Assumption A1 and are also (i) nested with $\goal(\nu_{i+1})\subset \goal(\nu_{i})$ for all $i \in [N-1]$, and (ii) half-bounded with $\init \in \goal(\nu_i)$ for all initial mass vectors $\init$ and all $i \in [N]$; see Fig. \ref{fig:b}. Then we arrive at an identical formulation to \eqref{eqn:stateful_b} since the minimal posterior mean beliefs for the agent outcomes to enter each $\goal(\nu_j)$ is an increasing sequence $\gamma_j$.

% \noindent Using a similar reduction as in stateless design, we can restrict our mechanism to induce a single posterior mean $\param_i$ to lie in each interval $[\gamma_{i-1},\gamma_{i})$ for $i \in [N+1]$. These $\param_i$ consequently induce equilibrium outcomes that lie in $\goal(\nu_j)$ if and only if $\param_i \geq \gamma_j$ or equivalently $i \geq j+1$. This implies that an optimal mechanism can be described by at most $N+1$ signals. In the proposition below, we provide a linear program (LP) to compute an optimal signalling mechanism for the stateful scaled capacity objective. We first introduce the LP:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% Using this result, we can efficiently compute the optimal objective $V^\ast$ and an optimal signalling mechanism $\pi^\ast$ in polynomial time. 

% \noindent If the $b_j$ and hence $\goal(\nu_j)$ were all identical, our setting becomes the stateless setting solved by Theorem $\ref{thm:stateless}$. In this special case, all $\nu_j$ correspond to a single $\gamma=\gamma_j$ and only two posterior means $\param_1 < \gamma \leq \param_2$ are required. If $\mu = \sum_{j \in [N]} p_j \nu_j \geq \gamma$ then this corresponds to regime R1 and non-informative mechanism is optimal. If $\mu < \gamma$ this corresponds to regime R4 and likewise we recover a discretized interval-based signalling mechanism over $\I = \{1,2\}$ by solving the LP and we can check that there exists a $\hat{j} \in [N]$ such that for all $j < \hat{j}$, $z_{\nu_j}(1) = 1$ and for all $j > \hat{j}$, $z_{\nu_j}(2) = 1$.  

% \noindent Finally, for any mechanism $\pi$, the probability of complying with the capacity limit conditioned on $\param = \nu_j$ can be represented by $V_j(\pi) \coloneqq  \mathbb{P}\{\final(i) \in \goal(\param)|\param=\nu_j\}$. Observe that $V_{\dist,\obj}(\pi) = p_j V_j(\pi)$ is a weighted average of the compliance for each possible realization of $\param$. However, practically planners may face significantly more adverse risks of being overcapacitated as the infectiousness increases, and weight compliance heterogeneously across realizations of $\param$. For this slightly more general objective, an optimal signalling mechanism for a different weighted sum $\sum_{j=1}^{N} \alpha_j V_j(\pi)$ for $\alpha_j \geq 0$ can likewise be solved using the linear program above by replacing the objective with $\max_{\{ z_{ji}\}} \sum_{i=j+1}^{N+1} \frac{\alpha_j}{p_j}z_{ji}$.

% \subsection{Numerical Experiments}
% % \textcolor{blue}{Outline: create analogous curve for the stateful setting for a discrete distribution - show the improved comparative benefit from stateful signalling in this regime relative to even the stateless setting. Here, we again have a stateful capacity based objective (simple LP solves this).}
% \noindent For the stateful capacity case, we highlight a specific instance where we scale-down the in-person capacity limit as the infectious risk increases. Consequently, the minimal posterior mean to induce outcomes in $\goal(\nu_j)$ are represented by $\gamma_j$ that are increasing in $j$. To gain intuition, we choose the specific set of tuples for $N=3$ where $\{p_i\}_{i \in \{1,2,3\}} = (0.3,0.3,0.4), \{\nu_i\}_{i \in \{1,2,3\}} = (0.4,0.6,1.0), \{\gamma_i\}_{i \in \{1,2,3\}} = (0.5, 0.9, 1.2)$ and compare the performance of the optimal mechanism against the same two benchmarks as in the stateless case.
% In Fig. \ref{table:stateful_vary_capacity}, we tabulate each information mechanism's performance. Observe that under no information, agents mean belief over $\theta = \mu = \sum_{j=1}^N p_j \nu_j = 0.7$. Since agents receive no signal, the equilibrium outcome is independent of $\theta$ and agents only comply if $\gamma_j < \mu$ which happens with probability $p_1 = 0.3$. Under full information, agents perfectly observe $\theta$, so the outcome is compliant with the limit if and only if $\theta_j \geq \gamma_j$. This occurs with probability $0$ in our example. Thus, the stateful design significantly improves the probability of compliance relative to both benchmarks. We also observe that the stateful design does no worse in this setting than either benchmark in any of the conditional compliance measures $V_j(\pi)$.
% \begin{figure}
%     \centering
%     \begin{tabular}{ |c|c|c|c|c| } 
%     \hline
%     Information Scheme & $V_{\dist,\obj}(\pi)$ & $V_1(\pi)$ & $V_2(\pi)$ & $V_3(\pi)$ \\     
%     \hline
%     No Information & 0.300 &1& 0& 0 \\ 
%     Full Information  & 0.000 & 0& 0 &0 \\ 
%     Stateful Design & 0.425 & 1& 0.417 &0 \\ 
%  \hline
% \end{tabular}
    
%     \caption{Comparison of non-informative, fully informative and optimal stateful signalling in terms of the overall probability of compliance and conditional probabilities of compliance. }
%     \label{table:stateful_vary_capacity}
% \end{figure}
% \label{sec:approximation}
% In the previous section, we demonstrated that MPS mechanisms can achieve optimal design for particular state-independent objective  functions. However, we also provided state-dependent counterexamples where no MPS mechanism is able to achieve or closely approximate optimal design. 
% In this section, we seek a methodology to provide \textit{approximate} optimal design for a general form of state-dependent objective functions. Because we seek a method that will generalize to a general form of objective functions $\obj$, observe that a closed-form description of the optimal signalling mechanism will be difficult to obtain under arbitrary objectives.
% % \srs{sentence seems unnecessary - The approach we  produces a signalling mechanism that will \textit{$\epsilon$-approximate} the optimal solution to \eqref{eqn:gen_objective_stateful} by using $O(\frac{1}{\epsilon})$ discrete signals and $O(\frac{1}{\epsilon^2})$ computational complexity.}

% % \begin{figure}
% %     \centering
% %     \input{presentations/stateful_c.tex}
% %     \caption{Caption}
% %     \label{fig:my_label}
% % \end{figure}
% \noindent Formally, we characterize an $\epsilon$-approximation of the optimal signalling mechanism using the following definition.

% The previous example demonstrates that generally one cannot expect to find MPS solutions under our model for general objectives, but we consider our second class of objectives which are state-dependent. Namely, we consider a scaling capacity objective where $\goal(\param) = \{y: y \geq b(\param)\}$ for some non-increasing function $b$. In this section, we consider stateful goal sets where generally the set of outcomes that the principal seeks to guide equilibrium for the true parameter $\param$ is $\goal(\param)$. In this stateful setting, we cannot reduce the search over $\pi$ by searching over the corresponding direct mechanisms $\mathcal{T}_\pi$. This is because a posterior mean $\param_i$ will induce a specific equilibrium outcome $\final(i)$ but we cannot evaluate whether $\final(i) \in \goal(\param)$ if we only know $\param_i$ and not the true $\param$.

% \noindent Observe that each design problem is tailored to an initial population allocation across the groups $\init$. For this particular $\init$, achievable equilibria lie on a one-dimensional manifold as shown in Lemma \ref{lemma:intervals}, so we can decompose the intersection of $\curve$ and each of our goal sets $\goal(\param)$ as the objects of interest. Namely we will impose the following assumptions to be as general as possible: \\
% \noindent \textbf{(A2)} $\goal(\param)$ is closed for all $\param$. \\
% \noindent \textbf{(A3)} $\goal(\param) \cap \curve = \cup_{i=1}^{P} [a_{i}(\param), b_{i}(\param)]$ for finite $P$, $0 \leq a_i(\param), b_i(\param) \leq 1$ for all $\param$.\\
% \noindent \textbf{(A4)} For all $i \in [P]$, $a_i(\cdot),b_i(\cdot)$ are $\eta_1$-Lipschitz. 

% \noindent Observe that \textbf{(A3)} can be satisfied if $\goal(\param)$ is convex for all $\param$, but the assumption allows for a more general description. Assumption \textbf{(A4)} while seemingly restrictive merely requires that the goal sets are smooth in $\param$ and that there are no sudden discontinuities. Observe that some of the $P$ intervals where we only assume $P$ is finite can be empty so the shape of the intersection can change significantly as $\param$ increases.

% \noindent The following proposition establishes a linear program that is capable of approximating the optimal solution to the information design problem posed in Equation \eqref{eqn:objective_stateful}. We first introduce the following LP:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}
% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%     \draw[->] (0,0) -- (\rb+0.5,0);
%     \draw[->] (0,0) -- (0,\rb);
%     % \draw[dashed] (\ra,0) -- (\ra,1) node[above] {$a$};
%     \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$1$};
%     \draw[] (\rb+0.5,-0.25) node[below] {$y$};
%     \draw[] (\rb-0.5,\rb-1) node[below] {$\obj(y;\cdot)$};
    
%     \draw[red, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{2*sin(deg(\x))+2});
%     \draw[red!90,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.9*sin(deg(\x))+1.9});
%     \draw[red!80blue!40,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.6*sin(deg(\x))+1.5});
%     \draw[red!70blue!30,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.4*sin(deg(\x))+1.2});
%     \draw[red!60!blue!40-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{1.2*sin(deg(\x))+0.9});
%     \draw[red!50!blue!50,-, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{sin(deg(\x))+0.8});
% \end{tikzpicture}
    
%     \begin{tikzpicture}
%     \draw[->] (0,0) -- (\rb+0.5,0);
%     \draw[->] (0,0) -- (0,\rb+0.5);
%     % \draw[dashed] (\ra,0) -- (\ra,1) node[above] {$a$};
% \draw[] (\rb,0) -- (\rb,-0.25) node[below] {$1$};
%     \draw[] (\rb+0.5,-0.25) node[below] {$y$};
%     \draw[] (\rb-0.5,\rb) node[below] {$\obj(y;\nu)$};
%     \draw[dotted,thick,red] (1.6,0) -- (1.3,-0.3) node[below] {$\theta_{s'}$};
%     \draw[dotted,thick,red] (1.8,0) -- (2.1,-0.3) node[below] {$\theta_{s''}$};
%     % \draw[dashed] (1.0,0) -- (1.0,-1.5) node[below] {$m(\gamma_{i+1})$};
    
%     %Right-Hand
%     \foreach \x in {1,...,\rb} % <--- my issues
%     \draw[thick, fill=red!25] (\x-.5,0) -- (\x-.5,{2*sin(deg(\x-0.25))+2.05}) -- (\x,{2*sin(deg(\x-0.25))+2.05}) -- (\x,0) -- cycle;
%     \foreach \x in {1,...,\rb} % <--- my issues
%     \draw[thick, fill=green!25] (\x-1,0) -- (\x-1,{2*sin(deg(\x-0.5-0.25))+2.05}) -- (\x-0.5,{2*sin(deg(\x-0.5-0.25))+2.05}) -- (\x-0.5,0) -- cycle;
    
%     % %Left-Hand
%     % \foreach \x in {\ra,-0.5,...,\rbtwo} % <--- my issues
%     % \draw[thick, fill=blue!25] (\x,0) -- (\x,{sin(deg(\x))}) -- (\x+.5,{sin(deg(\x))}) -- (\x+.5,0) -- cycle;
    
%     \draw[ultra thick, -, domain=0:\rb, smooth, samples=100, variable=\x] plot ({\x},{2*sin(deg(\x))+2});
    
% \end{tikzpicture}\caption{$\delta$-discretization of $F$ and $\omega$-discretization of $\obj$.}
%     \label{fig:discretization}
% \end{figure}
% Analogously, to adapt a continuous objective function $h(\cdot, \param)$ to a piecewise constant, we can parameterize the discretization by $\omega$ and choose to uniformly create intervals of length $\frac{1}{\omega}$ over $[0,1]$ with the discretized function taking a constant value over each interval equal to the average of the minimum and maximum on this interval. 
% \begin{defn}
% The \textit{$\omega$-discretization} $h_\omega$ of any continuous function $h:[0,1]\rightarrow \R$ is a piecewise constant function such that for all $k \in [\omega], x \in[\frac{k-1}{\omega},\frac{k}{\omega}]$:
% \begin{align*}
%     h_\omega(x) = \frac{\min_{x\in[\frac{k-1}{\omega},\frac{k}{\omega}]}h(x)+\max_{x\in[\frac{k-1}{\omega},\frac{k}{\omega}]}h(x)}{2} 
% \end{align*}
% \end{defn}

% Consider the following linear program parameterized by a sequence of parameters $\langle P, Q, \{\alpha_{ji}\}_{i \in [P], j\in[Q]},\{\gamma_{i}\}_{i \in [P]},\{\nu_{j}\}_{j\in[Q]}\rangle$:
% \begin{align*}
%     V^\ast &= \max_{\{ z_{ji}\}} \sum_{j=1}^N \sum_{i=j+1}^{N+1} \alpha_{ji}z_{ji} \\
%     &\text{s.t. }\sum_{i=1}^{N+1}  z_{ji} = p_j, \hspace{0.5cm}\forall j\in[N]\\
%     &\hspace{1cm} 0 \leq z_{ji} \leq p_j,\hspace{0.5cm} \forall i\in[N+1],j\in[N] \\
%     &\hspace{1cm} \gamma_{i-1}\sum_{j=1}^N z_{ji} \leq  \sum_{j=1}^N \nu_j z_{ji}, \hspace{0.5cm} \forall i\in[N+1] \\
%     &\hspace{1cm} \sum_{j=1}^N \nu_j z_{ji} \leq \gamma_{i}\sum_{j=1}^N z_{ji}, \hspace{0.5cm} \forall i\in[N+1]
% \end{align*}

% \noindent To eliminate instances of our problem when the objective is erratically constructed, we impose the following assumptions on the problem setting.

% \textbf{Assumptions}
% \\
% \noindent \textbf{A3} $\popdist$ is continuously differentiable with $0 < \frac{d\popdist}{dv} \leq \eta_\beta$. 

% \noindent \textbf{A4} $h(x; \cdot)$ is uniformly $\eta_{h,1}$-Lipschitz

% \noindent \textbf{A5} $h(\cdot; \theta)$ is uniformly $\eta_{h,2}$-Lipschitz

% \noindent \textbf{A6} $h(x; \theta)$ is jointly differentiably continuous

% \begin{theorem}\label{thm:stateful}
% Under assumptions A3-A5, the solution $\pi^\ast(F_\delta,h_\omega)$ for $\delta > \frac{2\eta_{2,h} +2\eta_{1,h} \eta_{\beta}}{\epsilon}$, $\omega > \frac{2\eta_{1,h}}{\epsilon}$ is $\epsilon$-optimal and $\pi^\ast(F_\delta,z_\omega)$ can be computed using \textbf{LP} with parameters:. 
% \end{theorem}
% \begin{proof}
% The proof proceeds in four major steps: (i) we first establish that the assumptions guarantee that the objective function as a function of the parameter and posterior mean belief is Lipschitz continuous, (ii) we next establish we can discretize the distribution over the risk parameter $\dist$ without loss, (iii) we then argue that we can replace a general objective function $\obj$ with a piecewise constant function without loss, (iv) we finally argue that the optimal solution using a discretized distribution $\dist$ and a piecewise constant $\obj$ can be solved using \textbf{LP}.
% First, we argue that there is Lipschitz continuity in the map $m$ from the posterior mean belief to the remote mass. By conservation of Lipschitz continuity under composition, this suggests that the planner's objective as a function of $\param$ and $\param_i$ is Lipschitz-continuous.
% \begin{subproof}
% \begin{lemma}
% \label{lemma:m_lipschitz}
% $m(t)$ is $C \eta_\beta$-Lipschitz.
% \end{lemma}
% \begin{subproof}
% Recall that $m(t) \coloneqq \inf\{u \geq 0: G^{-1}(u) \geq c_1(u)t+c_2(u)\}$ and, by Assumption \textbf{A3}, $G$ is continuously differentiable and monotone so $G^{-1}$ is continuous. Since $c_1, c_2$ are also continuous:
% \begin{align*}
%     m(t) &= \begin{cases}
%     u & G^{-1}(u) = c_1(u)t + c_2(u), 0 < u < 1 \\
%     0 & G^{-1}(0) \geq c_1(0)t + c_2(0) \\
%     1 & G^{-1}(1) \leq c_1(1)t + c_2(1)\\
%     \end{cases}
% \end{align*}
% Suppose by contradiction the claim is false, then there exists $0\leq t_1 < t_2 \leq M$ with $z_2 \coloneqq m(t_2)$, $z_1 \coloneqq m(t_1)$ such that $z_2 - z_1 > C \eta_\beta (t_2-t_1)$. Since $z_1 > z_2$:
% \begin{align*}
%     \popdist^{-1}(z_1) &\geq c_1(z_1)t_1+c_2(z_1)\\
%     \popdist^{-1}(z_2) &\leq c_1(z_2)t_2+c_2(z_2)
% \end{align*}
% Therefore:
% \begin{align*}
%     z_1 &\geq \popdist(c_1(z_1)t_1+c_2(z_1))\\
%     z_2 &\leq \popdist(c_1(z_2)t_2+c_2(z_2))
% \end{align*}
% Observe that:
% \begin{align*}
%     \popdist(c_1(z_2)t_2+c_2(z_2)) - \popdist(c_1(z_1)t_1+c_2(z_1)) &\geq z_2 - z_1\\
%     &> C \eta_\beta (t_2-t_1)
%     % \frac{G^{-1}(m(t_1))-c_2(m(t_1))}{c_1(m(t_1))} - \frac{G^{-1}(m(t_2))-c_2(m(t_2))}{c_1(m(t_2))} = t_2 - t_1 \\
%     % \frac{c_1(m(t_2))G^{-1}(m(t_1))-c_1(m(t_2))c_2(m(t_1))-c_1(m(t_1))G^{-1}(m(t_2))+c_1(m(t_1))c_2(m(t_2))}{c_1(m(t_1))c_1(m(t_2))} = t_2 - t_1     \\
%     % \frac{c_1(z_2)G^{-1}(z_1)-c_1(z_2)c_2(z_1)-c_1(z_1)G^{-1}(z_2)+c_1(z_1)c_2(z_2)}{c_1(z_1)c_1(z_2)} = t_2 - t_1    
% \end{align*}
% However:
% \begin{align*}
%     \popdist(c_1(z_2)t_2+c_2(z_2)) - \popdist(c_1(z_1)t_1+c_2(z_1)) &\leq \eta_\beta(c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1)) \\
%     &\leq \eta_\beta(c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_2))\\
%     &\leq \eta_\beta(c_1(z_2)t_2-c_1(z_1)t_1) \\
%     &\leq \eta_\beta(c_1(z_2)t_2-c_1(z_2)t_1) \\
%     &\leq C \eta_\beta(t_2-t_1)
%     % \popdist(c_1(z_2)t_2+c_2(z_2))-\popdist(c_1(z_1)t_1+c_2(z_1)) > \eta_\beta (t_2-t_1)\\
%     % t_2 - t_1 \leq t_2 - t_1) \\
%     %   c_1(z_2)t_2+c_2(z_2)-c_1(z_1)t_1-c_2(z_1) > t_2-t_1\\
%     % c_1(z_2)t_2-c_1(z_1)t_1+c_2(z_2)-c_2(z_1) > t_2-t_1\\
%     % c_1(z_2)t_2-c_1(z_1)t_1 > t_2-t_1\\
%     % c_1(z_2)(t_2-t_1) > t_2-t_1\\ 
% \end{align*}
% This is a contradiction, hence $m$ must be $C \eta_\beta$-Lipschitz. 
% \end{subproof}
% \end{subproof}
% \begin{subproof}
% \begin{lemma}
% \label{lemma:h_comp_lipschitz}
% $\tilde{h}(\param_i; \param) = h(m(\param_i);\param)$ is $C \eta_{h,1}\eta_\beta$-Lipschitz in $\theta_i$ for all $\param \in \paramspace$.
% \end{lemma}
% \begin{subproof}
% This follows directly from Lemma \ref{lemma:m_lipschitz} since the Lipschitz continuity is preserved under composition with constant as product. 
% \end{subproof}
% \end{subproof}
% Next, we establish a procedure that produces a solution $\pi'$ using $\dist_\delta$ that performs well compared to the optimal $\pi^\ast_{\dist,\obj}$. For readability, let $V_{\dist,\obj}(\cdot) \coloneqq V_{\dist,\obj}(\cdot), V_{\dist_\delta,\obj}(\cdot) \coloneqq V_{\dist_\delta,\obj}(\cdot), \pi^\ast \coloneqq \pi^\ast_{\dist,\obj} = \langle \{z_\param\}_{\param \in \paramspace}, \I\rangle, \pi^\ast_{\dist_\delta,\obj} \coloneqq \pi^\ast_{\dist_\delta,\obj}= \langle \{s_\param\}_{\param \in \{\nu_k\}_{k=1}^\delta \subseteq \paramspace}, \I_\delta \rangle$. Specifically, our approach, for sufficiently large $\delta$, will solve for optimality using the $\delta$-discretization of $\dist$, $\dist_\delta$, to produce $\pi^\ast_{\dist_\delta,\obj}$. We then modify the mechanism to $\pi' = \langle \{s'_\param \}_{\param \in \paramspace},\I_\delta \rangle$ which uses the same set of signals as $\pi^\ast_{\dist_\delta,\obj}$ but is expanded to the full domain of the distribution $\dist$ by having for all $k \in [N], \theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]$, $s_\theta'(\cdot) = s_{\nu_k}(\cdot)$. The following lemma establishes that using $\pi'$ is close to $\pi^\ast$ in the planner's true objective under the true distribution $\dist$.
% \begin{subproof}
% \begin{lemma}
% For $\delta > \frac{\eta_{2,h}+ C\eta_{1,h} \eta_{\beta}}{\epsilon}$, $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi^\ast)| \leq \epsilon$.
% \end{lemma}
% \begin{subproof}
% By definition, $V_{\dist,\obj}(\pi') \leq V_{\dist,\obj}(\pi^\ast)$ so it suffices to show that $V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\pi') \leq \epsilon$. 
% Observe that if we define $\hat{\pi} = \langle \{\hat{z}_\param\}_{\param \in \{\nu_k\}_{k=1}^{N} \subseteq \paramspace}, \I \rangle$ where for all $k \in [N], i \in \I, \hat{z}_{\nu_k}(i) = \frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}$:
% \begin{align*}
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\pi') &\leq
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\pi') + V_{\dist_\delta,\obj}(\pi') -V_{\dist,\obj}(\pi') \\
%     &=
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \\
%     &=
%     V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) + V_{\dist_\delta,\obj}(\hat{\pi})-V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) + V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi')\\
%     &\leq
%     \underbrace{V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi})}_{\textbf{(i)}} + \underbrace{V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi')}_{\textbf{(ii)}}
% \end{align*}
% The terms in expression (i) and (ii) can be simplified independently. Observe that in term (i), both $\pi^\ast$ and $\hat{\pi}$ use the same set of signals $\I$; in term (ii), both $\pi_{\delta}$ and $\pi'$ use the same set of signals $\I_\delta$. \\
% For (i), we can consider the corresponding direct mechanisms $T_{\pi^\ast} = \{(q_i^\ast, \param_i^\ast)\}_{i \in \I}$ for $\pi^\ast$ in combination with distribution $\dist$ and $T_{\hat{\pi}} = \{(\hat{q}_i,\hat{\param}_i)\}_{i \in \I}$ for $\hat{\pi}$ in combination with distribution $\dist_\delta$. Observe that by construction:
% \begin{align*}
%     \hat{q}_i &= \sum_{k=1}^{N} \mathbb{P}_{\dist_\delta}\big[\theta =\nu_k]\\ 
%     &= \sum_{k=1}^{N} \mathbb{P}_{\dist}\big[\theta \in [\frac{k-1}{\delta},\frac{k}{\delta}]\big] \hat{z}_{\nu_k}(i)\\
%     &=\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)\frac{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)}{\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} dF(\param)}\\
%     &=\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} z_\param(i) dF(\param)\\    
%     &= q_i^\ast
% \end{align*}
% Furthermore, for all $i \in \I$, we can bound the difference between $\param_i^\ast$ and $\hat{\param}_i$:
% \begin{align*}
% |\hat{\param}_i-\param_i^\ast| &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{\int_{0}^{M} \hat{z}_{\param}(i) d\dist_\delta(\param) }-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{\int_{0}^{M} z_{\param}(i) d\dist(\param) }\Big|\\
% &= \Big|\frac{\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) }{q_i^\ast}-\frac{\int_{0}^{M} \param z_{\param}(i) d\dist(\param) }{q_i^\ast}\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\int_{0}^{M} \param \hat{z}_{\param}(i) d\dist_\delta(\param) -\int_{0}^{M} \param z_{\param}(i) d\dist(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k)\hat{z}_{\nu_k}(i)d\dist(\param) -\sum_{k=1}^{N}\int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \param z_\param(i) dF(\param)\Big|\\
% &= \frac{1}{q_i^\ast}\Big|\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}(\nu_k-\param)z_{\theta}(i)d\dist(\param)\Big|\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\big|\nu_k-\param\big|z_{\theta}(i)d\dist(\param)\\
% &\leq \frac{1}{q_i^\ast}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}}\frac{1}{2\delta}z_{\theta}(i)d\dist(\param) \\
% &\leq \frac{1}{2\delta}
% \end{align*}
% Therefore, simplifying expression (i):
% \begin{align*}
%       V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &= \mathbb{E}_{i}[\mathbb{E}_{\param^\ast }[\obj(m(\theta_i^\ast); \param^\ast)|i]] - \mathbb{E}_{i}[\mathbb{E}_{\hat{\param}}[\obj(m(\hat{\param}_i); \hat{\param})|i]]
% \end{align*}\end{subproof}
% By Fubini's theorem:
% \begin{align*}
% V_{\dist,\obj}(\pi^\ast)-V_{\dist_\delta,\obj}(\hat{\pi}) &= \mathbb{E}_{\param^\ast \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i^\ast); \param^\ast)] - \mathbb{E}_{\hat{\param} \sim \dist_\delta, i \sim 
%       \hat{z}_{\param}}[\obj(m(\hat{\param}_i); \hat{\param})] \\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\param^\ast_i; \param)) z_{\param}(i) dF(\param)- \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \obj(m(\hat{\param}_i; \nu_k)) z_{\param}(i) dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( \obj(m(\param^\ast_i; \param)) -\obj(m(\hat{\param}_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\obj(m(\param^\ast_i; \param)) -\obj(m(\param^\ast_i; \nu_k))  \Big) z_{\param}(i)dF(\param)\\      
%       &=  \sum_{i \in \I}\sum_{k=1}^{N} \int_{\frac{k-1}{\delta}}^{\frac{k}{\delta}} \Big( 
%       \frac{C \eta_{h,1}\eta_\beta}{2\delta}+\frac{ \eta_{h,2}}{2\delta} \Big) z_{\param}(i)dF(\param)\\         
%   &\leq \frac{ C\eta_{\obj,1}\eta_{\beta}+\eta_{\obj,2}}{2\delta} \\
%   &\leq  \frac{\epsilon}{2}
% \end{align*}
% We also simplify expression (ii). Analogously, observe that if $\mathcal{T}_{\pi'} = \{(q_i',\param_i')\}_{i\in\I_\delta}$ for $\pi'$ in combination with $\dist$ and $\mathcal{T}_{\pi^\ast_{\dist_\delta,\obj}} = \{(q_i^\delta,\param_i^\delta)\}_{i\in\I_\delta}$ for $\pi^\ast_{\dist_\delta,\obj}$ in combination with $\dist_\delta$, then $q_i^\delta = q_i'$ for all $i\in\I_\delta$. The remainder of the proof is analogous so we can also establish that $V_{\dist_\delta,\obj}(\pi^\ast_{\dist_\delta,\obj}) -V_{\dist,\obj}(\pi') \leq \frac{\epsilon}{2}$ and consequently $|V_{\dist,\obj}(\pi')-V_{\dist,\obj}(\pi^\ast)| \leq \epsilon. \blacksquare$
% \end{subproof}
% The final step of the proof is to show that by approximating our general objective function $\obj$ by its $\omega-$discretization that we also achieve arbitrarily small loss. For readability, let $V_{\dist,\obj}(\cdot) \coloneqq V_{\dist_\delta,\obj}(\cdot), V_\omega(\cdot) \coloneqq V_{\dist_\delta,\obj_\omega}(\cdot), \pi^\ast \coloneqq \pi^\ast_{\dist_\delta,\obj} = \langle \{z_\param\}_{\param \in \paramspace}, \I\rangle, \pi_\omega \coloneqq \pi^\ast_{\dist_\delta,\obj_\omega}= \langle \{s_\param\}_{\param \in \{\nu_k\}_{k=1}^\delta \subseteq \paramspace}, \I_\delta \rangle$. 
% \begin{lemma}
% For $\omega > \frac{\eta_{\obj,1}}{\epsilon}$, $|V_{F,\obj}(\pi^\ast_{F_\delta,\obj_\omega})-V_{F,\obj}(\pi^\ast_{F_\delta,\obj})| \leq \epsilon$ 
% \end{lemma}
% \begin{subproof}

% Observe that:
% \begin{align*}
%     V_{\delta}(\pi)-V_{\dist,\obj}(\pi^\ast_{\dist_\delta,\obj}) &\leq
%     V_{\dist_{\delta},\obj}(\pi^\ast_{\dist,h})-V_{\dist,\obj}(\pi'_{F,h}) \\
%     &= \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[\obj(m(\theta_i), \param)] - \mathbb{E}_{\param \sim \dist_\delta, i \sim z_{\param}}[\obj(m(\theta_i), \param)] \\
%   &= \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\obj(m(\theta_i+\sigma_1), \param+\sigma_2)-\obj(m(\theta_i), \param)]] \\
%   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} +  \obj(m(\theta_i+\sigma_1), \param)-\obj(m(\theta_i), \param)]] \\
%   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} + \sigma_1 \eta_{1,h}\eta_{\beta}+ \obj(m(\theta_i), \param)-\obj(m(\theta_i), \param)]] \\
%   &\leq \mathbb{E}_{\param \sim \dist, i \sim z_{\param}}[E_{\sigma_1,\sigma_2}[\sigma_2 \eta_{2,h} + \sigma_1 \eta_{1,h}\eta_{\beta}]]
%     \\
%   &\leq \frac{\eta_{2,h} +  \eta_{1,h}\eta_{\beta}}{\delta} \\
%   &\leq  \epsilon
% \end{align*}
% \end{subproof}
% \begin{lemma}
% The result of \textbf{LP} is equivalent to $\pi^\ast(F_\delta,z_\omega)$.
% \end{lemma}
% \end{proof}

% The complexity of the above LP is consequently polynomial in $M,\eta_{1,g}, \eta_{2,g}, \eta_{\beta}$ and $\frac{1}{\epsilon^2}$. Observe that appealing to the results presented by Vaidya et al. (2018), the complexity of linear programming is $O(n^{2.5})$ for problem instances with $n$ variables. Consequently, we can bound the overall complexity in the following corollary:
% \begin{corollary}
% Under assumptions $A3-A5$, the linear program provided above has polynomial time complexity with $O(\frac{\eta_{1,\obj}^5\eta_{2,\obj}^{2.5} \eta_{\beta}^{1.5}}{\epsilon^5})$ runtime produces $\hat{\pi}$ such that $\big|V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\hat{\pi})\big| \leq \epsilon$.
% \end{corollary}
% \begin{proof}
% The linear program \textbf{LP} has $O(\delta \omega)$ variables $z_{ij}$. 
% \end{proof}
% \subsection{Numerical Experiments}
% In this subsection, we provide the results an reproduce the plot that exists in \cite{de_vericourt_informinz_2021} showing the improved gain and matching the mechanisms to the solutions they produce. Some additional pruning is necessary to compare apples to apples computationally. In this subsection, we provide the results for a more general setting than the DeVericourt analysis. We can consider another epidemiologically motivated setting with non-uniform cost distribution and non-concave objectives if sufficiently motivated and show our results.
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{img/DV.png}
%     \caption{Error of $\hat{V}$ against discretization of $\obj$}
%     \label{fig:results}
% \end{figure}

==> MSOM_Submission/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> archive/Bonus.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex

%\newpage

==> archive/Introduction.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex

% Sohil notes:
% Don't like the idea of talking too much about endemic risk/persistent risk since not really apropos since F is likely not very uncertain in those cases as in COVID unless talking about new strains etc.

\section{Introduction}
\subsection{Motivation}

\noindent The COVID-19 pandemic inspired tremendous interest in developing strategies to balance the preservation of in-person activities with the mitigation of disease spread \cite{ji_lockdown_2020,nowzari_analysis_2016,drakopoulos_efficient_2014, chernozhukov_causal_2021}. Despite the availability and success of pharmaceutical tools (i.e. medicines, vaccines), they can have short-lived efficacy as diseases evolve, are costly to develop and are costly to scale as diseases become widespread \cite{cakmakli_economic_2021,moore_approaches_2021}. To supplement these measures which are alone insufficient, one can distinguish between two categories of non-pharmaceutical interventions planners\footnote{Planners encompass a broad class of individual entities with well-defined objectives over community activity and community disease spread. These could include public health communities surveying a community, government agencies or private firms managing their workforce. Under our model, planners critically have an ability to centrally disseminate information to a community.} use: (i) hard and (ii) soft.

\noindent \textit{Hard interventions} are strict restrictions that prevent infectious spread, i.e., lockdowns, capacity limits or mask mandates. Hard interventions are highly effective at flattening the contagion curve in the early phases of disease spread when cures and vaccines are unavailable, but these measures are too economically and socially costly to be viable long-term as diseases become endemic \cite{anderson_how_2020,acemoglu_optimal_2020,acemoglu_optimal_2021,birge_controlling_2020}.

\noindent In contrast, \textit{soft interventions} aim to \textit{influence} agents to consider particular actions that impact their risk of disease spread, i.e. to self-test, to self-isolate, to work remotely \cite{ely_rotation_2021,hernandez-chanto_contagion_2021}. Previous studies have shown that a population's beliefs over the severity of a disease and the populations' aggregate in-person activity are affected by public information disclosure \cite{bursztyn_misinformation_2020,simonov_persuasive_2020,allcott_polarization_2020}. An ongoing area of research, this phenomenon presents an opportunity for planners to \textit{strategically} disclose information to align the affected aggregate in-person activity with the planner's preferences over the activity given the disease's infectiousness \cite{de_vericourt_informing_2021,hu_disclosure_2022}. While previous research has identified disclosure strategies that align with particular forms of practically-driven models of preference, modelling and analysis that is flexible to a broader class of planner preferences is required. 

In this paper, we develop a stylized model and computational approach that captures key features of this setting by considering a planner capable of provisioning information to a population facing uncertainty about a disease's infectious risk. The basic idea is that a planner who faces the same uncertainty over the risk as the population chooses a set of signals $\I$ (i.e. messages, highlighting particular research, news reporting)  and a distribution over these signals for each possible value of the infectious risk (i.e. choosing reporting service, recommendation algorithm) \cite{bursztyn_misinformation_2020, allcott_polarization_2020}. A single signal $\signal \in \I$ is randomly drawn from the distribution corresponding to the true infectious risk and is publicly disclosed before agents make strategic choices. The population uses the observed signal $\signal$ to perform a Bayesian update of their beliefs over the true infectious risk and correspondingly an equilibrium action profile is achieved. 
% The strategic choices the population makes is dependent aggregate outcome of these choices affect their tradeoff given the signal. 
Our model is suitable for optimization as a planner maintains preferences over the population's actions and must choose both a set of signals $\I$ and the distributions over these signals, i.e. a \textit{signalling mechanism}, that best induces the preferred actions. In Sec. \ref{subsec:model_signalling_cp}, we describe this class of signalling mechanisms and then formalize the planner's problem of designing the \textit{optimal} mechanism. We formulate this information design problem and motivate information provision as an effective behavioral control amidst disease spread by focusing on the increasingly relevant setting of managing strategic hybrid workers. This stylized model is generic enough that various preferences can be accounted for and we proceed to develop a computational approach. 

\noindent In our model, a workforce has a unit mass of non-atomic agents, each deriving value from working in-person instead of remotely in isolation. However, there is a stochastic cost associated with becoming infected that increases with the number of in-person contacts and an unknown continuous stochastic parameter, $\trueparam \in \paramspace$, measuring the disease's infectious risk. When $\trueparam$ is large, agents that choose to work in-person impose a larger negative externality on other agents that choose in-person work due to infectious risk. A planner has imperfect information about $\trueparam$, but generates signals into the value of $\trueparam$ by choosing a signalling mechanism. On observing the disclosed signal $\signal$ generated by the disclosed signalling mechanism, agents' public mean belief over $\trueparam$ is updated to $\posterior{\signal}$ and they simultaneously make equilibrium choices on where to work.\footnote{In practice, such signals can correspond to planner's broadcast on the virulence of a disease strain or reporting case counts in the workplace to a particular granularity.} In Proposition \ref{prop:eqbm_formula_prop_1}, we solve for the unique Bayes-Nash equilibrium, in which agents work in-person if and only if their benefit from in-person work exceeds a threshold which increases with the updated mean belief of the infectious risk $\posterior{\signal}$. As the infectious risk $\posterior{\signal}$ is believed to be higher, our result aligns with intuition as more agents work remotely in equilibrium. 

The planner supervising the agents is strategic and has preferences over the size of the agent mass working remotely that is informed by firm-specific utilities, i.e., firm-specific changes in productivity, workspace costs, risk of infectious spread, adherence to public health guidelines. For example, if the planner receives disutility from infectious spread, a larger $\trueparam$ corresponds to a higher expected number of new infections. Hence, the preferences maintained over the size of the mass working remotely possibly change as $\trueparam$ varies. Modelling the details of the preference is not a focus of this paper, so rather we abstract these preferences by considering a single utility function $\obj(\fin; \trueparam)$ over the fraction of remote workers at equilibrium $\fin$  and the infectious risk $\trueparam$.\footnote{Calibrating $\obj$ for a specific planner is not a focus of this paper, but various workforce and workspace characteristics will have an impact \cite{parker_return_2020}. The authors of \cite{vecherin_assessment_2022} provide a quantitative model to translate many of these characteristics into the expected number of new infections which planners could subsequently factor in with their own costs.} The planner seeks to maximize the expected utility achieved in equilibrium subject to public uncertainty in the true parameter and the uncertainty in the remote fraction arising from the randomness in the mean belief $\posterior{\signal}$ induced by the signalling mechanism. 

Since we are not considering a particular form of objectives, but broadly large classes of objectives functions we find the means to design the planner's optimal signalling mechanism is critically distinguished between state-independent and state-dependent objectives; in the former $\obj$ does not change as a function of the risk parameter, whereas in the latter it does. In this paper, we focus on four classes of objectives: 
\begin{enumerate}
    \item \textbf{State-independent indicator functions (Sec \ref{sec:static_id})}:  $\obj(\fin;\trueparam) \coloneqq \indicator{y \in \mathcal{Y}}$ \\
When specifying objectives from this class, as might be expected for adherence to externally determined restrictions for example, the planner specifies a set $\goal \subseteq [0,1]$ of remote masses that are equally ``acceptable" irrespective of the true infectious risk. Any other remote masses are deemed ``unacceptable" by the planner. For objectives of this form, the planner equivalently seeks to maximize the probability that the equilibrium outcome lies in the set $\goal$.
    % \item \textcolor{red}{\textbf{State-independent monotone, concave functions}: $\obj(\fin;\trueparam) \coloneqq h(y)$ where $h$ is concave and either strictly increasing or strictly decreasing (i.e. monotone)\\
    % Objectives of this form are motivated, for example, by planners unconcerned with infectious spread but with firm-specific workspace costs. The monotonicity and concavity of $\obj$ translates to the preference of planners to either influence more or less agents to work remotely with diminishing returns.}
    \item \textbf{State-dependent scaled capacity functions (Sec \ref{sec:scaled_cap_stateful})}:  $\obj(\fin;\trueparam) \coloneqq \indicator{y \ge b(\trueparam)}$ for some weakly increasing function $b$\\
    This class of objectives is motivated by planners seeking to comply with capacity limit guidance that becomes progressively strict as the infectiousness increases. The planner uses an objective of this form to categorize a remote mass (in-person mass) as ``acceptable" if and only if it exceeds (is below) some threshold that increases as the disease becomes more infectious. 
    \item \textbf{General state-dependent functions (Sec \ref{sec:approximation})}:  $\obj(\fin;\trueparam) $ where $\obj$ is jointly-Lipschitz continuous\\
    This most general class of objectives allows for the planner's preference to be state-dependent provided that $\obj$ is jointly-Lipschitz continuous.\footnote{Observe that carefully chosen, Lipschitz-continuous approximations can lower bound any objective from the previous three classes. Hence, this class can be thought of as the \textit{most general}. In this paper, we do not characterize the loss by performing such an approximation.} Designing optimal mechanisms for this class of objectives is the central focus of this work as the set of objectives is large enough to encapsulate previously considered practically-driven objectives and those that the literature has not previously considered. As an example, the authors of \cite{de_vericourt_informing_2021} consider a family of objectives that are jointly-Lipschitz continuous.  
\end{enumerate}

A key feature of our model, we allow $\trueparam$ to be a continuous parameter. Practically, agents have knowledge of several illnesses as baselines against which they can compare the infectiousness of new diseases. This motivates a need for beliefs over the infectious risk that are supported on a large set. Moreover, amidst disease spread, domain experts and predictive models generate differing forecasts that are most effective when combined in a multi-model ensemble forecast \cite{cramer_evaluation_2022}. Hence, a continuous distribution is also justified as individuals are uncertain across all forecasts but rely on the planner's ensemble forecast to dispel some uncertainty. Technically, allowing $\trueparam$ to be continuous instead of binary also significantly increases the analytic rigor necessary to search over feasible signalling mechanisms. 

\noindent For continuous uncertain parameters, a particularly relevant subclass of mechanisms is that in which  $\paramspace$ is partitioned into contiguous intervals and the parameters in each interval collectively map to a single interval-specific signal (see Fig. \ref{fig:mps}). These \textit{monotone partitional} signalling (MPS) mechanisms disclose the signal corresponding to the interval in which the true parameter belongs and consequently have an ordering corresponding to the ordering of the intervals. 

We can induce distributions over posterior mean beliefs that are extreme points of the set of all distributions capable of being induced by a signalling mechanism (Theorem 1 from \cite{kleiner_extreme_2021}). The literature has considered planner objectives where the extremal nature of this class of mechanisms contains an optimal mechanism, but our results consider objective classes sufficiently rich enough where monotone partitional signalling is not sufficient \cite{dworczak_simple_2019,guo_interval_2019,candogan_optimal_2021,ivanov_optimal_2015}.  We find MPS as optimal in some settings. In general settings we find some counterexamples. We exploit this structure to discretize.
\begin{figure}
    \centering
    \includegraphics[width=80mm]{img/mps.png}
    \caption{Three examples of monotone partitional signalling (MPS) mechanisms. The signal $\signal$ disclosed by the planner is strictly determined by which interval contains $\trueparam$.}
    \label{fig:mps}
\end{figure}

\noindent In the following table, we summarize the results of this paper. \\
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c}
      Planner Objective $\obj$ & State-dependent & Optimal Mechanism & Is MPS necessarily optimal?\\
      \hline
     \hyperref[sec:static_id]{$\mathbb{I}\{y \in \mathcal{Y}\}$} & No & Closed form (Theorem \ref{thm:stateless}) & Yes (Theorem \ref{thm:stateless}) \\
    %   {concave, monotone $\obj(\fin)$ } & No  & Approximation (Theorem \ref{thm:stateful}) & \textcolor{red}{Yes (Observation \ref{obs:to_prove})}\\      
     \hyperref[sec:approximation]{$\mathbb{I}\{y \geq b(\param)\}$} & Yes &  Approximation (Proposition \ref{prop:stateful}) & No (Example \ref{example:nonmps_stateful}) \\
      \hyperref[sec:approximation]{$\obj(\fin; \param )$} & Yes & Approximation (Theorem \ref{thm:stateful}) & No (Example \ref{example:nonmps_stateful}) 
    \end{tabular}
    \caption{Summary of results}
    \label{tab:results_tab}
\end{table}\\
In Section \ref{sec:static_id}, we solve for the optimal signalling mechanism for state-independent indicator objective functions. In Theorem \ref{thm:stateless} we establish sufficiency conditions for the optimal signalling mechanism to be monotone paritional. We also fully characterize the optimal signalling mechanisms in closed form provided the set of remote masses $\goal$ is contiguous or agents' prior beliefs over the risk are not too tightly concentrated to be affected by signalling.\\
In Section \ref{sec:stateful}, we consider discrete distributions $\dist$ and state-dependent scaled capacity objective functions. Our results in Proposition \ref{prop:stateful} present a linear program that approximates the optimal signalling mechanism. We demonstrate that the addition of state-dependence alone eliminates the sufficiency of monotone partitional signalling mechanisms from Theorem \ref{thm:stateless} to achieve optimality for this richer class of objectives. \\
For general state-dependent objective functions, the design of the optimal signalling mechanisms is intractable. We consequently focus on Lipschitz continuous objectives and provide an approximation result that produces a signalling mechanism that is close to optimality. The approximate solution is generated by discretizing both the continuous distribution of beliefs on risk and the objective function and using a linear program similar to that developed in Proposition \ref{prop:stateful}. In Theorem \ref{thm:stateful}, we bound the quality of the approximate solution as a function of the Lipschitz continuity of our objective. 

In Section \ref{sec:numerical}, we present a numerical comparison of our signalling mechanisms against two benchmarks: (i) directly revealing the true $\trueparam$ (full information) and (ii) revealing nothing (no information). Our signalling mechanisms significantly improve on these benchmarks for both state-independent indicator and state-dependent scaled capacity objectives. We then present a numerical study demonstrating how quickly the approximation error converges to zero as a function of the discretization for practically-motivated objective functions. Our results suggest that for concave objectives the approximation error converges significantly faster than the bound we establish in Theorem \ref{thm:stateful}.

\subsection{Related Literature}
\label{subsec:related_literature}
\noindent Information design has been active area of research in the economics community spawned by the seminal results shown by \cite{kamenica_bayesian_2011} (see \cite{candogan_information_2020, bergemann_information_2019, kamenica_bayesian_2019} for useful reviews). 
% The field has expanded to tackle several economic problems of interest, particularly in the public health space \cite{shi_information_2013}. 

\noindent Our contribution builds on the recent literature on information provision for multiple agents over a continuous unknown parameter. The authors of \cite{gentzkow_rothschild-stiglitz_2016} show the equivalence between signalling mechanisms over continuous parameters and mean-preserving contractions of the parameter's prior distribution. This insight is useful for reducing the complexity of search over signalling mechanisms. The authors in \cite{candogan_optimal_2021} build on this idea to characterize an optimal recommendation system for a discrete number of agents that are uncertain about a system state and must reveal a privately held type. Their results characterize how the designer must choose his recommended actions to maximize his quasilinear objective over these actions while retaining incentive compatibility. We instead focus on a setting with non-atomic agents and various classes of objectives that are rich enough to capture all practically-motivated settings. 

\noindent With regard to the design of soft interventions to mitigate disease spread, the authors of \cite{ely_rotation_2021} consider the optimal design of rotation schemes where in-person workers alternate on some schedule. Related to information provision, \cite{hernandez-chanto_contagion_2021} presents an activity-based model where the principal informs agents of the infection rate and identifies when full disclosure maximizes society's expected welfare. The authors of \cite{hu_disclosure_2022} study optimal information disclosure in a healthcare congestion game for a benevolent planner seeking to maximize global welfare. By contrast, the planner in our model is free to choose among many possible forms of objectives. Most closely related to our work, \cite{de_vericourt_informing_2021} presents a macro-perspective on how planners can provision information about unknown stochastic risk during a pandemic. Our setting is more general than \cite{de_vericourt_informing_2021}, as their planner seeks to globally optimize over an objective function that takes a weighted average of functional measures of the economic health and infectious health. In contrast, our setup allows for a broader class of objectives that can incorporate other practically relevant factors. Our results also extend their binary model of the infectious risk by considering the unknown parameter as being drawn from any bounded, continuous distribution. There is also significant recent literature on infection dynamics in mean-field games \cite{olmez_modeling_2021,la_torre_mobility_2022}, however our paper focuses on information design after a stochastic representation of infectious risk has been obtained. Finally, the implications of our results for designing soft interventions are complementary to the works on containing infectious spread through hard interventions \cite{acemoglu_optimal_2020,acemoglu_optimal_2021,birge_controlling_2020,cianfanelli_lockdown_2021,wu_optimal_2020}.

% Two other papers SA shared with me...

==> archive/Model.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex
\newpage
\section{Model and Problem Formulation}
\label{sec:model}

\noindent We consider a model where strategic hybrid workers (agents) for a particular firm decide whether to work at a shared workspace or to work remotely amidst the spread of a communicable disease. Agents face uncertainty over the true infectiousness of the disease (parameter), denoted by $\trueparam$, and thus face uncertainty over their likelihood of incurring the disutility associated with becoming infected. In Sec. \ref{subsec:model_agent}, we formally describe agents' utilities and their dependence on the parameter.

\noindent A central planner supervising the agents maintains a utility function $\obj(\fin; \trueparam)$ over the fraction of remote workers at equilibrium $\fin$ which possibly depends on $\trueparam$.  where $\trueparam$ is continuous. The planner maximizes the expected utility achieved in equilibrium subject to uncertainty in the true parameter and agent actions.

\begin{defn}
\label{defn:objs}
We classify the objective $\obj(\fin;\trueparam)$ accordingly:
\begin{enumerate}
    \item (State-independent indicator) There exists $\goal = \cup_{j=1}^N \Omega_j$ where $\Omega_j \coloneqq [\wll{j}, \wlh{j}]$ are disjoint, closed subsets of $\Omega_j \subseteq [0,1]$ such that $\obj(\fin;\trueparam) = \mathbb{I}\{y \in \goal\}$.
    % \item (State-independent, monotone, concave) In abuse of notation, there exists a strictly monotone, concave function $\obj(\fin;\param) = \obj(\fin)$.
    \item (Scaled-capacity) There exists some weakly increasing function $b(\cdot)$ such that $\obj(\fin;\trueparam) = \mathbb{I}\{\fin\geq b(\trueparam)\}$.
    \item (General objective) $\obj(\fin;\trueparam)$.
\end{enumerate}
\end{defn}



\noindent The literature on information design is not limited to designing signals over continuous distributions on continuous domains such as $\dist$ on $\paramspace$ since several works consider discrete distributions over finite uncertainty sets \cite{de_vericourt_informing_2021, kamenica_bayesian_2011}. While not characterized as monotone partitional, the optimal signalling mechanisms discovered in much of this literature maintains characteristics of this structure and coincides with a suitably modified definition.
\noindent While able to design a mechanism that takes $\trueparam$ as an input, the planner faces the same uncertainty over the parameter as the agents. However, the planner can strategically set the mechanism to send signals into the parameter's true value. The signal is revealed before agents make their choices, thereby influencing public belief over the parameter and affecting the equilibrium that is achieved. In Sec. \ref{subsec:model_signalling_cp}, we formalize this class of signalling mechanisms and introduce the planner's problem of designing the optimal mechanism.

\subsection{Agent Behavior and Infectious Risk}
\label{subsec:model_agent}

\noindent We consider a unit mass of risk-neutral, Bayesian-rational agents. Each agent simultaneously commits to either working in-person at a shared workspace ($\ws$) or working remotely ($\wrr$). Agents' choices result in a mass of agents $\fin$ who have chosen to work remotely where $0 \leq \fin \leq 1$. The \textit{in-person mass} is correspondingly $0 \leq 1-\fin \leq 1$.

\noindent Agents that work in-person each receive a privately-known benefit $\benefit$ that is heterogeneous across this continuum population where $\benefit$ follows a commonly-known distribution $\popdist$ over $\R_+$. The benefit encapsulates the personal value agents derive from working in-person net any travel costs. In order to interchange between agents' private benefits and the \textit{quantile} of their benefit, we define the inverse cumulative distribution $\popdist^{-1}$ where $\popdist^{-1}(u) \coloneqq \sup\{t: \popdist(t) \leq u\}$ as is standard practice.

\noindent Agents that work in-person also face both an uncertain risk of contracting the disease per infectious contact and also face uncertain costs in the event they do become ill. Both the transmissivity and severity of the disease are natural sources of public uncertainty as they cannot be easily estimated by individual agents. The overall risk agents can expect to incur directly depends on the in-person mass in a known way, as the increased frequency of contacts and likelihood of infected individuals being present can be easily estimated. 
% \textit{The perceived probability of infection for an individual engaging in social interactions is the product of the perceived infectiousness of the disease }
Since agents are risk neutral, we capture the product of the uncertain risk per contact and uncertain costs into an uncertain \textit{infectiousness (risk) parameter} $\trueparam \in \paramspace := [0,\maximal]$ for some $\maximal \in \R_+$. One can interpret $\maximal$ as the \textit{worst-case} infectious risk that agents feasibly could believe. Critically, we assume that the agents cannot perceive the value of the parameter $\trueparam$ that was realized for this specific disease, but that the agents and planner all commonly believe a prior distribution $\dist$ over $\paramspace$ from which $\trueparam \sim \dist$.

\noindent We model the (expected) stochastic infectious cost $\costfxn{\trueparam}{\fin}$ to be linear in $\trueparam$ and decreasing in the remote mass $\fin$ (increasing for in-person mass)\footnote{Observe that $\trueparam$ can be replaced with any injective function $c_0(\trueparam)$ so long as it is common knowledge as the setting can be reparameterized by adjusting $\dist$ to incorporate the transformation. }. Specifically, for commonly-known functions $c_1, c_2: [0,1] \rightarrow \mathbb{R}$:
\begin{align}
    \label{eqn:infectious_cost}
   \costfxn{\trueparam}{\fin} \coloneqq \trueparam \costperparam(\fin)+\constantcost(\fin)
\end{align}
\begin{ass*}
\begin{enumerate}
    \item[]
    \item[\textbf{A1}:] $c_1(1) = c_2(1) = 0$
    \item[\textbf{A2}:] $\costperparam$ is strictly decreasing, differentiable and bounded (denote $\costperparam(0) \coloneqq \maxcost$).
    \item[\textbf{A3}:] $\constantcost$ is weakly decreasing and differentiable.
\end{enumerate}
\end{ass*}
We further motivate this form of the infectious cost in greater detail in Appendix $\ref{appendix:aisys}$. Given the actions of all agents $\fin$ and the true parameter $\trueparam$, the utility of agents with type $\benefit$ working in-person is:
\begin{align}
\label{eqn:utility_fxn}
    u_\benefit(\ws,\fin;\trueparam) =  \benefit - \costfxn{\trueparam}{\fin}
\end{align} 

\noindent Any agents that work remotely face no infectious risk, but do not receive any benefit from the work environment. Consequently, the utility of an agent of type $\benefit$, $u_\benefit(\wrr,\fin;\trueparam) = 0$ independent of $\trueparam$ and $\fin$. 

\subsection{Signalling and Central Planner Objective}
\label{subsec:model_signalling_cp}

\noindent The planner can implement a \textit{signalling mechanism} which publicly provisions information into the true realization of $\trueparam$ to all agents. Specifically, we assume that the planner publicly commits to and discloses a mechanism $\pi = \langle \I, \{z_\param\}_{\param \in \paramspace} \rangle$ where $\{z_\param\}_{\param \in \paramspace}$ are a set of probability distributions with each $z_\param$ distributed over the set of \textit{signals} $\I$. The true realization of the infectious risk parameter $\trueparam$ is then realized unbeknownst to the agents and the planner. A signal $\signal \in \I$ is randomly chosen and disclosed with probability $z_{\trueparam}(\signal)$. The planner does not observe the true parameter value before committing to $\pi$. Thus, the planner cannot influence the mechanism after the true parameter is realized.

\noindent Prior to choosing their actions, all agents view $\signal \in \I$ and symmetrically update their belief over $\trueparam$ to a posterior distribution $\dist_\signal$ where:
\begin{align}
    \label{eqn:F_i}
    \dist_{\signal'}(t) &= \mathbb{P}[\trueparam \leq t|\signal=\signal'] = 
    \frac{\int_{0}^{t} z_\param(\signal') d\dist(\param)}{\int_0^\maximal z_\param(\signal') d\dist(\param)} 
\end{align}

\noindent For any given $\pi$, it is useful to represent the corresponding probability with which each signal $\signal \in \I$ is generated and the posterior mean of $\trueparam$ upon viewing each signal $\signal \in \I$. If agents' strategies only depend on their mean beliefs over $\paramspace$, this representation is equivalent to a \textit{direct mechanism} where the planner performs the update on the agents' behalf and simply shares the updated posterior mean with all agents. We denote such a mechanism by the set of tuples $\mathcal{T}_{\pi} = \{(q_\signal, \posterior{\signal})\}_{\signal \in \I}$ where:
\begin{align}
    q_\signal &\coloneqq \int_{0}^{\maximal} z_{\param}(\signal) d\dist(\param) \hspace{1em} [\text{signal probability}] \label{eqn:q_i}\\
    \posterior{\signal} &\coloneqq \frac{\int_{0}^{\maximal} \param z_{\param}(\signal) d\dist(\param) }{\int_{0}^{\maximal} z_{\param}(\signal) d\dist(\param) }\hspace{1em}  [\text{posterior mean}] \label{eqn:theta_i}
\end{align}

As the following mechanisms will be critical to the novelty of our results, we highlight a class of signalling mechanisms called \textit{monotone partitional} signalling mechanisms where there exists a finite partition of $\paramspace$, $\mathcal{P} \coloneqq \{\paramspace_j\}_{j=1}^m = \{[t_{j-1},t_j]\}_{j=1}^m$  for some $m$ with $t_0 = 0, t_m = \maximal$ and some increasing sequence $\{t_j\}_{j=1}^{m-1} \subseteq \paramspace$ such that $\I = [m]$ and for all $\param$, $z_\param(j) = \mathbb{I}\{\param \in [t_{j-1}, t_j]\}$. Observe from \eqref{eqn:q_i} and \eqref{eqn:theta_i} that for these mechanisms $q_j = \dist(t_j) - \dist(t_{j-1})$ and $\posterior{j} = \frac{\int_{t_{j-1}}^{t_j} \param d\dist(\param)}{q_j}$. 

To provide a discrete analog of this definition, consider a discrete distribution $D$ over a set $|\paramspace| = \{\nu_1, .., \nu_k\} < \infty$ for some $k$ with $\mathbb{P}[\trueparam = \nu_j] = p_j$. We designate a mechanism $\pi$ \textit{discrete monotone partitional} if there exists for finite $m$ a non-decreasing sequence $\{r_j\}_{j=1}^{m-1} \subseteq [k]$ with $r_0 = 1$ and $r_m = k$ such that $\I = [m]$ and (i) for all $j$ such that $\exists k$ with $r_{k-1} < j < r_{k}$, $z_{\nu_j}(k) = 1$, (ii) for all $j < r_{k-1}$ or $j > r_{k}$, $z_{\nu_j}(k) = 0$. As an example, if $k=2$ and $m=2$, observe that any signalling distributions $z_{\nu_1}, z_{\nu_2}$ are discrete monotone partitional if $z_{\nu_1}(1)z_{\nu_1}(2)z_{\nu_2}(1)z_{\nu_2}(2) = 0$ (at least one parameter almost surely maps to a single signal). 

\subsubsection{Game Structure}
\noindent Each instance of our game for a particular distribution over types $\popdist$ and public belief $\dist$ over $\paramspace$ can be expressed in normal form $\Gamma(\popdist, \dist) = \langle \popdist, (\mathcal{S}_v)_{\benefit \in \R_+},(u_\benefit)_{\benefit \in \R_+}\rangle$:

$\popdist$: private types of agents in the unit mass distributed $\benefit \sim \popdist$

$\mathcal{S}_\benefit$: type $\benefit$ agents' strategies, $\mathcal{S}_\benefit = \{\ws,\wrr\}$, $\forall \benefit \in \R_+$ 

$u_\benefit$: type $\benefit$ agents' utility functions $u_\benefit(s_\benefit, \fin; \trueparam)$ for strategy $s_\benefit \in \mathcal{S}_\benefit$, $\fin(\mathbf{s}) \coloneqq \int_{\R_+} \mathbb{I}\{s_\benefit = \wrr\}dG(\benefit)$ and parameter $\trueparam$

\noindent To implement the mechanism we consider the notion of a (Nash) equilibrium where no agents have an incentive to deviate from where they decided to work. In particular, agents of type $\benefit$ at an equilibrium $\profile^* \coloneqq (s_\benefit^*)_{\benefit\in\R_+}$ should always be choosing an action that generates utility equal to the best alternative of working remotely or in-person:
\begin{align*}
s_\benefit^* &= \argmax_{\ell \in \{\ws,\wrr\}}  \E[u_\benefit(\ell, \fin^*; \trueparam)]    
\end{align*}
For a given profile of strategies, observe that the induced remote mass is the measure of the mass of agents choosing strategies to work in-person: \begin{align*}
    \fin(\profile) \coloneqq \int_{\R_+} \mathbb{I}\{s_\benefit = \wrr\}dG(\benefit)
\end{align*}
The following definition encapsulates a necessary and sufficient description of solution concept we have described using the previous statements.
% Profile = \mathbf{s}, but this is ill-defined. 
It is easy to see that, in any equilibrium of the game, the set of types that choose remote work is exactly that of the form. 

\begin{defn}
\label{defn:pse}
The strategy profile $\profile^*$ is a Nash equilibrium of our game $\Gamma(\popdist,\dist)$ when $\E_{\trueparam \sim \dist}[u_\benefit(\ws, \fin(\profile^*); \trueparam)] > 0$ if and only if $s_\benefit^* = \ws$.
\end{defn}

\noindent Once signal $\signal \in \I$ is publicly revealed with the mechanism $\pi$, a signal-specific public belief $F_\signal$ over the risk parameter (computed using $\eqref{eqn:F_i}$) is induced and we denote the equilibrium strategies that agents choose in-response at equilibrium by $\profile_\pi^*(\signal)$ and the corresponding remote mass $\final(\signal) \coloneqq y(\profile_\pi^*(i))$.

\noindent In our model, the planner seeks to maximize their expected utility measured by the objective function $\obj(\fin;\trueparam)$ that depends on the equilibrium remote mass and the true risk parameter. 
\noindent We can express the (expected) objective $V_{F,\obj}(\pi)$ of the planner using $\pi$ by:
\begin{align}
    V_{F,\obj}(\pi) = \mathbb{E}_{\trueparam \sim \dist, i \sim z_{\trueparam}}[\obj(\final(i); \trueparam)] \label{eqn:gen_objective_stateful}
\end{align}
\noindent The planner seeks to design the optimal signalling mechanism $\pi_{F,\obj}^*$ such that: 
\begin{align}
    \pi_{F,\obj}^* &\in \argmax_{\pi: \langle\I,\{z_\param\}_{\param \in \paramspace} \rangle} V_{F,\obj}(\pi)
    \label{eqn:opt_v}
\end{align}

\noindent We highlight three classes of objective functions of interest. The first are what we denote as \textit{state-independent, indicator} objectives where for some $\goal \subset [0,1]$, $\obj(\fin;\trueparam) = \mathbb{I}\{\fin\in \goal\}$. Observe that the objective is critically piece-wise constant and does not depend on $\param$. The objective can be represented by a set $\goal$ of desirable in-person mass allowances (corresponding to remote masses). For objectives $\obj$ of this form, we can equivalently express the (expected) objective $V_{F,\obj}(\pi)$ of the planner using $\pi$ by:
\begin{align}
    V_{F,\obj}(\pi) = \mathbb{P}\{\final(i) \in \goal\} \label{eqn:objective_state_indpt}
\end{align} The second are \textit{state-dependent, indicator} objectives wherein we maintain sets of desirable remote masses $\goal(\param) \coloneqq [b(\param),\infty)$ that are nested half-intervals that shrink as $\param$ increases. Precisely, we focus on objectives of the form $\obj(\fin; \trueparam) = \indicator{\fin \geq b(\trueparam)}$ for some increasing function $b(\cdot)$. From a practical viewpoint, the stateful objective mimics capacity restrictions that are imposed on the shared workspace which are gradually scaled back as the infectiousness decreases. For these objectives, the expected objective under a mechanism $\pi$ can be represented by:
\begin{align}
    V_{F,\obj}(\pi) = \mathbb{P}\{\final(i) \geq b(\trueparam)\}
\end{align} 

The final class is the most general where we will only ourselves to a functional description of the planner objective. Namely, a function $\obj(\final(i);\trueparam)$ will be specified that will obey certain regularity and the design problems are captured in Equations \eqref{eqn:gen_objective_stateful} and \eqref{eqn:opt_v}.

==> archive/Preliminaries.tex <==
%!TEX root = Opt_Info_Provision_Hybrid.tex

\section{Preliminaries}
\label{sec:static_id}
% Consistent with the literature, probability π can be thought of as an abstraction of the intensity with which messages are sent (see, e.g., Alizamir et al. 2020), More precisely, µ corresponds to the product of (i) the (subjective) probability of disease transmission through contact between the individual and an infectious subject and (ii) the (perceived) proportion of infected individuals in the population engaging social interactions, can let alpha be $[0,1]$, Numerical study, partial adherence, A-SIYS, "COVID * persistent" boosters public health
\noindent In this section, we fully characterize the equilibrium $\profile^*(i)$ and corresponding masses $\final(i)$ as a function of the agent's posterior mean beliefs $\posterior{\signal}$.

\subsection{Equilibrium Characterization}
\noindent Recall from \eqref{eqn:utility_fxn} that agents' utilities have a linear dependence on $\theta$. Since agents are risk-neutral, it is clear from Definition \ref{defn:pse} that the equilibrium outcome $\final(\signal)$ should only vary as a function of the posterior means $\posterior{\signal}$. In other words, disparate signals inducing the same posterior mean should yield an identical equilibrium aggregate response. Observe that agents that work in-person incur the same expected costs but may derive different benefits, so the agents deriving the highest value from working in-person should do so in an equilibrium. The following proposition formalizes this insight and characterizes the equilibrium remote mass $\final(\signal)$ and the functional form it takes in terms of the posterior mean $m(\posterior{\signal}) \coloneqq \final(i)$. 
\label{subsec:static_eqn_char}
\begin{prop}
\label{prop:eqbm_formula_prop_1}
For any signal $i \in \I$ under any mechanism $\pi$, $\final(i)  = m(\posterior{\signal}) \coloneqq \inf\{u \geq 0: G^{-1}(u) \geq c_1(u)\posterior{\signal}+c_2(u)\}$ with:
\begin{align*}
    s_v^*(i) = \begin{cases}
\wrr & \text{ if } v \leq \final(i)\\
\ws & \text{ if } v > \final(i)
\end{cases}
\end{align*}
\end{prop}

\noindent Intuitively, the proposition sets the remote mass $m(\posterior{\signal})$ by having as few agents work remotely as possible until the agents that would need to move in-person find the infectious cost too high. The monotone, inverse function $G^{-1}(u)$ corresponds to the highest benefit amongst the mass of $u$ agents with the smallest benefits $v$. The computation merely decreases $u$ until $G^{-1}(u)$ no longer exceeds the expected infectious costs.

\begin{proof}
The following lemma
shows that \textit{under any equilibrium} $\final(i)$ as defined in Definition \ref{defn:pse}, there is a critical group $v^*(i) \in \R_+$ such that all agents of type $v \leq v^*(i)$ work remotely, and all agents of type $v > v^*(i)$ work in-person.
\begin{subproof}
\begin{lemma}
\label{lemma:rectangular_curve}
For any equilibrium $\final(i)$, there exists a critical group $v^*(i) \in \R_+$ such that for all $v \leq v^*(i)$, $s_v^*(i) = \wrr$ and all $v > v^*(i)$ $s_v^*(i) = \ws$.
\end{lemma}
\begin{subproof}
The proof proceeds by construction. Suppose that $s_v^*(i)$ is an equilibrium and let $v^*(i) = \sup\{t: s_t^*(i) = \wrr \}$. Suppose, by contradiction, that there exists $v < v^*(i)$ such that $s_v^*(i) = \ws$. Then, $v \geq c_1(\final(i))\posterior{\signal}+c_2(\final(i))$. However, this implies that $\hat{v} > c_1(\final(i))\posterior{\signal}+c_2(\final(i))$ for all $\hat{v} > v$ and hence by Definition $\ref{defn:pse}$, $s^*_{\hat{v}}(i) = \ws$. Hence, $\sup\{t: s_t^*(i) = \wrr\}\leq v$. This is a contradiction, so it is proven that for all $v \leq v^*(i)$, $s_v^*(i) = \wrr$ and hence $v^*(i)$ satisfies the conditions of the critical type.
\end{subproof}
\end{subproof}

\noindent The next lemma precisely computes the in-person equilibrium mass in response to signal $i$. Given the restriction on $s_v^*(i)$ established in the previous lemma, this will precisely identify the equilibrium remote mass $\final(i)$ that the agents will achieve as in the proposition statement and consequently proves the proposition result. 
\begin{subproof}
\begin{lemma}
\label{lemma:compute_inperson_mass}
In any equilibrium $\final(i)$, the equilibrium remote mass $\final(i) = \inf\{u \geq 0: \popdist^{-1}(u) \geq c_1(u)\posterior{\signal}+c_2(u)\}$.
\end{lemma}
\begin{subproof}
Let $\final(i) = z$ and $\inf\{u \geq 0: \popdist^{-1}(u) \geq c_1(u)\posterior{\signal}+c_2(u)\} = z+\epsilon$ for some $\epsilon$. By Definition \ref{defn:pse} and Lemma \ref{lemma:rectangular_curve}, all agents of type $v \leq \popdist^{-1}(z)$ are such that $v \leq c_1(z)\posterior{\signal}+c_2(z)$ and all agents of type $v > \popdist^{-1}(z)$ are such that $ v > c_1(z)\posterior{\signal}+c_2(z)$.

\noindent Suppose by contradiction $\epsilon > 0$. Since $c_1(u)\posterior{\signal}+c_2(u)$ is strictly decreasing in $u$, by definition of infinum, for all $t < z+\epsilon$, $\popdist^{-1}(t) < c_1(t)\posterior{\signal}+c_2(t)$. Hence, $\popdist^{-1}(z+\frac{\epsilon}{2}) < c_1(z+\frac{\epsilon}{2})\posterior{\signal}+c_2(z+\frac{\epsilon}{2})$. But since $\popdist^{-1}(z+\frac{\epsilon}{2}) \geq \popdist^{-1}(z)$ since $\popdist^{-1}$ is non-decreasing, $\popdist^{-1}(z+\frac{\epsilon}{2}) > c_1(z)\posterior{\signal}+c_2(z) > c_1(z+\frac{\epsilon}{2})\posterior{\signal}+c_2(z+\frac{\epsilon}{2})$. This is a contradiction.

\noindent Analogously, suppose by contradiction, that $\epsilon < 0$. Then, $\popdist^{-1}(z+\frac{\epsilon}{2}) \leq \popdist^{-1}(z) \leq c_1(z)\posterior{\signal}+c_2(z) < c_1(z+\frac{\epsilon}{2})\posterior{\signal}+c_2(z+\frac{\epsilon}{2})$. % by monotonicity, then by eq defn in 1st paragraph, by monotonicyt of cost
But, by infinum definition, $\popdist^{-1}(z+\frac{\epsilon}{2}) \geq c_1(z+\frac{\epsilon}{2})\posterior{\signal}+c_2(z+\frac{\epsilon}{2})$. % may need to show that this holds for all t > inf but small detail
This is a contradiction.

\noindent This implies that $\epsilon = 0$, so $\final(i) = \inf\{u \geq 0: \popdist^{-1}(u) \geq c_1(u)\posterior{\signal}+c_2(u)\}$. 
% \srs{Clean up proofs and edge case.}
\end{subproof}
\end{subproof}
\qed
\end{proof}

\noindent Proposition $\ref{prop:eqbm_formula_prop_1}$ identifies a threshold-based structure that the equilibrium must obey. Specifically, we can define a critical type $v^*(i) = G^{-1}(\final(i))$ where agents of type $v$ for $v > v^*(i)$ all work in-person and agents of type $v$ for $v < v^*(i)$ all work remotely. This characteristic allows the planner to only affect the mass of in-person workers as the types that will participate given the in-person mass is deterministically the highest types.

\noindent Moreover, as the posterior mean belief of the infectiousness $\posterior{\signal}$ increases, agents are more cautious to choose in-person work because the infectious cost increases on expectation. The following lemma establishes that the equilibrium remote mass is monotone and smooth in $\posterior{\signal}$. 

\begin{lemma}
$m(\theta)$ is non-decreasing, bounded and continuous in $\theta$.
\label{lemma:m_smooth}
\end{lemma}
\begin{proof}
\noindent Observe that $0 \leq m(\theta) \leq 1$ since from the definition above $m(\theta) \geq 0$ and $G^{-1}(1) > 0 = c_1(1) \theta + c_2(1)$ so $m(\theta) \leq 1$. Hence, $m(\theta)$ is bounded.
% \inf{u: \geq c_1(u)\posterior{\signal}+c_2(u)
\noindent Similarly, letting $f(u) = \frac{\popdist^{-1}(u) - c_2(u)}{c_1(u)}$, we equivalently have $m(\theta) = \inf\{u: f(u) \geq \theta \}$. Since $c_1(u)$ is a strictly decreasing function in $u$ and $\popdist^{-1}(u) - c_2(u)$ is a non-decreasing function, $f(\cdot)$ is strictly increasing. For any $\theta' \leq \theta''$ notice $\{u: f(u) \geq \theta'' \} \subseteq \{u: f(u) \geq \theta' \}$, so $m(\theta') \leq m(\theta'')$ and hence $m$ is non-decreasing. Applying Berge's Maximum Principle, we also determine that $m(\theta)$ is continuous.$\blacksquare$
\end{proof}

\noindent Using Proposition \ref{prop:eqbm_formula_prop_1} and Lemma \ref{lemma:m_smooth}, we conclude that as the posterior mean $\posterior{\signal}$ increases, the equilibrium remote mass smoothly increases as demonstrated in Figure \ref{fig:a}. Observe that the funciton $m$ is completely determined by the distribution of types $\popdist$ and has no dependence on with the true distributions over the infectiousness $\dist$. Also observe from Figure \ref{fig:a} that while monotone and continuous, we cannot comment generally on the convexity of $m$ over $\paramspace$. \footnote{The results in \cite{de_vericourt_informing_2021} include and sometimes depend on the concavity of the function $m$ which follows when $\popdist$ is uniform.} As a result, the design of the optimal signalling mechanism can be viewed as the problem of \emph{maximizing the probability} that \emph{posterior means} generated by the mechanism correspond to in-person masses $\final(i)$ that the \emph{planner deems desirable} (i.e. $\fin  \in \goal(\theta)$).

\begin{figure}[h]
\label{fig:m_fxn}
\centering     %%% not \center
\subfigure[Remote equilibrium mass as a function of posterior mean.]{\label{fig:a}\includegraphics[width=60mm]{img/m_theta.png}}
\subfigure[Critical type as a function of posterior mean.]{\label{fig:b}\includegraphics[width=60mm]{img/v_star.png}}
\end{figure}

==> notation.tex <==
\newcommand{\param}{\theta}
\newcommand{\paramspace}{\Theta}
\newcommand{\maximal}{M}
\newcommand{\trueparam}{\theta^*}
\newcommand{\priormean}{\mu^{\circ}}
\newcommand{\posterior}[1]{\mu_{#1}}
\newcommand{\fin}{y}
\newcommand{\indicator}[1]{\mathbb{I}\{#1\}}
\newcommand{\signal}{i}
\newcommand{\mfxn}{m}
\newcommand{\maxcost}{C}
\newcommand{\discpspace}{\Theta_\delta}
\newcommand{\final}{\fin_{\pi}^*}
\newcommand{\costfxn}[2]{\beta(#2; #1)}
\newcommand{\sigprob}[2]{z_{#1}(#2)}
\newcommand{\obj}{h}
\newcommand{\costperparam}{c_1}
\newcommand{\constantcost}{c_2}
\newcommand{\I}{\mathcal{I}}

\renewcommand{\P}{\mathbb{P}}

\newcommand{\benefit}{v}
\newcommand{\ws}{\ell_S}
\newcommand{\wrr}{\ell_R}
\newcommand{\profile}{\mathbf{s}}

\newcommand{\ubar}[1]{\text{\b{$#1$}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\dist}{F}
\newcommand{\popdist}{G}
\newcommand{\goal}{\mathcal{Y}}
\newcommand{\mean}{\mu}
\newcommand{\wll}[1]{\omega_{#1}^\ell}
\newcommand{\wlh}[1]{\omega_{#1}^h}
\newcommand{\lol}[1]{\ubar{\theta}_{#1}}
\newcommand{\hil}[1]{\bar{\theta}_{#1}}
\newcommand{\projgoal}{\bar{\mathcal{Y}}}
\newcommand{\norm}[1]{\|{#1}\|}

\newcommand{\numintervals}{K}

==> presentations/CDC_Slides/1_Novelty.tex <==
\begin{frame}
\frametitle{Motivation}
\begin{itemize}
    \item Public health messaging and news reporting impacted individual activity/isolation 
    levels during pandemic\footnote{Alcott et al. '20, Bursztyn et al. '20}
     \item \textcolor{red}{Bayesian information design} applied to risk of community transmission can be an effective tool for shaping agents' decisions, particularly in \textit{post-peak} phase 
     \end{itemize}
     \vspace{1cm}
  Our setup:    
     \begin{itemize}
     \item[Q.] How can a planner \textcolor{blue}{provision information} to manage \textcolor{blue}{strategic hybrid workers} who have \textcolor{blue}{choice to work in-person}?
    \item Planner's utility defined in terms of \textcolor{blue}{ranges of preferred in-person agent mass} to balance \textcolor{blue}{gains from in-person activity} at workplace against \textcolor{blue}{costs from disease spread} 
% \begin{itemize}
    %     \item e.g. managing hybrid work with congestive costs in workplace
    %     \item \textbf{Uncertainty about risk} of community disease spread
    % \end{itemize}

\end{itemize}
% \begin{figure}[h]
%     \centering
%     \scalebox{0.6}{
%     \begin{tabular}{cc|c|c|}
    
%       & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Intervention Type}}\\
%       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Hard}  & \multicolumn{1}{c}{Soft} \\
%       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(lockdowns)}  & \multicolumn{1}{c}{(info design)} \\
%       \cline{3-4}
%       {\textbf{}}  & Pre-peak & \greencheck & \xmark \\\cline{3-4}
%       & Post-peak & \xmark & \greencheck \\\cline{3-4}
%     \end{tabular}
%     }
%   \end{figure}
\end{frame}

\begin{frame}{Setup}
    \begin{itemize}
        \item Planner discloses \textcolor{blue}{public information} over uncertain state $\trueparam \sim \dist$ for \textbf{continuous} $\dist$ to unit mass of \textcolor{blue}{strategic} agents 
        %receiving \textbf{public information disclosure} over uncertain state $\trueparam \sim \dist$ for \textbf{continuous} $\dist$
        \item Mass (fraction) $1-\fin$ elect to work in office 
        \item Each agent gains personal benefit and incurs uncertain cost that depends on $\trueparam$ and $\fin$
        \item[] 
        \item We focus on design of \textcolor{blue}{optimal information provision} for broad classes of \textbf{planner preferences} $\obj(\fin;\trueparam)$
    \end{itemize}
\end{frame}

\begin{frame}{Overview of results}
    \begin{itemize}
        \item[A.] \underline{State-independent, set-based preference:} $\obj(\fin;\trueparam)=\mathbb{I}\{\fin\in\goal\}$
        \begin{itemize}
            \item \textbf{Motivation:} Capacity mandates
            \item For most distributions $\dist$, optimal mechanism just signals which of two intervals that partitions $\paramspace$ the true value lies in
            \item \textcolor{blue}{Interval-based structure}
        \end{itemize}
        \vspace{0.5cm}
        \item[B.] \underline{Scaled capacity:}  $\obj(\fin;\trueparam)=\mathbb{I}\{\fin\geq a(\trueparam)\}$ for increasing function $a$
        \begin{itemize}
            \item \textbf{Motivation:} Safe capacity limits
            \item Using \textcolor{blue}{linear programming} for algorithmic design of mechanism
        \end{itemize}
        \end{itemize}
\end{frame}


\begin{frame}{Related work}
\begin{tikzpicture}[sibling distance=15em,
  every node/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20}, foo/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=green!20}]]
  \node {Information Design Literature}
    child { node {binary $\trueparam$} child { node {Fixed \textbf{$\obj$}\\\tiny Kamenica et al. '11\\\tiny DeVericourt et al. '21} } }
    child { node {general $\trueparam$}
      child { node {$\obj$-agnostic\\ design}
        child { node[foo] {\textbf{set-based $\obj$}\\\textbf{\tiny SAJ22*}} }
        child { node[foo] {\textbf{scaled-capacity $\obj$}\\\textbf{\tiny SAJ22*}} }}
      child { node {Fixed \textbf{$\obj$}\\\tiny Gentzkow et al. '16\\\tiny Kolotlin '19\\\tiny Guo et al. '19\\\tiny Dworczak et al. '19\\\tiny Candogan et al. '21\\\tiny Ivanov '21} } };
\end{tikzpicture}
\vspace{0.5cm}
\hline\vspace{0.5cm}
\textbf{Hard interventions:} \\ 
Hu et al. '22, Birge et al. '20, Acemoglu et al. '20, \\Chernozhukov et al. '21, Moore '21, Drakopoulos et al. '14
% \begin{itemize}
%     \item Hu et al. '22, Birge et al. '20, Acemoglu et al. '20, Chernozhukov et al. '21, Moore '21, Drakopoulos et al. '14
% \end{itemize}
\end{frame}

==> presentations/CDC_Slides/2_Model.tex <==
\begin{frame}
\frametitle{Model: Uncertainty \& Signalling}
\begin{itemize}
\item Unknown state $\trueparam \in \paramspace \coloneqq [0,\maximal]$ where $\trueparam \sim \dist$ 
\begin{itemize}
    \normalsize
    \item $\dist$ is \textcolor{blue}{commonly known} and $\priormean = \E_F[\trueparam]$
    \item $\uparrow$ values of state $\Rightarrow$ $\uparrow$ risk of community transmisison
\end{itemize}
\item[] 
\item Planner \textit{publicly} commits and discloses \textcolor{blue}{signalling mechanism}:\;  \[\pi = \langle \{z_\param(\cdot)\}_{\param \in \paramspace},\I \rangle\]
    \begin{itemize}
    \normalsize
        \item $\I$ - set (alphabet) of signals
        % (e.g.\{ {\includegraphics[width=.03\textwidth]{presentations/pres_img/umbrella.png}},{\includegraphics[width=.03\textwidth]{presentations/pres_img/sunglasses.png}}\})
        \item $z_\param \in \Delta(\I)$ - distribution over signals
        \item Signal $\signal \in \I$ is drawn from $z_{\trueparam}$, and \textit{publicly} shared with agents before they make their choices
        \item \textcolor{red}{Planner does not observe $\trueparam$} when commits/discloses 
    \end{itemize}
\end{itemize}
\end{frame}

\begin{frame}
\frametitle{Model: Uncertainty \& Signalling}
\begin{itemize}
    \item Signal $\signal$ realized w.p. $q_i$ and induces posterior mean belief $\posterior{\signal}$
    \begin{align*}
        q_i &\coloneqq \mathbb{P}[\pi\rightarrow \signal] = \int_{\param \in \paramspace} z_\param(\signal) dF(\param)\\
        \posterior{\signal} &\coloneqq  \E[\theta|\pi \rightarrow \signal] = \frac{\int_{\param \in \paramspace} \param z_\param(\signal)dF\param}{\int_{\param \in \paramspace} z_\param(\signal) dF(\param)}
    \end{align*}
    % $\posterior{\signal}$\\\quad$q_i \coloneqq \mathbb{P}[\pi\rightarrow \signal] = \int_{\param \in \paramspace} z_\param(\signal) dF(\param)$\\
    % \quad$\posterior{\signal} \coloneqq  \E[\theta|\pi \rightarrow \signal] = \frac{\int_{\param \in \paramspace} \param z_\param(\signal)dF\param}{\int_{\param \in \paramspace} z_\param(\signal) dF(\param)}$
    \item $\pi$ has \textcolor{blue}{direct mechanism} representation $\mathcal{T}_\pi = \{(q_i, \mu_i)\}_{i \in \I}$
    \item \textbf{Blackwell 1953}: A distribution over posterior means \textcolor{blue}{$H$} is induced by some information structure if and only if:\\ $\textcolor{blue}{H}$ is \underline{mean-preserving contraction} of  $\textcolor{orange}{\dist}$, that is, $\textcolor{blue}{H} \succeq\textcolor{orange}{\dist}$ 
 % \item Any distribution \textcolor{blue}{$H$}  is a distribution \textit{over $\posterior{\signal}$} for some $\pi$ if and only if $\textcolor{blue}{H} \succeq\textcolor{orange}{\dist}$ is mean-preserving contraction\footnote{Blackwell '53}
\end{itemize}
\begin{center}
\vspace{-2em}
\scalebox{0.5}{
    \begin{tikzpicture}
    
    \begin{axis}[hide y axis,axis x line*=bottom,legend style={at={(axis cs:2.5,0.1)},anchor=south west},
        xtick={-4,4},
	xticklabels={$0$,$M$},ytick={},yticklabels={},ymin=0,ymax=0.5,enlargelimits=0.1]
    \addplot[name path=f,domain=-4:4,blue] {0.38*2^(-1*x*x)};
    \addplot[name path=g,domain=-4:4,orange] {0.19*2^(-0.25*x*x)};

    \path[name path=axis] (axis cs:0,0) -- (axis cs:1,0);
    \addplot [
        thick,
        color=orange,
        fill=orange, 
        fill opacity=0.05
    ]
    fill between[
        of=g and axis,
        soft clip={domain=-4:4},
    ];
    \addplot [
        thick,
        color=blue,
        fill=blue, 
        fill opacity=0.05
    ]
    fill between[
        of=f and axis,
        soft clip={domain=-4:4},
    ];
    % \node [rotate=-90] at (axis cs:  .7,  .59) {$y=x^2$};
    \addlegendentry{H}
    \addlegendentry{F}
    \end{axis}
\end{tikzpicture} }
\end{center}
\end{frame}

\begin{frame}
\frametitle{Model: Agents}
\begin{itemize}
    \item Unit mass of non-atomic agents; each making simultaneous location choice: $ a \in \{\ellC,\ellP\}$
    \begin{itemize}
        \item $\ellC$: in-person work (communal/hotspot location) 
        \item $\ellP$: remote work (peripheral location)
    \end{itemize}
    \item $y(\mathbf{a})$: aggregate mass choosing $\ellP$
    \item Each agent has private type from known distribution $v \sim G$
    \end{itemize}
\end{frame}

\begin{frame}
\frametitle{Model: Agents}
Each agent earns reward
\begin{itemize}
    \item $u^v(\ellP, \fin;\trueparam) = 0$ if $a = \ellP$ 
    \item $u^v(\ellC, \fin;\trueparam) = v-\beta(\fin;\trueparam)$ if $a = \ellC$, where \\ $\beta(y;\trueparam) \coloneqq \trueparam c_1(y) + c_2(y)$, with $c_1(\cdot), c_2(\cdot)$ decreasing and differentiable
    % \begin{itemize}
    % \item $\beta(y;\trueparam) \coloneqq \trueparam c_1(y) + c_2(y)$ where $c_1, c_2$ decreasing and differentiable
   % \end{itemize}
 %   \item \textcolor{blue}{Remote agent mass} at equilibrium: $y(a^*| \pi \rightarrow \signal) = \final(\signal)$
\end{itemize}
\vspace{0.5cm}
\textcolor{blue}{Remote agent mass} at equilibrium: $y(a^*| \pi \rightarrow \signal) = \final(\signal)$
\begin{alertblock}{Proposition}
\begin{enumerate}
    \item In equilibrium $\final(\signal)$, $\exists v^*$ s.t. agents at $\ellC$ $\iff v > v^*$
    \item $\exists$ weakly increasing, bounded, continuous $m: \paramspace \rightarrow [0,1]$ such that $\final(\signal) = m(\posterior{\signal})$
\end{enumerate}
\end{alertblock}
\begin{itemize}
    \item Larger remote agent mass needs (even) higher posterior means 
\end{itemize}
\end{frame}

\begin{frame}{Planner's Design Problem}
For given $\textcolor{red}{\pi}$, planner earns reward $V(\pi)$:
\begin{alertblock}{Optimal signalling mechanism}
\begin{align*}
    \pi^\ast &= \argmax_{\pi} V(\pi)\\
    &\coloneqq \argmax_{\pi} \E_{\trueparam \sim \dist, \signal \sim z_{\trueparam}(\cdot)}[\obj(\pi,\fin^\ast(\signal);\trueparam)]\\
    &= \argmax_{\pi} \E_{\trueparam \sim \dist,\signal\sim z_{\trueparam}(\cdot)}[\obj(\pi,m(\posterior{\signal});\trueparam)]
\end{align*}
\end{alertblock}
\end{frame}

\begin{frame}
\frametitle{State-Independent, Set-Based Preference}
\begin{itemize}
\item $\obj(\fin;\trueparam) = \mathbb{I}\{\fin\in\goal\}$
\item $\goal = \cup_{j=1}^\numintervals \Omega_j$ -- union of $\numintervals$ intervals $\Omega_j \coloneqq [a_j,b_j] \subseteq [0,1]$
\item For each~$j$, ``desirable" posterior means: $\bar{\Theta}_j \coloneqq m^{-1}(\Omega_j)$
    % \begin{itemize}
    %     \item 
    % \end{itemize}
\end{itemize}
\centering
\includegraphics[width=0.6\textwidth]{presentations/pres_img/workshop_slides.png}

\end{frame}

\begin{frame}{Equilibrium to Beliefs}
    Planner seeks  $\pi^*$: 
\begin{align*}\argmax_{\pi} V(\pi) &= \max_{\pi} \mathbb{P}\{\final(\signal) \in \mathcal{Y}\}\\
&= \max_{\pi} \mathbb{P}\{\posterior{\signal} \in m^{-1}(\mathcal{Y})\}\\
&= \max_{\pi} \sum_{i\in\I} q_i \mathbb{I}\{\posterior{\signal} \in \cup_{j=1}^{\numintervals} \bar{\Theta}_j\}
\end{align*}
\vspace{-1em}
\begin{itemize}
    \item We analyze by position of prior mean $\priormean$ relative to $\cup_{j=1}^{\numintervals} \bar{\Theta}_j$ \\($\ubar{a} \coloneqq \min \bar{\Theta}_1$, $\bar{b} \coloneqq \max \bar{\Theta}_\numintervals)$)
    \item Relative position of prior belief $\priormean$ to the desirable beliefs $\cup_{j=1}^{\numintervals} \bar{\Theta}_j$ is critical to structure of optimal design
\end{itemize}
    
\end{frame}


==> presentations/CDC_Slides/3_Theorem_1.tex <==

\begin{frame}{Optimal Design}
\begin{alertblock}{Theorem: Regimes with monotone partitional structure (MPS)}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{1.5cm} |p{2cm}  |p{1.5cm} | c }
     \toprule
      $F$ & $\pi^*$ & $V(\pi^*)$ & \\ \hline
    % \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}\cmidrule(lr){2-2}\
    $\priormean \in \bar{\Theta}_i$
    &$\I=\{\mathbf{1}\}$\newline 
      $[0,M] \rightarrow \mathbf{1}$
     &
     1
      & 
      \raisebox{-\totalheight}{\includegraphics[height=30mm]{presentations/pres_img/g1.png}}
      \\ \hline
      \only<1>{$\priormean < \ubar{a}$}\only<2>{$ \textcolor{blue}{\priormean > \bar{b}}$}
    &$\I=\{\mathbf{1},\textcolor{red}{\mathbf{2}}\}$\newline
      \only<2>{\small{$[0,t^\ast] \rightarrow \mathbf{1}$\newline $[t^\ast,M] \rightarrow \textcolor{red}{\mathbf{2}}$}}\only<1>{\small{$[0,t^\ast] \rightarrow \textcolor{red}{\mathbf{2}}$\newline$[t^\ast,M] \rightarrow \mathbf{1}$}}
     &
     \only<1>{$1-\dist(t^\ast)$}\only<2>{$ \textcolor{blue}{\dist(t^\ast)}$}
      & 
      \only<1>{\raisebox{-\totalheight}{\includegraphics[width=0.33\textwidth, height=28mm]{presentations/pres_img/g2.png}}}\only<2>{\raisebox{-\totalheight}{\includegraphics[width=0.33\textwidth, height=28mm]{presentations/pres_img/g6.png}}}
      \\ \bottomrule
      \end{tabular}
      \end{center}
      \end{table}
\end{alertblock}
\end{frame}

\begin{frame}{Optimal Design}
\begin{itemize}
\item Let $\ubar{s}(t) = \E[\theta|\theta<t]$ and $\bar{s}(t) = \E[\theta|\theta>t]$
\end{itemize} 
\begin{alertblock}{Theorem}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{2.9cm} |p{2cm}  |p{1cm} | c }
     \toprule
      $F$ & $\pi^*$ & $V(\pi^*)$ & \\ \hline
    % \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}\cmidrule(lr){2-2}
    $\ubar{a} \leq \priormean \leq \bar{b} \newline \priormean \notin \cup_{i=1}^\numintervals \bar{\Theta}_i\newline \exists t$,  $\ubar{s}(t), \bar{s}(t) \in \cup_{i=1}^\numintervals \bar{\Theta}_i$
    & $\I=\{\mathbf{1},\mathbf{2}\}$\newline $[0,t] \rightarrow \mathbf{1}$\newline $[t,M] \rightarrow \mathbf{2}$
     &
     1
      & 
      \raisebox{-\totalheight}{\includegraphics[height=25mm]{presentations/pres_img/g4.png}}
      \\ \bottomrule
      \end{tabular}
      \end{center}
      \end{table}
\end{alertblock}
\begin{itemize}
\item Disperse mean belief; but can't do so if too tightly concentrated
\item Can derive more general conditions without much complexity
\end{itemize}
\end{frame}

\begin{frame}{Optimal Design}
\begin{itemize}
\item $p(t,\lambda,\delta)$ and $q(t,\lambda,\delta)$ more diffused analogs of $\ubar{s}, \bar{s}$
\end{itemize}
\begin{alertblock}{Theorem}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{2.7cm} |p{2.5cm}  |p{1cm} | c }
     \toprule
      $F$ & $\pi^*$ & $V(\pi^*)$ & \\ \hline
    % \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}\cmidrule(lr){2-2}
    $\ubar{a} \leq \priormean \leq \bar{b} \newline\priormean \notin \cup_{i=1}^\numintervals \bar{\Theta}_i \newline \exists t$,  \small $p(t,\lambda,\delta), \newline {q(t,\lambda,\delta) \in \cup_{i=1}^\numintervals \bar{\Theta}_i}$
    & $\I=\{\mathbf{1},\mathbf{2}\}$
    \begin{align*}
        [0,t] \xrightarrow{\text{w.p }\lambda} \mathbf{1} \\ \xrightarrow{\text{w.p }1-\lambda} \mathbf{2} \\ [t,M] \xrightarrow{\text{w.p }\delta} \mathbf{2} \\ \xrightarrow{\text{w.p }1-\delta} \mathbf{1}
    \end{align*}
     &
     1
      & 
      \raisebox{-\totalheight}{\includegraphics[height=25mm]{presentations/pres_img/g5.png}}
      \\ \bottomrule
      \end{tabular}
      \end{center}
      \end{table}
\end{alertblock}
\end{frame}

\begin{frame}
\frametitle{Proof idea}
\begin{itemize}
    \item \underline{Part I:} Require at most $\numintervals+1$ signals ($|\I|\leq \numintervals+1$)
    \begin{itemize}
        \item $\bar{\Theta}_j$ are closed, convex intervals
        \item For each $j$, $\posterior{\signal_1},\posterior{\signal_2} \in \bar{\Theta}_j$ can be combined without loss 
    \end{itemize}
    \item \underline{Part II:} Objective fn. of $q_\signal, \posterior{\signal}$, so can search over $\mathcal{T}_\pi$'s
    \begin{itemize}
        \item Search directly over all $\textcolor{blue}{H} \succeq \textcolor{orange}{\dist}$
        \item Constraints: $\int_0^c \textcolor{blue}{H}^{-1}(t)dt \geq \int_0^c \textcolor{orange}{F}^{-1}(t)dt$ $\forall c \in [0,1]$        
    \end{itemize}
        \item<2-> \underline{Part III:} Know positions $\mu_i$
    \begin{itemize}
        \item If $\priormean < \ubar{a}$ or $\priormean > \bar{b}$, know position of $\mu_{\numintervals+1}$ relative to other posterior means in $\bar{\Theta}_j$
        \item If not, solve $\numintervals$ convex optimizations for possible locations of $\mu_{\numintervals+1}$ 
    \end{itemize}
     \item<2-> \underline{Part IV:} Combining (I) + (II) + (III)
    \begin{itemize}
        \item Know that $\textcolor{blue}{H}$ must be discrete by (I)
        \item Finite subset of constraints are sufficient so we reduce from an infinite \# of constraints to finite constraint problem
    \end{itemize}
\end{itemize}
\end{frame}

==> presentations/CDC_Slides/4_Theorem_2.tex <==
\begin{frame}{State-dependent preferences}
    \begin{itemize}
        \item Allowing preferences to depend on the state $\trueparam$ complicates the search problem (considering only $\mathcal{T}_\pi$ no longer sufficient)
    \item Motivates need for algorithmic solution for optimal design
    \item[]
    \item Consider \textbf{discrete} $\dist$ on finite number of states $\trueparam \in \{\nu_j\}_{j=1,..,N}$
    \item \textbf{Scaled-capacity}: Preferences specify an in-person capacity limit that gets progressively more strict as $\trueparam$ increases
    \begin{itemize}
    \normalsize
        \item $\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{\fin\in\goal(\trueparam)\} = \mathbb{I}\{\fin\geq a(\trueparam)\}$ where $a(\cdot)$ is  increasing function
        \end{itemize}
    \end{itemize}
\end{frame}

% in stateful setting we cannot reduce th search over pi by searching over direct mechanisms, because the posterior mean mu_i will induce an equilibrium outcome but we cannot evaluate whether that outcome is in desirable state-dependenct set since we do not know the true state. 
% in the second example, the posteriors are so generated that for certain ranges of true state, the posterior beliefs fall into desirable range of beliefs. 



\begin{frame}
\frametitle{Reduce \# of signals}
\vspace{-1em}
\begin{figure}
\only<1>{\input{presentations/pres_fig/stateful_e}}
\only<2>{\input{presentations/pres_fig/stateful_f}}
% \caption{$v(m(\cdot);\nu)$}
\end{figure}

\begin{itemize}
    \only<1>{\item $N$ curves
    \item At most one signal will correspond posteriors that have equilibrium in each interval $\mu_i \in [\gamma_i, \gamma_{i+1}]$}
   \only<2>{
    \item Signal $i$ will induce posterior $\mu_i$ that is large enough for states of the world $\nu_j$ where $j\leq i$}
\end{itemize}
\end{frame}

\begin{frame}{Solve Linear Program}
\begin{itemize}
    \item Variables $x_{ji}$ to represent probability in state $\nu_j$ under $F$ and signal $\signal$ is provisioned
    \begin{itemize}
        \item $z_{\nu_j}(i) = \frac{x_{ji}}{\sum_i x_{ji}}$
    \end{itemize}
    \item Objective and constraints on posterior can all be made linear
    \begin{itemize}
        \item Constraints on $\posterior{i}$: $\gamma_{i}\sum_{j=1}^N x_{ji} \leq \sum_{j=1}^N \nu_j x_{ji} \leq \gamma_{i+1}\sum_{j=1}^N x_{ji}$
    \end{itemize}
    \item LP algorithm outputs optimal solution $\pi^\ast$
\end{itemize}
\end{frame}



\begin{frame}
\frametitle{Conclusion}
\begin{itemize}
    \item New insights on structure and computation of optimal information mechanisms for managing hybrid workers amidst pandemic
    \item Future work: settings when planner needs to learn 
\end{itemize}
\vfill
thank you! feedback and questions? 
\end{frame}

==> presentations/Workshop_Slides/1_Novelty.tex <==
\begin{frame}
\frametitle{Our focus}
    \begin{itemize}
        \item[Q.] How can a planner \textcolor{blue}{provision information} to manage \textcolor{blue}{strategic agents} who face \textcolor{blue}{choice to move to congested hotspot}?
    %  \item \textbf{Information provision} to manage \textbf{strategic agents} who face \textbf{choice to move to congested hotspot}
        % \begin{itemize}
        %     \item Applications: pandemic management (\scalerel*{\includegraphics{presentations/pres_img/virus_clipart.png}}{B}), ride-hailing (\scalerel*{\includegraphics{presentations/pres_img/car_clipart.png}}{B})
        % \end{itemize}
        \item[-] Information governs \textcolor{blue}{agents' tradeoff of risk vs. value} at hotspot
        \item[-] Planner's utility defined in terms of \textcolor{blue}{ranges of preferred agent mass}
 at hotspot and can depend on \textcolor{blue}{unknown state} 
  \item[-] \textit{Applications:} pandemic management (\scalerel*{\includegraphics{presentations/pres_img/virus_clipart.png}}{B}), ride-hailing (\scalerel*{\includegraphics{presentations/pres_img/car_clipart.png}}{B})
       % \item Present novel model and introduce \textbf{classes of preferences} motivated by practical interest
       \item[] 
        \item Study preferences for which optimal information mechanism has \textcolor{blue}{interval-based} (esp. \emph{monotone partitional} structure).  
        \item Highlight how optimal information changes when \textcolor{blue}{dynamically provisioned} to long-run agents over a uncertain time-hotizon 
    \end{itemize}
\end{frame}

  \begin{frame}
  \vfill
  \centering
  \begin{beamercolorbox}[sep=8pt,center,shadow=true,rounded=true]{title}
    \usebeamerfont{title}Part I: Hybrid work under risk of infectious disease at worksplace\par%
  \end{beamercolorbox}
  \vfill
  \end{frame}

\begin{frame}
\frametitle{Motivation}
\begin{itemize}
    \item Public health messaging and news reporting impacted individual activity/isolation 
    levels during pandemic\footnote{Alcott et al. '20, Bursztyn et al. '20}
     \item \textcolor{red}{Bayesian information design} can be an effective tool for shaping agents' decisions, particularly in \textit{post-peak} phase 
     \end{itemize}
     \vspace{1cm}
  Our setup:    
     \begin{itemize}
    \item \textcolor{blue}{Information about risk} of community transmission at workplace can be a \textcolor{blue}{soft intervention} in hybrid work settings
    \item Planner aims to balance \textcolor{blue}{gains from in-person activity} at workplace (hotspot) against \textcolor{blue}{costs from disease spread} 
% \begin{itemize}
    %     \item e.g. managing hybrid work with congestive costs in workplace
    %     \item \textbf{Uncertainty about risk} of community disease spread
    % \end{itemize}

\end{itemize}
% \begin{figure}[h]
%     \centering
%     \scalebox{0.6}{
%     \begin{tabular}{cc|c|c|}
    
%       & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Intervention Type}}\\
%       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Hard}  & \multicolumn{1}{c}{Soft} \\
%       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(lockdowns)}  & \multicolumn{1}{c}{(info design)} \\
%       \cline{3-4}
%       {\textbf{}}  & Pre-peak & \greencheck & \xmark \\\cline{3-4}
%       & Post-peak & \xmark & \greencheck \\\cline{3-4}
%     \end{tabular}
%     }
%   \end{figure}
\end{frame}

\begin{frame}{Setup}
    \begin{itemize}
        \item Planner discloses \textcolor{blue}{public information} over uncertain state $\trueparam \sim \dist$ for \textbf{continuous} $\dist$ to unit mass of \textcolor{blue}{strategic} agents 
        %receiving \textbf{public information disclosure} over uncertain state $\trueparam \sim \dist$ for \textbf{continuous} $\dist$
        \item Mass (fraction) $1-\fin$ elect to move to hotspot 
        \item Each agent gains personal benefit and incurs uncertain cost that depends on $\trueparam$ and $\fin$
        \item[] 
        \item We focus on design of \textcolor{blue}{optimal information provision} for a broad class of \textbf{planner preferences} $\obj(\fin;\trueparam)$
    \end{itemize}
\end{frame}

\begin{frame}{Related work}
\begin{tikzpicture}[sibling distance=15em,
  every node/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20}, foo/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=green!20}]]
  \node {Information Design Literature}
    child { node {binary $\trueparam$} child { node {Fixed \textbf{$\obj$}\\\tiny Kamenica et al. '11\\\tiny DeVericourt et al. '21} } }
    child { node {continuous $\trueparam$}
      child { node {$\obj$-agnostic\\ design}
        child { node[foo] {\textbf{set-based $\obj$}\\\textbf{\tiny SAJ22*}} }
        child { node[foo] {\textbf{general $\obj$}\\\textbf{\tiny SAJ22*}} }}
      child { node {Fixed \textbf{$\obj$}\\\tiny Gentzkow et al. '16\\\tiny Kolotlin '19\\\tiny Guo et al. '19\\\tiny Dworczak et al. '19\\\tiny Candogan et al. '21\\\tiny Ivanov '21} } };
\end{tikzpicture}
\vspace{0.5cm}
\hline\vspace{0.5cm}
\textbf{Hard interventions:} \\ 
Hu et al. '22, Birge et al. '20, Acemoglu et al. '20, \\Chernozhukov et al. '21, Moore '21, Drakopoulos et al. '14
% \begin{itemize}
%     \item Hu et al. '22, Birge et al. '20, Acemoglu et al. '20, Chernozhukov et al. '21, Moore '21, Drakopoulos et al. '14
% \end{itemize}
\end{frame}

\begin{frame}{Overview of results (Part I)}
    \begin{itemize}
        \item[A.] \underline{State-independent, set-based preference:} $\obj(\fin;\trueparam)=\mathbb{I}\{\fin\in\goal\}$
        \begin{itemize}
            \item For most distributions $\dist$, optimal mechanism just signals which of two intervals that partitions $\paramspace$ the true value lies in
            \item \textcolor{blue}{Monotone partitional and interval-based structure}
        \end{itemize}
        \vspace{0.5cm}
        \item[B.] \underline{State-dependent preference:} 
        \begin{itemize}
            \item Using \textcolor{blue}{discretization} and \textcolor{blue}{linear programming} for algorithmic design of mechanisms with \textcolor{blue}{approximation guarantees}
            \begin{itemize}
                \item   \textbf{Scaled capacity:} $\obj(\fin;\trueparam)=\mathbb{I}\{\fin\geq a(\trueparam)\}$ for increasing, step function $a$
                \item \textbf{Lipschitz preference:} $\obj(\fin;\trueparam)$ is Lipschitz continuous
            \end{itemize}        
            \item Mechanism satisfies \textcolor{blue}{interval-based structure} by construction
          
        \end{itemize}
        \end{itemize}
\end{frame}

==> presentations/Workshop_Slides/2_Model.tex <==
\begin{frame}
\frametitle{Model: Uncertainty \& Signalling}
\begin{itemize}
\item Unknown state $\trueparam \in \paramspace \coloneqq [0,\maximal]$ where $\trueparam \sim \dist$ 
\begin{itemize}
    \normalsize
    \item $\dist$ is \textcolor{blue}{commonly known} and $\priormean = \E_F[\trueparam]$
    \item $\uparrow$ values of state $\Rightarrow$ $\uparrow$ risk of community transmisison
\end{itemize}
\item[] 
\item Planner \textit{publicly} commits and discloses \textcolor{blue}{signalling mechanism}:\;  \[\pi = \langle \{z_\param(\cdot)\}_{\param \in \paramspace},\I \rangle\]
    \begin{itemize}
    \normalsize
        \item $\I$ - set (alphabet) of signals
        % (e.g.\{ {\includegraphics[width=.03\textwidth]{presentations/pres_img/umbrella.png}},{\includegraphics[width=.03\textwidth]{presentations/pres_img/sunglasses.png}}\})
        \item $z_\param \in \Delta(\I)$ - distribution over signals
        \item \textcolor{red}{Planner does not observe $\trueparam$} when commits/discloses 
    \end{itemize}
\end{itemize}
\end{frame}

\begin{frame}
\frametitle{Model: Uncertainty \& Signalling}
\begin{itemize}
    \item Signal $\signal \in \I$ is drawn from $z_{\trueparam}$, and \textit{publicly} shared with agents before they make their choices
    \item Signal $\signal$ realized w.p. $q_i$ and induces posterior mean belief $\posterior{\signal}$
    \begin{align*}
        q_i &\coloneqq \mathbb{P}[\pi\rightarrow \signal] = \int_{\param \in \paramspace} z_\param(\signal) dF(\param)\\
        \posterior{\signal} &\coloneqq  \E[\theta|\pi \rightarrow \signal] = \frac{\int_{\param \in \paramspace} \param z_\param(\signal)dF\param}{\int_{\param \in \paramspace} z_\param(\signal) dF(\param)}
    \end{align*}
    % $\posterior{\signal}$\\\quad$q_i \coloneqq \mathbb{P}[\pi\rightarrow \signal] = \int_{\param \in \paramspace} z_\param(\signal) dF(\param)$\\
    % \quad$\posterior{\signal} \coloneqq  \E[\theta|\pi \rightarrow \signal] = \frac{\int_{\param \in \paramspace} \param z_\param(\signal)dF\param}{\int_{\param \in \paramspace} z_\param(\signal) dF(\param)}$
    \item $\pi$ has \textcolor{blue}{direct mechanism} representation $\mathcal{T}_\pi = \{(q_i, \mu_i)\}_{i \in \I}$
    \item \textbf{Blackwell 1953}: A distribution over posterior means \textcolor{blue}{$H$} is induced by some information structure if and only if:\\ $\textcolor{blue}{H}$ is \underline{mean-preserving contraction} of  $\textcolor{orange}{\dist}$, that is, $\textcolor{blue}{H} \succeq\textcolor{orange}{\dist}$ 
 % \item Any distribution \textcolor{blue}{$H$}  is a distribution \textit{over $\posterior{\signal}$} for some $\pi$ if and only if $\textcolor{blue}{H} \succeq\textcolor{orange}{\dist}$ is mean-preserving contraction\footnote{Blackwell '53}
\end{itemize}
\begin{center}
\vspace{-2em}
\scalebox{0.5}{
    \begin{tikzpicture}
    
    \begin{axis}[hide y axis,axis x line*=bottom,legend style={at={(axis cs:2.5,0.1)},anchor=south west},
        xtick={-4,4},
	xticklabels={$0$,$M$},ytick={},yticklabels={},ymin=0,ymax=0.5,enlargelimits=0.1]
    \addplot[name path=f,domain=-4:4,blue] {0.38*2^(-1*x*x)};
    \addplot[name path=g,domain=-4:4,orange] {0.19*2^(-0.25*x*x)};

    \path[name path=axis] (axis cs:0,0) -- (axis cs:1,0);
    \addplot [
        thick,
        color=orange,
        fill=orange, 
        fill opacity=0.05
    ]
    fill between[
        of=g and axis,
        soft clip={domain=-4:4},
    ];
    \addplot [
        thick,
        color=blue,
        fill=blue, 
        fill opacity=0.05
    ]
    fill between[
        of=f and axis,
        soft clip={domain=-4:4},
    ];
    % \node [rotate=-90] at (axis cs:  .7,  .59) {$y=x^2$};
    \addlegendentry{H}
    \addlegendentry{F}
    \end{axis}
\end{tikzpicture} }
\end{center}
\end{frame}

\begin{frame}{Monotone Partitional Structure}
    \begin{alertblock}{Monotone Partitional Structure (MPS)}
        A signaling mechanism~$\pi$ has MPS if:
        \begin{itemize}
            \item $\exists$ finite partition of $\paramspace$, $\mathbf{\mathcal{P}} \coloneqq \{\paramspace_j\}_{j=1}^m = \{[t_{j-1},t_j]\}_{j=1}^m$
            \item $0=t_0<t_1<\dots<t_{m-1}<t_m = \maximal$
            \item $\I=[m]$ and for all $\param\in\paramspace$, $z_\param(j) = \mathbb{I}\{\param \in [t_{j-1}, t_j]\}$ 
        \end{itemize}
    \end{alertblock}
    \begin{center}\includegraphics[width=0.5\textwidth]{img/mps.png}
    \end{center}
\end{frame}

\begin{frame}
\frametitle{Model: Agents}
\begin{itemize}
    \item Unit mass of non-atomic agents; each making simultaneous location choice: $ a \in \{\ellC,\ellP\}$
    \begin{itemize}
        \item $\ellC$: in-person work (communal/hotspot location) 
        \item $\ellP$: remote work (peripheral location)
    \end{itemize}
    \item $y(\mathbf{a})$: aggregate mass choosing $\ellP$
    \item Each agent has private type from known distribution $v \sim G$
    \end{itemize}
\end{frame}

\begin{frame}
\frametitle{Model: Agents}
Each agent earns reward
\begin{itemize}
    \item $u^v(\ellP, \fin;\trueparam) = 0$ if $a = \ellP$ 
    \item $u^v(\ellC, \fin;\trueparam) = v-\beta(\fin;\trueparam)$ if $a = \ellC$, where \\ $\beta(y;\trueparam) \coloneqq \trueparam c_1(y) + c_2(y)$, with $c_1(\cdot), c_2(\cdot)$ decreasing and differentiable
    % \begin{itemize}
    % \item $\beta(y;\trueparam) \coloneqq \trueparam c_1(y) + c_2(y)$ where $c_1, c_2$ decreasing and differentiable
   % \end{itemize}
 %   \item \textcolor{blue}{Remote agent mass} at equilibrium: $y(a^*| \pi \rightarrow \signal) = \final(\signal)$
\end{itemize}
\vspace{0.5cm}
\textcolor{blue}{Remote agent mass} at equilibrium: $y(a^*| \pi \rightarrow \signal) = \final(\signal)$
\begin{alertblock}{Proposition}
\begin{enumerate}
    \item In equilibrium $\final(\signal)$, $\exists v^*$ s.t. agents at $\ellC$ $\iff v > v^*$
    \item $\exists$ weakly increasing, bounded, continuous $m: \paramspace \rightarrow [0,1]$ such that $\final(\signal) = m(\posterior{\signal})$
\end{enumerate}
\end{alertblock}
\begin{itemize}
    \item $v^*$: private benefit of marginal agent indifferent over $\ellC$ \& $\ellP$
\end{itemize}
\end{frame}


\begin{frame}{Remote mass for different $\popdist$}
    \centering
    \includegraphics[width=.55\textwidth]{presentations/pres_fig/m_fig.png}
    \begin{itemize}
        \item Larger remote agent mass needs (even) higher posterior means 
        \item For simple preference and concave $m(\cdot)$, easy to maximize -- try to induce ``best" belief
    \end{itemize}
\end{frame}

\begin{frame}
\frametitle{Model: Planner Preferences}
For given $\textcolor{red}{\pi}$, planner earns reward $\obj(y;\trueparam)$
% \begin{itemize}
%     \item For given $\textcolor{red}{\pi}$, planner earns reward $\obj(y;\trueparam)$
% \end{itemize}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{1.8cm} |p{2.2cm}  |p{2cm} | p{3.5cm} }
     \toprule
      Class & $\obj(y;\trueparam)$ & Assumptions & Motivation \\ \hline
    State-indpt, set-based
    &$\mathbb{I}\{y \in \mathcal{Y}\}$
     &
     $\mathcal{Y} \subseteq [0,1]$
      & Capacity mandates, \newline Essential workers
      \\ \hline
      Scaled-capacity
    &$\mathbb{I}\{y \geq a(\trueparam)\}$
     &
     Increasing step \newline function $a$
      & Safe capacity limits
      \\ \hline
      Lipschitz
    &$\obj(y;\trueparam)$
     & jointly-Lipschitz &
    Community effects, \newline Multiple workspaces
      \\ \bottomrule
      \end{tabular}
      \end{center}
  \end{table}

\end{frame}

\begin{frame}{Planner's Design Problem}
\begin{alertblock}{Optimal signalling mechanism}
\vspace{-2em}
\begin{align*}
    \pi^\ast &= \argmax_{\pi} V(\pi)\\
    &\coloneqq \argmax_{\pi} \E_{\trueparam \sim \dist, \signal \sim z_{\trueparam}(\cdot)}[\obj(\pi,\fin^\ast(\signal);\trueparam)]\\
    &= \argmax_{\pi} \E_{\trueparam \sim \dist,\signal\sim z_{\trueparam}(\cdot)}[\obj(\pi,m(\posterior{\signal});\trueparam)]
\end{align*}
\end{alertblock}
\end{frame}

\begin{frame}
\frametitle{State-Independent, Set-Based Preference}
\begin{itemize}
\item $\obj(\fin;\trueparam) = \mathbb{I}\{\fin\in\goal\}$
\item $\goal = \cup_{j=1}^\numintervals \Omega_j$ -- union of $\numintervals$ intervals $\Omega_j \coloneqq [a_j,b_j] \subseteq [0,1]$
\item For each~$j$, ``desirable" posterior means: $\bar{\Theta}_j \coloneqq m^{-1}(\Omega_j)$
    % \begin{itemize}
    %     \item 
    % \end{itemize}
\end{itemize}
\centering
\includegraphics[width=0.6\textwidth]{presentations/pres_img/workshop_slides.png}

\end{frame}

\begin{frame}{Equilibrium to Beliefs}
    Planner seeks  $\pi^*$: 
\begin{align*}\argmax_{\pi} V(\pi) &= \max_{\pi} \mathbb{P}\{\final(\signal) \in \mathcal{Y}\}\\
&= \max_{\pi} \mathbb{P}\{\posterior{\signal} \in m^{-1}(\mathcal{Y})\}\\
&= \max_{\pi} \sum_{i\in\I} q_i \mathbb{I}\{\posterior{\signal} \in \cup_{j=1}^{\numintervals} \bar{\Theta}_j\}
\end{align*}
\vspace{-1em}
\begin{itemize}
    \item We analyze by position of prior mean $\priormean$ relative to $\cup_{j=1}^{\numintervals} \bar{\Theta}_j$ \\($\ubar{a} \coloneqq \min \bar{\Theta}_1$, $\bar{b} \coloneqq \max \bar{\Theta}_\numintervals)$)
    \item Relative position of prior belief $\priormean$ to the desirable beliefs $\cup_{j=1}^{\numintervals} \bar{\Theta}_j$ is critical to structure of optimal design
\end{itemize}
    
\end{frame}


==> presentations/Workshop_Slides/3_Theorem1.tex <==

\begin{frame}{Optimal Design}
\begin{alertblock}{Theorem: Regimes with monotone partitional structure (MPS)}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{1.5cm} |p{2cm}  |p{1.5cm} | c }
     \toprule
      $F$ & $\pi^*$ & $V(\pi^*)$ & \\ \hline
    % \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}\cmidrule(lr){2-2}\
    $\priormean \in \bar{\Theta}_i$
    &$\I=\{\mathbf{1}\}$\newline 
      $[0,M] \rightarrow \mathbf{1}$
     &
     1
      & 
      \raisebox{-\totalheight}{\includegraphics[height=30mm]{presentations/pres_img/g1.png}}
      \\ \hline
      \only<1>{$\priormean < \ubar{a}$}\only<2>{$ \textcolor{blue}{\priormean > \bar{b}}$}
    &$\I=\{\mathbf{1},\textcolor{red}{\mathbf{2}}\}$\newline
      \only<2>{\small{$[0,t^\ast] \rightarrow \mathbf{1}$\newline $[t^\ast,M] \rightarrow \textcolor{red}{\mathbf{2}}$}}\only<1>{\small{$[0,t^\ast] \rightarrow \textcolor{red}{\mathbf{2}}$\newline$[t^\ast,M] \rightarrow \mathbf{1}$}}
     &
     \only<1>{$1-\dist(t^\ast)$}\only<2>{$ \textcolor{blue}{\dist(t^\ast)}$}
      & 
      \only<1>{\raisebox{-\totalheight}{\includegraphics[width=0.33\textwidth, height=28mm]{presentations/pres_img/g2.png}}}\only<2>{\raisebox{-\totalheight}{\includegraphics[width=0.33\textwidth, height=28mm]{presentations/pres_img/g6.png}}}
      \\ \bottomrule
      \end{tabular}
      \end{center}
      \end{table}
\end{alertblock}
\end{frame}

\begin{frame}{MPS is not guaranteed}
\begin{alertblock}{Example}
\begin{itemize}
    \item $\dist \sim Unif[0,1]$ ($\priormean = 0.5$)
    \item $\bar{\Omega}_1 = [0.4-\epsilon,0.4+\epsilon], \bar{\Omega}_2 = [0.6-\epsilon,0.6+\epsilon]$
    \item[] 
    \item No mechanism with MPS achieves objective 1
    \begin{itemize}
        \item Consider first interval $[0,t_1]$ ($\mu_1 = \frac{t_1}{2}$, $\mu_i \geq \frac{1+t_1}{2}$ for all $i>1$)
    \end{itemize}
    \item[]
    \item $\I = \{1,2\}$ with $z_{\param}(1) = 0.7$ and $z_{\param}(2) = 0.3$ for all $\param \leq 0.5$, and $z_{\param}(1) = 0.3$ and $z_{\param}(2) = 0.7$ for all $\param \geq 0.5$
    \begin{itemize}
        \item $\posterior{1} = 0.4$ and $\posterior{2} = 0.6$
        \item Achieves objective of 1
    \end{itemize}
\end{itemize}
 
\end{alertblock}
\end{frame}

\begin{frame}{Optimal Design}
\begin{itemize}
\item Let $\ubar{s}(t) = \E[\theta|\theta<t]$ and $\bar{s}(t) = \E[\theta|\theta>t]$
\end{itemize} 
\begin{alertblock}{Theorem}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{2.9cm} |p{2cm}  |p{1cm} | c }
     \toprule
      $F$ & $\pi^*$ & $V(\pi^*)$ & \\ \hline
    % \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}\cmidrule(lr){2-2}
    $\ubar{a} \leq \priormean \leq \bar{b} \newline \priormean \notin \cup_{i=1}^\numintervals \bar{\Theta}_i\newline \exists t$,  $\ubar{s}(t), \bar{s}(t) \in \cup_{i=1}^\numintervals \bar{\Theta}_i$
    & $\I=\{\mathbf{1},\mathbf{2}\}$\newline $[0,t] \rightarrow \mathbf{1}$\newline $[t,M] \rightarrow \mathbf{2}$
     &
     1
      & 
      \raisebox{-\totalheight}{\includegraphics[height=25mm]{presentations/pres_img/g4.png}}
      \\ \bottomrule
      \end{tabular}
      \end{center}
      \end{table}
\end{alertblock}
\begin{itemize}
\item Disperse mean belief; but can't do so if too tightly concentrated
\item Can derive more general conditions without much complexity
\end{itemize}
\end{frame}

\begin{frame}{Optimal Design}
\begin{itemize}
\item $p(t,\lambda,\delta)$ and $q(t,\lambda,\delta)$ more diffused analogs of $\ubar{s}, \bar{s}$
\end{itemize}
\begin{alertblock}{Theorem}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ p{2.7cm} |p{2.5cm}  |p{1cm} | c }
     \toprule
      $F$ & $\pi^*$ & $V(\pi^*)$ & \\ \hline
    % \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}\cmidrule(lr){2-2}
    $\ubar{a} \leq \priormean \leq \bar{b} \newline\priormean \notin \cup_{i=1}^\numintervals \bar{\Theta}_i \newline \exists t$,  \small $p(t,\lambda,\delta), \newline {q(t,\lambda,\delta) \in \cup_{i=1}^\numintervals \bar{\Theta}_i}$
    & $\I=\{\mathbf{1},\mathbf{2}\}$
    \begin{align*}
        [0,t] \xrightarrow{\text{w.p }\lambda} \mathbf{1} \\ \xrightarrow{\text{w.p }1-\lambda} \mathbf{2} \\ [t,M] \xrightarrow{\text{w.p }\delta} \mathbf{2} \\ \xrightarrow{\text{w.p }1-\delta} \mathbf{1}
    \end{align*}
     &
     1
      & 
      \raisebox{-\totalheight}{\includegraphics[height=25mm]{presentations/pres_img/g5.png}}
      \\ \bottomrule
      \end{tabular}
      \end{center}
      \end{table}
\end{alertblock}
\end{frame}

\begin{frame}
\frametitle{Proof idea}
\begin{itemize}
    \item \underline{Part I:} Require at most $\numintervals+1$ signals ($|\I|\leq \numintervals+1$)
    \begin{itemize}
        \item $\bar{\Theta}_j$ are closed, convex intervals
        \item For each $j$, $\posterior{\signal_1},\posterior{\signal_2} \in \bar{\Theta}_j$ can be combined without loss 
    \end{itemize}
    \item \underline{Part II:} Objective fn. of $q_\signal, \posterior{\signal}$, so can search over $\mathcal{T}_\pi$'s
    \begin{itemize}
        \item Search directly over all $\textcolor{blue}{H} \succeq \textcolor{orange}{\dist}$
        \item Constraints: $\int_0^c \textcolor{blue}{H}^{-1}(t)dt \geq \int_0^c \textcolor{orange}{F}^{-1}(t)dt$ $\forall c \in [0,1]$        
    \end{itemize}
        \item<2-> \underline{Part III:} Know positions $\mu_i$
    \begin{itemize}
        \item If $\priormean < \ubar{a}$ or $\priormean > \bar{b}$, know position of $\mu_{\numintervals+1}$ relative to other posterior means in $\bar{\Theta}_j$
        \item If not, solve $\numintervals$ convex optimizations for possible locations of $\mu_{\numintervals+1}$ 
    \end{itemize}
     \item<2-> \underline{Part IV:} Combining (I) + (II) + (III)
    \begin{itemize}
        \item Know that $\textcolor{blue}{H}$ must be discrete by (I)
        \item Finite subset of constraints are sufficient so we reduce from an infinite \# of constraints to finite constraint problem
    \end{itemize}
\end{itemize}
\end{frame}

==> presentations/Workshop_Slides/4_Theorem2.tex <==
\begin{frame}{State-dependent preferences}
    \begin{itemize}
        \item Allowing preferences to depend on the state $\trueparam$ complicates the search problem (considering only $\mathcal{T}_\pi$ no longer sufficient)
    \end{itemize}
    \begin{alertblock}{Example}
    \begin{itemize}
        \item $\dist \sim Unif[0,1]$ ($\priormean = 0.5$)
        \item $\obj(\fin;\trueparam) = \mathbb{I}\{\fin\in\goal(\trueparam)\}$
        \item Desirable beliefs $\Omega(\trueparam) = m^{-1}(\goal(\trueparam)) = [\frac{2}{3}\trueparam,1]$

    \begin{figure}
    \includegraphics[width=45mm]{presentations/pres_img/ex_3.png}
    \end{figure}        
        \item $\I = \{\textcolor{blue}{\mathbf{1}},\textcolor{orange}{\mathbf{2}}\}, \mathcal{T}_\pi = \mathcal{T}_{\pi'} = \{\textcolor{blue}{(q_1=\frac{3}{4},\mu_1=\frac{7}{12})},\textcolor{orange}{(q_2=\frac{1}{4},\mu_2=\frac{1}{4})}\}$
    \item $V_{\dist,\obj}(\pi)\neq V_{\dist,\obj}(\pi')$
    \begin{itemize}
        \item If $\trueparam\in(\frac{3}{8},\frac{1}{2})$, success only under $\pi$ when induce belief \textcolor{blue}{$\mu_1$}
    \end{itemize}
    \end{itemize}
    \end{alertblock}
\end{frame}

\begin{frame}{State-dependent preferences}
    \begin{itemize}
        \item Allowing the preferences to depend on the state $\trueparam$ further reduces the possibility to obtain an optimal design with MPS
    \end{itemize}
    \begin{alertblock}{Example}
    \begin{itemize}
        \item $\dist \sim Unif[0,1]$ ($\priormean = 0.5$)
        \item $\obj(\fin;\trueparam) = \mathbb{I}\{\fin\in\goal(\trueparam)\}$
        \item Desirable beliefs $\Omega(\trueparam) = m^{-1}(\goal(\trueparam)) = [\frac{1}{3}\trueparam-\epsilon,\frac{1}{3}\trueparam+\epsilon]$
        
        \item $\pi = \langle \I, \{z_\param\}_{\param\in\paramspace}\rangle$ where $\I = \{\mathbf{1},\mathbf{2},\mathbf{3}\}$ and $z_{\theta}(s)$ is as follows:
    \begin{align*}
    z_\theta(\cdot) = \begin{cases}
    & \mathbf{1} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_1\coloneqq[0,0.12]\cup[0.52,0.56]\\
    & \mathbf{2} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_2\coloneqq[0.12,0.30]\cup[0.80,0.82]\\
    & \mathbf{3} \text{ w.p. } 1 \text{ if }\param\in\mathcal{S}_3\coloneqq[0,1]\setminus\{\mathcal{S}_1\cup\mathcal{S}_2\}
    \end{cases}
    \end{align*}
    \item $\posterior{\mathbf{1}} = 0.18, \posterior{\mathbf{2}} = 0.27$ and $\posterior{\mathbf{3}} = 0.65$
    \item $V_{\dist,\obj}(\pi) = \textcolor{red}{12\epsilon}$
    \item Opt Mechanism with MPS: $\textcolor{blue}{6\epsilon}$
    \end{itemize}
    \end{alertblock}
\end{frame}
% in stateful setting we cannot reduce th search over pi by searching over direct mechanisms, because the posterior mean mu_i will induce an equilibrium outcome but we cannot evaluate whether that outcome is in desirable state-dependenct set since we do not know the true state. 
% in the second example, the posteriors are so generated that for certain ranges of true state, the posterior beliefs fall into desirable range of beliefs. 

\begin{frame}{Approximately Optimal Design}
    \begin{itemize}
        \item Previous examples motivates need for \textit{approximate} solutions
    \end{itemize}
    \begin{alertblock}{Definition}
    A mechanism $\pi^{\epsilon}$ is $\epsilon$-optimal for a problem instance defined by distribution $\dist$ over $\paramspace$ and utility function $\obj$ (under $V_{\dist,\obj}$) if: \begin{align*}V_{\dist,\obj}(\pi^\ast)-V_{\dist,\obj}(\pi^{\epsilon})\leq \epsilon.\end{align*}
    \end{alertblock}
    How to produce \textcolor{blue}{interval-based} signalling mechanism $\pi^{\epsilon}$?
       % \begin{itemize}
        \begin{enumerate}
        \item Discretize $\dist$ appropriately to $\dist_\delta$ (intervals $\Theta_j \rightarrow \text{ points }\nu_j$)
        \item Reduce consideration to finite \# of signals
        \item Solve discrete analog using linear programming to get $\bar{\pi}^{\ast}$
        \item Translate the discrete solution $\bar{\pi}^{\ast}$ to $\pi^{\epsilon}$ \\ 
        by applying $\bar{z}_{\nu_j}$ signal distribution to all states in $\Theta_j$
        \end{enumerate}
 %   \end{itemize}
 %An interval-based signalling scheme!
\end{frame}
\begin{frame}{Preferences}
    \begin{itemize}
    \item \textbf{Lipschitz}: Preferences are smooth in the in-person mass and realized state
    \begin{itemize}
    \normalsize
        \item $\obj(\fin;\trueparam)$ is uniformly $\eta_1$-Lipschitz in $\fin$ \& $\eta_2$-Lipschitz in $\trueparam$
        \end{itemize}
    \item[]
    \item \textbf{Scaled-capacity}: Preferences specify an in-person capacity limit that gets progressively more strict as $\trueparam$ increases
    \begin{itemize}
    \normalsize
        \item $\obj(\fin;\trueparam) \coloneqq \mathbb{I}\{\fin\in\goal(\trueparam)\} = \mathbb{I}\{\fin\geq a(\trueparam)\}$ where $a(\cdot)$ is weakly increasing step function
        \end{itemize}
    \end{itemize}
\end{frame}

\begin{frame}
\frametitle{Discretization of $F$ to $F_\delta$}
\begin{itemize}
  \item Consider a finite number of states $\trueparam \in \{\nu_j\}_{j=1,..,N}$
   % \item Problem is more tractable if we only need to consider a finite number of states $\trueparam \in \{\nu_j\}_{j=1,..,N}$ 
    \item Partition $\paramspace$ into $N = M\delta$ intervals $\Theta_j$ of width $\frac{1}{\delta}$
    \item \textcolor{blue}{Pick smallest point} $\nu_j$ in each interval and assign all mass in $\Theta_j$ under $\dist$ to point $\nu_j$ in $\dist_\delta$
\end{itemize}
\begin{figure}
\only<1>{\input{presentations/pres_fig/stateful_0}}
\only<2>{\input{presentations/pres_fig/stateful_1}}
% \caption{$v(m(\cdot);\nu)$}
\end{figure}
\end{frame}



\begin{frame}
\frametitle{Reduce \# of signals}
\vspace{-1em}
\begin{columns}
\begin{column}{0.5\textwidth}
\begin{figure}
\only<1>{\input{presentations/pres_fig/stateful_a}}
\only<2>{\input{presentations/pres_fig/stateful_b}}
\only<3>{\input{presentations/pres_fig/stateful_c}}
% \caption{$v(m(\cdot);\nu)$}
\end{figure}
\end{column}
\begin{column}{0.5\textwidth}
\begin{figure}
\only<1>{\input{presentations/pres_fig/stateful_d}}
\only<2>{\input{presentations/pres_fig/stateful_e}}
\only<3>{\input{presentations/pres_fig/stateful_f}}
% \caption{$v(m(\cdot);\nu)$}
\end{figure}
\end{column}
\end{columns}

\begin{itemize}
    \only<1>{\item $N$ curves 
    \item Approximate $\obj$ 
   by piecewise const. fn. in $y$ without much loss for Lipschitz preference}
   \only<2,3>{
    \item At most one signal will correspond posteriors that have equilibrium in each interval $\bar{\mu_i} \in [\gamma_i, \gamma_{i+1}]$}
\end{itemize}
\end{frame}

\begin{frame}{Solve Linear Program}
\begin{itemize}
    \item Variables $x_{ji}$ to represent probability in state $\nu_j$ under $F_\delta$ and signal $\signal$ is provisioned
    \begin{itemize}
        \item $\bar{z}_{\nu_j}(i) = \frac{x_{ji}}{\sum_i x_{ji}}$
    \end{itemize}
    \item Objective and constraints on posterior can all be made linear
    \begin{itemize}
        \item Constraints on $\bar{\posterior{i}}$: $\gamma_{i}\sum_{j=1}^N x_{ji} \leq \sum_{j=1}^N \nu_j x_{ji} \leq \gamma_{i+1}\sum_{j=1}^N x_{ji}$
    \end{itemize}
    \item LP algorithm outputs optimal \textit{discrete} solution $\bar{\pi}^\ast \coloneqq \pi_{F_\delta,h}^\ast$
\end{itemize}
\end{frame}

\begin{frame}{Translate from discrete to continuous solution}
\begin{itemize}
    \item Apply signal distribution $\bar{z}_{\nu_j}$ from $\bar{\pi}^\ast$ to every point in the corresponding interval $\Theta_j$ to get $\pi^\epsilon$ 
    \item Similarly, unknown true optimal design $\pi_{F,h}^\ast$ has discrete analog $\bar{\pi}$ where aggregate signal distribution over interval $\Theta_j$ is applied to $\nu_j$
\end{itemize}
Quality of $\pi^\epsilon$ error bounded by how lossless we transition from discretized to continuous signalling mechanisms:
        \begin{align*}
            V_{F,h}(\pi_{F,h}^\ast)-V_{F,h}(\pi^\epsilon) \leq &\big(V_{F,h}(\pi_{F,h}^\ast)-V_{F_\delta,h}(\bar{\pi})\big) \\
            & + \big( V_{F_\delta,h}(\bar{\pi}^\ast)-V_{F,h}(\pi^\epsilon)\big)
        \end{align*}
\end{frame}

\begin{frame}
\frametitle{Translate from discrete to continuous solution}
\vspace{-1em}
\begin{columns}
\begin{column}{0.5\textwidth}
\begin{figure}
\input{presentations/pres_fig/stateful_g}
\end{figure}
\end{column}
\begin{column}{0.5\textwidth}
\begin{figure}
\input{presentations/pres_fig/stateful_h}
\end{figure}
\end{column}
\end{columns}
\begin{itemize}
    \item Posteriors are close under discretization: $0 \leq \mu_i-\bar{\mu}_i \leq \frac{1}{\delta}$
    \itemGuarantees continuous signalling mechanisms induce higher posteriors
\end{itemize}
\end{frame}

\begin{frame}{Translate from discrete to continuous solution}
\begin{itemize}
    \item Distribution over observed signals are identical
    \item This guarantees objective function values are also close 
\end{itemize}

\begin{alertblock}{Theorem: For both Lipschitz and scaled-capacity}
If cdf of $\popdist$ is Lipschitz, algorithm produces $\epsilon$-optimal mechanism with runtime:\\
\textbf{Lipschitz:} $O(\frac{1}{\epsilon^5})$\\
\textbf{Scaled Capacity:} $O(\frac{1}{\epsilon^5})$
\end{alertblock}
\end{frame}

==> presentations/Workshop_Slides/5_Dynamic.tex <==
  \begin{frame}
  \vfill
  \centering
  \begin{beamercolorbox}[sep=8pt,center,shadow=true,rounded=true]{title}
    \usebeamerfont{title}Part II: Dynamic information provision about demand surge in
    ride-hailing systems\par%
  \end{beamercolorbox}
  \vfill
  \end{frame}

\begin{frame}{Surge Pricing}

Mobility service providers need to deal with uncertain demand
\begin{columns}
\begin{column}{0.75\textwidth}

   \begin{itemize}
   % \item 
    \item \textbf{Wild Goose Chase (WGC):} Demand spikes $\Rightarrow$ drivers pick up far away passengers \\ $\Rightarrow$ fewer trips supplied $\Rightarrow$ matching failure \\ $\Rightarrow$ low welfare 
        (Castillo et al. '17)
    % \begin{itemize}
    %     \item 
    % \end{itemize}
    \item \textbf{Surge Pricing:}
    \begin{itemize}\normalsize 
        \item Subverts WGC
        \item Lower prices when demand is low
        \item $\uparrow$ total welfare and $\uparrow$ utilization rate
    \end{itemize}
\end{itemize}
\end{column}
\begin{column}{0.25\textwidth}  %%<--- here
\centering
\frame{\includegraphics[width=30mm]{presentations/pres_img/surgerhp.png}}
\end{column}
\end{columns}
\vspace{0.5cm}
Rich literature on market design for ride-hailing systems:
\begin{itemize}
    \item Bimpikis et al. '19, Besbes et al. '20, Borgs et al. '14, Castillo et al. '17, Castillo '20, Garg et al. '19
\end{itemize}
\end{frame}

\begin{frame}{Managing Strategic Drivers}
\begin{itemize}
    \item \textbf{Key issue:} Strategic drivers with uncertainty over surge patterns (i.e. when and where) proactively chase/skip surges
    \begin{itemize}
    \normalsize
        \item Unreliable service and supply-demand imbalance
        \item Congestive effect at surge hotspot
    \end{itemize}
    \item[] 
    \item[Q.] How can platform \textcolor{blue}{dynamically provision information}  about uncertain demand surge to manage \textcolor{blue}{strategic drivers}? 
    %avoid \textcolor{blue}{both overcrowding and no driver situations}? 
%    \textcolor{blue}{dispersed distribution} of drivers? 
\end{itemize}
\begin{figure}
    \centering
\begin{tikzpicture}
    \node[circle,fill=teal,minimum size=5em] at (360:0mm) (center) {\textcolor{white}{$Surge$}};
    \foreach \n in {1,...,4}{
        \node[circle,fill=black] at ({\n*360/8}:2 cm) (n\n) {\textcolor{white}{$\ell_\n$}};
        \draw[->,dashed] (n\n) edge (center) ;
        \draw[<-,dashed] (n\n) edge (center) ;
        \draw[->] (n\n) edge [loop left] (n\n) ;
    }
    \foreach \n in {5,...,8}{
        \node[circle,fill=black] at ({\n*360/8}:2cm) (n\n) {\textcolor{white}{$\ell_\n$}};
        \draw[->,dashed] (n\n) edge (center) ;
        \draw[->] (n\n) edge [loop right] (n\n) ;
    }
\end{tikzpicture}
\end{figure}
\end{frame}

\begin{frame}{Related work}
\begin{tikzpicture}[sibling distance=15em,
  every node/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20}, foo/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=green!20}]]
  \node {Dynamic Information Design}
    child { node {Fixed $T$} child { node {\tiny Ely et al. '17\\ \tiny Farhadi et al. '22, ..} } }
    child { node {Markovian $T$}
      child { node {Long-run receivers}
        child { node[foo] {Adaptive \\  \textbf{\tiny SAJ '22*}} }}
      child { node {Myopic receivers\\\tiny Vielle et al. '17} } };
\end{tikzpicture}

% Rich literature on \textbf{Ride-Hailing Market Design}:
% \begin{itemize}
%     \item Bimpikis et al. '19, Besbes et al. '20, Borgs et al. '14, Castillo et al. '17, Castillo '20, Garg et al. '19
% \end{itemize}
\end{frame}

\begin{frame}{Our setting}
\begin{itemize}
    \item Planner seeks to maximize number of periods where desirable masses are maintained across two location types
    \item Under full-information disclosure, this is not possible as all agents only move just before surge onsets
    \item Under no-information disclosure, agents distribution immediately converges
   \item \textbf{Key point:} Optimal disclosure induces the mass in the desirable set that is closest to the no-information mass 
 %  Optimal disclosure seeks to maximize probability desirable mass closest to no-information mass can be maintained
%    \item \textbf{Key point:} Optimal disclosure seeks to maximize probability desirable mass closest to no-information mass can be maintained
\end{itemize}
\end{frame}

==> presentations/Workshop_Slides/6_Dynamic_Model_Results.tex <==
\begin{frame}
\frametitle{Dynamic Model}
\begin{itemize}
\item Discrete time $t=1, 2, ..$
\item Unit mass of non-atomic \textcolor{blue}{long-run} agents; each make simultaneous location choice at time $t$: $ a_t \in \{\ellC,\ellP\}$
    \begin{itemize}
        \item $\ellC$ is communal (demand hotspot)
        \item $\ellP$ is peripheral (remote)
        \item Move from $\ellP$ to $\ellC$ is irreversible
    \end{itemize}
    \item Mass $y_t$ at $\ellP$ at end of $t$
\end{itemize}
\end{frame}

\begin{frame}
\frametitle{Model: Agents}
\begin{itemize}
    \item Each agent has private fixed per-period wage at $\ellP$ from known distribution $v \sim G$
\item Random time horizon $T \sim Geom(q)$ when surge onsets at congested hotspot
\begin{itemize}
    \item Horizon is memoryless 
    %(i.e. $\P[T=j+H|T=H] = \P[T=j]$)
    \item At end of period $T$, $1-y$ agents at $\ellC$ receive $\beta(1-y)$ where $\beta(\cdot)$ is decreasing
\end{itemize}
\item Agents seek to maximize total horizon wages
\end{itemize}
\end{frame}

\begin{frame}
\frametitle{Dynamic Information Provision}
\begin{itemize}
\item Planner seeks to maintain driver distribution in a goal set $\goal$ i.e., maximize \# of periods $t$ with $y_t \in \goal \coloneqq \cup_{j=1}^\numintervals \Omega_j$
\item Each $t$, planner first \textit{publicly} commits to and discloses \textit{signalling mechanism} $\pi_t = \langle \I , \{z_\param(\cdot)\}_{\param \in \paramspace_t}\rangle$
\begin{itemize}
    \item $\paramspace_t = \{S_t, S_t^c\}$ where $S_t = \{T = t\}$ (e.g. $\P[S_t] = q$)
    \item Planner can observe $y_{t-1}$, but not $S_t$
    \item An adaptive, sequential model 
\end{itemize}
\item Signal then publicly shared with all agents before they make their decisions 
\end{itemize}
\end{frame}

\begin{frame}
\frametitle{Memorylessness}
\begin{itemize}
\item By memorylessness, agents in $t$ play stationary strategies that only depend on belief over $\mu_t(i) \coloneqq \mathbb{P}[S_t|\pi \rightarrow \signal]$ and $y_{t-1}$
\item Planner also uses stationary strategy to prescribe $\pi_t$ that only depends on $y_{t-1}$
\item Can characterize map from current beliefs to equilibrium in next period $m_{y_{t-1}}(\mu_t) \coloneqq y_t^\ast$ (analogous to $m(\cdot)$ for Part I)
\end{itemize}
\end{frame}

\begin{frame}
\frametitle{Value of information}
\begin{itemize}
\item Solve for optimal strategy using dynamic programming on value functions $V(\mu_t; y_{t-1})$ 
%and iterate from when $y_{t-1}$ is low to when it is high
\item $V$ is piecewise concave (linear) in $\mu_t$
\begin{itemize}
    \item Concave regions correspond to the $\mu_t$ that yield $y_t^\ast$ in $\Omega_j$
\end{itemize}
\item Planner benefits by not dispersing beliefs in these intervals 
\end{itemize}
\scalebox{0.6}{
\begin{figure}
    \centering
    \begin{tikzpicture}
	\begin{axis}[xtick={0,0.2,0.6,1},
	xticklabels={$0$,$m_{y_{t-1}}^{-1}(b_K)$,$m_{y_{t-1}}^{-1}(a_1)$,$1$},ytick={0,1},yticklabels={0,1},ymin=-0.1,ymax=1.2,xlabel={$\posterior{t}$},ylabel={$V(\posterior{t};y_{t-1})$},
      x label style={at={(axis description cs:0.45,0)},anchor=north,font=\huge},
	  y label style={font=\huge,at={(axis description cs:-0.1,.35)},rotate=-90,anchor=south},
	  ]
   \addplot[domain=0.5:0.6,blue,thick] {0.6-0.3*x};	
	\addplot[soldot,blue] coordinates{(0.2,0.68)(0.333,0.6)(0.5,0.45)(0.6,0.42)};
	\addplot[holdotb] coordinates{(0.2,0)(0.333,0)(0.5,0)(0.6,0)};
	\addplot[domain=0:0.2,blue,thick] {0};
	\addplot[domain=0.333:0.5,blue,thick] {0};
	\addplot[domain=0.6:1,blue,thick] {0};
	\addplot[domain=0.2:0.333,blue,thick] {0.8-0.6*x};
	\end{axis}
	\end{tikzpicture} 
\end{figure}}
\end{frame}

\begin{frame}
\frametitle{Full and no disclosure: Benchmarks}
\begin{alertblock}{Lemma}
\begin{itemize}
    \item Under full disclosure, $y_1^* = .. = y_{T-1}^* > y_{T}^*$
    \begin{itemize}
        \item Agents move to $\ellC$ before $T$ iff $v \leq \hat{v}_{FI}$ where $\beta(G(\hat{v}_{FI})) = \hat{v}_{FI}$
    \end{itemize}
    \item Under no disclosure, $\tilde{y}^*(q) \coloneqq y_1^* = .. = y_{T}^*$
    \begin{itemize}
        \item Agents move (immediately) to $\ellC$ iff $v \leq v_{NI}^*$ where $\beta(G(v_{NI}^*))=\frac{v_{NI}^*}{q}$
        \item $\tilde{y}: [0,1] \rightarrow [0,1]$ is weakly decreasing, bounded, and continuous.
    \end{itemize}
\end{itemize}
\end{alertblock}

% \begin{alertblock}{Lemma}

% \end{alertblock}
\end{frame}

\begin{frame}{Dynamic Information Provision: Result}
\begin{figure}
    \centering
    
    \begin{tikzpicture}
	\begin{axis}[xtick={0,0.2,0.6,1},
	xticklabels={$0$,$\tilde{y}^{-1}(b_K)$,$\tilde{y}^{-1}(a_1)$,$1$},ytick={0,1},yticklabels={0,1},ymin=-0.1,ymax=1.2,xlabel={$\mathbf{q}$},ylabel={Fraction of\\ $T$-horizon},
      x label style={at={(axis description cs:0.45,0)},anchor=north,font=\small},
	  y label style={font=\normalstyle,at={(axis description cs:-0.1,.35)},rotate=-90,anchor=south},
	  ]
   \addplot[domain=0.5:0.6,blue,thick] {1};	
	\addplot[domain=0:1,black,thick] {0.01};
	\addplot[domain=0:0.2,violet,thick] {0.8+x};
	\addplot[soldot,blue] coordinates{(0.2,1)(0.333,1)(0.5,1)(0.6,1)};
	\addplot[holdotb] coordinates{(0.2,0)(0.333,0)(0.5,0)(0.6,0)};
	\addplot[domain=0:0.2,blue,thick] {0};
	\addplot[domain=0.333:0.5,blue,thick] {0};
	\addplot[domain=0.6:1,blue,thick] {0};
	\addplot[domain=0.2:0.333,blue,thick] {1};
	
	\addplot[domain=0.2:0.6,violet,thick] {0.99};
	\addplot[domain=0.6:1,violet,thick] {2.5-2.5*x};
 \addlegendentry{No Inf.}
 \addlegendentry{Full Inf.}
 \addlegendentry{Opt. }
	\end{axis}
	\end{tikzpicture} 
\end{figure}    
\end{frame}


\begin{frame}
\frametitle{Dynamic Information Provision: Result}
\begin{itemize}
    % \item When non-informative signalling is not optimal, show that planner objective is concave in belief across regimes
    % item Reduce optimization to just optimizing over few posterior beliefs
\end{itemize}
\begin{alertblock}{Theorem}
Optimal mechanism uses at most two signals and achieves values and posterior distributions: 
\begin{table}[h!]
     \begin{center}
     \resizebox{0.8\columnwidth}{!}{%
     \begin{tabular}{ p{3.8cm} |p{3.2cm}  |p{3cm}  }
       $\mathbf{q}$: & $\mathbf{V^*}:$ & $\mathbf{(\mu_1,\mu_2)}:$ \\\hline
      \small{$\mathbf{q} < \tilde{y}^{-1}(b_K)$} & $\frac{1+q-\tilde{y}^{-1}(b_K)}{q}$ & $(0, \tilde{y}^{-1}(b_K))$\\\hline
    \small{$\tilde{y}^{-1}(b_K) \leq \mathbf{q} \leq \tilde{y}^{-1}(a_1)$} & $\frac{1}{q}$ & $(\tilde{y}^{-1}(b_K),\tilde{y}^{-1}(a_1))$\\\hline
      \small{$\mathbf{q} > \tilde{y}^{-1}(a_1)$} & $\frac{1-q}{q(1-\tilde{y}^{-1}(a_1))}$ & $( \tilde{y}^{-1}(a_1),1)$
    %   & $\tilde{y}^{-1}(a_1),\tilde{y}^{-1}(b_K)$ & $1, \tilde{y}^{-1}(b_K)$
    %   & $\frac{1}{q}$ & $\frac{1}{\tilde{y}^{-1}(b_K)}$ \\\hline
    %   \small{$\tilde{y}^{-1}(b_K) > \mathbf{q}$} & $\frac{1-q}{1-\tilde{y}^{-1}(a_1)}$ & $\frac{1}{q}$ & $\frac{1}{q}$ \\\hline
    %   $\mathbf{y_{t-1}} < a_1$ & $0$ & $0$ & $0$\\
      \end{tabular}
      }
      \end{center}
      \end{table}
\end{alertblock}
\end{frame}

\begin{frame}
\frametitle{Conclusion}
\begin{itemize}
    \item New insights on structure and computation of optimal information mechanisms for managing congested hotspots
    \item Static and dynamic designs
    \item Future work: settings when planner needs to learn 
\end{itemize}
\vfill
thank you! feedback and questions? 
\end{frame}
